RTL2M$\mu$PATH: Multi-$\mu$PATH Synthesis with Applications to Hardware Security Verification

The Check tools automate formal memory consistency model and security verification of processors by analyzing abstract models of microarchitectures, called $\mu$SPEC models. Despite the efficacy of this approach, a verification gap between $\mu$SPEC models, which must be manually written, and RTL limits the Check tools' broad adoption. Our prior work, called RTL2$\mu$SPEC, narrows this gap by automatically synthesizing formally verified $\mu$SPEC models from SystemVerilog implementations of simple processors. But, RTL2$\mu$SPEC assumes input designs where an instruction (e.g., a load) cannot exhibit more than one microarchitectural execution path ($\mu$PATH, e.g., a cache hit or miss path) -- its single-execution-path assumption. In this paper, we first propose an automated approach and tool, called RTL2M$\mu$PATH, that resolves RTL2$\mu$SPEC's single-execution-path assumption. Given a SystemVerilog processor design, instruction encodings, and modest design metadata, RTL2M$\mu$PATH finds a complete set of formally verified $\mu$PATHs for each instruction. Next, we make an important observation: an instruction that can exhibit more than one $\mu$PATH strongly indicates the presence of a microarchitectural side channel in the input design. Based on this observation, we then propose an automated approach and tool, called SynthLC, that extends RTL2M$\mu$PATH with a symbolic information flow analysis to support synthesizing a variety of formally verified leakage contracts from SystemVerilog processor designs. Leakage contracts are foundational to state-of-the-art defenses against hardware side-channel attacks. SynthLC is the first automated methodology for formally verifying hardware adherence to them.

==> 01-intro.tex <==
\section{Introduction}
\label{sec:intro}
% \caroline{Abstract + Intro: 1.5 pages}
% In a \textit{hardware side-channel attack}, an attacker observes a victim program's hardware resource usage 
% % in space (what resources it uses) and time (when it uses them)
% and infers its secret data~\cite{Osvik:prime+probe+l1d,yarom:flush+reload+llc14,pandora:isca:21,cauligi:sok-spectre-sw-defense}. 
\textit{Hardware side-channel attacks}~\cite{Osvik:prime+probe+l1d,yarom:flush+reload+llc14,pandora:isca:21,cauligi:sok-spectre-sw-defense} can be understood using a telecommunications analogy~\cite{dawg:kiriansky}: a \textit{transmitter} (victim) modulates a \textit{channel} (hardware resource) in a secret-dependent manner, and a \textit{receiver} (attacker) infers the secret by observing the channel modulation.
% observes the channel modulation to infer the secret.
The transmitter is often a specific \textit{transmit instruction} in the victim program that modulates a channel in an operand-dependent manner~\cite{jiyong:stt}.
% , i.e., a \textit{transmit instruction}~\cite{jiyong:stt}.
This special case is so common that \textit{leakage contracts} based on transmit instructions, called \textit{constant-time (\ct{}) contracts}, are
%So often, in fact,
% that the notion of transmit instructions is
\textit{the} enabler for hardware side-channel defenses today ~\cite{arm:dit,intel:doit,riscv_zkt,pandora:isca:21}. 

% Such \textit{transmitter-centric}\footnote{Given the focus of this paper, we use the terms ``transmitter’’ and ``transmit instruction’’ interchangeably (\S\ref{sec:background:telecom}).} leakage 
A \ct{} contract enumerates a processor's transmit instructions and their unsafe (``leaky’’) operands. Hardware side-channel defenses then ensure that secrets \textit{never} reach  unsafe operands when programs execute.
% \textit{never} pass secrets to them.
This strategy is embodied in the \textit{\ct{} programming}\footnote{``Constant time'' is a legacy term that denotes ``data oblivious''~\cite{yu:oisa}.} discipline~\cite{Bernstein:curve25519, Bernstein:Poly1305-AES, Molnar:pc-security-model, Rane:Raccoon, Fisch:Iron,Shaon:SGX-BigMatrix, Zheng:Opaque, Eskandarian:OliDB, Mishra:Oblix,  Tople:oblivious-execution, Sasy2018ZeroTraceO, Ahmad2018OBLIVIATEAD, Coppens:timing-channel-x86, FactLanguage, synthct}---the gold standard for writing cryptopgraphic code~\cite{openssl, libsodium, hacl, mbedtls}.
% 
It is also central to
hardware~\cite{jiyong:stt,Taram:CSF,Bourgeat:m16, Schwarz:ConTExT, yu:oisa,jiyong:sdo,barber:specshield,weisse:nda,dolma} and software defenses~\cite{
barthe:highassurance,ctfoundations:pldi:20,guarnieri:spectector,vassena:blade,guanciale:inspectre,guarnieri:contracts,shivakumar:spectredeclassified,
guanciale:inspectre,cauligi:sok-spectre-sw-defense, serberus:mosier:2024} against \textit{transient execution attacks}, which exploit hardware faults and mispredictions to \textit{steer} secrets towards unsafe operands~\cite{spectre,canella2019systematic}.

% Owing to their importance, transmit instructions 
% are also foundational in 
Nascent ISA adoption further underscores the importance of \ct{} contracts for secure computation.
% Further underscoring their importance, several major ISAs have recently adopted \ct{} contracts.
% Nascent ISA \textit{leakage contracts} further underscore the relevance of transmit instructions for secure computation.
In particular, the Arm DIT~\cite{arm:dit} and Intel DOIT~\cite{intel:doit} \textit{hardware modes}
% \footnote{Enabling Arm DIT (Intel DOIT) is an unprivileged (privileged) operation.}
and the RISC-V Zkt~\cite{riscv_zkt} \textit{ISA extension}
% further underscore the role of transmit instruction in writing secure software.
% are also centered around transmitter instructions.
% underscore the transmit instructions in secure software design.
% In particular, Arm and Intel have introduced \textit{hardware modes} (DIT~\cite{arm:dit} and DOIT~\cite{intel:doit}, respectively),\footnote{Enabling Arm DIT (Intel DOIT) is an unprivileged (privileged) operation.} and RISC-V has defined an \textit{ISA extension} (Zkt), which define a ``safe'' instruction set under certain receiver assumptions.
% all of which transform transmit instruction  define ``safe'' subset of ISA instructions.
% , all of which provide ``safe'' versions \textit{some} ISA instructions according a particular threat model.
% , all of which provide ``safe'' versions of \textit{some} ISA instructions.
% In particular, 
% These industrial contracts 
flag \textit{all} instruction operands as unsafe by default.
% , i.e., all instructions are transmit instructions.
Programmers can then selectively enforce safety for \textit{some} instruction operands, subject to particular usage and receiver assumptions
% versions of \textit{some} instructions
% under certain receiver assumptions
(\S\ref{sec:background:sec-def}).
% Specifically, the \textit{data} operands of safe instruction variants are guaranteed to not impact the execution time (in cycles) of any in-flight instruction (including themselves), if executed in a particular mode (DIT, DOIT) or run on specific hardware (Zkt).

% That is, assuming a receiver who can measure execution time
% ,



% In this paper, we observe that 


% Often, the transmitter is a specific instruction in the victim program that modulates a channel in an operand-dependent manner, i.e., a \textit{transmit instruction}~\cite{}.
% So often, in fact, that \textit{the notion of transmit instructions forms the most ubiquitous hardware-software contract today for dealing with hardware side-channel attacks}. 
% Given a list of transmit instructions and their ``unsafe'' operands, hardware side-channel defenses can ensure that programs \textit{never} pass secrets to them.
% % their sensitive operands.
% In software, this approach is known as constant-time (CT) programming\footnote{``Constant time'' is a legacy term, which denotes ``data obliviousness''~\cite{}.}~\cite{Bernstein:curve25519, Bernstein:Poly1305-AES, Molnar:pc-security-model, Rane:Raccoon, Fisch:Iron, Shaon:SGX-BigMatrix, Zheng:Opaque, Eskandarian:OliDB, Mishra:Oblix, Tople:oblivious-execution, Sasy2018ZeroTraceO, Ahmad2018OBLIVIATEAD, Coppens:timing-channel-x86, FactLanguage, synthct}; it is the
% % . It is the
% gold standard for writing cryptographic code~\cite{openssl, libsodium, hacl, mbedtls}.
% % , which must process (and not leak) secrets.
% Transmit instructions are also central to hardware~\cite{jiyong:stt,Taram:CSF,Bourgeat:m16, Schwarz:ConTExT, yu:oisa,jiyong:sdo,barber:specshield,weisse:nda,dolma} and software defenses~\cite{todo, cauligi:sok-spectre-sw-defense, serberus:mosier:2024} against \textit{Spectre attacks}, which exploit hardware mispredictions to \textit{steer} secrets towards transmit instruction operands~\cite{spectre,canella2019systematic}.

% For over a decade, hardware side-channel defenses have relied on \textit{manually curated} lists of transmit instructions.
% % , making them brittle in the face of zero-day attacks that expose new ones.
% For a while, transmit instructions were restricted to control-flow~\cite{Kocher:RSA} and memory~\cite{Osvik:prime+probe+l1d,Yarom:flush+reload+llc13} instructions.
% % ---known to leak their condition and address operands, respectively.
% Researches then deemed some arithmetic instructions (e.g., integer division~\cite{Coppens:timing-channel-x86} and floating point~\cite{andrysco:subnormal} operations) unsafe on real processors. 
% Most recently, a survey of the Computer Architecture literature identified a set of hardware optimizations that would together render \textit{all} instruction operands
% % \textit{all instruction operands, results, and data at-rest}\footnote{Data ``at-rest'' refers to data contained in the architectural state of a processor~\cite{pandora:isca:21}.}
%  %vulnerable to side-channel leakage
% unsafe~\cite{pandora:isca:21}.


% Fortunately, modern ISAs are \textit{finally} (within the past two years) adopting \textit{\leakagecontracts{}} based on transmit instructions.
% For over a decade, hardware side-channel defenses have relied on \textit{manually curated} lists of transmit instructions.
% However, modern ISAs are \textit{finally} (within the past two years) adopting \textit{\leakagecontracts{}} based on transmit instructions.
% % , which we call \textit{CT contracts}.
% In particular, Arm and Intel have introduced hardware modes (DIT~\cite{arm:dit} and DOIT~\cite{intel:doit}, respectively),\footnote{Enabling Arm DIT (Intel DOIT) is an unprivileged (privileged) operation.} and RISC-V has introduced an ISA extension (Zkt), all of which
% % Arm DIT~\cite{arm:dit} and Intel DOIT~\cite{intel:doit} have introduced hardware modes which
% codify a subset of instructions whose \textit{data} operands specifically will \textit{not} impact the execution time (in cycles) of any in-flight instruction (including themselves).


% In particular, Arm DIT~\cite{arm:dit}, Intel DOIT~\cite{intel:doit}, and RISC-V Zkt~\cite{riscv_zkt} all codify a subset of instructions, whose \textit{data} operands specifically will \textit{not} impact the execution time (in cycles) of any in-flight instruction (including themselves).
% Arm DIT and Intel DOIT require \textit{only if} they are executed in a particular hardware mode.
% \caroline{Enabled in software.}

% Controlled by a model-specific register that cannot be changed by user space.
% Set of safe instructions is pretty small. 
% Generally belived that it will just make your processor run slower
% Rather than try to use optimized instructions in a safe way, they just disablle the optimizaitons altogether. This results is less performant software - performance will become an increasiningly big issue with more hardware optimizations.

% Industry-backed \leakagecontracts{} are a step in the right direction, but
% (at least) two important challenges remain.
% First, state-of-the-art leakage contracts are \textit{transmitter-centric}, enumerating transmit instructions and their unsafe operands, e.g., all instrution operands are unsafe \textit{except} some certain instructions' data operands when executed in a \textit{slower} DIT/DOIT/Zkt mode.
% Such a coarse-grained approach e between performance and security. 
% performance impact of DOITM may be "significantly higher on future processors". 
% On advanced microarchitecture, this coarse-grained approach means that performance overhead associated with DIT/DOIT/Zkt mode will be increasingly significant. 

\subsection{This Paper}
\label{sec:intro:this-paper}
\begin{figure}[t!]
\begin{subfigure}{0.52\linewidth} 
    \centering
     %\includegraphics[width=0.79\linewidth]{figs/mul_sub_l_6.png}
     %\includegraphics[width=0.82\linewidth]{figs/mul_sub_2.png}
     %\includegraphics[width=0.81\linewidth]{figs/mul_sub_3.png}
     \includegraphics[width=1.0\linewidth]{figs/mul_sub_3.png}
     %\vspace{-2pt}
     \caption{
     \upaths{}. Row(1/\llt{}): 1st/\llt{}-th visit to Row. Node label: value of \llt{} for \upath{}.
     %\yao{Updated}
     }
     %\upaths{}. Row\textsubscript{f}: \textit{final} visit to  Row. Node label \inst{n}: 1\textsuperscript{st} to \inst{n}\textsuperscript{th} visit to Row.}
     %, n: \# in node). \textcolor{myred}{$\rightarrow$}: in-order commit. }
     %\caption{\upaths{}. Row(f/l): exec. phase (first \inst{n}/last visit, \inst{n}: \# in node). }%, n: \# in node). \textcolor{myred}{$\rightarrow$}: in-order commit. }
     \label{fig:zero-skip-uhb}
\end{subfigure}%
~
%\hspace{0.01\linewidth}
\begin{subfigure}[b]{0.47\linewidth} %130pt} %.55\linewidth}
    \begin{tcolorbox}[left=0.1pt,right=0.2pt,top=1pt,bottom=1pt]
    %\begin{framed}
    \footnotesize
      \noindent\textcolor{ForestGreen}{{\RaggedLeft// 
      \inst{MUL} skips computation if it has zero operands or stays}}\\ % until \inst{done}}}\\
      %\inst{MUL} stays in \inst{mulU} for one cycle if it has zero operands, else stays four.}}\\
      %takes path 1 if at least one argument is 0, else it takes path 1.}}\\
%    {
%    \setlength{\arrayrulewidth}{1pt}
%       \renewcommand{\arraystretch}{1.3}
%     \begin{tabular}[t]{
%       @{}>{\raggedright\arraybackslash} m{113pt} %0.9\linewidth}
%       }
    %\noindent\textcolor{ForestGreen}{\RaggedLeft// Precondition}\newline
%     \centering\arraybackslash $\mathsf{visit(i0, mulUnit)}$ \\[2pt]
     %\rule{118pt}{0.4mm} 
    \hlt{\noindent$\mathsf{dst\;MUL\_mulU(MUL^N\;i0)\!:}$} %\textcolor{ForestGreen}{// Leakage function} 
    \newline
%        \indent$\;\;\mathsf{path\_id = ((}$\hlt{$\mathsf{i0.\iparg{arg0}}$}$\mathsf{== 0)\;\vee}$ \newline 
        \indent$\;\;\mathsf{\textcolor{blue}{return}\;ite((}$\hlt{$\mathsf{i0.\iparg{arg0}}$}$\mathsf{\;== 0)\;\vee}$ \newline
        \indent$\;\;\;\;\mathsf{(}$\hlt{$\mathsf{i0.\iparg{arg1}}$}$\mathsf{ \;== 0) \vee done, }$\newline
        %$\mathsf{(path\_id == 1), }$\newline 
        \indent$\;\;\;\;\hlt{$\mathsf{\{mulFin\},}$}$\hlt{$\mathsf{
        %\{mulUnitFin\}, 
        \{mulU\}}$}$\mathsf{)}$
%    \end{tabular}
%    }
    \\[3pt]
      \noindent\textcolor{ForestGreen}{{\RaggedLeft// \inst{SUB} proceeds or get stal-led by \inst{MUL} until it commits}} \\ % ($\mathtt{i1.cmt}$) }}\\
    %{
    %\setlength{\arrayrulewidth}{1pt}
    %   \renewcommand{\arraystretch}{1.3}
    % \begin{tabular}[t]{
    %   @{}>{\raggedright\arraybackslash} m{113pt} %0.95\linewidth}
    %   }
    %\noindent\textcolor{ForestGreen}{\RaggedLeft// Precondition}\newline
    % \centering\arraybackslash $\mathsf{visit(i0, scbFin)}$ \\[2pt]
    % \hline
    % 
    \hlt{\noindent$\mathsf{dst\;SUB\_scbFin(MUL^D\;i1)\!:}$}
    %\textcolor{ForestGreen}{// Leakage function} 
    \newline
        \indent$\;\;\mathsf{\textcolor{blue}{return}\;ite((}$\hlt{$\mathsf{i1.\itarg{arg0}}$}$\mathsf{\;== 0)\;\vee}$ \newline
        \indent$\;\;\;\;\mathsf{(}$\hlt{$\mathsf{i1.\itarg{arg1}}$}$\mathsf{ \;== 0)\vee i1.cmt, }$\newline
        % rdy should be seomthing like atH(i1) 
        \indent$\;\;\;\;$\hlt{$\mathsf{\{scbCmt\},}$}\hlt{$\mathsf{\{scbFin\}}$}$\mathsf{)}$
        %\newline
        %%$\mathsf{(path\_id == 1), }$\newline 
        %\indent$\;\;\;\;$\hlt{$\mathsf{
        %%\{mulUFin\}, 
        %\{mulU\}}$}$\mathsf{))}$
        %\indent$\;\;\mathsf{path\_id = ((}$\hlt{$\mathsf{i1.\itarg{arg0}}$}$\mathsf{ == 0)\;\vee}$\newline 
        %\indent$\;\;\;\;\mathsf{(}$\hlt{$\mathsf{i1.\itarg{arg1}}$}$\mathsf{ \;== 0))}$ \newline
        %\indent$\;\;\mathsf{\textcolor{blue}{return}\;ite((path\_id == 1), 
        %}$\newline
        %\indent$\;\;\;\;$\hlt{$\mathsf{\{scbCommit\}, \{scbFin\}}$}$\mathsf{)}$
    %\end{tabular}
    %}
    %\\[3pt]
    \end{tcolorbox}  
    %\vspace{10pt}
    \caption{\hlt{(Abstract)} leakage functions for \inst{MUL}/\inst{SUB}.{{\textcolor{orange}{\tiny[Yao: to myself, add text back]}}}}
    % \yao{TOFIX mathsf in cls is normal font}}
    \label{fig:leak_fun_muladd}
      %\noindent\textcolor{ForestGreen}{{\RaggedLeft// \textbf{Zero-skip multiply:} MUL in mulU fast/slow(1/0) path if it has zero operands}}\\
    
\end{subfigure}
%(a ``distinguished'' path selector function)
\caption{%leakage functions for \inst{MUL} and \inst{SUB}.
% Leakage functions for \inst{MUL} and \inst{SUB}.
Zero-skip 
\inst{MUL} takes a fast/slow \upath{}. In the latter case, it may stall a finished \inst{SUB} for one to three cycles.
% \\ {\footnotesize $dst$ $\mathsf{dst}$} $dst$ $\mathsf{dst}$% (\inst{m}: scoreboard size).
% \yao{Updated leakage function: add signals to indicate some uarch dependence..} \caroline{@Yao, make sure we have terms like hdRdy briefly defined.}
% \yao{fixed}
% \yao{l-font}
}
% takes a fast/slow \upath{} due to \textit{zero-skip}~\cite{arm:arm}; a completed \inst{SUB} may stall one to three extra cycles ($n$ = scoreboard size).
% on top of waiting for other instructions in the scoreboard (size $n$) to commit.
%    }
    \label{fig:zero-skip-example}
%\end{framed}
\end{figure}

% \noindent \textbf{Specification Challenge.}
We identify a fundamental limitation of \ct{} contracts.
% based on transmit instructions.
Specifically, the slowing of Moore's Law encourages
bespoke data-dependent hardware optimizations to maintain performance gains.
This phenomenon will soon render \textit{all instruction operands unsafe by default}~\cite{pandora:isca:21}.
Without ISA support, safe programming will be impossible.
% \nikos{Can't we claim that safe programming without ISA support is already impossible?}
With dedicated hardware features (à la DIT, DOIT, Zkt), increasingly poor performance of safe code compared to unsafe code will 
% become increasingly pronounced, 
discourage safe programming in practice~\cite{linuxct}. 
% advantages of safe code over unsafe code will become increasingly significant,  gap between safe and unsafe code will continue to widen, discouraging the~\cite{linuxct}.

% \subsubsection{The Leakage Contract Specification Challenge}
\label{sec:intro:this-paper:spec-challenge}


\textbf{Insight 1: Leakage is Circumstantial.}
% Our first insight, however, is
The phenomenon above follows from the ``all or nothing'' nature of \ct{} contracts:
% Current transmitter-centric leakage contracts are ``all or nothing.''
% That is,
instruction operands are \textit{entirely} safe or unsafe. 
However, we find that transmit instructions leak their unsafe operands in \textit{certain circumstances}.
% (\S\ref{todo}).
% We consider three primary scenarios.

For example, 
% it may be safe for a transmit instruction to process specific \textit{operand values}.
% of transmit instructions may be more unsafe than others.
consider a 32-bit multiply ($\mathtt{MUL}$) instruction executing on a processor whose multiplication unit ($\mathtt{mulU}$) implements the canonical \textit{zero-skip} optimization~\cite{andrysco:subnormal,Mult_leaky}. 
A $\mathtt{MUL}$ will spend a \textit{single} cycle in the $\mathtt{mulU}$ if it has at least one zero operand; else, it will spend a \textit{few} cycles~\cite{arm7TDMI}. %multiplier}.
% A $\mathtt{MUL}$ wih zero operand, it will spend a \textit{single} cycle in the multiplication unit. Otherwise, it will spend a \textit{few} cycles~\cite{arm-multiplier}.
Such a $\mathtt{MUL}$ is a transmit instruction: it modulates a channel (hardware resource) in the
% exhibits operand-dependent hardware resource usage with respect to the
$\mathtt{mulU}$ in an operand-dependent manner.
% in a transmitter-centric leakage contract.
% , such a $\mathtt{MUL}$ is a transmitter.
% classify 
However, if we can arrange for only non-zero values to be passed to \inst{MUL} operands, its usage is safe.
% a receiver that observes this channel, say by timing a $\mathtt{MUL}$'s execution latency,
% learns much more from a fast operation
% (at least one operand is zero) than a slow one (both operands are one of $2^{32}-1$ non-zero values).
% Hence, it is safe to pass non-zero secrets to these $\mathtt{MUL}$s.
% a 64-bit $\mathtt{MUL}$, say by timing its execution latency,
% all other $\mathtt{MUL}$s will spend a few cycles~\cite{arm-multiplier}.
% Transmitter-centric leakage contracts would flag $\mathtt{MUL}$ as a transmit instruction. Yet 
% \chris{how about we say: as long as we can arrange for only non-zeros or only zeros to be passed as mul operands, mul's usage is safe. ("more unsafe" sounds program dependent)}
% Arm multiplier cycle counts: https://developer.arm.com/documentation/ddi0180/a/instruction-cycle-summary-and-interlocks/instruction-cycle-times/multiplier-cycle-counts

% Consider an arithmetic-logic unit ($\mathtt{ALU}$) which supports \textit{operand packing}~\cite{gong:operand-packing,Gruss:cachetemplateattacks}. Respecting dependencies, if a pair of in-flight instructions in its reservation station ($\mathtt{aluRS}$) perform the same operation and feature narrow width operands (e.g., 32 bits or less for a 64-bit operation), they will be \textit{executed together}. Otherwise, they will be \textit{serialized} at the $\mathtt{ALU}$. 
% Such instructions are transmit instructions; they modulate a channel in the 
% % exhibit operand-dependent hardware resource usage within the
% $\mathtt{aluRS}$ in an operand-dependent manner.
% However, a receiver that observes this channel, say by timing an $\mathtt{SUB}$, learns a function of the $\mathtt{SUB}$'s operands only on a fast operation (the upper halves of its operands and the operands of another $\mathtt{SUB}$ it was merged with are zero).
% A slow $\mathtt{SUB}$, in contrast,
% % If a receiver observes 64-bit $\mathtt{SUB}$ (again, via timing), a fast operation indicates
% % % it can deduce
% % that the upper halves of its operands and the operands of another $\mathtt{SUB}$ it was merged with are zero.
% % A slow $\mathtt{SUB}$
% indicates that the upper halves of at least one of its operands \textit{may be} non-zero \textit{or} 
% % that operand-packing was not possible.
% % 
% that another $\mathtt{SUB}$ was not eligible to be packed together with it.
% Thus, a secret-dependent $\mathtt{ALU}$ instruction is safe
% % never co-resident in the ALU's reservation station.
% % ALU instructions are safe
% if it never resides in the $\mathtt{aluRS}$ with an identical operation.
% ALU operations can safely process secrets as long as scheduling decisions ensure that operand packing is never possible for a secret-dependent instruction it its reservation station.
% as long as a pair of identical ALU operations, where at least one is secret-dependent, can never resid
% ALU operation will never reside in the A  is safe as long as it is guaranteed to never be co-resident in the reservation station with an identical operation.

% Third, for a program with secret-dependent transmit instructions, certain \textit{receiver assumptions} may alleviate leakage in practice~\cite{metior}.
% % For example, consider an attacker (the receiver) that \textit{passively} monitors versus \textit{actively} engages with a victim's execution (\S\ref{sec:background:passive-active}).
% Suppose a receiver can directly time its own individual instructions but can only observe end-to-end execution time of a victim.
% Now, consider an 
% For the zero-skip multiply and operand packing examples, suppose that a receiver can directly time its own individual instructions but not the victim's.
% % cannot directly time individual.
% % victim $\mathtt{MUL}$s or $\mathtt{SUB}$s, respectively.
% Instead, it can \textit{passively} observe end-to-end victim program execution time or \textit{actively} 


% a passive attacker that observes end-to-end victim execution time may not be able reconstruct a program secret. However 
% \textit{active} attacker that interacts with the victim versus a \textit{passive} attacker that 


% it does not reach the reservation together with an identical operation.
% s may safely process secrets as long a secret-dependent the reservation station together.
% that the opportunity for operand-packing did not arise.
% another $\mathtt{SUB}$ was never co-resident in the ALU's reservation station.
% the opportunity for operand-packing did not arise.
% Thus, it is safe to supply secrets to such ALU operations as long as they are never co-resident in the ALU's reservation station.
% of the same instruction are ready to be issued in the same cycle, \textit{and} they operate on 
% Circumstance: particular scheduling decisions. It may also be okay for a transmitter to process a secret if a transmitter is spaced sufficiently far from some other instructions. E.g., Operand-packing: safe to process a secret if the same ops don’t reach the functional unit simultaneously. 

% consider the RISC-V $\mathtt{DIV}$ instruction as implemented on the CVA6 CPU~\cite{cva6}---a 64-bit, 6-stage, single-issue RISC-V core featuring speculation and limited out-of-order write-back (Fig.~\ref{}).




% \caroline{Left off here}
% All we need to do is ensure that a sensitive operand isn't 0 and multiply becomes safe again!

% Example: Multiply-zero-skip.  All we need to do is ensure that a sensitive operand isn't 0 and multiply becomes safe again!
% We propose Tspec models: precise yet abstract specifications that describe the necessary conditions for a transmit instruction to leak specific functions of its operands.
% The technical core of the paper develops a semantics that is sufficient to express the categories of conditions required for transmitters to leak, yet sufficiently abstract to hide microarchitectural details.
% We further show how our semantics enables a formal verification procedure capable of efficiently discovering (and synthesizing) Tspec constracts, given processor RTL as input.
% The above is non-trivial.  E.g., packed operands depend on understanding when multiple instructions can be in-flight together.


% Industry-backed \leakagecontracts{} are a step in the right direction. Yet, 
% % we identify and address
% % 
% % (at least)
% two important challenges that remain.
% First, state-of-the-art \leakagecontracts{} themselves exhibit several limitations---the \textit{Specification Challenge} (\S\ref{}).
% Most notably, they are \textit{transmitter-centric}, classifying instruction operands as entirely safe or unsafe.
% % highlights several limitations of ISA \leakagecontracts{} themselves. 
% % First, state-of-the-art \leakagecontracts{} are limited along a few dimensions---the \textit{Specification Challenge}.
% % For example, they are \textit{transmitter-centric}, classifying instruction operands as entirely safe or unsafe; target \textit{dynamic leakage}, protecting instructions' data operands only when the are actively in-use; and are\textit{threat model-specific}, exclusively targeting hardware side-channel leakage that manifests as execution time variability for a victim program.
% % ---the \textit{Specification Challenge}.
% % , and \textit{timing-specific}, targeting side-channel leakage that manifests as execution time variability for a victim program.
% % \caroline{Nothing about the effect on other instructions. Spec is fine, its limited, its by no means anywhere close to where we want to be.}
% % For example, all instruction operands are unsafe except for some specific instructions' data operands when executed in a \textit{slower} DIT/DOIT/Zkt mode.
% On advanced microarchitecture, the performance impact of this ``all-or-nothing'' approach
% %transmitter-centric and dynamic \leakagecontracts{}
% will be increasingly significant. Nearly all instruction operands may be unsafe be default~\cite{pandora:isca:21} with
% % making the performance impact of
% % . That is, nearly every instruction will t, discouraging use of
% secure processor modes and extensions disabling \textit{many} culprit hardware optimizations~\cite{lwn-doit}.
% % Plus, instructions which feature  \textit{static} 
% % Plus, a threat model-specific contract is easily voided when fundamental receiver assumptions are violated.
% % Second, ISA \leakagecontracts{} are \textit{receiver-specific}, targeting side-channel leakage that manifests as execution time variability for a victim program---the \textit{}.
% % approach directly translates to significant performance overhead associated with DIT/DOIT/Zkt mode will be increasingly significant. 
% % Such a coarse-grained approach can easily render all instructions unusable for safely processing secrets on advanced microarchitecture~\cite{pandora:isca:21}---the \textit{specification challenge}.
% % , rather than exposing \textit{culprit microarchitecture} (to support hardware designers) or precise \textit{leakage functions} (to support programmers).
% Second, a sound and complete approach for \textit{formally verifying} microarchitectural compliance with state-of-the-art leakage contracts remains elusive---the \textit{Verification Challenge}.

% \subsection{This Paper}
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=.5\linewidth]{isca2023-latex-template/figs/op-packing-uhb.png}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}


% This paper addresses the Specification and Verification Challenges via a novel class of leakage contracts, called \textit{\tspec{} models}, and an automated approach and tool for synthesizing \tspec{} models from processor RTL, called \tsynth{}. 



% \textbf{\tspec{} Models}
% Two key observations lead us to propose \tspec{} models as an alternative to standard \leakagecontracts{}.

% Our \textbf{first observation} is that transmitter-centric \leakagecontracts{} fail to expose opportunities for designing more precise and performant hardware side-channel defenses.
% Observe that if an $\mathtt{SUB}$ is never co-resident in instruction decode with another $\mathtt{SUB}$, the path selector function in Fig.~\ref{} reduces to $\mathtt{return(add.rdy)}$, which is \textit{operand-independent}. Given our CVA6 variant,
% %it is actually safe to supply secrets to the operands of $\mathtt{SUB}$s, as long as they are never co-resident with other $\mathtt{SUB}$s in the decode stage.
% % In our CVA6 variant, 
% a hardware side-channel defense could \textit{allow} secret-dependent $\mathtt{SUB}$s and \textit{disallow} multiple $\mathtt{SUB}$s in decode.
% % are never sent to decode with another $\mathtt{SUB}$.
% % More generally, 
% % (in hardware and software).



% Our second insight is that precisely defining the circumstances under which a transmit instruction leaks its operand(s) requires extending the transmitter-channel-receiver analogy with a new primitive to encode how channel modulations manifest as receiver observations. In particular, a receiver observes channel modulations indirectly through their (measurable) effects on the execution behavior of “special” instructions executed by the victim or itself. In this paper, we name such instructions transponder instructions, or simply transponders. More formally, a transponder is any instruction that exhibits microarchitectural execution path (\upath{}) variability as a direct result of a transmitter modulating a channel in an operand-dependent manner.

% \subsubsection{\tspec{} Models}


% By making programmers aware of these circumstances, we give them the ability to use transmit instructions for processing secrets \textit{safely}!

% \paragraph{Transponders: The Missing Enabler of Hardware Side-Channel Attacks}

% Exposing the circumstances under which transmit instructions leak their operand(s) has a couple key benefits. First, we give programmers the ability to use transmit instructions for processing secrets safely! Second, we give hardware designers the ability to enforce the safe execution of secret-dependent transmit instructions without blanket-disabling advanced performance optimizations.
\textbf{Insight 2: \upaths{} Enable Channel Observations.}
% \chris{"UPaths enable channel observations"}
% \chris{Not clear whether the next sentence is referring to the preious para or later text.  How about: We develop a formalism and automated analysis that captures and capitalizes on context-dependent leakage such as the mul example above.}
% \caroline{This sentence now feels out of places to me:}
To enable hardware side-channel defenses to
% We develop a formalism and automated verification procedure that capture and
capitalize on circumstantial leakage, as in the \inst{MUL} example above, we develop a formalism that captures the conditions
% By making hardware side-channel defenses aware of the conditions
under which transmit instructions leak their operand(s).
% , we can enable them
% can give them the ability
% to use transmit instructions for processing secrets \textit{safely}!
% \nikos{I am reading this again. Before we made the point that due to advanced hardware optimizations nearly all instructions leak information about their operands, in such a world knowing the per channel leakage functions doesn't really help program safely, it just highlights/quantifies the true risks.}
Intuitively, such conditions can be captured by per-channel \textit{leakage functions} that map the \textit{operand space(s)} of transmit instruction(s) that modulate a channel onto the \textit{observation space} of a receiver that observes it.
However, defining such functions 
is complicated by vague notions
in the literature of channels themselves, how their modulation is controlled by transmit instruction operands, and how their modulation manifests as receiver observations.
A recent attempt to resolve some of these issues writes down leakage functions manually~\cite{pandora:isca:21}.
Instead, we leverage the concept of \textit{microarchitectural execution paths} (\upaths{}), inspired by prior work~\cite{pipecheck, ccicheck, coatcheck, rtlcheck, checkmate, rtl2uspec:hsiao:2021}, to make these notions precise and support inferring leakage functions from RTL automatically.

% I would say that leave doesn't do anything with leakage functions. It has an observer model only - e.g., commit signal is observable.
% \chris{would it be accurate to say leakage functions are written down manually today? (eg pandora, LEAVE).  we want to automatically infer them.}
% \yao{concretized $\downarrow$}
% is not straightforward, since a pre characterization of how channel modulations m
% moddefinition of how channe 
% notion of a channel as well as how channel modulations manifest as receiver observations not precsiely defined in the literature.

% fist requires formalizing the notion of a channel as well as how channel modulations manifest as receiver observations.
% prior work leaves the notion of a channel highly abstract (it is a)

% s space.
% a transmit instruction's operand space onto a receiver observation space.
% However, 
%  space.

% However, defining these leakage functions is not straightforward.
% The main reason is that we don't have a formal notion of how channel modulations manifest as receiver observations. This means that the output space of such a leakage function is not well-defined.
% It also makes it difficult to articulate scheduling conditions. 
% Moreover, channel modulations typically involve interactions between multiple instructions (e.g., in the operand packing example). 
% Same transmitter may modulate moltiple channesl


% One reason is that we don't have a formal notion to describe how channel modulations manifest as receiver observations. Above we give some intuitive notion of fast and slow paths for particular instructions. Another reason is that we don't have a formal notion 

% However, doing so naïvely fails to cap


% For some transmit instructions, like the $\mathtt{MUL}$ above, this information can be captured
% Some of this information (e.g., operand value conditions) can be captured though \textit{leakage functions} that map the space of transmit instruction inputs onto distinct 
% leakage function isn't enough - we need to know how 


% requires extending the transmitter-channel-receiver analogy with a new primitive to encode \textit{how} channel modulations manifest as receiver observations. 
% defining the circumstances under which a transmit instruction leaks its operand(s)

% Exposing this information, however,
% % our second insight is that precisely exposing such information
% requires a formal definition of how channel modulations manifest as receiver observations---something that is not captured by the established transmitter-channel-receiver taxonomy.
% observe that above challenge can alleviated
%\rsout{made more concrete}\yao{

In particular, we observe that a transmit instruction's execution creates \upath{} variability for one or more \textit{transponder instructions}, or simply \textit{transponders},\footnote{In telecommunications~\cite{roddy2006satellite}, ``a transponder is the series of interconnected units which forms a single communications channel between the receive and transmit antennas in a communications satellite.''}
% We find that these notions can be made precise by adding
% To address this challenge, we propose adding a 
% We find that we can resolve this complication  by 
% a new primitive to the transmitter-channel-receiver taxonomy.
% Specifically, we observe that distinct channel modulations on behalf of a victim transmit instruction 
% (in the victim)
% create 
% when a transmit instruction modulates a channel, it creates
% distinct \textit{microarchitectural execution paths} (\upath{}s, \S\ref{sec:tspec:upaths}) for ``special''
executed by the victim or receiver.
% Clearly, a receiver (the attacker) does not peer into a processor and \textit{directly} observe operand-dependent channel modulations (hardware resource usage) on behalf of transmit instructions (in the victim).
% Rather, a receiver observes channel modulations \textit{indirectly} through their (measurable) effects on the
% \textit{microarchitectural execution behavior of instructions} executed by the victim or itself.
% We call these special instructions
% We name such instructions 
% , possibly including the transmit instruction itself.
A receiver ultimately observes 
a transmit instruction's channel modulations
% ,
% and infers its operands,
by detecting which \upath(s) its transponder(s) took at runtime, e.g., by measuring transponder execution time.
Thus, a leakage function (Fig.~\ref{fig:leak_fun_muladd}) can define how a channel, modulated by transmit instructions (function arguments), creates \upath{} variability (function outputs) for a transponder with respect to some phase of the transponder's execution (function name).
% A leakage function (Fig.~\ref{fig:leak_fun_muladd}) \textit{characterizes a channel} whose modulation creates \upath{} variability for a transponder. Its inputs are subscript-labeled transmit instructions, and its output is a distinct channel modulation encoded as the next-cycle execution phase(s) in the transponder's \upath{}.
% \chris{Suggestion: Start this paragraph saying utilize the uPath abstraction to automatically infer the leakage functions.  A key observation is that at the level of uPaths, a transmitter's execution creates uPath variations for other instructions called transponders.}


For example, Fig.~\ref{fig:zero-skip-uhb} shows \upaths{} for 32-bit $\mathtt{MUL}$ and $\mathtt{SUB}$ instructions executing on a variant of the RISC-V CVA6 CPU~\cite{cva6} that implements zero-skip multiplies~\cite{andrysco:subnormal,Mult_leaky}.
A $\mathtt{MUL}$ (transmit instruction) creates multiple \upaths{} for itself---it may spend one or four cycles computing its result in the $\mathtt{mulU}$. 
More subtly, a $\mathtt{MUL}$ creates multiple \upaths{} for concurrently in-flight $\mathtt{SUB}$s---a completed $\mathtt{SUB}$ may remain in the $\mathtt{scbFin}$ execution phase for one to three extra cycles before committing (three in Fig.~\ref{fig:zero-skip-uhb}).
% ) may be be forced to wait one to three additionally cycles before committing.
% it may conditionally delay their commit times by one to three cycles.
Hence, $\mathtt{MUL}$ transmitters implicate themselves \textit{and} $\mathtt{SUB}$s as transponders.
The top (bottom) leakage function in Fig.\ref{fig:leak_fun_muladd} defines how a channel modulated by a \inst{MUL} creates \upath{} variability for itself (a concurrently in-flight \inst{SUB}) with respect to its \inst{mulU} (the \inst{SUB}'s \inst{scbFin}) execution phase.
% , i.e., $\mathtt{MUL}$'s leak their operands to receivers who can their own or other 
% \caroline{Figure.}

%
% sdo needs to equivalence class information
% stt needs the set of all "interaction" among transmitter and transponder pairs or explicit branch
%}

\textbf{Insight 3: \upaths{} Enable Leakage Contract Synthesis.}
% \chris{see previous comment: I think we can hoist this point to earlier.}
A key benefit of \upaths{} and transponders is that they enable an automated procedure for synthesizing leakage functions from processor RTL
% In designing \tsynth{}, our third insight is that the notions of \upaths{} and transponders enable a leakage contract synthesis procedure
that relies \textit{primarily} on evaluating simple \textit{(single-)trace properties} on the design under verification (DUV). 
% \tsynth{}'s theoretical guarantees, automation, and scalability follow from the fact that it primarily relies on evaluating simple \textit{trace properties} on the design under verification (DUV).
% \footnote{We use the term \textit{contract verification} to encompass both \textit{contract satisfaction}.}
In contrast, all existing leakage contract verification
approaches, which target \ct{} contracts, \textit{exclusively} evaluate \textit{2-safety hyperproperties}~\cite{gleissenthall:iodine,gleissenthall:xenon,wang2023specification,deutschmann:upec-do, deutschmann2023scalable}.


% To make transponders more concrete, consider the aforementioned zero-skip optimization which implicates $\mathtt{MUL}$s as transmit instructions. As a function of its operands, a $\mathtt{MUL}$ creates a fast or slow path for itself. Hence, $\mathtt{MUL}$s are also transponders. Moreover, a $\mathtt{MUL}$ can create fast or slow paths for some subsequent instructions as function of its operands by conditionally delaying their commit times. Thus, all such instructs are also transponders.



% We say that a transponder is ``is part of the channel'' created by 
% A receiver infers a transmit instruction's operands, by deducing which \upath{} one of its transponder took at runtime.


% As a function of its own operands, a $\mathtt{MUL}$
% % The two left-most \upaths{} illustrate that $\mathtt{MUL}$s
% may spend one to four cycles computing its result in the multiplication unit ($\mathtt{mulU}$), yielding two \upath{} possibilities.
% Also as a function of a $\mathtt{MUL}$'s operands, a concurrently in-flight $\mathtt{SUB}$ may spend zero to three extra cycles in the scoreboard before it commits.
% That is, an $\mathtt{SUB}$ may be blocked from committing by a $\mathtt{MUL}$.


% As a function of a concurrently in-flight $\mathtt{MUL}$s, an 
% The remaining \upaths{} show that $\mathtt{SUB}$s may spend zero to three cycles, once completed, in the scoreboard before they commit.




% As we later explain (\S\ref{}), \upath{} variability for a $\mathtt{MUL}$ on this design results from the $\mathtt{MUL}$ itself modulating a channel during its first cycle in the $\mathtt{mulUnit}$.
% \upath{} variability for an  $\mathtt{SUB}$ results from a concurrently in-flight $\mathtt{MUL}$ modulating a channel while the $\mathtt{SUB}$ is completed in the scoreboard ($\mathtt{SCB.complete}$).
% phase of its execution.
% Hence, we say that $\mathtt{MUL}$'s transponders include itself and an

% As we later explain (\S\ref{}), the \upath{} variability for $\mathtt{MUL}$s and $\mathtt{SUB}$s on this processor var 

% \upath{} variability for a $\mathtt{MUL}$ can be attributed to a channel that is modulated when 
% % \upath{} variability for a $\mathtt{MUL}$ or $\mathtt{SUB}$ on this processor variant can both be attributed to the $\mathtt{MUL}



% A single transmit instruction may modulate one or more channels. 


% create a transponder is an instruction that exhibits \textit{microarchitectural execution path} (\upath{}, \S\ref{}) variability as a direct result of a transmit instruction modulating a channel in an operand-dependent manner. Notably, a transmit instruction creates \upath{} variability for one or more transponder instructions, possibly including itself.


% Exposing this information, however,
% % our second insight is that precisely exposing such information
% requires a formal definition of how channel modulations manifest as receiver observations---something that is not captured by the established transmitter-channel-receiver taxonomy.

 % CVA6 is a 64-bit, 6-stage, single-issue RISC-V core featuring speculation, diversified functional units, and limited out-of-order write back (Fig.~\ref{fig:cva6}).
% Informally, nodes represent instruction execution \textit{phases}, and edges encode \textit{one-cycle happens-before} orderings~\cite{lamport:happensbefore}.
% Thus, the execution latency (from $\mathtt{IF}$ to  $\mathtt{SCB.commit}$) of the left (right) path is four (eight) cycles.

% Consider the two left-most \upaths{} for $\mathtt{MUL}$s.
% The yellow nodes, which represent a $\mathtt{MUL}$'s first cycle in the $\mathtt{mulUnit}$s, are the source of a \textit{path divergence}---visually, the yellow nodes are followed by distinct nodes, colored green, in the two paths.
% Such a path divergence arises from a channel modulation.
% We use a notion of execution paths 



% In this paper, we associate channels with \upath{} divergences. Like that following the $\mathtt{mulUnit.mul}$ node for the $\mathtt{MUL}$'s \upaths{}. 

% The \textit{path divergence} illustrates that a channel is modulated when 


% From our previous explanation of the zero-skip optimization, it is clear that $\mathtt{MUL}$s modulate state in the $\mathtt{mulUnit}$ in an operand-dependent manner.
% Fig.~\ref{fig:zero-skip-example} shows that this modulation yields two \upath{} possibilities for $\mathtt{MUL}$s. We can define a leakage function that maps its operand space
% % This is because an $\mathtt{SUB}$ may be blocked from committing by an older $\mathtt{MUL}$.
% \caroline{Do we need to make any assumptions on ROB size here?}


% Comparing $\mathtt{MUL}$ paths, we not a \textit{path divergence} originating at



% in the completion state of the score 

% Intuitively, $\mathtt{MUL}$s are transmit instructions due to their operand-dependent hardware resource usage within the multiplication unit. 






% Give our first two insights, we propose
\textbf{Putting it all Together.}
% \yao{Should \pct{} Contracts?}
Based on our three insights, we first propose novel 
% our solution to the leakage contract specification challenge:
% \textit{transponder-centric} 
leakage contracts, called \textit{permissive constant-time (\pct{}) contracts}. 
Like \ct{} contracts, \pct{} contracts identify a microarchitecture's \textit{transmit instructions} and their \textit{unsafe operands}. Plus, they define specific \textit{leakage conditions} that render said operands unsafe.
%\yao{implicate the execution of transponders and} 

% \yao{The set of unsafe operands of transmitters support traditional CT programming; further, the set of leakage conditions }

% Note that \ct{} contracts are a class of PCT contracts where all leakage conditions are $true$.
% \chris{move the prev/last sentence to the end of the next para}
We find that \pct{} contracts with precise leakage conditions, related to transmit instruction \textit{operand values} and microarchitectural \textit{scheduling decisions}, can be derived
% by first identifying
% \tspec{} models have a the following defining features.
% First, 
% \tspec{} models
% they
% enumerate a
from a microarchitecture's leakage functions, which can be synthesized from RTL.
%pct{} contracts can support hardware side-channel defense in various ways. 
% which 
% a microarchitecture's \textit{transponders} and then constructing a comprehensive set of \textit{leakage functions} for each.
% ---instructions whose \upaths{} a receiver must observe to infer transmit instruction operands.
% . To infer a transmit instruction's operands, a receiver must deduce which \upath{} some transponder realized at runtime.
% instructions whose \upaths{} expose transmit instruction operands to a receiver that observes them.
% execution behavior a receiver must observe to infer transmit instruction operands.
% Second, for each transponder, \tspec{} models 
% \chris{the next few sentences are a bit intense for the intro.  if there is any way to depict the leakage function w/o getting into notation for intro, I suggest we do it.}
% A leakage function (Fig.~\ref{fig:leak_fun_muladd}) \textit{characterizes a channel} whose modulation creates \upath{} variability for a transponder. Its inputs are subscript-labeled transmit instructions, and its output is a distinct channel modulation encoded as the next-cycle execution phase(s) in the transponder's \upath{}.
% \textit{encoded as a particular \upath{}}.
% capture
% The function body captures
% leakage conditions related to transmit instruction \textit{operand values} and 
% .
% Input labels capture leakage conditions related to
% microarchitectural \textit{scheduling decisions}.
%denote circumstantial leakage related to particular
% or the use of selective microarchitectural \textit{state obfuscation}.
% In our zero-skip example, a $\mathtt{MUL}$ is both an intrinsic and dynamic (w.r.t. $\mathtt{SUB}$ transponders) transmit instruction.

% Fig.~\ref{} illustrates leakage functions for $\mathtt{MUL}$ and $\mathtt{SUB}$ transponders.
% \yao{leakage function output type is possibly not a path but segment of a set of paths though? Or it should be fine as it will be clarified?}

% is denoted by labeling function inputs 
% Its output 
% % is an integer identifier that
% encodes a particular channel modulation, and its inputs are transmit instructions whose operand values control its output.
% \tspec{} models 
% The function body captures circumstantial leakage related to particular transmit instruction operand values.
% Meanwhile, function inputs are dynamic \textit{scheduling decisions}
% thr
% \tspec{} models additionally classify a leakage function's inputs (transmit instructions) according to the circumstances under which they can create \upath{} variability for its associated transponder. 

% that illustrate this fact.

% \caroline{TODO}
% In our running zero-skip multiplier example, MUL, SUB, SUB, … are implicated as transponders. For MUL, its leakage function definition indicates that MULs leak their own operands – they are intrinsic transmit instructions. With respect to the SUB, SUB, …,  transponders, MUL is a dynamic transmit instruction. The function body precisely encodes how the space of transmitter operand values maps onto the channel modulation space. The function definition encodes the impact of scheduling decisions on leakage.

% These distinctions indicate whether a transponder's execution behavior is impacted by its own operands, the operands of a 

% Concretely, \tspec{} models enumerate a microarchitecture's \textit{transponders} and a set of \textit{leakage functions} for each.
% Given a transponder, each associated leakage function precisely models a channel whose modulation creates \upath{} variability within the transponder.

% A leakage function outputs a \upath{} identifier, which directs the execution behavior of the transponder.
% Leakage function inputs are instructions, including any transmit instructions whose operands influence its outputs.
% Moreover, \tspec{} models classify leakage function inputs as \textit{dynamic} (concurrently in-flight) or \textit{static} (previously in-flight) 


% \tspec{} models precisely capture how channel modulations are made visible to receivers (by exposing transponders) and the conditions under which channels can be modulated (by exposing leakage functions and characterizing leakage instruciton inputs as static/dynamic).

% The range of a leakage function indicates the number of distinct channel modulations.
% and thus the degree of \upath{} variability.
% transmit instructions 
% In a nutshell, a leakage function precisely describes how a enables hardware side-channel defenses that are tailored to particular \textit{threat models}, or which \textit{conditionally} pass secrets to transmit instructions or \textit{periodically} obfuscate hardware state.

% may leak to a receiver who observes the transponders execution behavior.
% Leakage function arguments are instructions  transmit instructions which leak their 
% , which are distinguished as the \textit{transponder} itself or other \textit{dynamic} (concurrently in-flight) or \textit{static} (previously in-flight).
% In a nutshell, a leakage function precisely describes how a enables hardware side-channel defenses that are tailored to particular \textit{threat models}, or which \textit{conditionally} pass secrets to transmit instructions or \textit{periodically} obfuscate hardware state.


% Concretely, \tspec{} models enumerate a microarchitecture's transponders, and a set of \textit{leakage functions} for each.
% % Given our observations, \tspec{} models are \textit{transponder-centric}, enumerating transponders and a set of leakage functions for each. 
% Leakage function arguments are transmit instructions, which are distinguished as the \textit{transponder} itself or other \textit{dynamic} (concurrently in-flight) or \textit{static} (previously in-flight).
% In a nutshell, a leakage function precisely describes how a enables hardware side-channel defenses that are tailored to particular \textit{threat models}, or which \textit{conditionally} pass secrets to transmit instructions or \textit{periodically} obfuscate hardware state.
% ($\mathtt{OP_T}$) or other \textit{dynamic} ($\mathtt{OP_D}$) or \textit{static} ($\mathtt{OP_S}$) instructions that it may interact with. Classifying arguments in this way
% indicates whether a transponder can expose its own operands or the operands of previously executed (static) or concurrently in-flight (dynamic) instructions.
% This information in turn




% However, our \textbf{second observation} is that the telecommunications analogy for characterizing hardware side-channel attacks---featuring a transmitter, channel, and receiver---is missing a key component.
% Clearly, a receiver does not \textit{directly} observe operand-dependent channel modulations (hardware resource usage) on behalf of transmit instructions (in the victim).
% Rather, channel modulations are observed \textit{indirectly} through their (measurable) effects on the execution behavior of ``special'' instructions (executed by the victim \textit{or} attacker).
% %, which we call 
% % In particular, secret-dependent channel modulations (hardware resource usage), induced transmit instructions (in the victim), are made visible to a receiver (the attacker) via their (measurable) effects on the dynamic execution behavior of \textit{other instructions}.
% % We call these other instructions
% In this paper, we name such instructions \textit{transponder instructions}, or simply \textit{transponders}.\footnote{``A transponder is the series of interconnected units which forms a single communications channel between the receive and transmit antennas in a communications satellite~\cite{roddy2006satellite}.''}
% % A transponder is any instruction that exhibits \textit{\upath{} variability} if and only if a transmit instruction modulates some channel.
% More formally, a transponder is any instruction that exhibits \textit{\upath{} variability} that can be ascribed to a leakage function---like the $\mathtt{SUB}$ in our motivating example.
% In our motivating example, an $\mathtt{SUB}$ is a transponder.
%, because it exhibits \upath{} variability (with respect to its $\mathtt{ID0}$ execution phase) that is associated with a leakage function (the one in Fig~\ref{fig:}).
% Further, an $\mathtt{SUB}$ instruction \textit{implicates} itself (i.e., its own dynamic instance) \textit{and} any dynamic $\mathtt{SUB}$ $\mathtt{i1}$ which is co-resident in the decode stage as transmit instructions. In other words, a receiver who can distinguish execution paths for an $\mathtt{SUB}$ may learn the data $\mathtt{SUB}$'s operands.
% The channel can be represented by the output of the leakage function.





% , which significantly advances the state-of-the-art in automated and formal guarantees.
% \tspec{} models extend transmitter-centric leakage contracts with details that express about 

% the precise mechanisms by which a transmit instruction leaks its operand(s) to a receiver via a channel.
% omit mechanistic descriptions of how hardware side-channel leakage manifests microarchitecturally.
% abstract away the mechanisms by which 
%
% 
% In particular, the following are not specified: 
% the mechanisms through which: 

% by a receiver based on observed channel modulations.
% how a receiver infers based on observed channel modulations.
% onto (a set of) inferred operand values.
% In particular,
% how a receiver (i) observes channel modulations and thereby (ii) infers a transmit instruction's operand(s) is not specified.

% the two mechanisms---(i) and (
%  still a huge scaling challeng - modern out of order cores

% augmenting state-of-the-art leakage contracts with these details enables more precise reasoning (by programmers \textit{and} hardware designers) about how microarchitecture impacts software security; \tspec{} models do just this.
% \caroline{Something like this somewhere: it may be safe to execute a transmit instruction with a secret operand under some circumstances, or in some programs.}
% Plus, it inspires a novel hardware verification approach.

% \tspec{} models are the first leakage contracts to incorporate both hardware side-channel leakage mechanisms---(i) and (ii)---above.

% Our \textbf{first insight} t
% In defining \tspec{} models, we make the important observation that the telecommunications analogy for characterizing hardware side-channel leakage---featuring a transmitter, channel, and receiver---is missing a key component.
% In particular, channel modulations (hardware resource usage), induced by a transmit instruction (in the victim), are made visible to a receiver (the attacker) \textit{via their (measurable) effects on the dynamic execution behavior of other instructions}.
% We call these ``other instructions'' \textit{transponder instructions}, or simply \textit{transponders}.\footnote{``A transponder is the series of interconnected units which forms a single communications channel between the receive and transmit antennas in a communications satellite~\cite{roddy2006satellite}.''}
% Informally, a transponder is any instruction whose \textit{microarchitectural execution path} is directly impacted by modulating some channel.
%; we say that a transponder is ``part of a channel.''
% We say that a transponder is ``part of the channel'' created by a transmitter.

% as a rule of thumb, the receiver (the attacker) cannot \textit{directly} observe channel modulations (hardware resource usage) on behalf of a transmit instruction (in the victim). Rather, the receiver \textit{indirectly} observes channel modulations via their measurable effect on the dynamic execution behavior of \textit{other instructions}, which 


% The arguments of such a leakage function are the operands of one or more transmit instructions; its range the number of distinct channel modulations.



% is equal to the degree of path variability it creates for the transponder.


% infer what input(s) could have induced the observed transponder execution path---(ii) above.
% , whose arguments are transmit instruction operands, 

% how operand values are inferred from observed channel modulations can be modeled with a per-transponder/module \textit{leakage function} associated with a channel, whose arguments are transmit instruction operands, to infer what input(s) could have induced the observed transponder execution path---(ii) above.


% The degree of path variability that a transponder exhibits with respect to a particular channel encodes the number of channel observations that a receiver may observer through the transponder.
% W.r.t. a particular channel, a receiver may 
 %With respect to a particular channel, the degree of path variability a transponder exhibits encodes the number of w of distinct observations that may be available to a receiver.

% , i.e., a $channel \rightarrow \{transponder_0, transponder_1, ...\}$ ---expressing mechanism (i). Notably, 


% multiple microarchitectural execution paths for one or more transponder instructions. Therefore, for each transmit instruction, mechanism (i) can be expressed as a \textit{set of transponders} for each channel it modulates.
% Second, 

% I.e., each channel modulation introduces some degree of path variability into a transponder instruction.
% A transponder may be be part of multiple channels.  



% First, each channel that a transmit instruction modulates can be represented as a \textit{set of transponders} which exhibit microarchitectural execution path variability as a result (i).


% can be represented as a set of transponderes 
% channel modulation manifests as multiple microarchitectural execution paths for one or more transponder instructions.

% Second, how some channel modulation is observed by a receiver can be encoded, per associated transponder, as the \textit{degree of path variability} that that the transponder may exhibit as as a result (ii).
% Third, how operand values are inferred from observed channel modulations can be modeled with a per-transponder/module \textit{leakage function} associated with a channel, whose arguments are transmit instruction operands, to infer what input(s) could have induced the observed transponder execution path---(ii) above.


% A transmitter modulates one or more channels in an operand-dependent manner.
% Each channel modulation manifests as multiple microarchitectural execution paths for one or more transponder instructions.
% I.e., each channel modulation introduces some degree of path variability into a transponder instruction.
% A transponder may be be part of multiple channels.  


% Each channle

% number of distinct execution paths each transponder may exhibit as a result (ii).
% Second, how operand values 
% as a list of transponder instruction which 
% Given the observation above, our \textbf{first key insight} is that a receiver observes a transmit instruction's operand-dependent channel modulations by deducing which \textit{microarchitectural execution path} its transponder(s) realized at runtime---(i) above.
% As we will show, 
% %a transmit instruction may be associated with more than one transponder instructions and vice versa.
% a transponder may be executed by the victim \textit{or} attacker, giving rise to side-channel leakage that is relevant for different threat models. Our \textbf{second key insight} is that a receiver leverages a \textit{leakage function} associated with a channel, whose arguments are transmit instruction operands, to infer what input(s) could have induced the observed transponder execution path---(ii) above.



% enables us to define \tspec{} models entirely in terms of hardware instructions and their operands.
% Specifically, we find that a receiver observes channel modulations by deducing which \textit{microarchitectural execution path} an \textit{amplifier instruction}, or simply \textit{amplifier} (our term), realized at runtime. An amplifier is any instruction whose execution path through a microarchitecture is directly impacted by modulating some channel.
% % That is, different channel modulations translate to different execution paths for the amplifier instruction at runtime.
% A receiver then leverages a \textit{leakage function} associated with the channel, whose arguments are transmit instruction operands, % to infer a set of operand values that 
% infer what input(s) could have induced the observed amplifier execution path.
% % We say that a transmit instruction modulates a channel in an operand-dependent manner, thereby directing the execution path of one or more amplifier instructions, which are deduced by a receiver.
% % We say that any such transmit instruction are ``
% % opvalues transmit instruction operands by mapping an observed path onto a set of operand values

% To make the notion of a \tspec{} model concrete, consider Fig.\ref{fig:zero-skip-example}, which features two microarchitectural execution paths for a multiply instruction (\texttt{MUL}) on a processor that implements a \textit{zero-skip multiplier}~\cite{}.
% % A \texttt{MUL} takes the left path if either of its operand is zero, else it takes the right path. 
% Note the yellow nodes, which represent a \texttt{MUL}'s first cycle in the \texttt{mulUnit} execution unit.
% It is clear that \textit{some} channel is modulated when \texttt{MUL}s enter the \texttt{mulUnit} due to the \textit{path divergence}---the yellow nodes are followed by different nodes, colored green, in the two paths.
% Suppose we know that if function $f_{mulUnit}(\texttt{MUL.arg0}, ~ \texttt{MUL.arg1}) \{ return(\texttt{MUL.arg0} == 0 ~||~ \texttt{MUL.arg1} == 0)\}$ returns one (zero), a \texttt{MUL} will take the left (right) path upon reaching the \texttt{mulUnit}.
% Because $f_{mulUnit}$ accepts instruction operands as augments (\texttt{MUL.arg0} and \texttt{MUL.arg1}), it is a \textit{leakage} function.
% Since $f_{mulUnit}$ is associated with a path divergence within the execution of \texttt{MUL}s, they are transponders. 
% In this (special) case, \texttt{MUL}s are transponders which implicate \textit{themselves} as transmit instructions---their own operands appear in the signature of $f_{mulUnit}$.
% Existing leakage contracts would flag \texttt{MUL}s as transmit instructions.
% \tspec{} models \textit{additionally} specify a tuple $\langle\texttt{MUL}, 2, f_{mulUnit}(\texttt{MUL.arg0}, ~ \texttt{MUL.arg1})~\{ return(...)\}\rangle$, indicating that a receiver who can differentiate between two execution paths of a \texttt{MUL} transponder learns a function of \texttt{MUL.arg0} and \texttt{MUL.arg1}, $f_{mulUnit}$.

% that a \texttt{MUL} modulate a channel (i) whose sole associated transponder is itself; (ii) which channel 

% a \texttt{MUL}'s sole transponder is itself, which 

% The operands of the leakage function implicate \texttt{MUL} as a transmit instruction, and the fact that \

% and \texttt{MUL} is a transponder---it exhibits microarchitectural execution path variability due to an an operand-dependent channel modulation.


% The arguments to this function (\texttt{MUL.arg0} and \texttt{MUL.arg1}) implicate \texttt{MUL}s as transmit instructions, and thereby render the function a \textit{leakage} function.
% % and render the funcntion a \textit{leakage function}. 
% Because the leakage function characterizes a channel modulation which directly impacts the execution behavior of \texttt{MUL}s, \texttt{MUL}s are also transponders.
% Putting it all together: \texttt{MUL}s are transmit instructions; their operand-dependent channel modulations implicate themselves as transponders; their channel modulations results in two observable execution path possibilities; and their operand values are inferred via the mulUnit funciton.

% may exhibit execution path variability due to a transmit instruction, 
% Moreover, \texttt{MUL} modulates a channel that creates variability within its


% However, since \texttt{MUL} exhibits execution path variability 

% decides whether a \texttt{MUL} takes the left or right path, 
% the left or right path is take  \tereturns one (zero), then the left (right) path is taken.
% The arguments to this function (\texttt{MUL.arg0} and \texttt{MUL.arg1}) implicate \texttt{MUL} itself as a transmit instruction


% It happens, that \texttt{MUL}'s operand-dependent channel modulation

% Hence, \texttt{MUL} is a transponder.
% %source of a \textit{path divergence}.
% % at which the two paths diverge:
% %, marked by the yellow nodes,
% %the \textit{path divergence} originating at the yellow node, which 
% % the yellow nodes, which represent \texttt{MUL}'s first cycle in the \texttt{mulUnit} functional unit, 
% % In particular, the yellow nodes are followed by different (green) nodes in the two paths.
% The following leakage function is associated with the channel: $mulUnit(\texttt{MUL.arg0}, ~ \texttt{MUL.arg1}) = (\texttt{MUL.arg0} == 0 ~||~ \texttt{MUL.arg1} == 0)$. Its arguments, implicate \texttt{MUL} itself as a transmit instruction; a transmit instruction and its transponder(s) \textit{may} be the same instruction as in this case. If the function returns one (zero), the left (right) path is taken.
% % If the function returns one, the left path is tak, else the left path is. Note that the rance of the function is two, 
% A receiver that can deduce which path is taken by a \texttt{MUL} at runtime (e.g., by measuring its execution time) learns the return value of this leakage function.

% In a nutshell, \tspec{} models are \textit{transponder-centric}. For each transponder instruction, \tspec{} models enumerate the \textit{degree} (how many divergent paths) and \textit{leakage function} associated with each path divergence it may exhibit. \tspec{} models are strictly richer than transmitter-centric contracts, which can be produced by inspecting leakage function operands.
% and each path divergence it may exhibit, \tspec{} models enumerate, for each path divergence it may For each accomplice instruction, \tspecA{} models further define a set of \textit{leakage functions}, whose arguments are the operands of transmit instructions, and whose range denotes a degree of path variability experienced by the accomplice instruction.
% \tspecU{} models \textit{additionally} include user-friendly descriptions of accomplice \textit{execution paths} on the target microarchitectures and \textit{design signals} which implicate a transmitter as contributing to its path variability.
%
%
% can be useful towards identifying special scenarios in which it may actually be safe to supply secrets to transmitters.
% For example, consider operand-packing execution units, which are optimized to improve throughput by packing together two distinct operations (e.g., ALU operations) and executing them as one, when their operand bit-widths are sufficiently narrow~\cite{brooks:operand-packing,gong:operand-packing}.
% Such ``packable'' operations clearly create operand-dependent hardware resource usage (i.e., they are transmit instructions)~\cite{pandora:isca:21}.
% % Suppose that a receiver can observe whether a packable operation was merged with another instruction or not by measuring its execution time, and further that its upper operand bits are zero executing the same operation with a low bit-width alongside it.
% However, 
% % is the same opermay be safe as long a pair of ``packable'' operations, whose operands have mis-matched secrecy labels, cannot arrive the execution unit concurrently.
% % where at least as the receiver cannot execute alongside the victim in a sibling SMT thread.
%
% Naïvely defining a \tspec{} model for a microarchitecture requires exposing a degree of implementation detail beyond what industrial hardware vendors would deem acceptable. Taken literally, enumerating channels naïvely requires naming specific hardware structures. Plus, a list of culprit hardware resources is not readily usable by software defenses. Thus, we consider two \tspec{} model variants, \tspecA{} models (``A'' for ``architecture'') and \tspecU{} models (``$\mu$'' for microarchitecture), which are intended for use by programmers and hardware designers, respectively.  
%
% % Towards defining \tspecA{} models, 
% Our \textbf{first key insight} enables
% % is a novel taxonomy for characterizing how channel modulations manifest microarchitecturally. This taxonomy enables
% us to define \tspecA{} models exclusively in terms of hardware instructions and their operands.
% % \footnote{In this paper, we focus on ISA instructions, but \tspec{} models can be easily defined in terms of micro-ops or ghost instructions.} and their operands.
% In particular, we observe that operand-dependent channel modulations on behalf of a transmit instruction manifest as \textit{multiple microarchitectural execution paths} for one or more \textit{\accomp{} instructions}, or simply \textit{\accomps{}} (our terminology). Ultimately, a receiver infers (a function of) a transmit instruction’s operands by indirectly observing which execution path one of its \accomp(s) took at runtime, e.g., by measuring the \accomp(s) execution time or its contention with other instructions. Phrased differently, an \accomp{} instruction is ``part of the channel'' created by a transmit instruction.
% Thus, \tspecA{} models indirectly expose the channels modulated by a transmit instruction by instead exposing its \accomp(s).
%
% For each accomplice instruction, \tspecA{} models further define a set of \textit{leakage functions}, whose arguments are the operands of transmit instructions, and whose range denotes a degree of path variability experienced by the accomplice instruction.
% \tspecU{} models \textit{additionally} include user-friendly descriptions of accomplice \textit{execution paths} on the target microarchitectures and \textit{design signals} which implicate a transmitter as contributing to its path variability.
%
% \textbf{\tsynth{} Approach \& Tool}
% Lead with the example -- here are specs today, here are the specs were proposing, and here's why we thing software will benefit.
% This is what information is contained. 
% Switch to operand-packing
% Leaning on -- what is the information contained in the spec, motivated by operand packing (fist thing to convey)
% Give the example, explain why its good - leakage function, multiple instructions interacting
% Instructions which are important for the channel modulated by the to measurable.
% Spec is build on this abstraction of execution paths - this abstraction itself need not be based in this abstract
% Analysis uses this abstraction 
% Second thing to lean on -- idea of path abstractions that you get from rtl2uspec
% The idea for what abstraction we want to use - these abstract execution paths.
% Great abstraction that compromises in that it visually allows you to reason about what software has going 
% \tspec{} models are based on \uspath{} abstraction for modeling instruction execution bahvior on a microarchitecture. As it turns out, this abstraction also enable formal analysis to derive \tspec{} models from RTL efficiently and fully-automatically. \tspec{} also produces high-utility conterexamples, which unlike signal traces, precisely communicate how the microarchitecture is enabling program level information leakage - how leakage functions and the path divergences they create manifest as \upath{} variability.
%
% As with all \leakagecontracts{}, the utility of \tspec{} models depends on the degree to which they accurately reflect microarchitecture.
% Hence, % this paper takes a substantial step towards 

% \subsubsection{The Leakage Contract Verification Challenge}
\label{sec:intro:this-paper:verify-challenge}
% Like all hardware-software contracts, 
In particular, since \pct{} contracts are useful only if we can guarantee hardware compliance, we propose
% Unfortunately, a sound and complete approach for formally verifying that a microarchitecture implements even a transmitter-centric leakage contract remains elusive (Table~\ref{tab:related:lc-verification}).
% \caroline{Left off here.}
% hardware lekage contract verification  for \textit{formally verifying} microarchitectural adherence to lea with state-of-the-art leakage contracts remains elusive
% Our third insight is that the notion of a transponder enables an automated leakage contract verification procedure that relies primarily on evaluating simple trace properties on the design under verification (DUV). 
% \textbf{\tsynth{} Approach \& Tool}
% Thus, beyond \textit{defining} \pct{} contracts, we propose
an approach and tool, called \tsynth{}, for \textit{formally verifying} microarchitectural adherence to them.
%\footnote{https://anonymous.4open.science/w/kULzwlgP0ouCgGfoFiP1/}
% for \textit{formally verifying} microarchitectural adherence to \tspec{} models.
% that a \tspec{} model accurately reflects microarchitecture.
% which takes a substantial step towards formally verifying that a hardware implementation satisfies the \tspec{} model it claims to.
% it claims to with an approach and tool, called \tsynth{}.
% Hence, we have developed \tsynth{},
% \textit{sound and complete}, and first \textit{automated}, approach and tool for formally verifying that a microarchitecture satisfies some \tspec{} model.
% Thus, a core contribution of this paper is the \tsynth{}
% % Thus, we have designed \tsynth{}, a \textit{sound and complete}
% approach and tool for synthesizing (i.e., reverse-engineering) \tspec{} models from RTL.
% , and transmitter-based \leakagecontracts{} which they subsume, from RTL.
% In particular, we design \tsynth{} conducts \textit{contract synthesis}. 
Given modest (mostly standard) design metadata, \tsynth{} \textit{automatically} synthesizes a formally-verified
% \rsout{\textit{partial}}
\pct{} contract
% \rsout{, called \tspecA{} models,}
from processor RTL
using static netlist analysis, linear temporal logic (LTL) property generation~\cite{pnueli:ltl,manna:ltl-textbook}, and model checking~\cite{baier:principles_of_model_checking, clarke:model_checking}.
% \rsout{\tspecA{}}\yao{\tspec{}} 
In particular, our current \tsynth{} implementation synthesizes a class of \pct{} contracts, called \pctA{} contracts, that are 
% class of \tspec{} model s \tspec{} models from automatically synthesized 
% \tspec{} models are derived from \tsynth{}'s intermediate output--
derived from \textit{abstract leakage functions} (highlighted fields in Fig.~\ref{fig:leak_fun_muladd})---the intermediate synthesis result. Since these functions leave the function body abstract, \pctA{} contracts capture leakage conditions related to scheduling decisions (S) exclusively.
% Hence, the \tspec{} models we verify in this paper 
% \yao{and include complete labeled input arguments and output range}.
% enumerate transponders and a set of \textit{abstract leakage functions} for each that leave the function body details abstract.
% (e.g., Fig.~\ref{??} for the running zero-skip multiply example).
% Fig.~\ref{fig:operand-packing-function} (bottom) shows an abstract leakage function; it defines which instructions' 
% %(\caroline{TODO: }classified as $\mathtt{OP_T}$, $\mathtt{OP_D}$, or $\mathtt{OP_S}$)
% operands are rendered unsafe and the range of return values. 
% Synthesized \tspec{} models are partial in that for each t they define which instruction operands leave leakage functions abstract while defining which instruction opearnds they leak and the rage of path d
% Notably, both \tspec{} and \tspecA{} models subsume standard \leakagecontracts{}~\cite{arm:dit,intel:doit,riscv_zkt}

% , let alone \tspec{} models.
% We instead advocate for \textit{contract synthesis}, whereby a \leakagecontract{} is incrementally derived (i.e., reverse-engineered) from processor RTL. In particular,


% In doing so, \tsynth{} automatically verifies microarchitectural adherence to state-of-the-art \leakagecontracts{}, which \tspec{} models subsume, \textit{for the first time}.
% \tspecU{} models from RTL, which are abstracted to produce \tspecA{} models. Since \tspecU{} models subsume \tspecA{} models, we refer to them collectively and \tspec{} models when the distinction is irrelevant.
% Since \tspec{} models subsume state-of-the-art \leakagecontracts{}, \tsynth{} synthesizes these too \textit{for the first time}.
% Importantly, \tspecA{} models subsume, and are thus easily exportable to, standard transmitter-centric \leakagecontracts{}.


% Spec is build on this abstraction of execution paths - this abstraction itself need not be based in this abstract

% Analysis uses this abstraction 
% Second thing to lean on -- idea of path abstractions that you get from rtl2uspec
% The idea for what abstraction we want to use - these abstract execution paths.
% Great abstraction that compromises in that it visually allows you to reason about what software has going 


% , which require a model checker to explore two copies of the DUV~\cite{}.
% In a nutshell,
% % Leveraging the notion of a transponder, 
% \tsynth{} first uses trace properties to uncover all possible \upaths{} for each implemented instruction. Instructions with more than one \upath{} are \textit{candidate} transponders.
% % \textit{\upath{} discovery} for each implemented instruction using trace properties.
% % , using trace properties uncover all possible microarchitectural execution paths for each implemented instruction
% % Next, for instructions with
% % Instructions 
% % which may exhibit more than one \upath{} (\textit{candidate transponders}),
% % For each candidate transponder, 
% % \caroline{Fix this part:}
% Next, \tsynth{} compares \textit{all pairs of \upaths{}} (akin to evaluating a 2-safety hyperproperty on an abstract representation of the DUV) for each candidate transponder to identify \textit{path divergences} (e.g., $\mathtt{mulUnit}$ and $\mathtt{scb.complete}$ in Fig.~\ref{??}).
% % ---common nodes in a pair of \upaths{} that are followed by different nodes.
% % identifies divergences across the \upaths{} of each candidate transponder.
% %  to localize path divergences.
% % compares its execution paths to localize path divergences. Third, f
% % \yao{update below to reflect what I actually did...}
% For each divergence, \tsynth{}
% % \textcolor{purple}{\sout{\tsynth{} uses static netlist analysis to identify
% identifies which RTL signals are responsible for the divergence.
% %R evaluated by its path selector function.
% Finally, \tsynth{} uses symbolic taint analysis~\cite{} to determine whether these signals
% %\textcolor{purple}{\sout{these signals} signals for the execution phase involved in the divergence}
% are operand-dependent on the candidate transponder (indicating an intrinsic transmitter) and/or other dynamic or static instructions (indicating a dynamic or static transmitter).
% If so, \tsynth{} has identified a true transponder and its abstract leakage function.
% (transmit) instruction operands or not. 
% In designing, \tsynth{} we make our \textbf{third observation}

% The key to \tsynth{}'s theoretical guarantees, automation, and scalability is 
% % (soundness and completeness) and automation is that it
% % \textit{the first} approach for hardware leakage contract verification\footnote{We use the term \textit{contract verification} to encompass both \textit{contract satisfaction}.}
% relies primarily on evaluating simple \textit{trace properties} on the design under verification (DUV).
% and \textit{contract synthesis}.}procedure for formally evaluating microarchitectural adherence to \leakagecontracts{} that relies \textit{mostly} on evaluating simple \textit{trace properties} on the design under verification (DUV).
% Meanwhile, all prior \leakagecontract{} verification
% % \footnote{We use the term \textit{contract verification} to encompass both \textit{contract satisfaction}.}
% approaches exclusively evaluate \textit{2-safety hyperproperties}~\cite{}, which require a model checker to explore two copies of the DUV~\cite{}.
% Leveraging the notion of a transponder, \tsynth{} first conducts \textit{path discovery}, using trace properties uncover all possible microarchitectural execution paths for each implemented instruction. Instructions which may exhibit more than one path are \textit{transponders}. Second, for each transponder, \tsynth{} compares its execution paths to localize path divergences. Third, for each path divergence, \tsynth{} identifies a handful of \textit{control signals} in the RTL, which ultimately select a particular path possibility for the transponder at runtime. Finally, \tsynth{} uses symbolic taint analysis to determine whether these control signals may be derived from (transmit) instruction operands or not. 


% Our \textbf{second insight} enables our trace property-based approach: given that channel modulations manifest as multiple execution paths for amplifiers, \tsynth{} can first uncover all amplifier instructions and then identify their associated transmit instructions.
% Thus, \tsynth{} first conducts microarchitectural execution path discovery for all implemented hardware instructions. This exploration is conducted form a hard reset of the DUV (unlike prior work which relies on symbolic initial states for scalability).
% % and on a single copy of the design.
% Next, \tsynth{} flags instructions with more than one execution path as \textit{candidate amplifiers}. Third, it pinpoints path divergences within the execution paths of candidate amplifiers. These path divergences implicate signals in the DUV which may leak to a receiver who observes the execution path taken by the amplifier at runtime. Finally, \tsynth{} leverages symbolic taint analysis, to color these signals as operand-dependent on one or more transmit instructions.

% \caroline{TODO: define path selector function earlier. MUL example: have variable execution paths for MUL, SUB, SUB, …; show a reorder buffer and execution stage of a pipeline. Illustrate how the multiply my take variable cycles in the MUL unit and how other instructions may be compile in the ROB for variable cycles. Also include the leakage functions (aka path selector functions for each).}

\yao{Notably, beyond supporting CT programming, \pct{} contracts' leakage conditions also support implementing state-of-the-art hardware defenses against speculative execution attacks~\cite{jiyong:sdo, jiyong:stt}, which rely heavily on manual reasoning. Further, the rich contracts also enables future hardware-software co-design of defenses. %side-channel mitigation. 
% Specifically, there exists no tool to automatically and comprehensively collect the information needed to implement the \pct{} contracts also, for the first time, enable automatic and comprehensive 
% about side-channel arising from instruction interactions
% \pct{} contracts also, for the first time, enable automatic and comprehensive collection of i
}

\textbf{Contributions} We summarize our contributions as follows.

\begin{itemize}
    \item \textbf{Transponders:} We extend the hardware side-channel attack taxonomy
    %  propose the notion of \textit{transponders}
    to capture \textit{how} receivers observe channel modulations---as distinct \upaths{} for \textit{transponders}.
    \item \textbf{Leakage Functions:} We show how to formulate each instance of \upath{} variability for a transponder as a function of transmit instruction operands, i.e., a leakage function.
    % We show how leakage functions can be used to characterize each instance of \upath{} variability For each channel whose modulation creates \upath{} variability a transponder, and  we define leakage functions to characterize channels whose modulation creates \upath{} variability for transponders.
    % leverage transponders to encode the conditions under which transmit instructions leak their unsafe operands via particular channels.    
    % modulations on behalf of a transmit instruction. 
    \item \textbf{\pct{} Contracts:} We propose \pct{} contracts, which extend \ct{} contracts with precise leakage conditions, derived from a microarchitecture's leakage functions.
    % and
    % derived from a processor's leakage functions, which capture the conditions under which transmit instructions leak their unsafe operands.
    % use transponders and their associated leakage functions to 
    % , called \tspec{} models, and 
    %  use them to model various ``leaky'' processor optimizations~\cite{pandora:isca:21}.
    % show how they enable more precise defenses. Notably, \tspec{} models can be define 
    % and show that they can be defined purely in terms of architectural constructs (assembly instructions and their operands), minimizing the exposure of proprietary implementation details.
    % We further find that aforementioned details can be defined purely in terms of architectural constructs (assembly instructions and their operands), minimizing the exposure of proprietary implementation details.
    % \item Significantly richer leakage contracts, called \tspec{} models, which expose to programmers (i) operand-dependent channel modulations on behalf of transmit instructions are observed by a receiver---via execution path variability for transponder instructions---and (ii) leakage functions which map channel observations onto a set of possible operand values.
    
    \item \textbf{\tsynth{}:} We propose
    % take a significant step towards formally verifying hardware adherence to \tspec{} models with
    \tsynth{} for synthesizing % \rsout{\tspecA{}}\yao{\tspec{}} 
    % \tspecA{} models 
    \pctA{} contracts from RTL.\footnote{https://anonymous.4open.science/w/kULzwlgP0ouCgGfoFiP1/} Notably, \tsynth{} is the 
    %first 
    % \textit{sound} and \textit{complete}, and first \textit{automated}, 
    first automated approach and tool
    % (Table~\ref{table:relatedwork}) 
    for verifying hardware adherence to
    % both \tspecA{} models \textit{and}
    \ct{} contracts~\cite{arm:dit,intel:doit,riscv_zkt}, where all leakage conditions are $true$.
    % which \pctA{} 
    % transmitter-centric \leakagecontracts{}~\cite{arm:dit,intel:doit,riscv_zkt} which \tspecA{}
    % \rsout{\tspecA{}}\yao{\tspec{}}
    % contracts subsume.
   %  A formal and fully automatic approach and tool, called \tsynth{}, synthesizing (i.e., ``reverse engineering'') \tspec{} models from RTL.
    % Since \tspec{} models subsume transmitter-based leakage contracts, \tsynth{} also represents both the \textit{first sound and complete} and \textit{first automated} approach for verifying microarchitectural adherence to them.
    
    
    \item \textbf{\upaths{}:} We propose the \upath{} abstraction, which
    % to encode instruction execution behavior on a microarchitecture. Beyond
    beyond enabling the specification of \pct{} contracts and design of \tsynth{}, offers a friendlier alternative to waveforms for viewing violations of hardware side-channel safety (Def.~\ref{def:sc_safe}).
    %This abstraction enables our definition of transponders, our trace property-based approach to \leakagecontract{} synthesis, and a designer-friendly alternative to wave-forms for viewing leakage counterexamples.
    
    % We finde that \upaths{} have several benefic  as concise execution path-based abstraction that encodes instruction execution behavior on a microarchitecture. , path-based abstraction for visually representing operand-dependent hardware resource usage manifests on a microarchitecture on a microarchitecture. Enables hardware designers to root cause information leakage and make targeted hardware changes if needed.
    
    \item \textbf{CVA6 Case Study:} We use \tsynth{} to synthesize a complete \pctA{} model from the RISC-V CVA6 processor core~\cite{cva6}, surfacing
    %---a 64-bit, 6-stage, single-issue RISC-V core featuring speculation, limited out-of-order write-back, diversified functional units, and a data cache.
    % Across all 72 instructions in the RV64I ISA and M extension, and \tsynth{} identifies
    94 unique abstract leakage functions, 72 transponder instructions, and 26 transmit instructions. \tsynth{} uncovers a novel channel that leaks store/load addresses, compared to prior work that analyzes the same design~\cite{deutschmann:upec-do,deutschmann2023scalable}.
    % \caroline{We find a new channel compared to prior work!} 
    % \yao{An attempt: Compared to prior works, \tsynth{} uncovers a novel channel associated with store.} \caroline{First to analyze cache!}
    % \caroline{identifies 32 transmit instructions and N abstract leakage functions.}\yao{identifies 26 transmit instructions and 97 abstract leakage functions.}
\end{itemize}





==> 14-formal-synth-proof.tex <==
In \S\ref{sec:tool:security-arg}, we claim that \synthlc{} produces a \textit{complete} set of leakage signatures,  which capture all violations of \textit{hardware side-channel safety}.
%security guarantees of \synthlc{} 

Below we present a formal proof on this claim. 
To do so, we first presents a microarchitectural execution semantics (\S\ref{a:sec:uarch-semantics}) so as to define hardware side-channel safety (i.e., Def.~\ref{def:scsafe}) \textit{formally} (\S\ref{a:sec:background:sec-def}). 
Next we concretize our receiver \Rupath{} (\S\ref{sec:tool:security-arg} of main paper) by formally defining $\mathcal{O}_{\mathcal{R}_{\upath{}}}$ (\S\ref{a:sec:tspec:receiver-assumptions}). 
% Next we discuss receiver assumptions  to which reasoning on channels is done with respect to. 
%on the set of all channels on a microarchitecture is done with respect to some receiver assumption, which a sufficiently powerful and realistic receiver (attacker) assumptions, which we introduce in . 
Then we define in \S\ref{a:sec:spec:upathdecformal} the \upaths{} and decisions formally in order to support the formal proof on leakage signature synthesis in the next section (\S\ref{a:sec:tool-approach-formal}). % and thus contract verification (\S\ref{}).

% \subsection{Hardware Side-Channel Safety}
%Foundation For Reasoning About Side-Channel Leakage} 
%Leakage Signatures Synthesis Formal Foundation Supplementary Proof and Reasoning}
% To argue the soundness and completeness of leakage contracts requires that \PathFinder{} and \synthlc{} uncovers \textit{all} leakage signatures corresponding to \textit{all} channels on a microarchitecture \M{}, under some realistic receiver (attack) assumption. 
%it is sufficient for leakage signature synthesize to collecting all decisions from a complete set of \upaths{} for all instruction
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   To do so we first need a notion of what means secure and side-channel free formally. \\ 
%[x]    1. (2.2 Microarchitectural Execution Semantics)  \\
%[x]    2. (2.3 security definition) \\
%[x]    Next we detail the receiver assumption \\ 
%[x]    3. (3.2.3 Receiver Assumptions. We define and verify PCT contracts with respect to a novel receiver r upath) \\ 

%[ ]    To facilitate the proof that all channels correspond to all decisions taken by transponders \\ 
%[ ]    4. (3.2.4 upaths Formalized.) \\
%[ ]    5. (3.3.1 Decisions) \\ 
%[ ]    If the leakage contract is incomplete, then there exists some way to have countereample \\ 
%[ ]    6. (4.2 Counterexample Discovery) \\
%[ ]    7. (4.3 leakage signatures Discovery) as the signautre synthsis 
%   
%   This amounts to finding all leakage signatures 
%   all leakage signatures leakage againstsynthesize a complete set of  
%   \yao{TODO}
% \yao{TODO}


% \yao{\textless{}\textless{}\textless{}}

%Since it is the leakage contracts that should expose all side-channel on a microarchitecture, we first need to establish a formal notion of side-channel free. 

\subsection{Microarchitectural Execution Semantics}
\label{a:sec:uarch-semantics}
% Formally defining a program's susceptibility to hardware side-channel attacks is the first step towards uncovering and characterizing all channels on a given hardware implementation. %, synthesizing and verifying leakage contracts against hardware implementation. % against hardware implementation. 
% requires d
This section presents an execution semantics for an abstract processor microarchitecture (inspired by~\cite{guarnieri:contracts}) to support such a security definition.
% (\S\ref{sec:background:sec-def}).

% This paper proposes \tspec{} models, a novel class of \textit{transponder-centric} leakage contracts to support a \textit{conditional constant-time defense} ($\mathcal{D}_{cct}$), and the \tsynth{} approach and tool to formally verify hardware compliance with \tspec{} models (and transmitter-centric leakage contracts with they subsume).
% We propose \tspec{} models to precisely expose the conditions under which transmitters leak their operands

% % (discussed abstractly in \S\ref{sec:background:telecom:channels} and \S\ref{sec:background:telecom:receiver})
% to programmers and the \tsynth{} approach and tool to verify hardware compliance to \tspec{} models. This section presents microarchitectural execution semantics for a simple processor, which we use to argue the correctness of \tsynth{} 
% we use to define hardware side-channel safety, 

% \subsection{Threat Model}
% \label{sec:background:threat-model}



% Leakage contracts offer the possibility of safely executing victim programs on unsafe hardware (i.e., hardware containing transmit instructions). 
% % The core contributions of this paper are \tspec{} models, which resolve fundamental limitations associated with transmitter-centric leakage contracts, and the \tsynth{} approach and tool, which formally verifies microarchitectural adherence to leakage contracts.
% % The sole purpose of leakage contracts is to support hardware side-channel defenses.
% This section formalizes what it means for a program to be susceptible to hardware side-channel attacks and how leakage contracts enable hardware side-channel defenses.


% The primary goals of this paper are to resolve limitations associated with transmitter-centric leakage contracts and to devise an automated approach to verifying hardware adherence to leakage contracts. 


% \caroline{
% \begin{itemize}
%     \item \textbf{Receiver Assumptions:}
%     \begin{itemize}
%         \item \textbf{Observer Models:}
%         \begin{itemize}
%             \item \textbf{Prior work:} Defines Observer Models that expose a subset of microarchitectural state to the receiver at each time-step of an execution trace. E.g., a receiver that can measure instruction execution time can be captured with an an Observer Model that exposes the commit signal at every cycle.
%             \item \textbf{Our work:} We consider a receiver that can observe the \upaths{} of instructions as the execute. A \upath{} is a partial order on the \ufsm{} states visited by an instruction during its execution; \upaths{} capture both speculatively and non-speculatively executed instructions. To achieve this, our Observer Model exposes the \ufsm{} state of the microarchitecture at each time-step of an execution trace. There is always one \ufsm{} that capture the commit signal, our Observer Model describes a strictly more powerful receiver that prior work.
%         \end{itemize}
%         \item \textbf{Attack Strategy:}
%         \begin{itemize}
%             \item \textbf{This work:} The distinction between passive vs. active attackers is typically considered orthogonally to the discussion of leakage contracts.
%             \item \textbf{Our work:} However, the \tspec{} models we propose support more precise definitions of these Attack Strategies.
%         \end{itemize}
%     \end{itemize}
%     \item \textbf{Hardware Side-Channel Defenses:}
%     \begin{itemize}
%         \item For most realistic Observer Models (e.g., commit signal or \ufsms{}), an arbitrary program will be susceptible to hardware side-channel leakage. Hardware side-channel defenses thus require some cooperation between hardware and software:
%         \begin{itemize}
%             \item \textbf{Hardware:} Hardware exposes a hardware-software contract.
%             \item \textbf{Software:} The space of programs is restricted according to information in the contract.
%             \item If hardware satisfies the contract, and the space of programs is restricted per the contract, then there will be no hardware side-channel leakage.
%             \item TODO: I'm having a bit of trouble formalizing this in a non-confusing way. Technically the property I have written, requires the hardware contract to consist of both an Execution Model and a Leakage Model (à la~\cite{guarnieri:contracts}. But I think it's probably unwise to get into this level of detail.
%         \end{itemize}
%         \item \textbf{Prior Work:} Considers transmitter-centric leakage contracts. Contract exposes transmit instructions and their unsafe operands. Programs are written to never pass secrets to transmit instructions. Prevents hardware side-channel leakage across all sequential executions. 
%         \item \textbf{Our work:} Considers transponder-centric leakage contracts. Contract exposes transponders and leakage functions for each. Programs are written such that secrets never reach transmitters under certain circumstances. Widens the space of programs + can enable safe programming in situations where transmitter-centric leakage contracts cannot.
%         \item MAYBE: Possibly mention that we're synthesizing transponder-centric contracts from hardware. In doing so we synthesize transmitter-centric contracts implicitly.
%         \item TODO: Maybe I can write ``defense'' abstractly. Then I can only focus on the leakage model component and not the execution model component?
%     \end{itemize}
% \end{itemize}
% }
% p, s, s’, u, u’
% O(uarch(P(p, s), u)) = O(uarch(P(p, s), u’)) - ensures there aren’t secrets left over in microarchitecture to create divergence
% \paragraph*{Microarchitecture}

% \textbf{A Simple Microarchitectural Execution Semantics (inspired by~\cite{guarnieri:contracts})}
% \label{sec:background:uarch-semantics}
% We first define a simple microarchitectural execution semantics.
% \caroline{Currently using similar notation to~\cite{guarnieri:contracts}.}
Consider a processor \textit{microarchitecture} $\mathcal{M} = (S_0, S, T)$, where $S$ is a set of \textit{states}, $S_0 \subseteq S$ is a set of \textit{initial states}, and $T \subseteq S \times S$ is a deterministic \textit{transition relation}. 
% \yao{
% across a cycle (i.e., time step).}
%\yao{Should be obvious(?): Initial states include any states reachable from running any valid program from a hard reset.}
% \footnote{Our semantics is inspired by recent work on hardware-software contracts for secure speculation~\cite{guarnieri:contracts}.}
% \chris{say somewhere around here that we use this $\sigma(v)$, $\mu(w)$ notation to associate specific state elements $v$ $w$ with arch or uarch state.}

A processor state $\langle\sigma, \mu\rangle \in S$ consists of an architectural state $\sigma$ and a microarchitectural state $\mu$. An \textit{architectural state} $\sigma = \langle m, a\rangle$ denotes the contents of \textit{main memory} $m : loc \rightarrow \mathcal{V}$ and the contents of the \textit{architectural register file} $a : reg_a \rightarrow \mathcal{V}$, where $\mathcal{V}$ is the set of values that memory locations and registers can assume, $loc$ is a set of memory locations, and $reg_a$ is a set of architectural registers.
% We define a special register identifier $pc \in reg_a$ for the processor's program counter.
% , which is assigned the special value $\bot \in \mathcal{V}$ when a program terminates.
A \textit{microarchitectural state} $\mu : reg_\mu \rightarrow \mathcal{V}$ denotes the contents of all other state elements in the processor, where $reg_\mu$ is a set of microarchitectural registers.

Consider state $s = \langle \sigma, \mu \rangle$, where $\sigma = \langle m, a \rangle$. We use $s(\sigma)$ and $s(\mu)$ to refer to the architectural and microarchitectural state components of $s$; $\sigma(m)$ and $\sigma(a)$ to refer to the main memory and architectural register file components of $\sigma$; $m(j)$
% , $a(k)$, and $\mu(l)$
to refer to the value assumed by memory location $j$ in $m$;
% , architectural register, and microarchitectural register;
$s(\sigma)(m)(j)$ to refer to the value assumed by memory location $j$ in $s$; and so on.
% We define a special set of \textit{operand register} identifiers $reg_{op} \subset reg_\mu$, which represent state elements that hold an instruction's operands just before it is issued/dispatched.
% \footnote{In practice, which \textit{physical} registers represent \textit{architectural} registers may change cycle by cycle. Our semantics assumes a constant set of architectural register identifiers $reg_a$ that abstracts away this implementation detail.}
% \chris{re:the footnote commented out here in the tex.  When we define $\sigma$, can we say that $m$ denotes the contents of main memory and $r$ denotes the contents of the arch reg \emph{file}? (That way, its pretty clear what static structures they refer to/clarifies what state elements $\mu$ is exactly and doesn't sound defensive.)}


% ($reg \cap \mu reg = \varnothing$). 
% \chris{it's not clear exactly what state elements $\sigma$ and $\mu$ will encompass.  Will $reg$ and $ureg$ change cycle by cycle?}

% not to overflow
\sloppy An execution \textit{trace} $\langle \sigma_0, \mu_0 \rangle, \langle \sigma_1, \mu_1 \rangle, ...$ of \M{} is an infinite sequence of states, such that $\langle \sigma_0, \mu_0 \rangle \in S_0$,
%$\sigma_n[pc] = \bot$,
and $(\langle \sigma_k, \mu_k \rangle, \langle \sigma_{k+1}, \mu_{k+1} \rangle) \in T$ for $k \geq 0$. % < n$.
By $\lbbar p \rbbar_{\mathcal{M}}^{\langle \sigma, \mu \rangle}$ we denote the execution trace obtained from running a \textit{program} $p$ on \M{} from initial state $\langle \sigma, \mu \rangle$, such that
$\sigma(m)$ is initialized with $p$'s instructions and data and %\textcolor{olive}{
$\mu(\mathtt{IM\_PC})$ contains the address of the first instruction to fetch in $p$. $\mathtt{IM\_PC}$ is the \textit{instruction memory program counter} signal in \M{}~\cite{rtl2uspec:hsiao:2021}. %}.
%\yao{Defined but not used anywhere. Possibly trim the highlighted to "and program counter in $\mu$ is initialized to the first instruction in $p$"}
% $\mathtt{IM\_PC}$ is used to fetch instructions from memory in \M{}.
If $\langle \sigma, \mu \rangle \notin S_0$, then $\lbbar p \rbbar_{\mathcal{M}}^{\langle \sigma, \mu \rangle}$ returns the empty trace.
% $()$.
% $\sigma_0(m)$ is initialized with $p$'s instructions and data.
% We are sometimes interested in fast-forwarding a trace to a particular state.
By $t[n]$ we denote the state corresponding to the $n$th \textit{step}/\textit{cycle} of trace $t$, i.e., $t[0] = \langle \sigma, \mu \rangle$ for $t = \lbbar p \rbbar_{\mathcal{M}}^{\langle \sigma, \mu \rangle}$ .
% $\langle \sigma_0, \mu_0 \rangle$.
% \rsout{By $\langle \sigma_0, \mu_0 \rangle \Downarrow^p_{\mathcal{M}} \langle\sigma_k, \mu_k\rangle$, we denote state $\langle\sigma_k, \mu_k\rangle \in \lbbar p \rbbar_{\mathcal{M}}^{\langle \sigma_0, \mu_0 \rangle}$.}
% \yao{The notation is never used.}
% , reached via execution trace $\langle \sigma_0, \mu_0 \rangle, ..., \langle\sigma_i, \mu_i\rangle$.
% Hence, $\lbbar i \rbbar_{M}^{\langle \sigma_0, \mu_0 \rangle \Downarrow \langle\sigma_i, \mu_i\rangle}$ captures the observation trace obtained by \R from running $i$ on $M$ from state $\langle \sigma_i, \mu_i \rangle$.


%is referred to any instance of a particular fixed opcode.
%, whereas ``a dynamic/unique instruction'' is a particular instance in pipeline of a particular opcode and program counter.}
%and its encoding can include additionally one or two operands. }
% and immediate fields. For an instruction, we consider secret can only be in register operand fields}

% State $\langle\sigma_i, \mu_i\rangle$ marks the state where $\mu_i(IFR) = i$. That is, $i$ as just been fetched from instruction memory into the \textit{instruction fetch register} (IFR), i.e., $i$ has just materialized in the processor $M$. 


%\textit{labeled} \textit{memory} $m_l$ and \textit{architectural register} $r_l$ contents.
% Memory $m_l : \mathbb{N} \rightarrow \mathcal{V_L}$ maps natural numbers to labeled values $\mathcal{V_L}$, where $l = \{\textsc{pub}, \textsc{sec}\}$ and $\mathcal{V_L} = Vals \times l$.

% \mathcal{M} : loc \rightarrow \mathcal{V}_L$ and the architectural \textit{register file} $\mathcal{R} : reg \rightarrow \mathcal{V}_L$, where $loc \subseteq \mathbb{Z}$ is the set of memory addresses $reg = $ is a finite set of general purpose registers 
% An \textit{architectural state} $\sigma = \langle \mathcal{M}, \mathcal{R} \rangle$ defines the contents of \textit{memory} $\mathcal{M} : loc \rightarrow \mathcal{V}_L$ and the architectural \textit{register file} $\mathcal{R} : reg \rightarrow \mathcal{V}_L$, where $loc \subseteq \mathbb{Z}$ is the set of memory addresses $reg = $ is a finite set of general purpose registers 
% $\mathcal{V} \subseteq \mathbb{Z}$ is the set of data values that registers and data memory locations can assume ($0 \in \mathcal{V}$);



% Consider a victim \textit{program} $p$ running on a processor \textit{microarchitecture} $M = (S_0, S, T)$, a finite state transition system, where $S$ is the set of processor \textit{states}, $S_0 \subseteq S$ is the set of \textit{initial states}, and $T \subseteq S \times S$ is the \textit{transition relation}.

 
% where $M$
% Microarchitecture $M = (S_0, S, T) $
% is a finite state transition system,
% \begin{itemize}
%     \item $S$ is a set $2^n$ of hardware states for a design with $n$ flip-flop bits,
%     \item $S_0 \subseteq S$ is the set of initial states, and
%     \item $T \subseteq S \times S$ is the transition relation.
% \end{itemize}


\subsubsection{Security Definition}
\label{a:sec:background:sec-def}

% \textbf{Formalizing Hardware Side-Channel Safety}
% \label{sec:background:hw-sc-safety}

% \chris{the rest of SII is a mix of known / our contribution. 
%  The latter should not be in SII.}
We define a program's susceptibility to hardware side-channel attacks using an \textit{information-flow} property below~\cite{sabelfeld2003language,goguen1982security}.
Our definition assumes a \textit{static privacy policy} $\pi : loc \rightarrow \{\textsc{l}, \textsc{h}\}$ that labels memory locations in $m$ 
% \chris{in $m$?}
% ($loc \cup reg_a$)
% , and thus all registers ($reg_a$, $reg_\mu$) and memory locations ($loc$),
% labels each architectural state element ($\in \{loc \cup reg\}$)
% state element ($\in \{loc \cup reg \cup \mu reg\}$) 
% each memory location
% according to whether they store 
as storing \textit{low} (\textsc{l}, public) or \textit{high} (\textsc{h}, private) data.
A program's instruction memory is always low~\cite{serberus:mosier:2024,deutschmann:upec-do}.\footnote{W.l.o.g., \emph{only} locations in $m$ are assigned security types in \textit{static} privacy policy $\pi$, and taint does not propagate, e.g., to elements in $r$ or $\mu$.}
% \chris{suggest a footnote here: static = w.l.o.g. \emph{only} locations in $m$ are tainted = taint doesn't propagate, e.g., to elements in $mu$.}
% \textsc{l}-labeled in $\pi$.


Hardware side-channel safety is defined with respect to an observer model $\mathcal{O_R}$.
Given state $\langle \sigma, \mu \rangle \in S$, $\mathcal{O_R}(\langle \sigma, \mu \rangle)$ returns the value of 
each memory location, architectural register, and microarchitectural register  that is assumed to be \textit{visible} to \textit{receiver} $\mathcal{R}$. 
% \yao{Space-saving idea?: each state element assumed \textit{visible} to the \textit{receiver}.}
% the subset of architectural and microarchitectural state that is
We lift functions over sequence elements to functions over sequences in the natural way, e.g., for execution trace $t = \langle \sigma_0, \mu_0 \rangle, \langle \sigma_1, \mu_1 \rangle, ...$, we define the \textit{observation trace} obtained by receiver \R{} from $t$ as $\mathcal{O_R}(t) = \mathcal{O_R}(\langle \sigma_0, \mu_0 \rangle), \mathcal{O_R}(\langle \sigma_1, \mu_1 \rangle), ...$.
% That is, $\mathcal{O_R}(t)$ captures
%  (\S\ref{sec:background:telecom:receiver}).
% \chris{the current text in \S\ref{sec:background:telecom:receiver} doesn't clarify what we mean by this.}
% Given an execution trace $t = \langle \sigma_0, \mu_0 \rangle, \langle \sigma_1, \mu_1 \rangle, ..., \langle \sigma_n, \mu_n \rangle$, $\mathcal{O_R}(t) = O_0, O_1, ..., O_n$
% captures the \textit{observation trace} obtained by receiver \R{} from execution trace $t$.
% \chris{(to improve flow) I suggest moving this next para up to where we define $\mathcal{O_R}$.}
Industrial leakage contracts~\cite{arm:dit, intel:doit, riscv_zkt} 
% and recent work~\cite{wang2023specification}
%Most prior work~\cite{gleissenthall:iodine, gleissenthall:xenon, deutschmann:upec-do, deutschmann2023scalable, wang2023specification}, including industrial leakage contracts~\cite{arm:dit, intel:doit, riscv_zkt}, 
assume a receiver $\mathcal{R}_C$ that observes \M{}'s $\mathtt{commit}$ signal, or
$\mathcal{O}_{\mathcal{R}_C}(\langle \sigma, \mu \rangle) = \mu(\mathtt{commit})$,
% Recent work assumes the same~\cite{wang2023specification} or similar~\cite{deutschmann:upec-do, deutschmann2023scalable}.
% that observes the commit signal at every time step.
modeling a receiver that perceives channel modulations through their impact on instruction or program execution time.

\paragraph{Program Assumptions}:
\label{a:sec:background:sec-def:program}
For virtually all realistic receivers, including $\mathcal{R}_C$,
%Eq.~\ref{a:eq:non-interference} is trivially invalid for 
any program that features secret-dependent control-flow can leak the secret. For example, consider the code listing, 
\inst{if(sec)\{seq~/\mathord{*}latency~L\mathord{*}/\}else\{seq'~/\mathord{*}latency~L'\mathord{*}/\}}, 
%\inst{if~(sec)~\{seq~/*latency~L\hspace{-2pt}*\hspace{-2pt}/\}~else~\{seq'~/*latency~L'\hspace{-2pt}*\hspace{-2pt}/\}}, 
which features a secret-dependent conditional branch. Clearly, and independent of microarchitecture, 
there exists instruction sequences \inst{seq} and \inst{seq'} whose latencies \inst{L} and \inst{L'},
respectively, are different (\inst{L \neq L'}).
Given our focus on \textit{microarchitectural} side-channels, we assume that all programs $p$ feature the same sequence of instructions along all branches of secret-dependent control-flow instructions, i.e., \inst{seq = seq'} for the code listing above. That is, we assume $p$ satisfying $ArchCtrl(p)$ (\S\ref{sec:tool:security-arg}).  %(or  as in \S\ref{sec:tool:security-arg}) That is we consider program $p$ if $PublicCtrl(p)$ returns true.  


With the above foundation, Def.~\ref{def:scsafe} in \S\ref{sec:tool:security-arg} of main paper (copied below) is formally defined. 

\begin{definition}[Hardware Side-Channel Safe]
\label{a:def:sc_safe}
A microarchitecture ${\mathnormal{M}}$ is
\textit{hardware side-channel safe}
with respect to receiver ${\mathnormal{R}}$, or
$\mathrm{SC\hbox{-}Safe}({\mathnormal{M}}, {\mathnormal{R}})$, iff:
\begin{equation}
\begin{split}
      \forall p.\forall \pi.\forall \sigma, \sigma'. \forall \mu. ArchCtrl(p) \implies \\
      (\sigma \approx_{\pi} \sigma'
      \implies \mathnormal{O_{R}}(\lbbar {p} \rbbar^{\langle\sigma, \mu\rangle}_{\mathnormal{M}}) = \mathnormal{O_{R}}(\lbbar {p} \rbbar^{\langle\sigma', \mu\rangle}_{\mathnormal{M}}))
\end{split}
\label{a:eq:non-interference}
\end{equation}
\end{definition}

Eq.~\ref{a:eq:non-interference} quantifies over all programs $p$ and security policies $\pi$ (which label program inputs as public or secret), all pairs of initial architectural states $\sigma, \sigma'$ and all initial microarchitectural states $\mu$.
Looking at the second line, the antecedent, $\sigma \approx_{\pi}\sigma'$, checks that the initial architectural states
are \textit{low-equivalent} with respect to $\pi$: they agree on the values of low data in $\pi$, i.e., $p$'s public data inputs.
The consequent, $\mathnormal{O_R}(\lbbar p \rbbar_{\mathnormal{M}}^{\langle\sigma, \mu\rangle}) = \mathnormal{O_R}(\lbbar p \rbbar_{\mathnormal{M}}^{\langle\sigma', \mu\rangle})$, asserts that \R{} obtains identical observation traces when $p$ runs on microarchitecture \M{} from initial states $\langle \sigma, \mu \rangle$ and $\langle \sigma', \mu \rangle$.

Eq.~\ref{a:eq:non-interference} violations indicate the observation trace obtained by receiver \R{} from running program $p$ with privacy policy $\pi$ on microarchitecture \M{} \textit{indisputably} a function of $p$'s high inputs. Note that secret-dependent control-flow instructions can still cause Eq.~\ref{a:eq:non-interference} violations, e.g., if they trigger operand-dependent squashes.



% \begin{definition}[Hardware Side-Channel Safe]
% Program ${\color{MidnightBlue}p}$ with privacy policy ${\color{MidnightBlue}\pi}$ is \textit{hardware side-channel safe}
% %is \textit{safe} from hardware side-channel attacks
% with respect to receiver ${\color{MidnightBlue}\mathcal{R}}$ on microarchitecture ${\color{MidnightBlue}\mathcal{M}}$, or $\mathrm{SC\hbox{-}Safe}({\color{MidnightBlue}\mathcal{M}}, {\color{MidnightBlue}\mathcal{R}}, {\color{MidnightBlue}p}, {\color{MidnightBlue}\pi})$, iff:
% \footnote{{\color{MidnightBlue}Blue} highlights constants, which are not quantified.}
% % , where:
% % iff Eq.~\ref{a:eq:non-interference} is valid:
% \begin{equation}
% \begin{split}
%       \forall \sigma, \sigma'. \forall \mu. \mathrm{NI}({\color{MidnightBlue}\mathcal{M}}, {\color{MidnightBlue}\mathcal{R}}, {\color{MidnightBlue}p}, {\color{MidnightBlue}\pi}, \sigma, \sigma', \mu)
% \end{split}
% \label{a:eq:non-interference}
% \end{equation}
% where $\mathrm{NI}({\color{MidnightBlue}\mathcal{M}}, {\color{MidnightBlue}\mathcal{R}}, {\color{MidnightBlue}p}, {\color{MidnightBlue}\pi}, \sigma, \sigma', \mu)$ denotes \textit{microarchitectural non-interference} as follows:
% \begin{equation}
% \begin{split}
%       \sigma \approx_{\color{MidnightBlue}\pi} \sigma'
%       \implies \mathcal{O_{\color{MidnightBlue}R}}(\lbbar {\color{MidnightBlue}p} \rbbar^{\langle\sigma, \mu\rangle}_{\color{MidnightBlue}\mathcal{M}}) = \mathcal{O_{\color{MidnightBlue}R}}(\lbbar {\color{MidnightBlue}p} \rbbar^{\langle\sigma', \mu\rangle}_{\color{MidnightBlue}\mathcal{M}})
% \end{split}
% \label{a:eq:uni}
% \end{equation}
% %\label{def:hw-sc-safety}
% \end{definition}
% % Via Eq.~\ref{eq:uni}, 
% Eq.~\ref{a:eq:non-interference} quantifies over all pairs of initial architectural states, $\sigma$ and $\sigma'$, and all initial microarchitectural states, $\mu$.
% % considers all \textit{pairs of traces} obtained from running $p$ on \M{} from all pairs of initial states, where the architectural state components 
% % $\sigma_0$ and $\sigma'_0$
% % may differ ($\sigma_0$ and $\sigma'_0$), but the microarchitectural state components are identical ($\mu_0$).
% % $\mu_0$ is identical.
% % (possibly) distinct architectural states,
% % all \textit{pairs} of initial architectural states, 
% % $\sigma_0$ and $\sigma'_0$, and all identical microarchitectural states, $\mu_0$.
% % and $\mu'_0$. 
% The antecedent (Eq.~\ref{eq:uni}), $\sigma \approx_{\pi}\sigma'$, checks that the initial architectural states
% % , $\sigma_0$ and $\sigma'_0$,
% are \textit{low-equivalent} with respect to $\pi$: they agree on the values of low data in $\pi$, i.e., $p$'s public data inputs.
% %does not have secret-dependent control-flow decision, meaning fetch stream is independent of secret value in the $\pi$.}
% % \textcolor{Maroon}{\mathcal{O_R}(\lbbar p \rbbar_{\mathcal{M}}^{\langle \sigma_0, \mu_0 \rangle}) = \mathcal{O_R}(\lbbar p \rbbar_{\mathcal{M}}^{\langle\sigma_0, \mu'_0\rangle})}
% % \chris{it's not clear whether the initial states in the definition need to be $\in S_0$}
% % Eq.~\ref{a:eq:non-interference} an \textit{information-flow} property.
% % We define \textit{hardware side-channel safety} for a program $p$ running on a microarchitecture $M$ using an
% % a program's susceptibility to hardware side-channel attacks using an
% % \textit{information-flow} property~\cite{}.
% % To do this, we 
% % We say architectural states $\sigma$ and $\sigma'$ are \textit{low-equivalent} with respect to privacy policy $\pi$, or $\sigma \approx_{\pi_\textsc{l}} \sigma'$, iff $\sigma$ and $\sigma'$ agree on the values of low data.
% % memory locations.
% % \yao{Updated $p$ color above and $\pi_L$}
% % \caroline{I realize I need to update text below to accommodate equation changes, but I'm not ready to do that yet.}
% % \yao{Maybe?: Eq.~\ref{a:eq:non-interference} asserts that $\sigma$ is non-interfering with $p$'s execution on \M{} from any microarchitectural state $\mu_0$ with respect to $\pi$.
% % $\sigma$ is non-interfering iff Eqn.~\ref{def:hw-sc-safety} is satisifed: for all pairs of ..
% % } 
% % \textit{both} of the following hold:
% % consists of the logical conjuction of two predicates, which enforce that the consequent need only hold:
% % predicate enforces that:
% % \begin{itemize}
% %     \item $\sigma_0 \approx_{\pi_\mathtt{L}}\sigma'_0$: 
% %     % Asserts that $\sigma$ and $\sigma'$ are low-equivalent.
% %     % For pairs of p
% %     Initial architectural states, $\sigma_0$ and $\sigma'_0$, are \textit{low-equivalent} with respect to $\pi$; they agree on the values of low data in memory (i.e., $p$'s public data inputs).
% %     % , but may disagree on high data values.
% %     % data, but may disagree on high data.
% %     % , are considered.
% %     \item ${\color{Maroon}\mathcal{O_R}(\lbbar p \rbbar_{\mathcal{M}}^{\langle \sigma_0, \mu_0 \rangle}) = \mathcal{O_R}(\lbbar p \rbbar_{\mathcal{M}}^{\langle\sigma_0, \mu'_0\rangle})}$: 
% %     Initial microarchitectural states, $\mu_0$ and $\mu'_0$, \textit{cannot} contribute to distinct observations of $p$'s execution on \M for receiver \R. % That is, running $p$ with the same inputs ($\sigma$) on $M$ produces the same observation trace regardless of the initial microarchitectural state ($\mu$ or $\mu'$).
% % \end{itemize}
% % The first (${\color{RedOrange} \sigma \approx_{\pi_\mathtt{L}}\sigma'}$) asserts that $\sigma$ and $\sigma'$ are low-equivalent.
% % The second (${\color{Maroon} \mathcal{O_R}(\lbbar p \rbbar_{M}^{\langle \sigma, \mu \rangle}) = \mathcal{O_R}(\lbbar p \rbbar_{M}^{\langle\sigma, \mu'\rangle})}$) asserts that running $p$ with the same inputs ($\sigma$) on $M$ produces the same observation trace regardless of the initial microarchitectural state ($\mu$ or $\mu'$). 
% % Intuitively, the former will consider all pairs of program inputs which agree on low data but (possibly) disagree on high data.
% % The latter will ensure that \textit{only the program inputs} can contribute to distinct receiver observations.
% % \yao{maroon for $\mu$ removed }
% The consequent, $\mathcal{O_R}(\lbbar p \rbbar_{\mathcal{M}}^{\langle\sigma, \mu\rangle}) = \mathcal{O_R}(\lbbar p \rbbar_{\mathcal{M}}^{\langle\sigma', \mu\rangle})$, asserts that \R{} obtains identical observation traces when $p$ runs on \M{} from initial states $\langle \sigma, \mu \rangle$ and $\langle \sigma', \mu \rangle$.
% produces the same observation trace for \R{} regardless of the initial state.
% A counterexample to Eq.~\ref{a:eq:non-interference} means that the observation trace obtained by \R{} from running $p$ on $M$ is \textit{exclusively a function of high inputs} to $p$.
% , i.e., $\mathcal{R}'s$ observations are not entirely a funciton of low inputs.

% Observe that for every pair of traces compared by the consequent, the initial microarchitectural states are the same, and the initial architectural states are low-equivalent.
% $\mu_0$ is identical for every pair of compared traces,
A violation of Eq.~\ref{a:eq:non-interference} indicates that the observation trace obtained by receiver \R{} from running program $p$ with privacy policy $\pi$ on microrarchitecture \M{} is \textit{indisputably} a function of $p$'s high inputs. 
Intuitively, with respect to $\mathcal{R}_C$, Eq.~\ref{a:eq:non-interference} is valid if no instruction in $p$ can influence the commit signal's value as a function of its operands. 



% ${\color{Maroon}\mathcal{O_R}(\lbbar p \rbbar_{\mathcal{M}}^{\langle \sigma_0, \mu_0 \rangle}) = \mathcal{O_R}(\lbbar p \rbbar_{\mathcal{M}}^{\langle\sigma_0, \mu'_0\rangle})}$: Initial microarchitectural states, $\mu_0$ and $\mu'_0$, \textit{cannot} contribute to distinct observations of $p$'s execution on \M for receiver \R{}
% \chris{we should say this is a form of observational determinism adapted for uarch attacks; I think there's 3 papers to cite (see Sanjit paper).}

\label{a:sec:background:sec-def:imprecise}
\textbf{Other Security Definitions}:
Some prior definitions of hardware side-channel safety omit $\mu$ in Eq.~\ref{a:eq:non-interference}, leaving the initial microarchitectural states for pairs of traces compared by the consequent implicitly unconstrained~\cite{deutschmann:upec-do, deutschmann2023scalable, gleissenthall:iodine, gleissenthall:xenon}.
%\yao{removed from previous and add to next \cite{guarnieri:contracts}}
% do not explicitly require the pairs of compared traces in Eq.\rsout{~\ref{a:eq:non-interference}}\yao{~\ref{def:hw-sc-safety}} to be run from the \textit{same} initial microarchitectural states, i.e., \rsout{the red text}\yao{$\mu_0$} is omitted~\cite{guarnieri:contracts, deutschmann:upec-do, deutschmann2023scalable, gleissenthall:iodine, gleissenthall:xenon}.
% \chris{people may get confused here because low equivalence is well known.  should we say prior work doesn't say anything about uarch state? (just arch state)}
% \yao{I think the text above already indicates that prior work doesn't say anything about "uarch"(?).}
% work omits details of the initial microarchitectural state (the red text in Eq.~\ref{a:eq:non-interference}) when \textit{defining} hardware side-channel safety~\cite{guarnieri:contracts, gleissenthall:iodine, gleissenthall:xenon, deutschmann:upec-do, deutschmann2023scalable}.
However, like prior work~\cite{guarnieri:contracts, wang2023specification}, we observe that constraining these traces' initial microarchitectural states (e.g., to be equivalent)\footnote{Eq.~\ref{a:eq:non-interference} must constrain the initial microarchitectural states in both traces to be \textit{non-interfering w.r.t. $p$ and $\pi$}. Any $\mu$ and $\mu'$ for which $\mathcal{O_R}(\lbbar p \rbbar_{\mathcal{M}}^{\langle \sigma, \mu \rangle}) = \mathcal{O_R}(\lbbar p \rbbar_{\mathcal{M}}^{\langle\sigma, \mu'\rangle})$ holds in the antecedent of Eq.~\ref{a:eq:non-interference} suffices,
% to prove hardware side-channel safety of $p$,
% evaluates to true form an equivalence class of microarchitectural states which are \textit{non-interfering w.r.t. $p$}. Any such pair is sufficient
% to prove hardware side-channel safety of $p$, 
but we select $\mu = \mu'$ for simplicity.} is required to prevent Eq.~\ref{a:eq:non-interference} from \textit{mis-classifying} a safe program $p$ running on microarchitecture \M{} as \textit{unsafe} with respect to security policy $\pi$ and receiver \R{}.
As an example, consider $p = \{\mathtt{LI~r1,3}; \mathtt{SUB~r1, r1, r1}\}$
% consisting of a single $\mathtt{ADD}$
executing on \M{} from initial states, $\langle \sigma, \mu \rangle$ and $\langle \sigma', \mu' \rangle$, where $\mu \neq \mu'$ and $\sigma \approx_{\pi}\sigma'$. Suppose $\mu$ and $\mu'$ feature an in-flight $\mathtt{MUL}$ with  
%Suppose the $\mathtt{ADD}$'s arguments $args \in reg_a$ are \textsc{h}-labeled in $\pi$, and both $\mu_0$ and $\mu'_0$ feature an in-flight $\mathtt{MUL}$. Suppose also that the $\mathtt{MUL}$
at least one zero operand in $\mu$ and no zero operands $\mu'$, and \M{} implements zero-skip multiplies (\S\ref{sec:intro}). 
It is possible that $\mathcal{O}_{\mathcal{R}_C}(\lbbar p \rbbar_{\mathcal{M}}^{\langle\sigma, \mu\rangle}) \neq \mathcal{O}_{\mathcal{R}_C}(\lbbar p \rbbar_{\mathcal{M}}^{\langle\sigma', \mu'\rangle})$ in Eq.~\ref{a:eq:non-interference}, despite $p$'s execution time being \textit{independent} of its high inputs.

Some procedures for verifying hardware side-channel safety side-step the imprecision of a security definition that omits $\mu$ by assuming equivalent initial microarchitectural states for all pairs of compared traces in their \textit{implementations}~\cite{deutschmann:upec-do, deutschmann2023scalable}.
% \yao{removed LEAVE~\cite{wang2023specification}}
% implicitly addressing the imprecise definition above.
Other such procedures directly check this imprecise security definition and require users to navigate false counterexamples as a result~\cite{gleissenthall:iodine, gleissenthall:xenon}.
% \yao{HW-SW contract~\cite{guarnieri:contracts} does leave uarch unconstrained. But in this paragraph we want to cite LEAVE though. LEAVE requires initial uarch to be the same as precondition for ''contract satisfaction'', which in our framework boils down to side-channel free though, without mentioning why. 
%%Prior definitions of hardware side-channel safety omit $\mu$ in Eq.~\ref{a:eq:non-interference}, leaving the initial microarchitectural states for pairs of traces compared by the consequent implicitly unconstrained~\cite{guarnieri:contracts, deutschmann:upec-do, deutschmann2023scalable, gleissenthall:iodine, gleissenthall:xenon}.
%%Prior definitions of hardware side-channel safety either omit $\mu$ in Eq.~\ref{a:eq:non-interference} and left the initial microarchitectural states for pairs of traces compared by the consequent implicitly unconstrained~\cite{deutschmann:upec-do, deutschmann2023scalable, gleissenthall:iodine, gleissenthall:xenon}.
% }
% this imprecision when verifying hardware side-channel safety~\cite{gleissenthall:iodine, gleissenthall:xenon}.




% Meanwhile, other verification procedures consider arbitrary initial microarchitectural states at the cost of imprecise analyses~\cite{gleissenthall:iodine, gleissenthall:xenon}.
% \rsout{The same}\yao{Some of the same} prior works~\cite{guarnieri:contracts, deutschmann:upec-do, deutschmann2023scalable} do implicitly acknowledge the imprecision above by constraining hardware side-channel verification procedures to consider equivalent initial microarchitectural states, as we do.\yao{; while some ~\cite{gleissenthall:iodine, gleissenthall:xenon} unnecessarily assume equality may be too constrained and allow initial states to have non-equal microarchitectural states. }
%\yao{Or: prior works~\cite{wang2023specification, deutschmann:upec-do, deutschmann2023scalable} do not explicitly reason about why the equality is required; some~\cite{gleissenthall:iodine, gleissenthall:xenon} unnecessarily assume equality may be too constrained and allows initial states to have non-equal microarchitectural states. }


% details of definitions of hardware side-channel omit the red text in Eq.~\ref{a:eq:non-interference}
% Note that Eq.~\ref{a:eq:non-interference} features a more precise definition of hardware side-channel safety than prior work, which omits the red text~\cite{guarnieri:contracts, gleissenthall:iodine, gleissenthall:xenon, deutschmann:upec-do, deutschmann2023scalable}.
% % , thereby exclusively considering the case where $\mu_0 = \mu'_0$~\cite{guarnieri:contracts, others}.
% % \footnote{Prior work only considers the case where $\mu_0 = \mu'_0$~\cite{}.}
% % \chris{might want to add a footnote saying that the new property is sound but more precise because prior work only considers the case when $\mu=\mu'$, which the above also checks}
% We find that the red text is required to avoid \textit{mis-classifying} a safe program $p$ running on microarchitecture \M as \textit{unsafe} with respect to receiver \R{}.
% As an example, consider $p = \{\mathtt{li~r1,3}$; $\mathtt{li~r2,2}$; $\mathtt{ADD~r1, r1, r2}\}$
% % consisting of a single $\mathtt{ADD}$
% executing on \M from initial states, $\langle \sigma_0, \mu_0 \rangle$ and $\langle \sigma'_0, \mu'_0 \rangle$. 
% Supposed that $\mu_0$ and $\mu'_0$ feature an in-flight $\mathtt{MUL}$, which  
% %Suppose the $\mathtt{ADD}$'s arguments $args \in reg_a$ are \textsc{h}-labeled in $\pi$, and both $\mu_0$ and $\mu'_0$ feature an in-flight $\mathtt{MUL}$. Suppose also that the $\mathtt{MUL}$
% has at least one zero operand in $\mu_0$ and no zero operands $\mu'_0$.
% Assume also that \M implements zero-skip multiplication (\S\ref{sec:intro:this-paper:spec-challenge}). 
% Here, it is possible that $\mathcal{O}_{\mathcal{R}_C}(\lbbar p \rbbar_{\mathcal{M}}^{\langle\sigma_0, \mu_0\rangle}) \neq \mathcal{O}_{\mathcal{R}_C}(\lbbar p \rbbar_{\mathcal{M}}^{\langle\sigma'_0, \mu'_0\rangle})$, despite $p$'s execution time being \textit{independent} of its own high inputs.
% Program $p$ only operates on immediate fields which are \textsc{h}-labeled in $\pi$.
% Receiver $\mathcal{R}_C$ may observe distinct execution times for $p$ that are \textit{independent} of $p$ its operands, yet Eq.~\ref{a:eq:non-interference} will fail. 
% \artem{Conceptually, the orange text makes perfect intuitive sense. Pragmatically, is it obvious to the reader why there would be two initial states differing only by the uarch parts?}
% \chris{Is this example sending the right message?  Don't we need a case where the antecedant holds for a set of initial states not considered by the prior work?}



%We here present a formal reasoning on how leakage contracts exported from the synthesized leakage signatures are sound and complete.
% 
% Recall an RTL leakage contract verification procedure is complete ...
% and 
% soudn ... 


\subsubsection{Receiver Assumptions}
\label{a:sec:tspec:receiver-assumptions}
% Given our definitions of \upaths{} (\S\ref{sec:tspec-upaths-by-example}) and PLs (\S\ref{sec:tspec:pls}),
% A \pct{} contract may be defined with respect to any receiver \R{}.
%We verify all variety of leakage contracts exported from leakage signatures with respect to a novel receiver \Rupath{} that observes instruction \upaths{}.
In \S\ref{sec:tool:security-arg} of main paper, we assume a receiver $\mathcal{R}_{\upath{}}$ and thus $\mathcal{O}_{\mathcal{R}_{\upath{}}}$  abstractly. 
Here we provide the formal definition of it.

% on a microarchitecture. 
% $\mathcal{R}_{\upath{}}$
% A key novelty of \pct{} contracts is that they assume a receiver $\mathcal{R}_{\upath{}}$, which observes the \upaths{} of instructions as they execute.
We define $\mathcal{O}_{\mathcal{R}_{\upath{}}}$ using one auxiliary definition.
%(\S\ref{sec:background:sec-def})
% s. First, we say that ``instruction $i$ is in-flight in state $\langle \sigma, \mu \rangle$,'' or $in\hbox{-}flight(i, \langle \sigma, \mu \rangle)$, iff $i.\mathtt{II} \in \mu(\mathtt{IIRs})$. Second, 
We say that ``dynamic instruction $i$ \textit{visits} PL $pl$ in state $\langle \sigma, \mu \rangle$,'' or $visit(i, pl, \langle \sigma, \mu \rangle$), iff $\mu(pl.\mathtt{IIR}) = i.\mathtt{II} \land \mu(pl.\mu \mathtt{FSM}) = pl.\mathtt{state}$.
Thus, $\mathcal{O}_{\mathcal{R}_{\upath{}}}(\langle \sigma, \mu \rangle) = \{pl \mid \exists i. visit(i, pl, \langle \sigma, \mu \rangle) \}$, or \Rupath{} observes, at each cycle, the set of PLs visited by in-flight instructions. 
% \yao{in-flight = dynamic? Should this be $i_I$?  }
% for any instruction $i$ in an executing program $p$, $\mathcal{R}_{\upath{}}$ observes all PLs that it visits in each state.
% \yao{The sentence sounds like $O$ knows exact mapping of $i$ and the PLs it visited, and as we discussed before observer doesn't need to know which $i$ is in which PL. Propose: ``i.e., $\mathcal{R}_{\upath{}}$ observes, at each cycle, all PLs resided by any inflight instruction $i$ in an executing program $p$.''}% Sometimes, we are interested in identifying only the PLs in which a particular instruction $i$ resides in state $\langle \sigma, \mu \rangle$, i.e.,  $\mathcal{O}^i_{\mathcal{R}_{\upath{}}}(\langle \sigma, \mu \rangle) = \{pl \mid visit(i, pl, \langle \sigma, \mu \rangle) \}$.
% $\mathcal{O}_{\mathcal{R}_{\upath{}}}(\langle \sigma, \mu \rangle) = \{pl \mid in\hbox{-}flight(i) \land visit(i, pl, \langle \sigma, \mu \rangle) \}$. 

% $\mathcal{O}_{\mathcal{R}_{\upath{}}}(\langle \sigma, \mu \rangle) = \mu (\mathrm{IDRs}, \mu \mathrm{FSMs})$. 
Informally, for $\mathcal{R}_{\upath{}}$, Eq.~\ref{a:eq:non-interference} is valid for an arbitrary program (that satisfies our assumptions in \S\ref{a:sec:background:sec-def:program}) if no instruction can create \upath{} variability for any instruction (including itself) as a function of its operands on the target microarchitecture.
Note that $\mathcal{R}_{\upath{}}$
% $\mathit{commit} \in \mu \mathrm{FMSs}$, so $\mathcal{R}_{\upath{}}$
is strictly more powerful than $\mathcal{R}_C$ (\S\ref{a:sec:background:sec-def}), capturing a receiver that perceives channel modulations via their impact on execution time and more~\cite{perf_counter_sc, acousticexploit, radiationexploit,KocherDPA,sok_em_side_channels,portsmash,memjam,xu:controlledchannelattacks}.
% drama, tlb_bleed, powerexploit 
%
%perf_counter_sc,powerexploit, acousticexploit, radiationexploit,KocherDPA,sok_em_side_channels}.
%resource contention~\cite{branchpred_sc, andrysco:subnormal, portsmash, memjam, xu:controlledchannelattacks, drama, tlb_bleed}, etc.
%~\cite{perf_counter_sc,powerexploit, acousticexploit, radiationexploit,KocherDPA,sok_em_side_channels}.



\subsection{\texorpdfstring{\upaths{}}{upaths} And Decisions Formalized}
\label{a:sec:spec:upathdecformal}
\subsubsection{\texorpdfstring{\upaths{}}{upaths} Formalized}
\label{a:sec:tspec:upathsdef}
%\rsout{
We define 
% A dynamic instruction $i$ with type $I$ exhibits one out of a set
$\boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathcal{M}$ as the set of all possible \upaths{} that a dynamic instance of instruction \textit{type} $I$ may exhibit when it runs on micraorchitecture \M{}.
% ; $\boldsymbol{\mu \textsc{\textbf{path}}^i_\mathcal{M}}$ as the set of all \upaths{} that $i$ may exhibit on \M{}.
% more than one \upath{} when it runs on a microarchitecture \M{}.
% }\yao{already mentioned in scene setting text earlier}
% We now
% \caroline{Please use this notation below:}
%we formally define the set $\mu \textsc{path}^{I}_\mathcal{M}$ of all \upaths{} that instruction $i$ may exhibit on microarchitecture \M{}.
% define the set $\boldsymbol{\mu \textsc{\textbf{path}}^i_\mathcal{M}}$ of all \upaths{} that instruction $i$ may exhibit on \M{}.
%
%
% \rsout{
% Then, $\upath_i = \{(pl, pl') \mid \exists t. con(pl, pl') \wedge visit(i, pl, t[k]) \wedge
% visit(i, pl', t[k+1])\}$.} \caroline{This is not capturing a notion of edge weights/revisits.}
% %
%\yao{$pl$ can be equal to $pl'$; we summarize consecutive revisits using node weight $w: (nodes ,\mathbb{N}) = \{ (pl, n) | \arg\max_n \exists t. (\forall j. 0 \le j < n, visit(i, pl, t[k+j])) \}$}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%To define a \upath{} for $i$, we first collect an ordered sequence of PLs visited by $i$ in trace $t$: $V = (s_0, s_1, .. s_j)$ where $ s_j = \{pl \mid visit(i, pl, t[k+j]\}\}$. The \upath{} for $i$ is thus an ordered list of tuples $E = (e_1, e_2, ..)$ where $e_j = \{(pl, pl')  \mid conn(pl, pl') \wedge pl \in s_{j-1} \wedge pl' \in s_j\} $
%\\
%\\
% \yao{
% As described below, e
Each
$p \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathcal{M}$ 
% $\mu \textsc{path}^{I}_\mathcal{M} \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathcal{M}$ 
% represents some \upath{} that $i$ may exhibit on \M{} in some trace $t$. It
is a tuple $(V, E)$, where $V$ and 
$E$ are sequences of \textit{sets of PLs} and \textit{sets of happens-before edges}, respectively, as defined below.

% \chris{how are edge weights/time encoded in this representation?}
%\yao{A post-processing pass summarizes the revisited PLs using the node weight (numbers after row labels) for consecutively-visited (non-consecutively-visited) PLs.}
% is a sequence of partial orders defined as follows. 
Consider an execution trace $t$, where a dynamic instruction of type $I$, $i_I$,  materializes in \M{} (i.e., appears in some PL) in state $t[j]$, and dematerializes (i.e., disappears from all PLs) in state $t[k]$, where $j<k$.
Suppose $i_I$ exhibits $p = (V, E) \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathcal{M}$ from $t[j]$ through $t[k-1]$.
We define $V = (v_0, v_1, ..., v_{k-j-1})$, where $v_n = \{pl \mid visit(i_I, pl, t[j+n]) \}$ captures the set of PLs visited by $i_I$ in step $n$ of its execution.
% , sequenced sets of PLs visited at $n$-step of $i$'s execution.   
We define $E = (e_0, e_1, ..., e_{k-j-2})$, where $e_n = \{(pl, pl') \mid con(pl, pl') \wedge pl \in v_n  \wedge pl' \in v_{n+1}\}$ captures happens-before ordering between $i_I$'s visits to PLs in consecutive trace steps.
% captures happens-before ordering between \upath{} nodes. 
% We use dashed edge with label \inst{l} in Fig.~\ref{fig:upaths-example} to summarize \inst{l} consecutive revisits to the same PL where only first or last visit is incident with any edge. 
% Old def w/o weights:
% We define $V = (v_0, v_1, ..., v_{k-j-1})$, where $v_n = \{pl \mid \exists i. visit(i, pl, t[j+n])\}$ captures the set of PLs visited by $i$ in step $n$ of its execution. We define $E = (e_0, e_1, ..., e_{k-j-2})$, where $e_n = \{(pl, pl') \mid  con(pl, pl') \wedge pl \in v_n  \wedge pl' \in v_{n+1}\}$ captures happens-before ordering between $i$'s visits to PLs in consecutive trace steps.
% \yao{remove $\exists i.$ since this is constrained under an $i$}.  
 %\yao{Updated to match figure: }
%  New def w/weights:
% \rsout{We define $V = (v_0, v_1, ..., v_{k-j-1})$, where $v_n = \{(pl, l) \mid l > 0 \land \neg visit(i, pl, t[j+n-1]) \wedge (\wedge_{q = 0}^{l} visit(i, pl, t[j+n+q]))\} \cup \{(pl, 1) \mid visit(i, pl, t[j+n]) \wedge \neg visit(i, pl, t[j+n+1])\}$. The first set builder captures consecutively revisited PLs that are newly visited in $t[j+n]$ and assigns them label $l$. The second set builder captures all PLs visited for the last consecutive cycle in $t[j+n]$ and assigns them label $1$.
% We define $E = (e_0, e_1, ..., e_{k-j-2})$, where $e_n = \{(pl, pl') \mid  \exists l, l'. \land con(pl, pl') \wedge (pl, l) \in v_n  \wedge (pl', l') \in v_{n+1}\}$ captures happens-before ordering between \upath{} nodes.}
% \yao{FIGTWO:
% We define $V = (v_0, v_1, ..., v_{k-j-1})$, where $v_n = \{pl \mid visit(i, pl, t[j+n]) \}$, sequenced sets of PLs visited at $n$-step of $i$'s execution.   
% We define $E = (e_0, e_1, ..., e_{k-j-2})$, where $e_n = \{(pl, pl') \mid con(pl, pl') \wedge pl \in v_n  \wedge pl' \in v_{n+1}\}$ captures happens-before ordering between \upath{} nodes. 
% We use dashed edge with label \inst{l} in Fig.~\ref{fig:upaths-example} to summarize \inst{l} consecutive revisits to the same PL where only first or last visit is incident with any edge. 
% If there is not out/in-going edges to $pl$ across multiple visits $\wedge_{n=k}^{n=k+l} (pl, pl)$ we summarize using 
% } 
% $i$'s first/final visits to PLs in consecutive trace steps.
% visited captures PLs visited across $l$ consecutive cycles as one PL with node label $l$ and another with node label $1$ (representing final visit), for a total of $l+1$ consecutive visits. \caroline{All pls such that its the first cycle we visit them plus all pls such that it is the last cycle we visit them.}
% \yao{Maybe obvious as from bottom of p.5 when \inst{l} is first used, $l > 0$}
%\yao{Add quantified $l > 0$ (Or maybe obvious, then can be omitted): 
%We define $V = (v_0, v_1, ..., v_{k-j-1})$, where $v_n = \{(pl, l)\mid \exists l > 0. \neg visit(i, pl, t[j+n-1]) \wedge (\wedge_{q = 0}^{l} visit(i, pl, t[j+n+q]))\} \cup \{(pl, 1) \mid visit(i, pl, t[j+n]) \wedge \neg visit(i, pl, t[j+n+1])\} $ captures PLs visited across $l$ consecutive cycles as one PL with node label $l$ and another with node label $1$ (representing final visit), for a total of $l+1$ consecutive visits.
%}
% \yao{the q should be range from 0 to $l-1$ so the total number is $l$ cycles.}
% the set of PLs visited by $i$ consecutively starting in step $n$ of its execution via the first $w-1$ and the final visits. 

% We define $V = (v_0, v_1, ..., v_{k-j-1})$, where $v_n = \{(pl, w-1)\mid \neg visit(i, pl, t[j+n-1]) \wedge (\wedge_{q = 0}^{w-1} visit(i, pl, t[j+n+q]))\} \cup \{(pl, 0) \mid visit(i, pl, t[j+n]) \wedge \neg visit(i, pl, t[j+n+1])\} $ captures the set of PLs visited by $i$ consecutively starting in step $n$ of its execution via the first $w-1$ and the final visits.

%We define $E = (e_0, e_1, ..., e_{k-j-2})$, where $e_n = \{(pl, pl') \mid  \exists l. l'. m. m \le n + l \land con(pl, pl') \wedge (pl, l) \in v_n  \wedge (pl', l') \in v_{m}\}$ captures happens-before ordering between $i$'s visits to PLs in consecutive trace steps.
% We define $E = (e_0, e_1, ..., e_{k-j-2})$, where $e_n = \{(pl, pl') \mid  \exists l, l', m. n < m \le n + l \land con(pl, pl') \wedge (pl, l) \in v_n  \wedge (pl', l') \in v_{m}\}$ captures happens-before ordering between $i$'s first/final visits to PLs in consecutive trace steps.

% We define $E = (e_0, e_1, ..., e_{k-j-2})$, where $e_n = \{(pl, pl') \mid  \exists l, l'. con(pl, pl') \wedge (pl, l) \in v_n  \wedge (pl', l') \in v_{n+1}\}$ captures happens-before ordering between $i$'s visits to PLs in consecutive trace steps.
% \caroline{Yao: fix.}
%Then, a \upath{} for $i$ within a trace $t$, $ \mu \textsc{path}^{I}_\mathcal{M}$, is $(V, E)$: $V$ is a sequence of node sets $\exists k, (v_0, v_1, ...)$, where $v_j = \{pl \mid visit(i, pl, t[k+j])\}$.
%$E$ is a sequence of partial orders set $(e_0, e_1, ..)$ where $e_j = \{(pl, pl') \mid  con(pl, pl') \wedge pl \in v_j  \wedge pl' \in v_{j+1}\}$. 
% In short, $\mu \textsc{path}^{I}_\mathcal{M}$ collects the set of partial orders among $pl$ visited by $i$ in two consecutive steps. 
% }
%We define a \upath{} exhibited by $i$ within a trace $t$, 
%$ \mu \textsc{path}^{I}_\mathcal{M}$, as $(V, E)$, where 
%$V = \{ (pl, r) \mid \forall r. 1 \le r \le (\sum_k visit(i, pl, t[k]))  \}$,  and \\
%$E = \{ ((pl, r), (pl', r')) \mid con(pl, pl') \wedge visit(i, pl, t[k]) \wedge visit(i, pl', t[k+1]) \wedge \sum_{l < k} visit(i, pl, t[l]) = r-1\;\wedge $ \\
%$ \sum_{l' < k} visit(i, pl', t[l']) = r'-1 \}$. \\
%In other words, a path $p \in \boldsymbol{\mu \textsc{\textbf{path}}^i_\mathcal{M}}$ is a set of tuples $((pl, r), (pl', r'))$, where $i$'s $r$-th visit to $pl$ happens one cycle before $r'$-th visit to $pl'$ in some execution trace $t$.
%$\boldsymbol{\mu \textsc{\textbf{path}}^i_\mathcal{M}}$ is thus the set of $\mu \textsc{path}^{I}_\mathcal{M}$ under any trace $t$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \rsout{In other words, a path $p \in \upath_i$ is a set of tuples $(pl, pl')$, where $i$ visits $pl$ one cycle before $pl'$ in some execution trace $t$.}

Above, the predicate $con(pl, pl')$ returns true iff \ufsms{} corresponding to $pl$ and $pl'$ are connected purely by combinational logic in \M{}'s netlist. It requires that \upaths{} exclusively capture \textit{causal} happens-before relationships among visited PLs.

%\yao{TODO}
Note that we use upper-case, like $I$, to denote an instruction \textit{type} (e.g., \inst{MUL~rd, rs1, rd2}) and lower-case, like $i$ to denote a \textit{dynamic} instruction; $i_I$ denotes a \textit{dynamic} instruction of type $I$.
% \yao{\textless{}\textless{}\textless{}}


\subsubsection{Decisions}
\label{a:sec:tspec:transponders:decisions}

% \chris{its hard to tell whether the subscript $i$ refers to an instruction or an index.}
% \yao{Possibly superscript? $(src^i, \mathbf{dst^i})$}

Recall a \textit{\upath{} decision}
$d^{I}_\mathcal{M} = (src, \mathbf{dst})$ 
% $d^{I}_\mathcal{M} = (src^{I}_\mathcal{M}, \mathbf{dst}^{I}_\mathcal{M})$
made by an instruction $I$ on microarchitecture \M{} is a tuple, where 
% $src^{I}_\mathcal{M}$
$src$
is a single \textit{decision source} PL and $\mathbf{dst}$
% $\mathbf{dst}^{I}_\mathcal{M}$
is a set of \textit{decision destination} PLs, that 
distinguishes \textit{at least two} of $I$'s \upaths{} on \M{}.
% of instruction $i$.
% localizes variability in one \upath{} compared to another \upath{} for the same instruction $i$.
We define the set of all decisions $\mathbf{d}^{I}_\mathcal{M}$ that $I$ makes on \M{} below.
% Given an instruction $i$ (e.g., \inst{ADD} in our running example), we can define the set of decisions $\mathbf{d_i}$ across all of $i$'s \upaths{} as follows.
% , corresponding to two dynamic instances of the same instruction.
% \chris{define $\upath_i$}
% \yao{new subsubsection\S\ref{sec:tspec:upathsdef}}

% \rsout{First, we define the set of $i$'s \textit{decision source} PLs as}
% % consider all pairs of $i$'s \upaths{}, $p$ and $p'$, to derive the set of \textit{decision sources}
% \caroline{Please fix this definition:}
% \rsout{$\mathbf{src}^I_\mathcal{M} = \{ pl \mid \forall p, p' \in \upath_i, ~pl \in p.nodes \land pl \in p'.nodes \land next(p, pl) \neq next(p', pl)\}$.
% In other words, a decision source PL $src^{I}_\mathcal{M} \in \mathbf{src}^I_\mathcal{M}$ is followed by a distinct set of \textit{decision destination} PLs in at least two of $i$'s \upaths{} on \M{}.
% Next, we can construct the set of decisions \caroline{Please fix this definition:}
% $\mathbf{d}^{I}_\mathcal{M} = \{(src^{I}_\mathcal{M}, \mathbf{dst}^{I}_\mathcal{M}) \mid \forall  p \in \upath_i, \forall src^{I}_\mathcal{M} \in \mathbf{src}^I_\mathcal{M}, ~\mathbf{dst}^{I}_\mathcal{M} = next (src^{I}_\mathcal{M}, p) \}$.}
% \yao{Below is new text \textgreater\textgreater\textgreater} 
% % $\mu \textsc{path}^{I}_\mathcal{M}

For \upath{} $p = (V, E)$, let 
% $\mathbf{pl}_p = \{pl \mid \exists v_n \in V. pl \in v_n \}$
% \yao{
$\mathbf{pl}_p = \{pl \mid \exists v_n \in V. pl \in v_n \}$
% }
select the set of all PLs that are visited
in $p$.
Let  $next(p, pl) = \{pl' \mid \exists e_n \in E. (pl, pl') \in e_n \}$ select the set of all PLs visited the cycle after $pl$ in $p$.
%\yao{Let  $next(p, pl) = \{pl' \mid \exists e_n \in E. ((pl, w), (pl', w')) \in e_n \}$ select the set of all PLs visited the cycle after $pl$ in $p$.}
We define the set of $I$'s decision source PLs on \M{} as $\mathbf{src}^I_\mathcal{M} = \{ pl \mid \exists p, p' \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathcal{M}. ~pl \in \mathbf{pl}_p \land pl \in \mathbf{pl}_{p'} \land next(p, pl) \neq next(p', pl)\}$.
%For a \upath{} $p = (V, E)$, $v_k \in V, e_k \in E$, %\upath{} of $i$, $p$, 
%%and $pl \in .v_k$, then 
%let $p.e_k(pl) = \{pl' \mid pl \in v_k \wedge (pl, pl') \in e_k \}$, the set of connected PLs visited by $i$ after visiting $pl$ in $v_k$.
%The set of $i$'s \textit{decision source} PLs, $\mathbf{src}^I_\mathcal{M} = \{pl \mid  \forall p, p' \in \boldsymbol{\mu \textsc{\textbf{path}}^i_\mathcal{M}}, \exists k, k', ~pl \in p.v_k \land pl \in p'.v_{k'} \land p.e_k(pl) \neq p'.e_{k'}(pl)\}$.
%% $\mu \textsc{path}^{I}_\mathcal{M}
In other words, a decision source
$src \in \mathbf{src}^I_\mathcal{M}$ 
% $src^{I}_\mathcal{M} \in \mathbf{src}^I_\mathcal{M}$
is followed by a distinct set of \textit{decision destinations} in at least two of $I$'s \upaths{} on \M{}.
We then define the set of \upath{} decisions for $I$ on \M{} as 
$\mathbf{d}^{I}_\mathcal{M} = \{(src, \mathbf{dst}) \mid \exists p \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathcal{M}. src \in \mathbf{src}^I_\mathcal{M} \land 
\mathbf{dst} = \{pl \mid pl \in next(p, src)\}
\}$.
% \yao{%no $\cup$. \\%just $\mathbf{dst} = \{pl \mid \exists (V, E) \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathcal{M}. \exists e_n \in E. (src, pl) \in e_n\}$; %why not use $\mathbf{dst} = \{pl \mid \exists p \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathcal{M}. pl \in next(p, src)$?
% It should be:
% $\mathbf{d}^{I}_\mathcal{M} = \{(src, \mathbf{dst}) \mid \exists p \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathcal{M}. src \in \mathbf{src}^I_\mathcal{M} \land 
% \mathbf{dst} = \{pl \mid pl \in next(p, src)\}
% \}$.
% %$\mathbf{dst} = \exists p \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathcal{M}. \{pl \mid  pl \in next(p, src)$
% }
% \yao{there shouldn't be any $src^I_\mathcal{M}$ to refer to element of $\mathbf{src}^I_\mathcal{M} $}
% \caroline{Check}
% $\mathbf{d}^{I}_\mathcal{M} = \{(src^{I}_\mathcal{M}, \mathbf{dst}^{I}_\mathcal{M}) \mid src^{I}_\mathcal{M} \in \mathbf{src}^I_\mathcal{M} \land \mathbf{dst}^{I}_\mathcal{M} = \bigcup \{pl \mid \exists (V, E) \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathcal{M}. \exists e_n \in E. (src^{I}_\mathcal{M}, pl) \in e_n\}\}$.
% $ \forall  p \in \boldsymbol{\mu \textsc{\textbf{path}}^i_\mathcal{M}}. \forall src^{I}_\mathcal{M} \in \mathbf{src}^I_\mathcal{M}, ~\mathbf{dst}^{I}_\mathcal{M} = next (p, src^{I}_\mathcal{M}) \}$.
%
%Next, we can construct the set of decisions 
%$\mathbf{d}^{I}_\mathcal{M} = \{(src^{I}_\mathcal{M}, \mathbf{dst}^{I}_\mathcal{M}) \mid \forall  p \in \boldsymbol{\mu \textsc{\textbf{path}}^i_\mathcal{M}}, \forall src^{I}_\mathcal{M} \in \mathbf{src}^I_\mathcal{M}, \forall k, \mathbf{dst}^{I}_\mathcal{M} = p.e_k(src^{I}_\mathcal{M}) \}$.
%src^{I}_\mathcal{M} \in p.v_k,
%
%First, we define the set of $i$'s \textit{decision source} PLs as
%$\mathbf{src}^I_\mathcal{M} = \{ pl \mid \forall p, p' \in \boldsymbol{\mu \textsc{\textbf{path}}^i_\mathcal{M}}, \exists r_j \in p, r_{j'} \in p', ~pl \in p.nodes \land pl \in p'.nodes \land (next(pl, r_j) \neq next(pl, r_{j'}))\}$, where $p.nodes$ are all $pl$ visited by $i$ in $p$, and $next(pl, r_j)$ is the set $\{pl' \mid (pl, pl') \in r_j\}$. % for $r_j \in p$. %the $j$-th step for $i$ in $p$. 
%In other words, a decision source PL $src^{I}_\mathcal{M} \in \mathbf{src}^I_\mathcal{M}$ is followed by a distinct set of \textit{decision destination} PLs in at least two of $i$'s \upaths{} on \M{}.
%Next, we can construct the set of decisions 
%$\mathbf{d}^{I}_\mathcal{M} = \{(src^{I}_\mathcal{M}, \mathbf{dst}^{I}_\mathcal{M}) \mid \forall  p \in \boldsymbol{\mu \textsc{\textbf{path}}^i_\mathcal{M}}, \forall r_j \in p, \forall src^{I}_\mathcal{M} \in \mathbf{src}^I_\mathcal{M}, ~\mathbf{dst}^{I}_\mathcal{M} = next (src^{I}_\mathcal{M}, r_j) \}$.
%%%%%%%%
%First, for a path $p \in \boldsymbol{\mu \textsc{\textbf{path}}^i_\mathcal{M}}$, let $next(p, pl)$ be the set $\{\{pl' \mid \forall pl'. \exists r'. ((pl, r), (pl', r')) \in p.E \} \mid \forall r. (pl, r) \in p.V \}$. 
%We define the set of $i$'s \textit{decision source} PLs as
%$\mathbf{src}^I_\mathcal{M} = \{ pl \mid \forall p, p' \in \allpaths. \exists s, s'. s \in next(p, pl) \wedge s' \in next(p', pl) \wedge s \neq s'\}$. 
%%$. (pl,r) \in p.V \land (pl, r') \in p'.V \land next(p, (pl,r)) \neq next(p', (pl, r'))\}$.
%In other words, a decision source PL $src^{I}_\mathcal{M} \in \mathbf{src}^I_\mathcal{M}$ is followed by a distinct set of \textit{decision destination} PLs in at least two of $i$'s \upaths{} on \M{}.
%Next, we can construct the set of decisions 
%%\caroline{Please fix this definition:}
%$\mathbf{d}^{I}_\mathcal{M} = \{(src^{I}_\mathcal{M}, \mathbf{dst}^{I}_\mathcal{M}) \mid \forall  p \in \upath_i. \forall src^{I}_\mathcal{M} \in \mathbf{src}^I_\mathcal{M}.\forall  ~\mathbf{dst}^{I}_\mathcal{M} \in next (p, src^{I}_\mathcal{M}) \}$.
%%Next, we can construct the set of decisions 
%%%\caroline{Please fix this definition:}
%%$\mathbf{d}^{I}_\mathcal{M} = \{(src^{I}_\mathcal{M}. \mathbf{dst}^{I}_\mathcal{M}) \mid \forall  p \in \upath_i. \forall src^{I}_\mathcal{M} \in \mathbf{src}^I_\mathcal{M}.\forall r.  ~\mathbf{dst}^{I}_\mathcal{M} = next (p, (src^{I}_\mathcal{M}, r)) \}$.
% \\ \yao{\textless\textless\textless}

% \caroline{Check once we make other minor changes:}
% Fig.~\ref{fig:upaths-example} highlights decision source PLs (\textcolor{orange}{orange} nodes) and decision destination PLs (\textcolor{Cerulean}{blue} nodes) in the \upaths{} of various instructions according to their execution on CVA6-OP (from our running example) and the original CVA6 design.
% With respect to its two \upaths{} in Fig.~\ref{fig:upaths-example}, \inst{ADD} on CVA6-OP (\M{}) has $\mathbf{src^\mathtt{ADD}_{\mathcal{M}}} = \{\mathtt{ID}\}$ and $\mathbf{d^\mathtt{ADD}_\mathcal{M}} = \{(\mathtt{ID}, \{\mathtt{issue}, \mathtt{scbIss}\}), (\mathtt{ID}, \{\mathtt{ID}\})\}$.

\subsection{Formal Foundation For Leakage Signature Synthesis}
\label{a:sec:tool-approach-formal}
\label{sec:proof_transponder}
% \yao{TODO, reference}

We now prove our claim that \synthlc{} produces a \textit{complete} set of leakage signatures,  which capture all violations of \textit{hardware side-channel safety} (Def.~\ref{a:def:sc_safe}).


% We now present the formal foundation for, and give an overview of, the \synthlc{} approach. 
% \synthlc{} systematically derive a complete set of leakage signatures and thus a set of formally-verified leakage contracts from the RTL of processor microarchitectures \M{}, under the assumption of receiver \Rupath{}, using commercial model checkers~\cite{cadence:jasper_gold}.



% %the \synthlc{} \textit{contract synthesis} approach. \synthlc{} systematically 
% %We now present the formal foundation for, and give an overview of, the \synthlc{} \textit{contract synthesis} approach. \synthlc{} systematically 
% %% and an overvie provide the formal foundation for an automated \textit{leakage contract synthesis} procedure, called \synthlc{}, which systematically
% %derives formally-verified % \textit{partial} 
% %\pct{} contracts from the  RTL of processor microarchitectures \M{}, under the assumption of receiver \Rupath{}, using commercial model checkers~\cite{cadence:jasper_gold}. 
% %\synthlc{}'s intermediate output is a complete set of
% %% \pct{} contracts 
% %% These partial \pct{} contracts, called \tspecA{} models \tspecACupath{},
% %% are derived from a microarchitecture's
% %\textit{leakage signaturess} for \M{}, from which a \pct{} contract is produced via the procedure in \S\ref{sec:tspec:lf-to-tspec}. 
% %% \yao{3.4 did not explicitly mention, I added a sentence.}
% %% \chris{we shouldn't introduce non-leakage signaturess (beyond, say, a brief mention in the text) if we aren't going to use them}
% %a leakagesignatures is a leakage function that is restricted to precisely the yellow-highlighted components of Figs.\ref{fig:leak_fun_muladd}~and~\ref{fig:leakage_func_examples}.
% %% That is, the function body is abstract.
% %% A \pct{} contract 
% %% \caroline{I will edit \S\ref{sec:tspec:lf-to-tspec} and then rephrase this last part.}
% %Hence, \synthlc{}-synthesized \pct{} contracts capture leakage conditions that correspond to \textit{scheduling decisions} only, while ignoring those that correspond to unsafe operand values, i.e., assertion $v = true$ always (\S\ref{sec:tspec:lf-to-tspec}). We call the resulting leakage contracts \pctA{} contracts \tspecHatCupath{} to make our assumptions clear.


% % \tspecCupath{} captures leakage conditions that correspond to rules (ii) and (iii) in \S\ref{sec:tspec:lf-to-tspec}...
% % , but not (i). \textit{except} those which encode how changes in transmitter \textit{operand values} effectuate changes in transponder \upaths{}, i.e., those which correspond to rule (i).
% % \yao{But rule (ii) and (iii) also do not show how changes in op value effectuate changes in upath???}
% % \chris{isn't that underselling?  we capture operand dependencies but just don't say how a change in operand value effectuates a change in uPath.}
% % (rule (i) in \S\ref{sec:tspec:lf-to-tspec}), for the $\mathcal{R}_\upath$ receiver.
% % \yao{1) Not quite sure conditions here means. 2) ``all leakage conditions'' is inexact, unless we have full tspec body. 3) I think you're saying: ``\tspecACupath{} captures all leakage conditions to the granularity of the operand of a transmitter and the type of side-channel that it implicates a transponder with.''}

% % While a significant step, we believe it is possible to synthesize complete \pct{} contracts in future work
% % We propose an automated \textit{leakage contract synthesis} procedure, called \synthlc{}, for synthesizing formally-verified \textit{partial} \pct{} contracts from processor RTL.
% % These partial \pct{} contracts, called \tspecA{} models, enumerate a microarchitecture's (i) transponders and (ii) a set of \textit{abstract} leakage functions for each. a leakagesignatures, which models a channel, contains the highlighted components of Figs.\ref{fig:leak_fun_muladd}~and~\ref{fig:leakage_func_examples}:
% % \begin{itemize}
% %     \item A \textit{transponder} that exhibits \upath{} variability and its relevant \textit{decision node} (function name);
% %     \item All \textit{transmitters} that modulate the channel, \textit{labeled} as intrinsic, static, or dynamic, (function argument list);
% %     \item Which \textit{transmitter operands} control channel modulations (function's transmitter operand dependencies); and 
% %     \item The set of possible channel \textit{modulations} (function range). 
% % \end{itemize} 
% % leakage signaturess, and thus \tspecA{} models, leave details of the function body abstract.

% %In synthesizing \pctA{} contracts from RTL,
% %% of a processor microarchitecture $\mathcal{M}$,
% %\synthlc{} significantly advances the state-of-the-art in leakage contract verification~\cite{gleissenthall:iodine, gleissenthall:xenon, wang2023specification, deutschmann:upec-do, deutschmann2023scalable}.
% %% , which encompasses \textit{contract synthesis}~\cite{deutschmann:upec-do} and \textit{contract satisfaction}~\cite{gleissenthall:iodine, gleissenthall:xenon, wang2023specification, deutschmann2023scalable} approaches (\S\ref{sec:related}).
% %% ~\cite{wang2023specification, deutschmann2023scalable}\yao{$\leftarrow$ I list both synthesis and satisfaction; it seems we should say 'for both synthesis and satisfaction?' as it is followed by a contract satisfaction example$\rightarrow$}.
% %First, \synthlc{} is the first automated approach for formally verifying hardware adherence to \ct{} contracts $\mathcal{C}_{ct}^{\mathcal{M}, \mathcal{R}_C}$ and \ctCupath{}, which \tspecHatCupath{} subsumes (\S\ref{sec:related}).
% %% \footnote{\caroline{We need to have this somewhere, but it should move to where this is discussed:}\yao{\sout{Possibly remove this text...}Moved to related work section} \rsout{We say a contract verification procedure is \textit{sound} if it never classifies an instruction as safe for processing secrets (in certain circumstances for \pct{} contracts) when it is actually unsafe. A contract verification procedure is \textit{complete} if it never classifies an instruction as unsafe for processing secrets (in certain circumstances) when it is actually safe. In general, most prior work is conservatively sound while sacrificing completeness.}}. %~\cite{gleissenthall:iodine, gleissenthall:xenon, deutschmann:upec-do, deutschmann2023scalable, wang2023specification}.}.}
% %% This is because 
% %% \chris{simpler way to say it? $\mathcal{R}_C$ is a projection of $\mathcal{R}_\upath$}
% %% $\mathcal{R}_C \subseteq \mathcal{R}_\upath$ (\S\ref{todo}) and $xmit \subseteq \mtspecHatCupath$ (\S\ref{todo}).
% %% \chris{can we state here precisely what we mean by soundness/completeness in the context of the previous definitions}
% %% \yao{A contract verification procedure is complete if it \textit{always} classifies ``truly'' safe instruction/system as safe. That is, it never raises false alarm by misclassifying safe as unsafe. 
% %% A procedure is sound if it \textit{only} classify ``truly'' safe instruction/system as safe, and thus never miss catching unsafe situations.}
% %% \chris{If we tweak the notation, $\mathcal{R}_C \subseteq \mathcal{R}_\upath$ makes sense and says something precise.}
% %Second, \pctA{} contracts are the first to enable hardware side-channel defenses that account leakage conditions based on scheduling decisions.
% %% for dynamic and static leakage conditions for transmitters, i.e., those which correspond rules (ii) and (iii) in \S\ref{sec:tspec:lf-to-tspec}.
% %% scheduling decisions and state obfuscation on the safety of secret-dependent transmitters.
% %
% % This section provides a formal foundation for our \synthlc{} leakage contract synthesis procedure (\S\ref{}) and gives an overview of the \synthlc{} approach (\S\ref{}), whose implementation we detail in (\S\ref{sec:tsynth-tool}).
% % We are excited to explore synthesis of complete \pct{} contracts in future work (\S\ref{}).

% % Moreover, we lack scalable and automated approaches for formally verifying microarchitectural adherence to \leakagecontracts{}~\cite{arm:dit,intel:doit,riscv_zkt}---\textit{the verification challenge}.
% % A few \textit{contract satisfaction} methodologies have been proposed~\cite{gleissenthall:iodine, gleissenthall:xenon, guaniere:leave, upec-dit-v2}, where a circuit's adherence to a \leakagecontract{} is formally proven or refuted. However, these schemes either target \textit{signal-centric} \leakagecontracts{}~\cite{gleissenthall:iodine,gleissenthall:xenon}, which are too coarse-grained to support CT code, or require significant \textit{manual effort and designer knowledge} to formulate inductive invariants, inspect (possibly spurious) counterexamples, and generally guide the proof effort~\cite{guaniere:leave, deutschmann:upec-do, upec-dit-v2}.


% % \caroline{\tspec{} Approach: 1.5 pages}

% % \caroline{\textbf{Leakage Contract Verification:}
% % \begin{itemize}
% %     \item Contract synthesis instead of contract satisfaction
% %     \item Mostly evaluate trace properties on the DUV
% %     \item No manual invariant writing
% %     \item Path-based cex inspection - to detect imprecise taint analysis only, not spurious cex that correspond to unreachable states
% %     \item Automatic, Sound, Complete (?)
% %     \item Amenable to decomposition (illustrated by looking at cache and core separately)
% % \end{itemize}
% % }

% \subsubsection{Leakage Signature Synthesis Roadmap}
% % \subsection{Formal Foundations for Contract Synthesis}
% \label{a:sec:tsynth-formal-foundation}
% As pointed earlier (\S\ref{a:sec:background:sec-def:program}), most microarchitecture does not enforce Eq.~\ref{a:eq:non-interference} for an arbitrary program (satisfying our assumptions in \S\ref{a:sec:background:sec-def:program}) and privacy policy, given a realistic receiver, like $\mathcal{R}_C$~\cite{arm:dit,intel:doit,riscv_zkt,pandora:isca:21}.

% A violation of Eqn.~\ref{a:eq:non-interference} thus indicates a side-channel leakage that requires the side-channel defense to protect against. 
% It is leakage contracts that summarize all such counterexamples on the targeted microarchitecture and inform succinctly a defense strategy about how program can leaks secret data. 

% Thus to synthesize a complete set of leakage signatures (each of which corresponds to a channel) requires finding all counterexamples to Eqn.~\ref{a:eq:non-interference}, given a realistic receiver. 

% With this in mind, \PathFinder{} and \synthlc{} cooperate to synthesize leakage signatures from \M{}. 
% First, \PathFinder{} effectively discovers an over-approximation of \textit{all} counterexamples to Eq.~\ref{a:eq:non-interference}.
% Second, \synthlc{} refines this over-approximation to the set of true counterexamples and, in doing so, discovers all of \M{}'s leakage signatures (\S\ref{a:sec:tsynth:approach:lf-discovery}).

% %To be exhaustive, defenses often rely on leakage contracts to summarize for them the characteristics of all counterexamples. 

% %that effectively summarizes all counterexapmles in certain structure and inform them the    the cooperation of software anleakage contracts and  



% %Most microarchitecture will produce \textit{counterexamples} when a proof of Eq.~\ref{eq:tspec-defense-NI} is attempted with an empty \pct{} contract.
% %% Most microarchitecture does not enforce hardware side-channel safety by default for an arbitrary program and privacy policy, given a realistic receiver (\S\ref{sec:background:hw-sc-defense}). Hence, attempting to prove Eq.~\ref{eq:tspec-defense-NI} for an empty \pct{} contract will produce \textit{counterexamples}.
% %With this in mind, \synthlc{} synthesizes  \tspecHatCupath{} from $\mathcal{M}$ in three steps.
% %First, it discovers an over-approximation of \textit{all} counterexamples to Eq.~\ref{eq:tspec-defense-NI}  when ${\mathcal{C}_{pcts}^{\mathcal{M}, \mathcal{R_{\upath}}} = \varnothing}$ (\S\ref{sec:tsynth:approach:cex-discovery}). 
% %% Thanks to our \upath{} abstraction (\S\ref{sec:tspec:upaths}), this exploration is exhaustive and automatic.
% %Second, it refines this over-approximation to the set of true counterexamples and, in doing so, discovers all of \M{}'s leakage signaturess (\S\ref{sec:tsynth:approach:lf-discovery}). Third, \synthlc{} derives $(I, op, c)$ tuples from \M{}'s leakage signaturess per \S\ref{sec:tspec:lf-to-tspec} to produce $\mathcal{C}_{pcts}^{\mathcal{M}, \mathcal{R_{\upath}}}$.
% %% , soundly ignoring leakage conditions due to unsafe operand values by assigning $v$ to $true$ always (\S\ref{sec:tspec:lf-to-tspec}).
% %We detail the first two steps below.
% %% outline \synthlc{}'s counterexample discovery and leakage signatures discovery procedures next.

% % and identifies all $(I, op, c) \in \mathcal{C}_{\tau \textsc{spec}}^{\mathcal{M}, \mathcal{R_{\upath}}}$ tuples required to eliminate them .
% % that satisfy:
% % \begin{equation}
% % \begin{split}
\subsubsection{Counterexample Discovery}
\label{a:sec:tsynth:approach:cex-discovery} 
Finding all \textit{counterexamples} to Eq.~\ref{a:def:sc_safe} given an \textcolor{MidnightBlue}{\M{}}, and \textcolor{MidnightBlue}{\Rupath{}}, equates to finding all satisfying \textit{solutions} to:
\begin{equation}
\begin{split}
      \exists p. \exists \pi. \exists \sigma, \sigma'. \exists \mu. (p) \land \\
      \sigma \approx_{\color{Black}\pi} \sigma' \land \underbrace{\mathcal{O_{\color{MidnightBlue}R_{\upath{}}}}(\lbbar p \rbbar^{\langle\sigma, \mu\rangle}_{\color{Black}\mathcal{M}})}_{\mathcal{O}_A}
      \neq \underbrace{\mathcal{O_{\color{MidnightBlue}R_{\upath{}}}}(\lbbar p \rbbar^{\langle\sigma', \mu\rangle}_{\color{MidnightBlue}\mathcal{M}})}_{\mathcal{O}_B}
\end{split}
\label{a:eq:non-interference-cex}
\end{equation}
That is, \synthlc{} must find all ways in which a program $p$ with security policy $\pi$ can produce distinct observations for \Rupath{}, called $\mathcal{O}_A$ and $\mathcal{O}_B$, when running on $\mathcal{M}$ from a pair of low-equivalent architectural states, $\sigma$ and $\sigma'$, and microarchitectural state, $\mu$.
% In particul.ar, \tsynth{] }
% \tspecACupath{} for receiver $\mathcal{R}_\upath$ is the same as exploring the counterexample space for Eq.~\ref{a:eq:non-interference} under the same receiver.
% In particular, we need to find all ways in which a program $p$ that executes from a pair of low-equivalent architectural states, $\sigma_0$ and $\sigma'_0$, and common microarchitectural state $\mu_0$, resulting in traces may produce distinct observation traces for $\mathcal{R}_\upath$.

To do this, \synthlc{} leverages an important observation about all solutions to Eq.~\ref{a:eq:non-interference-cex}.
% that all solutions to Eq.~\ref{eq:non-interference-cex} have something in common.
Namely, 
all distinct valuations of $\mathcal{O}_A$ and $\mathcal{O}_B$ indicate that the same dynamic transponder $i_P$ exhibits distinct decisions at the same decision source PL
%\chris{"For all pairs of traces where $\mathcal{O}_A$ and $\mathcal{O}_B$ are distinguishable, both traces share a common prefix that ends in the same transponder $i_P$ that exhibits different decisions at the same decision..."?}
in traces $t = \lbbar p \rbbar_{\mathcal{M}}^{\langle \sigma, \mu \rangle}$ and $t' = \lbbar p \rbbar_{\mathcal{M}}^{\langle \sigma', \mu \rangle}$,
% where $\sigma \approx_{\pi} \sigma'$, 
as a function of \textsc{h}-labeled data in $\pi$. 
% \yao{TODO: Reference to \S\ref{sec:proof_transponder}}
% \yao{h-labeled data}
We provide the proof in section below (\S\ref{a:sec:proof_transponder}). 
%sketch a proof of this claim in \S\ref{sec:proof_transponder}.
% The argument above yields a powerful result: 
Hence, all valuations of $\mathcal{O}_A$ and $\mathcal{O}_B$ in satisfying solutions to Eq.~\ref{a:eq:non-interference-cex} are captured by identifying all decisions that may be exhibited by transponder instructions on \M{}. 
% To provide more intuition for the above claim, observe that
% We provide more intuition below.

\paragraph{Counterexamples and Transponder Relation}
\label{a:sec:proof_transponder}

Observe that traces $t$ and $t'$, as defined above, satisfy
% consider traces $t = \lbbar p \rbbar_{\mathcal{M}}^{\langle \sigma_0, \mu_0 \rangle}$ and $t' = \lbbar p \rbbar_{\mathcal{M}}^{\langle \sigma'_0, \mu_0 \rangle}$, where $\sigma_0 \approx_{\pi} \sigma'_0$, which satisfy
Eq.~\ref{a:eq:non-interference-cex} iff:
% A counterexample to
% Eq.~\ref{a:eq:non-interference} iff:
\begin{equation}
\begin{split}
      \exists k. \forall j. 0 \leq j < k \land  \mathcal{O}_{\mathcal{R}_\upath}(t[j]) = \mathcal{O}_{\mathcal{R}_\upath}(t'[j])
      \\ \land~\mathcal{O}_{\mathcal{R}_\upath}(t[k]) \neq \mathcal{O}_{\mathcal{R}_\upath}(t'[k])
\end{split}
\label{eq:NI-cex}
\end{equation}
That is, there exists an \textit{earliest} step $k$ of $t$ and $t'$ at which the traces produce distinct 
%is the first step for which $t$ and $t'$ produce distinct
observations for $\mathcal{R}_\upath$.
Given the definition of $\mathcal{O}_{\mathcal{R}_\upath}$ (\S\ref{a:sec:tspec:receiver-assumptions}), the PLs occupied by all in-flight instructions are the same in $t$ and $t'$ from step $0$ through step $k-1$, but different in step $k$.
Distinct observations in step $k$ indicates that some instructions $i$ and $i'$, in-flight in $t$ and $t'$, respectively, visited the same source ($s$) PL in step $k-1$, but distinct destination ($d$) PLs in step $k$: 
% \caroline{Make sure ``in-flight'' is defined somewhere.}\yao{\S\ref{sec:tspec:transponders:path-selector}}
% or $visit(i, pl, t[k-1]) \land visit(i', pl, t'[k-1])$, but distinct destination PLs in step $k$, or $visit(i, pl', t[k]) \land \neg visit(i, pl', t[k])$ for some PL $pl'$.
\begin{equation}
\begin{split}
      \exists i, i'. \exists s. \exists d.
       visit(i, s, t[k-1]) \land visit(i', s, t'[k-1]) \\
      \land~visit(i, d, t[k]) \land \neg visit(i, d, t[k])
\end{split}
\label{eq:NI-cex-transponder}
\end{equation}

Suppose $i$ and $i'$ are the \textit{same} in-flight instruction. We say instructions in trace $t$ and $t'$ are the same if they have the same encoding and feature the same program counter.
% Since only program inputs can be \textsc{h}-labeled in $\pi$, d
Different decisions made by the same instruction at the same decision source PL necessarily indicates different inputs to some path selector function. Since only high data can differ under Eq.~\ref{a:eq:non-interference-cex}'s low-equivalence constraint and only program inputs can be \textsc{h}-labeled in $\pi$, said path selector function inputs must be operand-dependent on some transmitter. Hence, $i = i'$ is a transponder $P$ (\S\ref{sec:synth-lc-approach}).

Now suppose $i$ and $i'$ are \textit{different} in-flight instructions, which may occur in two cases.
We show that under our assumptions, some
% they imply that some
transponder $i_P$ exhibits distinct decisions at the same decision source PL in $t$ and $t'$.

\textit{Case 1 (Control-Flow):} 
In the first case, $t$ and $t'$ feature distinct \textit{fetch streams}, where a fetch stream denotes the sequence of instructions that populate \M{}'s \textit{instruction fetch register} (\inst{IFR}, \S\ref{sec:tool:metadata}). 
% As discussed in \S\ref{sec:tsynth-tool:metadata}, a processor's \inst{IFR} holds instructions when they are first fetched from memory.
% Distinct fetch streams for $t$ and $t'$ is indicative of private data-dependent control-flow in $p$. Since, we are interested in \textit{hardware} side-channels, we assume that 
Recall however, given our program assumptions in \S\ref{a:sec:background:sec-def:program}, that the fetch streams are identical in $t$ and $t'$, yielding a contradiction.
% . This is analogous to assuming that $p$ features the same sequence of instructions along all control-flow paths.
Note that \synthlc{} still flags control-flow instructions as transmitters in this setting, as they may conditionally flush mis-speculated instructions as a function of their operands.

\textit{Case 2 (Delayed Observation):} 
In the second case, some same-instruction pair $j$ and $j'$, in traces $t$ and $t'$, respectively, exhibited different decisions at the same source PL some step \textit{before} $k-1$. Hence, $j = j'$ is a transponder $P$.
However, this \upath{} variability was not detected until $j$ and $j'$  transitively impacted the execution of $i$ and $i'$, respectively. 

% \rsout{Recall that \Rupath{} observes the \textit{set of occupied PLs} in each trace step, but not which instructions occupy each PL.}
% are the same instruction  made different decisions at the same decision source PL at The second scenario arises due to the transitive effects of another same-instruction pair $j$ and $j'$ in-flight in $t$ and $t'$, respectively, which made distinct decisions at the same source PL at some step $0 \leq l < k-1$.
%
\begin{figure}[t]
    \centering
     % \includegraphics[width=0.9\linewidth]{figs/taint_cases.png}
     % \vspace{-7pt}
     % \caption{Constraints on SVA property to classify transmitter as intrinsic (i), dynamic (ii-a/b), or static (iii).
     % }
     % \label{a:fig:taint_cases}
     %\includegraphics[width=0.8\linewidth]{figs/corner_case_1.png}
     \includegraphics[width=0.8\linewidth]{figs/corner_case_2.png}
     % \vspace{-7pt}
     \caption{
     Delayed observation at step $k$ arising from transponder exhibiting distinct decision earlier than step $k-1$.} %   A scenario of case 2b in \S\ref{sec:tsynth:approach:cex-discovery}.
     %
     %at step $k$ can be attributed to same $i$ making distinct decision at step earlier than $k-1$. 
     %Both trace features same fetch stream. While $i_1$ exhibit distinct decisions at step $k-2$, distinct observation happens at step $k$.
     
     \label{a:fig:corner_case}
\end{figure}
% \vspace{-5pt}
% \caroline{This needs a pass after merging:}\yao{Fixed}
% \caroline{Discuss}
Such scenario is illustrated in Fig.~\ref{a:fig:corner_case}. 
%and results % illustrates this scenario: 
%We here discuss ``delayed observation'' case for Eq.~\ref{eq:NI-cex-transponder} in \S\ref{sec:tsynth:approach:cex-discovery} where $i$ and $i'$ are different instructions from same program $p$ occupying the same $pl$ at step $k-1$. % visiting the same $src$ in both $t$ and $t'$ at step $k-1$ and cause a violation of observation equivalence at step $k$. 
% Such case results 
% from same instruction pair $j$ and $j'$ ($j=j'$) in trace $t$ and $t'$ respectively that  
%can be attributed to same instruction $j$ in program already 
% makes distinct decision at step \textit{earlier than} $k-1$. An example is in Fig.~\ref{fig:corner_case}, where 
%both traces feature same fetch stream and at step $k-1$, 
At step $k-2$, $j=j'=i_0$ makes distinct decisions at $pl_B$ in $t$ compared to $t'$.
% , such that at step $k-1$.
In $t$, $i_0$ disappears from all PLs (i.e., progresses to the ``empty'' PL). In $t'$, it remains in $pl_B$.
% $pl_B$ is followed by empty set in $t$ and $\{pl_B\}$ in $t'$. 
However, distinct observations for $\mathcal{R}_\upath$, involving $i = i_2$ and $i' = i_1$ where $i_1 \neq i_2$, do not manifest until later in step $k$. 
% $i=i_1$ and $i'=i_2$ both visit $pl_A$ followed by distinct observation for $\mathcal{R}_\upath$ at step $k$.
% Such distinct observation arises from $j=j'=i_1$ making distinct decision at decision source PL $pl_A$ during step $k-2$. 
%, but distinct observation does not arise until step $k$.
%Both $t$ and $t'$ feature same fetch stream where $i_1$ exhibits \upath{} variability at step $k-1$ already while no violation of Eq.~\ref{eq:NI-cex-transponder} happens until step $k$.


% \chris{its not clear why the instructions where the divergences occur need to be transponders.}
Given the observation above, \synthlc{}'s counterexample discovery using \PathFinder{} over-approximates Eq.~\ref{a:eq:non-interference-cex}'s solution space by
% Equivalently,  Given the discussion above, the set of valuations for  $\mathcal{O}_A$ and $\mathcal{O}_B$ in 
% the set of distinct observations that can satisfy
% Eq.~\ref{eq:non-interference-cex} can be over-approximated as the set of all distinct decisions that can be exhibited by each instruction on \M{} for each decision source.
% are exactly all pairs of distinct decisions that can be exhibited by a transponder instruction for each decision source.
% Hence, \synthlc{}'s counterexample discovery step uncovers
first uncovering all possible \upaths{} for each implemented instruction $I$ on $\mathcal{M}$. Those instructions with more than one \upath{} are flagged as \textit{candidate transponders}. A set of decisions $\mathbf{d}^{P}_\mathcal{M}$ is collected for each candidate transponder $P$ as described \S\ref{a:sec:tspec:transponders:decisions}.
Enabled by user-annotated \ufsms{} (\S\ref{sec:tool:metadata}), \synthlc{} conducts this counterexample discovery step automatically, using commercial model checkers~\cite{cadence:jasper_gold} to evaluate \textit{(single-)trace} properties on \M{} (\S\ref{sec:both-tool}). 



\subsection{Leakage Signature Discovery}
\label{sec:tsynth:approach:lf-discovery}
\synthlc{}'s counterexample discovery procedure (\S\ref{a:sec:tsynth:approach:cex-discovery}) over-approximates the solution space to Eq.~\ref{a:eq:non-interference-cex}, because unique decisions for \textit{candidate} transponders may not represent legitimate valuations of $\mathcal{O}_A$ and $\mathcal{O}_B$ when $p$ with $\pi$ executes \textit{from low-equivalent initial states} on \M{}.
% Counterexample discovery step over-approximates the solution space to Eq.~\ref{eq:non-interference-cex}. We need to determine which valuations of $\mathcal{O}_A$ and $\mathcal{O}_B$ are possible from low-equivalent initial states and further what contract tuples exclude them.
Finding which decisions do represent valid solutions to Eq.~\ref{a:eq:non-interference-cex}, requires finding which decision may depend on \textsc{h}-labeled data in $\pi$.
Since $\pi$ labels program inputs, this is equivalent to finding which decisions  may depend on \textit{transmitter operands}.

\subsubsection{Instantiating Eq.~\ref{a:eq:non-interference-cex}}
\label{a:sec:checking-eq-8}
\begin{figure}[t!]
    \centering
     \includegraphics[width=0.9\linewidth]{figs/taint_cases.png}
     \vspace{-5pt}
     \caption{Constraints on SVA properties to uncover and classify transmitters as (1) intrinsic, (2a/b) dynamic, or (3) static. 
     }
     \label{a:fig:taint_cases}
\end{figure}

To do this, \synthlc{} considers each candidate transponder in turn and systematically derives all of its leakage signatures. A candidate transponder may have \textit{at most one} leakage signatures \textit{per decision} (if it is not a true transponder, it will have none). % So, \synthlc{} considers each decision in turn. 
Consider candidate transponder $P$ and its various decisions on \M{} (in $\mathbf{d}^{P}_\mathcal{M}$) that originate at decision source $src \in \mathbf{src}^P_\mathcal{M}$.
% \yao{$src \in \mathbf{src}^P_\mathcal{M}$}.
% and decision $(src, \mathbf{dst}) \in \mathbf{d}^{P}_\mathcal{M}$. 
Our goal is to derive a its leakage signature \inst{P\_src} (if one exists), which features four components: the signature's (i) \textit{name} (i.e., ``$P$'' concatenated with PL ``$src$''), (ii) \textit{range} (i.e., the set of PL sets $\{\mathbf{dst} \mid (src, \mathbf{dst}) \in \mathbf{d}^{P}_\mathcal{M}\}$), (iii) labeled \textit{transmitters} (i.e., explicit inputs labeled \textit{intrinsic} (\inst{N}), \textit{static} (\inst{S}), or \textit{dynamic} (\inst{D})), and (iv) \textit{unsafe operands} (i.e., operands of explicit inputs that appear in the function body). 
% The decisions gathered for $i_P$ give us
Clearly, we already have (i) and (ii).

We can obtain (iii) and (iv) by instantiating Eq.~\ref{a:eq:non-interference-cex} in various ways as follows. First, select a pair of decisions $d_0, d_1 \in \mathbf{d}^{P}_\mathcal{M}$ for transponder $P$, which feature the same decision source $src$, but distinct decision destinations.
% such that $d_0 \neq d_1$ (i.e., their decision destination PLs $\mathbf{dst}^{I_P}_\mathcal{M}$ are different).
Next, consider all possible (candidate) pairs $(T, op)$ of a transmitter $T$ and its unsafe operand $op$. 
For each pair, constrain program $p$ according to the following three cases below (illustrated in Fig.~\ref{a:fig:taint_cases}) to determine if $P$ exhibits decision $d_0$ versus $d_1$ as a function of $op$. For all cases, assume some $i_T, i_P \in p$ and that the only operand of any instruction in $p$ to be supplied with high data is $op$ of $i_T$ specifically.

%\yao{Could be trimmed since they correspond to three bullets in 3.4 by a) removing below b) update previous sentence: For each pair, constrain program $p$ according to conditions for each of the three labels listed in \S\ref{sec:tspec:lf-to-tspec} to determine if $i_P$ exhibits $d_0$ versus $d_1$ as a function of $op$. For all cases, assume $i_T, i_P \in p$ and that the only operand of any instruction in $p$ to be supplied with high data is $op$.
%Concretely, program conditions are depicted in Fig.\ref{a:fig:taint_cases}, where  \textit{Case 2} is broken into two sub-cases: one where $i_T$ materializes in \M{} before $i_P$ (\textit{Case 2a}) and vice versa (\textit{Case 2b}). }
\textit{Case 1} determines whether $T$ is an intrinsic transmitter with respect to \inst{P\_src} by constraining 
% $i_T = i_P$, i.e., constraining
$i_T$ and $i_P$ to be the same dynamic instruction.
\textit{Case 2} determines whether $T$ is a dynamic transmitter by constraining $i_T$ to be in-flight when $i_P$ visits its decision source $src$.
\textit{Case 3} determines whether $T$ is a static transmitter by constraining $i_T$ to have materialized and dematerialized in \M{} \textit{before} $i_P$ reaches $src$.
These cases are depicted in Fig.\ref{a:fig:taint_cases}, where \textit{Case 2} is broken into two sub-cases: one where $i_T$ materializes in \M{} before $i_P$ (\textit{Case 2a}) and vice versa (\textit{Case 2b}).
% Then, instantiate Eq.~\ref{eq:non-interference-cex} with $\mathcal{O}_A = d_0$ and $\mathcal{O}_B = d_1$, where $i_T, i_P \in p$ such that the only operand of any instruction in $p$ to be supplied with \textsc{h}-labeled data is operand $op$ of $i_T$. 
% To identify intrinsic inputs, $i_T = i_P$ (i.e., they are the same instruction). To identify dynamic inputs, consider the case where $i_T$ first materializes in \M{} before $i_P$ \textit{and} the case where $i_P$ materializes before $i_T$, and only consider executions where $i_T$ is in-flight when $i_P$ reaches $src^i_\mathcal{M}$. To identify static inputs, consider the case where $i_T$ materializes before $i_P$, and only consider executions where $i_T$ has dematerialized when $i_P$ reaches $src^i_\mathcal{M}$. 
If Eq.~\ref{a:eq:non-interference-cex} is satisfied in any of these cases, we have \textit{labeled} transmitter $T$ with unsafe operand $op$.



% have left copy featuring two ADD that pack together while right copy of two ADD do not pack implies (left copy can fetch new instruction earlier than right copy.), which contradicts with the constraint of two copies issue new instruction always at same cycle


% However, this stalling will misclassify transponder decisions as \textit{independent} of \textit{dynamic} transmitters in particular. For example, suppose $i_T$ is fetched in both traces in time step $0$ and that one trace is stalled due to back-pressure in time step $1$. The other trace will wait to catch up.
% which stalls one trace from fetching in time step $1$ stalling a trace may allow an in-flight dynamic transmitter to progress far enough in its execution such that it can no longer impact a transponder's 
% One option is to construct assumptions for each fetch instruction in advances for the two traces. However, since the number of assumptions must be finite, this requires bounding the number of instructions that appear between $i_T$ and $i_P$. Another option is to lock-step the two copies such that they always issue instructions at the same cycle. However, this constraint as an assumption limits interaction between transmitter and transponder and causes missing cases such as operand packing (since the assumption will preclude back-to-back ADD that will fast-forward one copy).
% Alternatively, 

% synchronizes the two copies by stalling one copy to wait for the other with respect to some constraint. E.g., stalling the instruction fetch of one copy if it has fetch more instructions than the other. However, such synchronization will prevent Suppose we have a pair of $i_T = \mathtt{MUL}$ fetched in the two copies, where one is slow and the other is fast. The slow \inst{MUL} will prevent its trace from fetching a new instruction, so the trace with the fast \inst{MUL} will wait for the slow trace to catch up. Once it does, subsequent instructions will no longer exhibit distinct decisions due to \inst{MUL}. This is particularly an issue for dynamic transmitters.

\subsubsection{Symbolic IFT}
\label{a:sec:tsynth-approach:symb-ift}
In theory, the various instances of Eq.~\ref{a:eq:non-interference-cex} described can checked on \M{} by: (i) constructing a \textit{product circuit}, where \M{} is instantiated twice, to check the property directly~\cite{wang2023specification, deutschmann:upec-do}, or (ii) augmenting \M{} with \textit{information flow tracking} (IFT) circuitry to check the property indirectly~\cite{gleissenthall:xenon, gleissenthall:iodine}.
The first strategy is regarded as more precise~\cite{yang2018lazy}. However, with our goal of attributing transponder decisions to transmitter operands, it exhibits a soundness limitation as we discuss in a separate section (\S\ref{a:sec:product-circuit-limitations}).

% We refer the interested reader to \S\ref{} for more details.
% Due to issues outlined in 
% the limitations associated with the product circuit formulation of % these limitations, we decide to instantiate
% \S\ref{sec:product-circuit-limitations}, 

Hence, \synthlc{} checks Eq.~\ref{a:eq:non-interference-cex} using symbolic IFT
% using symbolic information flow tracing (IFT) formulation.
% In particular, we create 
% $\mathcal{M}_{IFT}$, which a augments 
by augmenting \M{} with cell-level IFT
% \rsout{gate-level}\yao{More precise: ``cell-level'' (ref Table 14.3 in ~\cite{weste1985principles}} IFT
circuitry~\cite{solt2022cellift} to produce $\mathcal{M}_{IFT}$.
% \yao{~\cite{solt2022cellift}}.
% .
For \textit{Case 1} (intrinsic) and \textit{Case 2} (dynamic) in \S\ref{a:sec:checking-eq-8}, $\mathcal{M}_{IFT}$ features a single ``taint'' bit per data bit in \M{}'s netlist. 
To enforce that only $op$ of $i_T$ may be supplied \textsc{h}-labeled data (\S\ref{a:sec:checking-eq-8}), \synthlc{} exclusively sets the taint bit associated with $op$ and prevents taint propagation from $i_T$'s output to the input of any other instruction (architecturally or speculatively).
% primary inputs of other instructions (architecturally or speculatively).
For \textit{Case 3} (static) in \S\ref{a:sec:checking-eq-8}, $\mathcal{M}_{IFT}$ features two taint bits per data bit in \M{}'s netlist (\S\ref{sec:tsynth-tool:f-leak-syn}). 
This implementation choice allows \synthlc{} to effectively flush ``sticky'' taint that is associated with $op$'s dynamic influence on transponders \upaths{}, thereby considering its static influence exclusively.
We briefly describe the implementation as follows.

\paragraph*{Symbolic IFT for Static Transmitter}

%Recall from \S\ref{sec:tsynth-approach:symb-ift} that for \textit{Case 3} (static) in \synthlc{}'s symbolic IFT analysis, $\mathcal{M}_{IFT}$ features two taint bits (upper and lower) per data bit in \M{}'s netlist. 
Taint flows exclusively within upper taint bits or lower taint bits. However, when a data bit's upper taint bit is set, it clears the lower taint bit.

To enforce that only $op$ of $i_T$ may be supplied with \texttt{h}-labeled data, \synthlc{} exclusively sets the \textit{lower} taint bit associated with $op$ and prevents taint propagation from $i_T$'s output to the input of any other instruction (architectural or speculatively).

To uncover static transmitters, \synthlc{} effectively flushes $i_T$'s dynamic influence by setting the \textit{higher} taint bit associated with the operands of all instructions that are fetched after $i_T$ and before $i_P$. These intermediate instructions are constrained such that when $i_P$ is issued the lower taint bits for all \ufsms{} are cleared.



% For static transmitter, % aside from the constraint on issuing of instructions, 
% %we augment design with 
% two-bit IFT circuit is set up and \synthlc{} supplies \inst{h}-labeled data by setting \textit{lower} taint bit associated with \inst{op} when $i_T$ is at issue stage. 
% To flush the dynamic influence, \synthlc{} first introduces taints at \textit{higher} taint bit for instructions that are fetched after $i_T$ and before $i_{P}$.
% %of such that 
% %taint at bit zero  at bit 0 for $i_T.op$ (i.e., supplied with \inst{h}-labeled data), and bit 1 for operands of interim instructions that are fetched after $i_T$ and before $i_{P}$.
% %For each register, taint at bit 1, if high, resets taint at bit 0 a cycle before the issue of transponder $i_{P}$. 
% %%at \ufsms{} specifically a cycle before the issue of $i_{P}$.
% The interim instructions are then constrained such that when $i_{P}$ is issued, lower taint bit for all \ufsms{} are cleared.   
% Under the assumption that a static channel, if exists, is not written by all implemented instructions, the constraint eliminates the dynamic influence induced at \ufsms{} by $i_T$, but does not imply all feasible traces featuring flushes of the static channel induced by $i_T$.
% %per the assumption that a static channel, if exists, is not written by all implemented instructions. 
Given this two-bit IFT approach, the state space in Table~\ref{table:relatedwork} for \synthlc{} is $2^n$ for path exploration and $2^{3n}$ for symbolic taint tracking respectively.




%\subsection{Figures}



% \subsection{Different Defenses and Contracts}
% %{
%    \begin{table}[t]
%    \renewcommand{\arraystretch}{1.4}
%    \setlength\tabcolsep{0.8pt}
%    \centering
%    \footnotesize
%    %\tiny
%    \begin{tabular}[t]{
%            |>{\centering\arraybackslash} m{15mm} %0.001\textwidth}
%            |>{\centering} m{15mm} %0.001\textwidth}
%            |>{\centering} m{12mm} %0.001\textwidth}
%            |>{\centering} m{14mm} %0.001\textwidth}
% %            |>{\centering} m{15mm} %0.001\textwidth}
%            |>{\centering\arraybackslash} m{15mm}|
%            }
%            \hline
%            Side-channel defense & Constant-time (CT) defense & CT defense w.r.t $\mathcal{R}_C$ & \pct{} defense &  
%            \pct{} defense w.r.t $\mathcal{R}_\upath$ \\
%            \hline
% $\mathcal{D}^{\mathcal{R},\pi}$     &  
% \ctD{} &
% $\mathcal{D}_{ct}^{\mathcal{R}_C, \pi}$ & %$\mathcal{C}^{\mathcal{M}, {\mathcal{R}_C}}_{xmit}$ & 
% \tshieldD{} &
% \tshieldDupath{} 
% \\
% \hline 
% $\mathcal{C}^{\mathcal{M}, \mathcal{R}}$ & 
%  \ctC{} &
% $\mathcal{C}^{\mathcal{M}, {\mathcal{R}_C}}_{xmit}$ & %$\mathcal{C}_{ct}^{\mathcal{R}_C}$  &
% \tspecC{} &
% \tspecCupath{} \\ 
% \hline
%    \end{tabular}
% %   \\ [3pt]
%    \caption{Defenses facilitated by the leakage contracts. }
%    %\yao{The example where CT defense is not w.r.t $\mathcal{R}_C$ includes say $\mathcal{R}$ observing perf counter value or like value of memory request control output value?} 
%    \label{table:defenses}
% \end{table}
% %\vspace{-20pt}
% \yao{Not referenced anywhere. Probably could killed. Or we could reference in the sec 4?}
% Table.~\ref{table:cds} summarizes the different defenses and corresponding contracts discussed in \S\ref{sec:tspec} and \S\ref{sec:tsynth-approach}. \tsynth{} synthesizes a class of  \tspecCupath{} -- \tspecHatCupath{}. 


%\subsection{To replace}
%\subsubsection{Fig. 1}
%\yao{Todo:  \\
%- Fig. 1a source change to \texttt{figs/mul\_sub\_1\_10.png} shown as below \\ 
%- Fig. 1a caption change to:  ``\upaths{}. Row\textsubscript{r}: \textit{remaining} visit to Row. Node tag \inst{l}: \inst{l} last visit to Row.''
%- Relevant main text doesn't need to change 
%}
%\begin{figure}[h!]
%\begin{subfigure}{0.52\linewidth} 
%    \centering
%     \includegraphics[width=0.8\linewidth]{figs/mul_sub_2.png}
%     %\vspace{-2pt}
%     \caption{\upaths{}. Row\textsubscript{1/l}: 1st/\inst{l}-th visit to Row. Subpath tag \inst{l}: \inst{l} visits to Row.}
%     %, n: \# in node). \textcolor{myred}{$\rightarrow$}: in-order commit. }
%     %\caption{\upaths{}. Row(f/l): exec. phase (first \inst{n}/last visit, \inst{n}: \# in node). }%, n: \# in node). \textcolor{myred}{$\rightarrow$}: in-order commit. }
%     %\label{fig:zero-skip-uhb}
%\end{subfigure}%
%~
%\hspace{0.01\linewidth}
%\begin{subfigure}{0.44\linewidth} %130pt} %.55\linewidth}
%    \begin{tcolorbox}[left=0.2pt,right=0.2pt,top=1pt,bottom=1pt]
%    %\begin{framed}
%    \footnotesize
%      \noindent\textcolor{ForestGreen}{{\RaggedLeft// 
%      \inst{MUL} skips computation if it has zero operands or stays until \inst{done}}}\\
%      %\inst{MUL} stays in \inst{mulU} for one cycle if it has zero operands, else stays four.}}\\
%      %takes path 1 if at least one argument is 0, else it takes path 1.}}\\
%%    {
%%    \setlength{\arrayrulewidth}{1pt}
%%       \renewcommand{\arraystretch}{1.3}
%%     \begin{tabular}[t]{
%%       @{}>{\raggedright\arraybackslash} m{113pt} %0.9\linewidth}
%%       }
%    %\noindent\textcolor{ForestGreen}{\RaggedLeft// Precondition}\newline
%%     \centering\arraybackslash $\mathsf{visit(i0, mulUnit)}$ \\[2pt]
%     %\rule{118pt}{0.4mm} 
%    \hlt{\noindent$\mathsf{dst\;MUL\_mulU(MUL_I\;i0)\!:}$} %\textcolor{ForestGreen}{// Leakage function} 
%    \newline
%%        \indent$\;\;\mathsf{path\_id = ((}$\hlt{$\mathsf{i0.\iparg{arg0}}$}$\mathsf{== 0)\;\vee}$ \newline 
%        \indent$\;\;\mathsf{\textcolor{blue}{return}\;ite((}$\hlt{$\mathsf{i0.\iparg{arg0}}$}$\mathsf{\;== 0)\;\vee}$ \newline
%        \indent$\;\;\;\;\mathsf{(}$\hlt{$\mathsf{i0.\iparg{arg1}}$}$\mathsf{ \;== 0) \vee done, }$\newline
%        %$\mathsf{(path\_id == 1), }$\newline 
%        \indent$\;\;\;\;\hlt{$\mathsf{\{mulFin\},}$}$\hlt{$\mathsf{
%        %\{mulUnitFin\}, 
%        \{mulU\}}$}$\mathsf{)}$
%%    \end{tabular}
%%    }
%    \\[3pt]
%      \noindent\textcolor{ForestGreen}{{\RaggedLeft// \inst{SUB} proceeds or get stalled by \inst{MUL} until it commits ($\mathtt{i1.cmt}$) }}\\
%    %{
%    %\setlength{\arrayrulewidth}{1pt}
%    %   \renewcommand{\arraystretch}{1.3}
%    % \begin{tabular}[t]{
%    %   @{}>{\raggedright\arraybackslash} m{113pt} %0.95\linewidth}
%    %   }
%    %\noindent\textcolor{ForestGreen}{\RaggedLeft// Precondition}\newline
%    % \centering\arraybackslash $\mathsf{visit(i0, scbFin)}$ \\[2pt]
%    % \hline
%    % 
%    \hlt{\noindent$\mathsf{dst\;SUB\_scbFin(MUL^D\;i1)\!:}$}
%    %\textcolor{ForestGreen}{// Leakage function} 
%    \newline
%        \indent$\;\;\mathsf{\textcolor{blue}{return}\;ite(((}$\hlt{$\mathsf{i1.\itarg{arg0}}$}$\mathsf{\;== 0)\;\vee}$ \newline
%        \indent$\;\;\;\;\mathsf{(}$\hlt{$\mathsf{i1.\itarg{arg1}}$}$\mathsf{ \;== 0))\vee i1.cmt, }$\newline
%        % rdy should be seomthing like atH(i1) 
%        \indent$\;\;\;\;$\hlt{$\mathsf{\{scbCmt\},}$}\hlt{$\mathsf{\{scbFin\}}$}$\mathsf{)}$
%        %\newline
%        %%$\mathsf{(path\_id == 1), }$\newline 
%        %\indent$\;\;\;\;$\hlt{$\mathsf{
%        %%\{mulUFin\}, 
%        %\{mulU\}}$}$\mathsf{))}$
%        %\indent$\;\;\mathsf{path\_id = ((}$\hlt{$\mathsf{i1.\itarg{arg0}}$}$\mathsf{ == 0)\;\vee}$\newline 
%        %\indent$\;\;\;\;\mathsf{(}$\hlt{$\mathsf{i1.\itarg{arg1}}$}$\mathsf{ \;== 0))}$ \newline
%        %\indent$\;\;\mathsf{\textcolor{blue}{return}\;ite((path\_id == 1), 
%        %}$\newline
%        %\indent$\;\;\;\;$\hlt{$\mathsf{\{scbCommit\}, \{scbFin\}}$}$\mathsf{)}$
%    %\end{tabular}
%    %}
%    %\\[3pt]
%    \end{tcolorbox}  
%    \vspace{-3pt}
%    \caption{\hlt{(Abstract)} leakage functions for \inst{MUL}/\inst{SUB}. }
%    %\label{fig:leak_fun_muladd}
%      %\noindent\textcolor{ForestGreen}{{\RaggedLeft// \textbf{Zero-skip multiply:} MUL in mulU fast/slow(1/0) path if it has zero operands}}\\
%    
%\end{subfigure}
%%(a ``distinguished'' path selector function)
%\caption{%leakage functions for \inst{MUL} and \inst{SUB}.
%% Leakage functions for \inst{MUL} and \inst{SUB}.
%Zero-skip 
%\inst{MUL} takes a fast/slow \upath{}. In the latter case, it may stall a finished \inst{SUB} for one to three cycles. % (\inst{m}: scoreboard size).
%% \yao{Updated leakage function: add signals to indicate some uarch dependence..} \caroline{@Yao, make sure we have terms like hdRdy briefly defined.}
%% \yao{fixed}
%}
%% takes a fast/slow \upath{} due to \textit{zero-skip}~\cite{arm:arm}; a completed \inst{SUB} may stall one to three extra cycles ($n$ = scoreboard size).
%% on top of waiting for other instructions in the scoreboard (size $n$) to commit.
%%    }
%    % \label{fig:zero-skip-example}
%%\end{framed}
%\end{figure}
%
%% \newpage
%
%\subsubsection{Fig. 2}
%\yao{Todo:  \\
%- Fig. 2 source change to \texttt{figs/paths\_3\_9\_7.png} shown as below \\ 
%- Fig. 2 caption change to:  ``Left: \inst{ADD} \upaths{} on CVA6-OP (\S\ref{sec:tspec:upaths}). Right: A sample of \upaths{} (\S\ref{sec:results}) synthesized by \tsynth{} from the CVA6 core (for \inst{BEQ}, \inst{LD}) and data cache (for \inst{ST}). Row\textsubscript{\inst{r}}: \textit{remaining} visit to Row. Node label \inst{l}: \inst{l} last consecutive visits to Row. Orange/Blue nodes: decision source/destination PLs (\S\ref{sec:tspec:transponders}).'' \\ 
%- Relevant main text change suggest are made directly with comment started with 'FIGTWO' 
%}
%
%\begin{figure}[h]
%    \centering
%     \includegraphics[width=0.95\linewidth]{figs/paths_5.png}
%     \caption{Left: \inst{ADD} \upaths{} on CVA6-OP (\S\ref{sec:tspec:upaths}). 
%     Right: A sample of \upaths{} (\S\ref{sec:results}) synthesized by \tsynth{} from the CVA6 core (for \inst{BEQ}, \inst{LD}) and data cache (for \inst{ST}). 
%     Row\textsubscript{\inst{1}/\inst{l}}: 1st/\inst{l}-th visit to Row. Subpath labeled \inst{l}: \inst{l} consecutive visits to Row. % summarized with brace label. 
%     %Brace label \inst{l}: \inst{l} consecutive visits to Row at the end. %1\textsuperscript{st} to \inst{n}\textsuperscript{th} consecutive visit to Row.
%     Orange/Blue nodes: decision source/destination PLs (\S\ref{sec:tspec:transponders}).
%     }
%     %\label{fig:upaths-example}
%\end{figure}
%
%
%%\begin{figure}[h!]
%%    \centering
%%     %\includegraphics[width=0.95\linewidth]{figs/paths_3_9_3.png}
%%     \includegraphics[width=0.2\linewidth]{figs/test_upath.png}
%%     % \includegraphics[width=0.95\linewidth]{figs/paths_3_9_6.png}
%%     \caption{Left: \inst{ADD} \upaths{} on CVA6-OP (\S\ref{sec:tspec:upaths}). 
%%     Right: A sample of \upaths{} (\S\ref{sec:results}) synthesized by \tsynth{} from the CVA6 core (for \inst{BEQ}, \inst{LD}) and data cache (for \inst{ST}). 
%%     Row\textsubscript{\inst{r}}: \textit{remaining} visit to Row. Node label \inst{l}:
%%     $l$ remaining consecutive visits to Row.}
%%\end{figure}
%
%


% % \subsection{\caroline{Transplanted}}
% \subsection{Implication of Undetermined Results} % and IFT Imprecision}
% \label{sec:undet-result}
% % \caroline{DISCUSS: What are we trying to get across in this section compared to in the main text?} 
% \caroline{However, our approach can synthesize contracts for the first time fully-automatically. These contracts are also substantially richer than those in prior work. Our approach is amenable to performance improvements via decomposition. If someone wanted to do a fully proof on our synthesized contract, they could and the human effort would be reduced.}
% \yao{To address concerns about undetermined result and unsoundness with some reasons:
 %richer contract, it is fully automatic, and amendable to modularization. 
% }

% Some undetermined model checker outcomes indicate that \tsynth{} is prone to standard scalability challenges associated with model checking complex hardware designs.
% \yao{I think this is already addressed in results:}
% Nevertheless, we believe \tsynth{} is an important contribution for a few reasons. First, it synthesizes significantly richer leakage contracts than can be verified by prior work for a more powerful receiver. Second, it is fully automatic and requires no designer effort manually craft inductive invariants. Even with undetermined outcomes, \tsynth{} can be highly effective at debugging RTL.
% % before a \rsout{culminating proof with manual invariant writing is performed, complementing works such as \textsc{LeaVe}~\cite{wang2023specification}}.
% Third, \tsynth{} is the only leakage contract verification approach amenable to modularity, which we show in a limited setting with our CVA6 cache evaluation.

% \yao{I believe most are mentioned within ``False-Positives from IFT'' in \S\ref{sec:results} except the emphasis that ``even with these extra conditions, the resulting \pctA{} contract is much richer than the traditional \ct{} alternative.''}

% \rsout{Empirically, our results (\S\ref{sec:results}) show that the impact of \tsynth{}'s theoretical incompleteness (due to IFT, \S\ref{sec:tsynth-approach:symb-ift}) is tolerable in practice. In particular,
% % From the evaluation result (\S\ref{sec:results}), the incompleteness is relatively constrained compared to that of prior works: 
% the \pctA{} contract synthesized from CVA6 features a
% % it affects the final \pctA{} contracts by adding
% handful of extra (spurious) conditions under which it is unsafe for a transmitter to process secrets. Even with these extra conditions, the resulting \pctA{} contract is much richer than the traditional \ct{} alternative.
% % (i.e., by identifying a few extra cases - involving dynamic transmitters -- where transmitters cannot safely be supplied secrets during a dynamic execution). 
% Notably, the \ct{} contract synthesized from CVA6 features no spurious instruction-operand pairs.
% }
% However, despite such imprecision, the synthesized \pctA{} is a much richer contracts that enables processing of secret by transmitter for the first time.
% Moreover, we believe this can be addressed in the future work of  synthesizing leakage function body via symbolic execution combined with model checking to determine if a condition is truly feasible or not. In contrast, prior works relies on manual constraint writing and suggests no solution to automatically address imprecision due to symbolic initial resets. 


%Pruning cannot (resp. can) result in false positives (resp. negatives): an IUV being classified as unsafe (resp. safe) when it is safe (resp. unsafe). 
%\tsynth{} can miss paths for ``deemed safe IUVs'' due to undetermined node or edge pruning.
%
%Undetermined node pruning may lead to missed paths featuring divergent decisions that are operand-dependent.
%Empirically, such pruned paths feature PLs in likely-unrelated functional units to the deemed-safe instruction (e.g., the store buffer for \texttt{ADD}). 
%
%Undetermined edge pruning may cause \tsynth{} to miss divergent decision nodes and target PLs involved in their decisions.
%In a nutshell, undetermined edges indicate a potentially missed additional partial order for a covered PL Set (\S\ref{subsec:hbedge_assert}); if a PL Set is covered, the model checker has already found one partial order. 
%Empirically we did not observe this case: all PLs that are sources of undetermined edges are already divergent decision nodes in the CVA6 case study. 
%%
%Regarding missed destination PLs (target of the pruned edges),
%% divergent decision nodes associated with these PLs,
%we will only miss them if the destination PL of an undetermined edge is not involved in any decisions across all $IUV_A$'s execution paths (thus the will not be flagged for manual inspection). 
%For our case study, we did not observe this case; that is, every destination PL $pl_d$ of all undetermined edges is already involved in some decision $(n, plset) \notin d_{m}$, where $pl_d \in plset$, and thus undergos manual inspection (\S\ref{sec:divergent_decisions}).
%
%
%We believe we can reduce (or even eliminate) undetermined results by modularizing \tsynth{}. We also plan to investigate “design for verification” approaches where cheap-to-verify runtime monitors are used to dynamically detect execution behaviors deemed impossible due to undetermined results.
% \subsection{security definition}
% \yao{TODO to myself}
% As an example, consider $p = \{\mathtt{LI~r1,3}; \mathtt{SUB~r1, r1, r1}\}$
% % consisting of a single $\mathtt{ADD}$
% executing on \M{} from initial states, $\langle \sigma, \mu \rangle$ and $\langle \sigma', \mu' \rangle$, where $\mu \neq \mu'$ and $\sigma \approx_{\pi}\sigma'$. Suppose $\mu$ and $\mu'$ feature an in-flight $\mathtt{MUL}$ with  
% %Suppose the $\mathtt{ADD}$'s arguments $args \in reg_a$ are \textsc{h}-labeled in $\pi$, and both $\mu_0$ and $\mu'_0$ feature an in-flight $\mathtt{MUL}$. Suppose also that the $\mathtt{MUL}$
% at least one zero operand in $\mu$ and no zero operands $\mu'$, and \M{} implements zero-skip multiplies (\S\ref{sec:intro}). 
% It is possible that $\mathnormal{O}_{\mathnormal{R}_C}(\lbbar p \rbbar_{\mathnormal{M}}^{\langle\sigma, \mu\rangle}) \neq \mathnormal{O}_{\mathnormal{R}_C}(\lbbar p \rbbar_{\mathnormal{M}}^{\langle\sigma', \mu'\rangle})$ in Eq.~\ref{a:eq:non-interference}, despite $p$'s execution time being \textit{independent} of its high inputs.

% Some procedures for verifying hardware side-channel safety side-step the imprecision of a security definition that omits $\mu$ by assuming equivalent initial microarchitectural states for all pairs of compared traces in their \textit{implementations}~\cite{deutschmann:upec-do, deutschmann2023scalable}.
% % \yao{removed LEAVE~\cite{wang2023specification}}
% % implicitly addressing the imprecise definition above.
% Other such procedures directly check this imprecise security definition and require users to navigate false counterexamples as a result~\cite{gleissenthall:iodine, gleissenthall:xenon}.

% \yao{, discussed more in \S\ref{sec:ift_static_t}}. % \rsout{As discussed in \S\ref{sec:tsynth-tool:f-leak-syn},}, 
% and foc
% \caroline{TODO. }


\subsubsection{Synthesizing Leakage Signatures} 

To synthesize a leakage signatures \inst{P\_src}, \synthlc{} considers each decision
% In all cases, for transponder $P$ and decision source $src$, \tsynth{} considers each decision
$(src, \mathbf{dst}) \in \mathbf{d}^{P}_\mathcal{M}$ paired with each (candidate) transmitter. Using commercial model checkers~\cite{cadence:jasper_gold}, \synthlc{} checks if taint can flow to (the \ufsm{} associated with) any $ dst \in \mathbf{dst}$. If so, $P$ is a transponder, and $T$ is recorded as a transmitter (explicit input) along with its label and unsafe operand $op$ (\S\ref{a:sec:checking-eq-8}).
% can become tainted.
% \caroline{\tsynth{} uses commercial model checkers combined with information-flow tracking (IFT). checks if taint can propagate to any destination PL $dst \in  \mathbf{dst^{t_P}_\mathcal{M}}$.}




% \tsynth{} uses commercial model checkers combined with information-flow tracking (IFT), where \M{} is augmented with a gate-level IFT circuit~\cite{solt2022cellift}, to perform this step. In a nutshell, \tsynth{} injects taint at a candidate transmitter's unsafe operand and checks if taint can propagate to any destination PL $dst \in  \mathbf{dst^{t_P}_\mathcal{M}}$. 



% (rather than a pair of decisions as in ) and check



% $d_0, d_1 \in \mathbf{d}^i_\mathcal{M}$ $i_P$ and decision $(src^{I_P}_\mathcal{M}, \mathbf{dst}^{I_P}_\mathcal{M}) \in \mathbf{d}^{I_P}_\mathcal{M}$. 

% only  instantiate Eq.~\ref{eq:non-interference-cex} as described in \S\ref{sec:checking-eq-8}, we We then instantiate traces as discussed above. However, to communicate that $op$ of $i_T$ accepts \textsc{h}-labeled data, we inject ``taint'' only at $i_T$'s operand-holding register (\S\ref{}). We also prevent taint from flowing from the transmitters primary output to the primary inputs of other instructions (architecturally or speculatively). To check for intrinsic, we check to see if taint can reach any of the PLs corresponding to $d_0$, and so on. To check for intrinsic, we see if taint can reach $d_0$ subject to constraints above. Same for static. 





% To do this, \tsynth{} considers each unique decision for each candidate transponder in turn. For a given transponder-decision pair \rsout{$(i_P, d_{I_P} = (src_{I_P}, \mathbf{dst_{I_P}}))$}\yao{$(i_P, d^{I_P} = (src^{I_P}, \mathbf{dst^{I_P}}))$}, \tsynth{} attempts to uncover a leakagesignatures to characterize it, where the function name is $i_P\_src_{I_P}$ and the function range is \yao{all} $\mathbf{dst^{I_P}_\mathcal{M}}$ \yao{such that $(src^{I_P}_\mathcal{M},\mathbf{dst^{I_P}_\mathcal{M}}) \in \mathbf{d}^{I_P}_\mathcal{M}$}. The following procedure searches for all transmitters that serve as function inputs and their unsafe operands that appear in the function body.
% If no such inputs are found, the function is discarded.

% determines if depends on the value(s) of any \textit{candidate} transmitter operand(s), where each operand of each ISA instruction is considered as a candidate transmitter operand in turn.


% This step is sufficient to derive $(I, op)$ tuples. To simultaneously derive conditions, and thus $(I, op, c)$ tuples, \tsynth{} instantiates four variants of this property as defined below.

% Given a set of candidate transponders and their corresponding decisions \tsynth{} considers each to determine if it is dependent on \texttt{l}-labeled data and under what conditions. In particular, \tsynth{} uses the output of Step 1 to produce leakage signaturess for each decision (if one exists).

% Each variant involves considering a program $p$ that features a single transmitter instruction $i_T$ and a single transponder instruction $i_P$. We consider four cases illustrated in Fig.~\ref{a:fig:taint_cases}. In the first, the transponder and transmitter are the same instruction.
% \yao{In the second case, $i_T$ is fetched before $i_P$ and is still in-flight when $i_P$ visits $src^{I_P}_\mathcal{M}$. In this case, $i_T$ is dynamic transmitter if the property return true.
% Third case is similar to second, but $i_T$ is fetched after $i_P$ but is still in-flight when $i_P$ is at decision source PL. 
% Last case correspond to static transmitter when $i_P$ is issued after $i_T$ is not in-flight.}
% %
% (i) $...i_P = i_T...$ (Intrinsic) (i-a) $...i_P, n, i_T...$ (Dyanmic-a),(ii-b) $...i_T, n, i_P...$ (Dyanmic-b), (iii) $...i_T...i_P...$ (Static).
% We consider each decision for each $i_p$ in each case. We look to see if the decision is secret dependent one of $i_T$'s operands in each scenario.

% We conduct this analysis using model checking and information flow tracking.
% % \yao{Appendix Fig.~\ref{a:fig:taint_cases}}
% We derive $i.op.c$ tuples form leakage signaturess as outlined in \S\ref{}.



% Need to identify transmitters and I/S/D labeling to eliminate each counterexample. We consider each decision one at a time and use symbolic IFT to attribute a decision to the operands of a transmitter under one of these conditions.

% \chris{these two steps make sense, but the following text doesn't give enough details about the algorithm that orchestrates them (if that is supposed to come later, ok).  E.g., Do we find a CEX then find the c to block that CEX?  Do we find all the CEX then look for the set of c to block all the CEX? 
% Do we identify symmetric/redundant c?  Etc.}


% The first counterexample to NI returns the first cycle in which the PLs occupied by the instructions in the two traces are different. This can be due to one of two reasons. First, the in-flight instructions are different meaning (speculative) control-flow diverged in the two traces. Second, in-flight instructions are the same, but one transponder instruction made a different decision at a decision source in the previous cycle. If we assume the fetch streams of the two traces are the same, i.e., branches execute the same instruction along transient and non-transient control-flow paths, all remaining counterexamples are due to transponders making different decisions. Each pair of unique decisions for each transponder gives a distinct way to violate Eq.~\ref{a:eq:non-interference}. Note: even if fetch streams are the same, we can still observe \upath{} variability for branch transponders which conditional squash mis-speculated instructions as a function of their operands.


% Suppose we have traces t and t' which produce identical observation traces for $\mathcal{R}_\upath$ up until state $\langle \sigma_k, \mu_k \rangle$ where the $\mathcal{R}_\upath$'s observations differ.



% To start, we will rewrite Eq.~\ref{a:eq:non-interference} in a way that enables us to isolate observation traces produced by executing individual instructions in a program.
% % In other words, for we need to prove that for all programs $p$, with respect to receiver $\mathcal{R}$ and policy $\pi$, if $p$ enforces conditional constant-time defense when running on $\mathcal{M}$ (Eq.~\ref{eq:tspec-defense}), then it is hardware side-channel safe when running on $\mathcal{M}$ (Eq.~\ref{eq:NI-per-inst-trace}).
% To do this, we will extract the set of \textit{instruction execution traces} from a program execution trace $\lbbar p \rbbar_{\mathcal{M}}^{\langle \sigma_0, \mu_0 \rangle}$, as follows:
% % obtained from running a program $p$ on a microarchitecture $\mathcal{M}$ from initial state $\langle \sigma_0, \mu_0 \rangle$, as follows:
% \begin{equation}
% \begin{split}
%       {\lbkt p \rbkt}_{\mathcal{M}}^{\langle \sigma_0, \mu_0 \rangle} = \{ \lbbar i \rbbar_{\mathcal{M}}^{\langle \sigma_k, \mu_k \rangle} | \langle \sigma_0, \mu_0 \rangle \Downarrow_\mathcal{M}^{p} \langle \sigma_k, \mu_k \rangle \\ \land~\mu_k[\mathtt{IFR.inst}] = i \land \mu_k[\mathtt{IFR.vld}] = 1 \}
% \end{split}
% \label{eq:per-inst-traces}
% \end{equation}
% Eq.~\ref{eq:per-inst-traces} captures an execution trace for any valid instruction that is fetched from instruction memory into the \textit{instruction fetch register} (IFR).
% % execution of any fetched instruction, so captures both speculative and non-speculative traces.
% Using Eq.~\ref{eq:per-inst-traces}, we can write Eq.~\ref{a:eq:non-interference} as follows:
% \begin{equation}
% \begin{split}
%       \forall \sigma_0, \sigma'_0. \forall \mu_0. (\sigma_0 \approx_{\pi_\mathtt{L}} \sigma'_0 
%       % \hspace{-12pt} \bigcup_{t_0 \in {\lbkt p \rbkt}_{\mathcal{M}}^{\langle \sigma_0, \mu_0 \rangle}} \hspace{-20pt} \mathcal{O}_{\mathcal{R}} (t_0)
%       % = \hspace{-20pt} \bigcup_{t_1 \in {\lbkt p \rbkt}_{\mathcal{M}}^{\langle \sigma_0, \mu'_0 \rangle}} \hspace{-20pt} \mathcal{O}_{\mathcal{R}} (t_1)) \hspace{-4pt}
%       \implies \hspace{-20pt} \bigcup_{t_0 \in {\lbkt p \rbkt}_{\mathcal{M}}^{\langle \sigma_0, \mu_0 \rangle}} \hspace{-20pt} \mathcal{O}_{\mathcal{R}} (t_0)
%       = \hspace{-20pt} \bigcup_{t_1 \in {\lbkt p \rbkt}_{\mathcal{M}}^{\langle \sigma'_0, \mu_0 \rangle}} \hspace{-20pt} \mathcal{O}_{\mathcal{R}} (t_1))
% \end{split}
% \label{eq:NI-per-inst-trace}
% \end{equation}

% \caroline{Really I should change $\mathcal{O}_{\mathcal{R}}$ to $\mathcal{O}_{\mathcal{R}_{\upath}}$ to make this point, so writing this as a comment for now. Essentially I want the observable execution trace of each instruction (so each element in the union) to just be extracting its individual execution phases at each time step. So, in a given cycle an instruction's observable trace is only going to be capturing the \ufsm{} states containing its unique instruction identifier. If you take the full observation trace corresponding to a single instruciton it should capture its full \upath{} on the design over time. As I'm writing this, I might need to tweak def 7, because $\mathcal{O}_{\mathcal{R}_{\upath}}$ technically grabs all of the \ufsm{} state and not the \ufsm{} state for a particular instruction --- but latter is what I'm going for here. Hence, the observations of different executions of various in-flight instructions can be unioned to produce the overall observable execution path for the whole program according to $\mathcal{O}_{\mathcal{R}_{\upath}}$.}

% \chris{the unions need clarification because each $\mathcal{O}_{\mathcal{R}} (...)$ looks like a state vector (AFAICT), not a set.}



% To synthesize a $\mathcal{C}^\mathcal{R}_{\tau}$, we first use the notions of transponders and \upaths{} to explore all possible violations of Eq.~\ref{eq:tspec-defense-NI}, assuming an empty contract and substituting Eq.~\ref{eq:NI-per-inst-trace} for Eq.~\ref{a:eq:non-interference}.
% %R when the contract is empty. 
% % We will start with an empty contract $\mathcal{C}^\mathcal{R}_{\tau}$ which means that we assume that Eq.~\ref{eq:NI-per-inst-trace} holds for all programs running on $\mathcal{M}$.
% % We want to synthesize $\mathcal{C}^\mathcal{R}_{\tau}$ such that Eq.~\ref{eq:tspec-defense} is valid.
% % We can do this by first finding all ways in which we can violate Eq.~\ref{eq:NI-per-inst-trace}, i.e., finding all satisfying solutions to:
% This amounts to finding all possible satisfying solutions to:
% \begin{equation}
% \begin{split}
%     \exists p. \exists \sigma_0, \sigma'_0. \exists \mu_0. \sigma_0 \approx_{\pi_\mathtt{L}} \sigma'_0 
%     \land \hspace{-18pt} \bigcup_{t_0 \in {\lbkt p \rbkt}_{\mathcal{M}}^{\langle \sigma_0, \mu_0 \rangle}} \hspace{-18pt} \mathcal{O}_{\mathcal{R}} (t_0)
%     \neq \hspace{-18pt} \bigcup_{t_2 \in {\lbkt p \rbkt}_{\mathcal{M}}^{\langle \sigma'_0, \mu_0 \rangle}} \hspace{-18pt} \mathcal{O}_{\mathcal{R}} (t_2) 
% \end{split}
% \label{eq:NI-per-inst-trace-cex}
% \end{equation}
% Note that we consider a single initial microarchitectural state $\mu_0$, rather than a pair of initial microarchitectural states as in Eq.~\ref{eq:NI-per-inst-trace}. Intuitively, all $\mu_0$ and $\mu'_0$ that satisfy the red predicate in Eq.~\ref{a:eq:non-interference} are in an equivalence class of microarchitectural states that do not contribute to observably distinct execution behavior for $p$. 
% Any pair of these states is sufficient for exploring counterexamples to hardware side-channel safety.
% % the characteristics of $p$'s executions on $\mathcal{M}$ that must be capture in a \pct{} contract.
% % This is because, intuitively, if a program $p$ can violate Eq.~\ref{eq:NI-per-inst-trace} for distinct $\mu_0$ and $\mu'_0$, then these microarchitectural states do not contribute to observably disntinct execution behavior for $p$. Any pair of microarchitectural states that do not interfere with $p$'s observable execution behavior are sufficient for exploring all counterexampels.
% \chris{yea, if we ditch the antecedant in Eqn 9, that's another +1 to purge it from SII.}

% Given our observation that operand-dependent channel modulations on behalf of transmitters manifest as \upath{} variability of transponders, we rewrite Eq.~\ref{eq:NI-per-inst-trace-cex} in terms of transponders.
% To do this, we first extract the fetch stream of the $\mathcal{M}$ as follows:
% \begin{equation}
% \begin{split}
%     |p|_\mathcal{M}^{\langle \sigma_0, \mu_0 \rangle} = \{\mu_k[\mathtt{IFR.inst}] | \\
%     \langle \sigma_k, \mu_k \rangle \in \lbbar p \rbbar_{\mathcal{M}}^{\langle \sigma_0, \mu_0 \rangle} \land \mu_k[\mathtt{IFR.vld}] = 1\}
% \end{split}
% \label{eq:fetch-stream}
% \end{equation}

% Using Eq.~\ref{eq:fetch-stream}, we can re-write Eq.~\ref{eq:NI-per-inst-trace-cex} as:
% Given our observation that channel modulations on behalf of a transmitter manifest as \upath{}, we can re-write Eq.~\ref{eq:NI-per-inst-trace-cex} as:
% \begin{equation}
% \begin{split}
%     \exists p. \exists \sigma_0, \sigma'_0. \exists \mu_0. \exists i_P. i_P \in p
%     \\ \land~\sigma_0 \approx_{\pi_\mathtt{L}} \sigma'_0 
%     % \land t = \{i_1, i_2, ...\} \\
%     \land~ |p|_\mathcal{M}^{\langle \sigma_0, \mu_0 \rangle} = |p|_\mathcal{M}^{\langle \sigma'_0, \mu_0 \rangle} \\
%     \land~\textcolor{Orange}{\mathcal{O}_{\mathcal{R}_{\mu \textsc{path}}}(\lbkt p \rbkt[i_P]_\mathcal{M}^{\langle \sigma_0, \mu_0 \rangle}) \neq \mathcal{O}_{\mathcal{R}_{\mu \textsc{path}}}(\lbkt p \rbkt[i_P]_\mathcal{M}^{\langle \sigma'_0, \mu_0 \rangle})}
% \end{split}
% \label{eq:NI-transponder-cex}
% \end{equation}
% Eq.~\ref{eq:NI-transponder-cex} states that there exists a program $p$ containing a transponder $i_P$, such that when $i_P$ executes on $p$, it exhibits distinct \upaths{}.
% % I.e., there exists a program $p$ containing a transponder $i_p$ that exhibits \upath{} variability as a function of $p$'s high inputs.
% % Given as list \inst{asm} of all instruction encodings in the ISA, \tsynth{} searches for all \textit{candidate} transponders $i_{p_c} \in \mathtt{asm}$, i.e., all instructions that may exhibit \upath{} variability on $\mathcal{M}$ and thereby satisfy the orange predicate in Eq.~\ref{eq:NI-transponder-cex}. Importantly, \upath{} exploration can be conducted using solely trace properties.
% % We want to find all possible ways in which the orage predicate can be satisfied. This amounts to finding all instructions that can exhibit \upath{} variability and then considering all pairs of paths for such an instruction to localize all decisions.

% \subsection{\tsynth{} Approach}
% Based on the formal foundation in the previous section, \tsynth{} synthesizes \pct{} contracts from RTL in two high-level steps: (i) enumerating all possible solutions to the orange predicate in Eq.~\ref{eq:NI-transponder-cex}, and (ii) for each solution, identifying all $(I, op, c)$ tuples that prevent it. 

% Each possible solution to the orange predicate involves a particular transponder $i_P$ and one of its unique \textit{decisions}.
% To find all solutions, we must then find all transponders on the DUV and all decisions for each.
% To do this we first conduct \upath{} exploration where we find all \upaths{} of all implemented instructions on the microarchitecture.
% Instructions with more than one execution path are candidate transponders.
% Then we use Algorithm~\ref{alg:find-cex} to find all counterexamples which involves comparing all pairs of distinct \upaths{} for a transponder to identify decision nodes and then finally decisions.

% \begin{algorithm}
% \caption{TODO}
% \begin{algorithmic}[1]
% \Procedure{FindDecisions}{i}
%     \ForAll{\(p_0, p_1 \in \mu \textsc{path}(i)\)} 
%         \State \(src = p_0.\mathtt{pl} \cap p_1.\mathtt{pl}\)
%         \If{\(p_0[src].\mathtt{dst} \neq p_1[src].\mathtt{dst}\)} 
%             \State \(dec[i] \gets dec[i] \cup (src, p_0[d].\mathtt{dst}) \cup (d, p_1[src].\mathtt{dst})\)
%         \EndIf
%     \EndFor
% \EndProcedure
% \label{alg:find-cex}
% \end{algorithmic}
% \end{algorithm}

% Once we find all candidate transponders/decisions, we want to find (i) if it is operand-dependent on a operand $op$ of transmitter $i$, and (ii) if it is, the $i.op.c$ tuple to add to our contract in order to preclude this \upath{} variability.
% We do the former using a symbolic taint analysis. We do the latter by enforcing particular conditions on our taint analysis.
% Find all of the ways in which we could observe a NI violation. The notion of transponders and \upaths{} makes this task manageable. For each possiblity, find the $i.op.c$ tuple to rule it out.

% \begin{algorithm}
% \caption{TODO}
% \begin{algorithmic}[1]
% \Procedure{FindTransmitters}{i}
% \For{\((src, dst) \in dec[i]\)}
%     \For{\(i_T \in \mathtt{asm}\)} 
%         \For{\(op \in \mathtt{operands}\)} 
%             \For{\(c \in \{\mathtt{I}, \mathtt{D}, \mathtt{S}\}\)} 
%                 \If{\(i.op.c \implies (src.dst)\)}
%                 \State \(\mathcal{C}^\mathcal{R}_{\tau} = \mathcal{C}^\mathcal{R}_{\tau} \cup i.op.c\)
%                 \EndIf
%             \EndFor
%         \EndFor
%     \EndFor
% \EndFor
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}




% \upath{} exploration finds all \textit{candidate} transponders \inst{I_{P_C}}, i.e., all instructions that may \upath{} variability on $\mu arch$. 

% These are instructions whose executions on $\mu arch$ can satisfy
% We can conduct this exclusively using trace properties.
% We conduct \textbf{\upath{} Exploration} to find 





% In order to use the trace property in Eq.~\ref{eq:ct-defense}, we need to verify that our target microarchitecture $\matcal{M}$ uploads its leakage contract---$\mathcal{C}_{\tau}^\mathcal{R}$ in our case.


% Given a \pct{} contract $\mathcal{C}_{\tau}^\mathcal{R}$, we can replace the blue predicate in Eq.~\ref{eq:ct-defense} (\S\ref{sec:background:threat-model-summary}) with
% \textcolor{myorange}{$\mathrm{Safe}(i.op, s_0) \notin \mathcal{C}^\mathcal{R}_{\tau}$} 
% % and \textcolor{myorange}{$\neg \mathrm{Safe}(i.op1, s_0) \in \mathcal{C}^\mathcal{R}_{\tau}$}, respectively,
% to yield $\mathcal{D}_{\tau}^{\mathcal{R}, \pi}$. This defense avoids supplying secrets to transmitter operands \textit{unless} $\mathcal{C}^\mathcal{R}_{\tau}$ indicates that it is safe to do so in state $s_0$.

% Given a receiver $\mathcal{R}$ and a privacy policy $\pi$, we need to verify once that a 

% Suppose we start with an empty contract $\mathcal{C}_{ct}^\mathcal{R}$, such that for all $p$, Eq.~\ref{eq:ct-defense} holds. If $Eq.~\ref{eq:ct-defense} \implies Eq.~\ref{eq:NI-per-inst-trace}$ is valid, then for such a contract, Eq.~\ref{eq:NI-per-inst-trace} must hold for all $p$. Of course, we know that Eq.~\ref{eq:NI-per-inst-trace} does not hold for arbitrary $p$ on realistic microarchitecture. So we want to construct $\mathcal{C}_{ct}^\mathcal{R}$.
% For a transmitter-centric contract, constructing $\mathcal{C}_{ct}^\mathcal{R}$ involves finding all instructions $i$ and all operands $op$ such that $(i.op \notin \mathcal{C}_{ct}^\mathcal{R}) \implies \neg (Eq.~\ref{eq:ct-defense} \implies Eq.~\ref{eq:NI-per-inst-trace})$. For a transponder-centric contract (a \pct{} contract) we also want to find all ways in which we can satisfy the former. Satisfying $\exists i. \exists op. (i.op \notin \mathcal{C}_{ct}^\mathcal{R}) \implies \neg (Eq.~\ref{eq:ct-defense} \implies Eq.~\ref{eq:NI-per-inst-trace})$ is the same as satisfying $\exists i. \exists op. (i.op \notin \mathcal{C}_{ct}^\mathcal{R}) \implies  (Eq.~\ref{eq:ct-defense} \land \neg Eq.~\ref{eq:NI-per-inst-trace})$. Fining all transponders involves finding all ways that we can satisfy $\neg Eq.~\ref{eq:NI-per-inst-trace}$. 

% We extract the fetch stream of the processor as follows:
% \begin{equation}
% \begin{split}
%     |p|_\mathcal{M}^{\langle \sigma_0, \mu_0 \rangle} = \{\mu_k[\mathtt{IFR.inst}] | \\
%     \langle \sigma_k, \mu_k \rangle \in \lbbar p \rbbar_{\mathcal{M}}^{\langle \sigma_0, \mu_0 \rangle} \land \mu_k[\mathtt{IFR.vld}] = 1\}
% \end{split}
% \label{eq:NI-per-inst-cex}
% \end{equation}




% Recall that our goal is to synthesize a transponder-centric leakage contract ${LC_P}$, such that
% $\forall p. (\lbbar p \rbbar_{\mu arch} \vdash_{LC_P} \mathcal{D}_{CT_C}) \rightarrow \mathrm{Property~\ref{a:eq:non-interference}}$ for receiver $\mathcal{R}_{\mu \textsc{path}}$ (\S\ref{sec:background:threat-model-summary}).
% Given a microarchitecture $\mu arch$, we synthesize $LC_P$ in three steps: \textit{\upath{} Exploration} (\S\ref{}), \textit{2-\upath{} Comparison} (\S\ref{}), and \textit{Transponder Implication} (\S\ref{}). To understand these, steps, consider an alternate formulation of Property~\ref{a:eq:non-interference} below.

% \begin{equation}
% \begin{split}
%       \forall \sigma_0, \sigma'_0. \forall \mu_0, \mu'_0. 
%       (\textcolor{BurntOrange}{\sigma_0 \approx_{\pi_\mathtt{L}} \sigma'_0} \\ \land~
%       \textcolor{BrickRed}{\bigcup_{i \in p} \mathcal{O_R}(\lbbar i \rbbar_{\mu arch}^{\langle \sigma_0, \mu_0 \rangle \Downarrow \langle \sigma_i, \mu_i \rangle}) = \bigcup_{i \in p} \mathcal{O_R}(\lbbar i \rbbar_{\mu arch}^{\langle \sigma_0, \mu'_0 \rangle \Downarrow \langle\sigma_i, \mu'_i\rangle})}) \\
%        \rightarrow 
%       \textcolor{Violet}{\bigcup_{i \in p} \mathcal{O_R}(\lbbar i \rbbar_{\mu arch}^{\langle \sigma_0, \mu_0 \rangle \Downarrow \langle\sigma_i, \mu_i}\rangle) = \bigcup_{i \in p} \mathcal{O_R}(\lbbar i \rbbar_{\mu arch}^{\langle \sigma'_0, \mu'_0 \rangle \Downarrow \langle\sigma'_i, \mu'_i\rangle})}
% \end{split}
% \label{eq:non-interference-inst}
% \end{equation}

% % the trace of observations produced by running instruction $i$ from a state $\langle \sigma, \mu \rangle$, reachable from initial state $\langle \sigma_i, \mu_i \rangle$, where $\mu_i(IF) = i$. That is, $i$ as just been fetched from instruction memory, i.e., $i$ has just materialized in the processor.


% To synthesize a contract $LC_P$ for a microarchitecture $\mu arch$, we start with an \textit{empty contract}. That is, $\mathcal{D}_{CT_C}$ trivially holds for all programs $p$ executing on $\mu arch$, i.e., $\forall p.$ Property~\ref{a:eq:non-interference} (or equivalently  $\forall p.$ Property~\ref{eq:non-interference-inst}):
% \begin{equation}
% \begin{split}
%       \forall p. \forall \sigma_0, \sigma'_0. \forall \mu_0, \mu'_0. (\textcolor{BurntOrange}{A} \land \textcolor{BrickRed}{B}) \rightarrow \textcolor{Violet}{C}
% \end{split}
% \label{eq:non-interference-no-contract}
% \end{equation}

% The color coding in Property~\ref{eq:non-interference-inst} and Property~\ref{eq:non-interference-no-contract} align.
% Our \tsynth{} approach for synthesizing a $LC_P$ for $\mu arch$ will derive counterexamples to Property~\ref{eq:non-interference-no-contract} by finding satisfying solutions to the following:
% \begin{equation}
% \begin{split}
%       \exists p. \exists \sigma_0, \sigma'_0. \exists \mu_0, \mu'_0. (\textcolor{BurntOrange}{A} \land \textcolor{BrickRed}{B}) \land \neg \textcolor{Violet}{C}
% \end{split}
% \label{eq:non-interference-cex}
% \end{equation}

% From \S\ref{sec}, we know that transmitters, as a function of their operands, create execution path variability for transponders. Thus, we instantiate Property~\ref{eq:non-interference-cex} as follows:
% \begin{equation}
% \begin{split}
%       \exists p. \exists \sigma_0, \sigma'_0. \exists \mu_0.
%       p = \{i_1, i_2, ... i_n\} \land i_T = i_1 \land i_P = i_n \\ \land~\pi(\sigma_0 \setminus \{i_T.args \}) = \textsc{l}  
%        \bigwedge\limits_{j=2}^n \neg DataDep(i_1,i_j)
%       % \bigwedge\limits_{j=2}^n \pi(i_j.args = \textsc{l}) \\
%       \land \textcolor{BurntOrange}{\sigma_0 \approx_{\pi_\mathtt{L}} \sigma'_0} \\
%       % \land~\textcolor{BrickRed}{\mathcal{O_R}(\lbbar i_P \rbbar_{\mu arch}^{\langle \sigma_0, \mu_0 \rangle \Downarrow \langle \sigma_{I_P}, \mu_{I_P} \rangle}) = \mathcal{O_R}(\lbbar i_P \rbbar_{\mu arch}^{\langle \sigma_0, \mu'_0 \rangle \Downarrow \langle\sigma_{I_P}, \mu_{I_P}'\rangle})} \\
%       % \land~\pi(i_T.arg0 = \textsc{l}) \land~\pi(i_T.arg1 = \textsc{l}) \\
%       \land~\textcolor{Violet}{\mathcal{O_R}(\lbbar i_P \rbbar_{\mu arch}^{\langle \sigma_0, \mu_0 \rangle \Downarrow \langle\sigma_{I_P}, \mu_{I_P}\rangle}) \neq \mathcal{O_R}(\lbbar i_P \rbbar_{\mu arch}^{\langle \sigma'_0, \mu_0 \rangle \Downarrow \langle\sigma'_{I_P}, \mu_{I_P}\rangle})}
% \end{split}
% \label{eq:non-interference-inst-cex-detailed}
% \end{equation}


% A satisfying solution to Property~\ref{eq:non-interference-inst-cex-detailed}, gives us a program $p$ containing a transmitter $i_T$ and a transponder $i_P$ such that $i_T$ processes a secret and creates execution path variability for $i_P$ that is observed by $\mathcal{R}$. 
% Note that we only consider a single initial microarchitectural state $\mu_0$. \caroline{TODO: this is because of the existential...}

% \caroline{Maybe say that we synthesize $LC_T$ to support $\mathcal{D}_{CT}$ first and then we synthesize $LC_P$ to support $\mathcal{D}_{CT_C}$ later.}

%The \tsynth{} procedure discovers all satisfying solutions to Property~\ref{eq:non-interference-inst-cex-detailed} incrementally.






% \subsection{Formalizing Instruction Execution Behavior as Microarchitectural Execution Paths}
% \label{sec:upath-def}
% \yao{Formal definition in Sec 3?} 
% Transponder instruction is one that experience channel modulation and exhibits distinct execution behavior observable by some attacker in terms of hardware resource usage. 
% \subsubsection{Microarchitectural Execution Paths}

% \subsubsection{\ufsm{} and Performing Locations}
% \begin{itemize}
%     \item Metadata for Identifying Performing Locations
% \end{itemize}

% \subsubsection{Requirements for SVA-Directed Path Discovery}
% \begin{itemize}
%     \item Controlling DUV instruction stream
%     \item Detecting and Tracking IUV execution
%     \item Identifying the End of an Instruction Execution Path
% \end{itemize}




%\subsection{An Abstraction for Hardware Resource Usage - \upath{}}
%\subsection{Controlling the DUV Instruction Stream}


\subsection{Product Circuit Limitations}
\label{a:sec:product-circuit-limitations}
% for this scenario below.
%
In \S\ref{a:sec:tsynth-approach:symb-ift}, we note that 
% for leakage function synthesis, two approaches are possible to evaluate
Eq.~\ref{a:eq:non-interference-cex} can be evaluated with a product circuit or symbolic IFT.
% : (i) constructing a \textit{product circuit}, or (ii) symbolic IFT. 
\synthlc{} chooses the latter, because we find that the product circuit formulation 
% symbolic IFT over the former, % one for soundness reason: 
%mainly because product circuit approach suffers from soundness issue. 
% Below we discuss limitation of the product circuit approach. 
% In \S\ref{sec:tsynth-approach:symb-ift} for leakage function synthesis, 
% \tsynth{} chose symbolic IFT over 
%to determine whether a transponder exhibiting distinct decisions depends on some transmitter operands, one needs to 
% there are two approach to formally evaluate  and attribute distinct observation to candidate transmitter operands: (i)
% Each case above can be instantiated in theory using a product circuit, whereby two copies of \M{} are instantiated. However, we find that directly checking Eq.~\ref{eq:non-interference-cex} as a two-trace property in this manner suffers from soundness limitations. 
% because product circuit approach 
is vulnerable (in our usage scenario) to \textit{misclassifying} a particular transponder decision as \textit{independent} of some 
% dynamic 
transmitter's operand. We here provide intuition below.

Consider a candidate pair of a transmitter $T$ and its unsafe operand $op$. To establish causality between $op$ and a decision made by $i_P$ at decision source $src \in \mathbf{src}^P_\mathcal{M}$, $op$ must be the only instruction operand in $p$ to be supplied with high data. This requires constraining the operands of all instructions in $p$, except $op$ of $i_T$, to be equal in both traces.
% in both traces must be equal except for $op$ of $i_T$.
However, once $i_T$ materializes in \M{}, it may create \upath{} variability for many instructions \textit{before} $i_P$ reaches $src$. This variability will soon render the fetch streams of the two traces \textit{out of sync}, i.e., the traces will fetch new instructions in different steps.
% of the two traces becoming asynchronous relative to each other.
Such asynchrony makes it difficult to constrain all non-$op$ operands in $p$ as required.
% to 
% the operands of all instructions in $p$, except $op$ of $i_T$, 
% to be equal in the two traces.
% is difficult. 
% \yao{Possibly into appendix?}
There are a few plausible solutions to this challenge but all  suffer from a soundness issue. 
%\textit{mis-classify} a transponder decision as \textit{independent} of some transmitter's operands (\S\ref{sec:product-ckt-limit}).

% \subsection{Product Circuit Limitation}
% \label{sec:product-ckt-limit}
%\caroline{TODO}
% \rsout{We here discuss two plausible solutions to the challenges discussed in \S\ref{sec:product-circuit-limitations}.} \caroline{be more specific: "what challengs"???} 
% \yao{Revised. }
%Recall \S\ref{sec:product-circuit-limitations} discussed that product circuit approach is prone to asynchrony issue that causes difficulty to constrain equality of all instructions in $p$ except $op$ of $i_T$. We here discuss some plausible solutions to such a problem and show respective insufficiency.
%to \caroline{be more specific: "what challengs"???} the challenges discussed in \S\ref{sec:product-circuit-limitations}.  
% the number of instructionsn
First, by \textit{bounding} the number of instructions in $p$, it is possible to write a finite set of constraints over the operand values in both traces.
This may fail to attribute a transponder decision to $op$ if $i_T$ and $i_P$ must be separated by more instructions than the bound permits.

Second, both traces could be constrained to operate in a \textit{lock-step} fashion, such that they always fetch instructions at the same trace steps~\cite{deutschmann:upec-do, deutschmann2023scalable, gleissenthall:iodine, gleissenthall:xenon}.
Consider the operand-packing optimization from \S\ref{sec:op-packing-example}. If a trace operand-packs after decoding two instructions, it may fetch more instructions in the next cycle, else it may not. Lock-stepping thus enforces that one trace can operand-pack iff the other trace does. Hence, \upath{} variability for \inst{ADD}s will be deemed independent of their operands. 
%That is, lock-stepping could \textit{misclassify} a transponder decision as \textit{independent} of some transmitter's operand. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \yao{START}
% Third, a \textit{stuttering circuit} can be used to prevent one trace from fetching instructions when the other lags behind~\cite{wang2023specification}.
% Suppose in two traces $t$ and $t'$ featuring issue of $i_T$ and $i_P$. 
% %is fetched in both at step $k$ and $i_P$ is fetched at step $k+1$. Then later on, 
% In $t$, a back-pressure happens at fetch during execution of $i_T$, 
% % creates back-pressure in the fetch stream,  % before $i_P$ has reached a decision source PL, $src^{i_P}_\mathcal{M}$, 
% while $t'$ does not experience such back-pressure.
% % but in $t'$ but not $t'$ before 
% The trace $t'$ that is ready to fetch new instruction $i_P$ now waits for $t$ to continue execute until the fetch is ready.
% As a result, 
% % trace $t$ effectively features extra symbolic number of invalid instructions fetched compared to $t'$. 
% % Moreover, 
% during the catch-up, $i_T$ in $t$ may progress far enough in its execution such that it can no longer create variability for $i_P$ at some decision source PL $src^{i_P}_\mathcal{M}$.
% Therefore, this approach can also be unsound. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Third, a \textit{stuttering circuit} could be used to prevent one trace from fetching instructions when the other lags behind~\cite{wang2023specification}.
% \caroline{Discuss: I don't recall this explanation:}
% \yao{Updated:}
Suppose $i_T$ is fetched in both traces in step $k$ and $i_P$ is fetched in step $k+1$. Then suppose $i_T$ creates back-pressure in the fetch stream of one trace before $i_P$ has reached its decision source PL $src \in \mathbf{src}^P_\mathcal{M}$. The trace that has run ahead will wait for the other to catch up. However, in this time, $i_T$ may progress far enough in its execution such that it can no longer create variability for $i_P$ with respect to $src$. 
% \yao{To myself (For discussion/rebuttal): As an example, this could miss the case of \inst{DIV} as dynamic transmitter for \inst{REM} at \inst{ID} on CVA6. Consider $p = $ \inst{DIV};  \inst{REM}. When \inst{DIV} (candidate transmitter with varying operand value) is in division circuitry, it creates back-pressure for \inst{REM} at ID stage, and in return creates back-pressure in fetch stages. Stuttering now freeze the trace featuring \inst{DIV} that took fast path when its \inst{DIV} finishes and lets slower trace to catch up. By the time the late one catches up, the \inst{DIV} is already out of the division circuitry, and can no longer impact \inst{REM} to exhibit stall at ID stage versus not. The next step where both progress, both \inst{REM} in both traces progress to the division circuitry. }

%%
%However, constraining instruction fetch is not sufficient to enforce equality of operands, because most realistic processors, such as CVA6, have fetch and issue (where instructions bind their operand values) separated into different stages. 
%One could additionally constrain that issue or register-read stage of same instruction happens at same cycle, but this limits the dynamic interaction among instructions (such as precluding out-of-order issuing when the processor supports it) and thus renders synthesized leakage functions unsound. 
%%%
%this will likely  across two-trace two traces may not issue/register-read same instruction at the same cycle.  

In summary, all three approaches may \textit{mis-classify} a particular transponder decision as \textit{independent} of some transmitter’s operand, resulting in lack of soundness of synthesized leakage signatures. 
% stuttering circuit~\cite{wang2023specification} synchronizes the two copies by stalling one copy to wait for the other with respect to some constraint.

% {\color{red}
% ~\cite{liu2000automatic,song2013automatic
% }. }
% in advance that constrain operand values in both traces.
% The latter two solutions may .
%For the second solution, 



==> depr.tex <==
%\begin{figure}[t!]
%\begin{subfigure}{0.52\linewidth} 
%    \centering
%     %\includegraphics[width=0.79\linewidth]{figs/mul_sub_l_6.png}
%     %\includegraphics[width=0.82\linewidth]{figs/mul_sub_2.png}
%     %\includegraphics[width=0.81\linewidth]{figs/mul_sub_3.png}
%     \includegraphics[width=1.0\linewidth]{figs/mul_sub_3.png}
%     %\vspace{-2pt}
%     \caption{
%     Row(1/\llt{}): 1st/\llt{}-th visit to Row. Node label: value of \llt{} for \upath{}. 
%     %\yao{Updated}
%     }
%     %\upaths{}. Row\textsubscript{f}: \textit{final} visit to  Row. Node label \inst{n}: 1\textsuperscript{st} to \inst{n}\textsuperscript{th} visit to Row.}
%     %, n: \# in node). \textcolor{myred}{$\rightarrow$}: in-order commit. }
%     %\caption{\upaths{}. Row(f/l): exec. phase (first \inst{n}/last visit, \inst{n}: \# in node). }%, n: \# in node). \textcolor{myred}{$\rightarrow$}: in-order commit. }
%     \label{fig:zero-skip-uhb}
%\end{subfigure}%
%~
%%\hspace{0.01\linewidth}
%\begin{subfigure}[b]{0.47\linewidth} %130pt} %.55\linewidth}
%    \begin{tcolorbox}[left=0.1pt,right=0.2pt,top=1pt,bottom=1pt]
%    %\begin{framed}
%    \footnotesize
%      \noindent\textcolor{ForestGreen}{{\RaggedLeft// 
%      \inst{MUL} skips computation if it has zero operands or stays}}\\ 
%    \hlt{\noindent$\mathsf{dst\;MUL\_mulU(MUL^N\;i0)\!:}$} %\textcolor{ForestGreen}{// Leakage function} 
%    \newline
%        \indent$\;\;\mathsf{\textcolor{blue}{return}\;ite((}$\hlt{$\mathsf{i0.\iparg{arg0}}$}$\mathsf{\;== 0)\;\vee}$ \newline
%        \indent$\;\;\;\;\mathsf{(}$\hlt{$\mathsf{i0.\iparg{arg1}}$}$\mathsf{ \;== 0) \vee done, }$\newline
%        %$\mathsf{(path\_id == 1), }$\newline 
%        \indent$\;\;\;\;\hlt{$\mathsf{\{mulFin\},}$}$\hlt{$\mathsf{
%        %\{mulUnitFin\}, 
%        \{mulU\}}$}$\mathsf{)}$
%    \\[3pt]
%      \noindent\textcolor{ForestGreen}{{\RaggedLeft// \inst{SUB} proceeds or get stal-led by \inst{MUL} until it commits}} \\ % ($\mathtt{i1.cmt}$) }}\\
%    \hlt{\noindent$\mathsf{dst\;SUB\_scbFin(MUL^D\;i1)\!:}$}
%    \newline
%        \indent$\;\;\mathsf{\textcolor{blue}{return}\;ite((}$\hlt{$\mathsf{i1.\itarg{arg0}}$}$\mathsf{\;== 0)\;\vee}$ \newline
%        \indent$\;\;\;\;\mathsf{(}$\hlt{$\mathsf{i1.\itarg{arg1}}$}$\mathsf{ \;== 0)\vee i1.cmt, }$\newline
%        % rdy should be seomthing like atH(i1) 
%        \indent$\;\;\;\;$\hlt{$\mathsf{\{scbCmt\},}$}\hlt{$\mathsf{\{scbFin\}}$}$\mathsf{)}$
%    \end{tcolorbox}  
%    %\vspace{10pt}
%    \caption{\hlt{Leakage signatures} for \inst{MUL}/\inst{SUB}.}
%    \label{fig:leak_fun_muladd}
%\end{subfigure}
%% \begin{subfigure}[b]{1.0\linewidth} 
%% \begin{minipage}{\linewidth}
%% \begin{lstlisting}[style=uspecStyle]
%% Axiom MUL_paths: forall microops i, IsMultiply i $\Rightarrow$
%% AddEdges [((i, IF), (i, ID)); ((i, ID), (i, issue)); ...]
%% /\ (AddEdge((i, mulU(1)), (i, mulFin)) \/  
%%     AddEdge((i, mulU(1)), (i, mulU(l))).  % left or right
%% Axiom InOrderCmt: forall microops i0, i1, ProgramOrder
%% i0 i1 $\Rightarrow$ AddEdge((i0, scbCmt), (i1, scbCmt)).
%% \end{lstlisting}
%% \end{minipage}
%
%%     \caption{Top (bottom) axiom 
%%     %instantiates nodes and edges 
%%     %within a column (across columns), 
%%     corresponds to \upaths{} realizable by \inst{MUL} (dependencies between instructions).
%%     %describes \upaths{} realizable by \inst{MUL} (structural dependencies between instructions). 
%%     \yao{Possibly put inline to save space(?)}}
%%     \label{fig:uspec-mul-add}
%
%% \end{subfigure}
%%(a ``distinguished'' path selector function)
%\caption{%leakage functions for \inst{MUL} and \inst{SUB}.
%% Leakage functions for \inst{MUL} and \inst{SUB}.
%Zero-skip 
%\inst{MUL} takes a fast/slow \upath{}. In the latter case, it stalls a finished \inst{SUB} for one to three cycles.
%}
%    \label{fig:zero-skip-example}
%\end{figure}


\section{deprcated Introduction}
\yao{\textgreater{}\textgreater{}\textgreater{}Testing new intro}
\subsection{Topic sentences... (Expanded intro in next section)}
\begin{enumerate} [topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex] 
% \item \textbf{Microarchitectural Execution Paths.} \rtltouspec{}~\cite{rtl2uspec:hsiao:2021} synthesizes an axiomatic model of hardware, called \uspec{}, automatically from RTL design to enable, with the \textit{Check} family of tools~\cite{checkweb}, correctness proof of memory consistency model implementation down to the RTL level for the first time. However, the \textit{single-execution-path assumption}, where an instruction type exhibits exactly one kind of execution in all situations, limits its support of any modern hardware that has data-dependent behavior (e.g., cache hit versus miss path).

% \item To address the limitation, we extend concepts from the \uspec{}~\cite{pipecheck, ccicheck, coatcheck, rtlcheck, checkmate, rtl2uspec:hsiao:2021} and formalize the notion of \textit{microarchitectural execution paths} (\upaths{}) consisting of instruction's visits to different execution phases on hardware. 

% \item Beyond supporting the synthesis of complete \uspec{} models, multi-\upaths{} indicate variable hardware resource usage exhibited by an instruction type. Importantly, when an instruction's \upaths{} variability is operand-dependent on some instruction(s), this implies a hardware side-channel, from which we can for the first time define precisely hardware side-channel leakage. 
% MUL example?

% \item \textbf{Hardware side-channel attack.} In a hardware side-channel attack, transmitter (victim) modulates a channel (hardware resource) in a secret-dependent manner, and a receiver (attacker) infers the secret by observing the channel modulation.

% \item Minimally a defense requires flagging the unsafe operands of transmit instructions on a microarchitecture, often summarized in the so-called constant-time (CT) contracts. 
%, so as to, for example, block the channel modulation using software-based or hardware-based solution. 

\item \caroline{I do think this is good to mention somewhere, but probably not in the intro.} Nevertheless, defenses solely based on CT contracts can be increasingly impractical due to 1) performance overhead from increasing amount of secret to protect~\cite{spectre} and 2) growing number of transmitters due to growing number of data-dependent optimization deploy~\cite{pandora:isca:21}.

% \item Given the trends, hardware-based defenses require and exploit details regarding each channel modulation and observation to design performant and secure hardware. 
%(e.g., conditions under which channel modulation is induced and observed) 

% \item Common to both software and hardware based defenses is \textit{leakage contracts} of varying granularity that describe leakage on a microarchitecture.
%(informal and implicit in the case of hardware-based defense).
% These defenses are effective only if leakage contracts are provably upheld by the hardware, but there exists yet an automatic and scalable tool to synthesize or verify a CT contract against hardware, not to mention the exact details on channels required by hardware-based defenses.

% \item \textbf{This Paper.} A fundamental challenge in constructing and verifying leakage contracts is that there exits no formal way to describe side-channel leakage.  
%so as to synthesize and verify them against the hardware. We observe that \upaths{} enables channel observation.
% Insight 1: leakage function supports enforcement of defenses
% Insight 2: upath enables channel observation
% Insight 3: upath enable synthesis of leakage function

% \item \textbf{Putting it all Together.} In addressing the challenge, we propose 1) \upaths{}-based \textit{per-channel leakage function} as a unifying framework to captures what operand(s) of transmitter(s) induces modulation of channels that render distinct observation, and 2) an automatic tool that synthesizes and verifies leakage function against the hardware.

\end{enumerate}

\subsection{Contribution List}

\begin{enumerate} [topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex] 
\item \upaths{}
\item Leakage function: Per-channel description that map the operand(s) space of transmitter(s) to the distinct behaviors of transponder instruction execution made by the receiver
    \begin{itemize} [topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
    \item Extending side-channel attack taxonomy with notion of transponder
    \end{itemize}
\item \synthlc{} and CVA6 case study
\end{enumerate}

\subsection{Bullets summarizing related works}
\begin{itemize} [topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
\item Intrinsic transmitters are required in Dolma (called variable-time micro-ops), STT family of works including STT, SDO, SPT (called explicit channels)
\item Dynamic transmitters are required in MI6 (called Strong Timing Independence), STT family of works (called implicit channels), ConTExt (called instruction that influece the microarchitectural state that it has to stall), and Dolma (called resolvent micro-ops). 
\item Static transmitter are required in MI6 (for its microarchitectural state flushes), OISA (for its requirement on branch predictor), STT family of works (included in the implicit channels), ConTExt (called operations that influence "uncore" or off-core microarchitectural elements), and Dolma (micro-ops that produce persistent state modifications).
\item Decisions source PL are required in MI6 (to enforce strong timing independence), STT family of works (for the point where ``the effects of branch resolution'' take place), SDO (for implementing the control to select DO invariants), and Dolma (for the poitn where ``prediction resolves for inducive micro-ops''). 
\item upaths are required in NDA (for checking if speculative-store-bypass is a threat), and SDO (for DO invariants). 
% decision source PL is not enough, take MUL for eample, one needs to know a total of 64 paths can spawn from the mulU corresponding to 64 DO invariants (non-interfereing w.r.t the input operand value)
\end{itemize}

%\clearpage

\noindent \textgreater{}\textgreater{}\textgreater{} Expanded introduction...

\section{Introduction}
%\label{sec:intro}


% \rtltouspec{}~\cite{rtl2uspec:hsiao:2021} synthesizes an axiomatic model of hardware, called \uspec{}, automatically from RTL design to enable, with the \textit{Check} family of tools~\cite{checkweb}, correctness proof of memory consistency model implementation down to the RTL level for the first time. However, the \textit{single-execution-path assumption}, where an instruction type exhibits exactly one kind of execution in all situations, limits its support of any modern hardware that has data-dependent behavior (e.g., cache hit versus miss path).

% \textbf{Microarchitectural Execution Paths.} To address the limitation, we extend concepts from the \uspec{}~\cite{pipecheck, ccicheck, coatcheck, rtlcheck, checkmate, rtl2uspec:hsiao:2021} and formalize the notion of \textit{microarchitectural execution paths} (\upaths{}) consisting of instruction's visits to different execution phases on hardware. 
%     \begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
%     \item For example, consider a 32-bit multiply (\inst{MUL}) instruction executing on a processor whose multiplication unit ($\mathtt{mulU}$) implements the canonical \textit{zero-skip} optimization~\cite{andrysco:subnormal,Mult_leaky}. A \inst{MUL} will spend a \textit{single} cycle in the $\mathtt{mulU}$ if it has at least one zero operand; else, it will spend a \textit{few} cycles~\cite{arm7TDMI}.
%     \item Fig.~\ref{fig:zero-skip-uhb} shows two \upaths{} (a column of graph is a \upath{}) for 32-bit \inst{MUL} on a variant of the RISC-V CVA6 CPU~\cite{cva6} that implements zero-skip multiplies~\cite{andrysco:subnormal,Mult_leaky}.
% %and \inst{SUB} instructions executing 
%     \end{enumerate}


% Beyond supporting the synthesis of complete \uspec{} models, multi-\upaths{} indicate variable hardware resource usage exhibited by an instruction type. Importantly, when an instruction's \upaths{} variability is operand-dependent on some instruction(s), this implies a hardware side-channel, from which we can for the first time define precisely hardware side-channel leakage. 
%     \begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
%     \item Cotinuing our running example of \inst{MUL}, a \inst{MUL} creates multiple \upaths{} for itself---it may spend one or four cycles computing its result in the $\mathtt{mulU}$. 
%     \item Shown simultaneously in Fig.~\ref{fig:zero-skip-uhb}is a concurrent \inst{SUB} with two \upaths{}: a \inst{MUL} creates \upath{} variability for itself (a concurrently in-flight \inst{SUB}) with respect to its \inst{mulU} (the \inst{SUB}'s \inst{scbFin}) execution phase
%     %may exhibit either left or right \upath{} with respect when \inst{SUB} is in \inst{scbFin} execution phase depending which 
%     \end{enumerate}
%creates multiple \upaths{} for concurrently in-flight \inst{SUB}s---a completed \inst{SUB} may remain in the $\mathtt{scbFin}$ execution phase for one to three extra cycles before committing (three in Fig.~\ref{fig:zero-skip-uhb}).

% Fig.~\ref{fig:zero-skip-uhb} shows two \upaths{} (a column of graph is a \upath{}) for 32-bit \inst{MUL} on a variant of the RISC-V CVA6 CPU~\cite{cva6} that implements zero-skip multiplies~\cite{andrysco:subnormal,Mult_leaky}.

% For example, consider a 32-bit multiply (\inst{MUL}) instruction executing on a processor whose multiplication unit ($\mathtt{mulU}$) implements the canonical \textit{zero-skip} optimization~\cite{andrysco:subnormal,Mult_leaky}. A \inst{MUL} will spend a \textit{single} cycle in the $\mathtt{mulU}$ if it has at least one zero operand; else, it will spend a \textit{few} cycles~\cite{arm7TDMI}.
%    \item Fig.~\ref{fig:zero-skip-uhb} shows two \upaths{} (a column of graph is a \upath{}) for 32-bit \inst{MUL} on a variant of the RISC-V CVA6 CPU~\cite{cva6} that implements zero-skip multiplies~\cite{andrysco:subnormal,Mult_leaky}.
%and \inst{SUB} instructions executing 
%    \end{enumerate}

% \textbf{Hardware side-channel attack.} In a hardware side-channel attack, transmitter (victim) modulates a channel (hardware resource) in a secret-dependent manner, and a receiver (attacker) infers the secret by observing the channel modulation.
%     \begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
%     \item Initially, transmitter was primarily a specific \textit{transmit instruction} executed by victim.
%     \item With the introduction of transient execution attacks, more ways to induce channel modulation emerges through speculatively-executed transmit instructions or even non-instructions (such as hardware prefetcher~\cite{pandora:isca:21, augury:2022:vicarte:oakland22}). 
%     \item Channel types, attacker strategy, and observation model also expand as a result of various hardware structures and optimization technique found to be exploitable. 
%     \end{enumerate}

Minimally a defense requires flagging the unsafe operands of transmit instructions on a microarchitecture, often summarized in the so-called constant-time (CT) contracts~\cite{arm:dit,intel:doit,riscv_zkt,pandora:isca:21}. 
%, so as to, for example, block the channel modulation using software-based or hardware-based solution. 
    \begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
    \item Give a \ct{} contract, software-based defenses~\cite{Bernstein:curve25519, Bernstein:Poly1305-AES, Molnar:pc-security-model, Rane:Raccoon, Fisch:Iron,Shaon:SGX-BigMatrix, Zheng:Opaque, Eskandarian:OliDB, Mishra:Oblix,  Tople:oblivious-execution, Sasy2018ZeroTraceO, Ahmad2018OBLIVIATEAD, Coppens:timing-channel-x86, FactLanguage, synthct} ensure that secrets \textit{never} reach unsafe operands during program execution, a strategy called \textit{\ct{} programming}\footnote{``Constant time'' is a legacy term that denotes ``data oblivious''~\cite{yu:oisa}.} 
    \item Software-based defenses~\cite{barthe:highassurance,ctfoundations:pldi:20,guarnieri:spectector,vassena:blade,guanciale:inspectre,guarnieri:contracts,shivakumar:spectredeclassified, guanciale:inspectre,cauligi:sok-spectre-sw-defense, serberus:mosier:2024} against transient execution attacks~\cite{spectre,canella2019systematic} similarly rely heavily on \ct{} contracts by using serialization instruction to prevent secret leaking under hardware faults and mispredictions. 
%as a result of hardware from reaching unsafe operands of speculatively executed transmitters. 
%Defenses both transient~\cite{barthe:highassurance,ctfoundations:pldi:20,guarnieri:spectector,vassena:blade,guanciale:inspectre,guarnieri:contracts,shivakumar:spectredeclassified, guanciale:inspectre,cauligi:sok-spectre-sw-defense, serberus:mosier:2024} and non-transient attacks~\cite{ct works} rely heavily on these contracts. 
    %\item They aim to ensure that secrets never reach unsafe operands of (speculatively or non-speculatively executed) transmit instructions (through automatic program transformation~\cite{} or serialization~\cite{}). 
    \item Nascent ISA adoption of CT contracts, including Arm DIT~\cite{arm:dit} and Intel DOIT~\cite{intel:doit} \textit{hardware modes}, and the RISC-V Zkt~\cite{riscv_zkt} \textit{ISA extension}, further underscores their importance. 
    \end{enumerate}

Nevertheless, defenses solely based on CT contracts can be increasingly impractical. % due to 1) performance overhead from increasing amount of secret to protect and 2) growing number of transmitters due to growing number of data-dependent optimization deploy~\cite{pandora:isca:21}.
    \begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
    \item For one, performance overhead increases when the secrets to protect ballon from a handful of keys in cryptographic code~\cite{openssl, libsodium, hacl, mbedtls} to almost entire memory of general programs~\cite{jiyong:stt,choudhary:2021:spt,Bourgeat:m16, Schwarz:ConTExT, yu:oisa,jiyong:sdo,barber:specshield,weisse:nda,dolma} due to transient execution attacks.
    %\item For one, there are more information to protect from a handful of keys in cryptographic code in the early days to the entire memory of general programs.
    \item For the other, the slowing of Moore's Law encourages bespoke data-dependent hardware optimizations to maintain performance gains. This phenomenon will soon render \textit{all instruction operands unsafe by default}~\cite{pandora:isca:21}.
    %\item There exists not yet automatic and scalable verification method to construct and verify the CT contracts.
    \end{enumerate}

Given the trends, hardware-based defenses~\cite{jiyong:stt,choudhary:2021:spt,Bourgeat:m16, Schwarz:ConTExT, yu:oisa,jiyong:sdo,barber:specshield,weisse:nda,dolma} require and exploit details regarding each channel modulation and observation to design performant and secure hardware (\S\ref{sec:tspec} and \S\ref{sec:related}). % explained more in related work and motivating example?
%(e.g., conditions under which channel modulation is induced and observed) 
    \begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
    % intrinsic transmitter
    %\item Some works~\cite{dolma, jiyong:stt,choudhary:2021:spt,jiyong:sdo} requires to classify whether or not a transmit instruction can induce channel modulation and manifest distinct observation in itws own execution as well. 
    % dynamic transmitter 
    \item For example, some works~\cite{Bourgeat:m16, jiyong:stt,choudhary:2021:spt,jiyong:sdo, Schwarz:ConTExT, dolma} requires if a transmit instruction induces channel modulation that causes ``other'' instruction(s) to exhibit distinct execution behavior or not.
    % decision source PL
    \item When channel is induced from ``instruction interaction'', some of these defenses~\cite{Bourgeat:m16, jiyong:stt,choudhary:2021:spt,jiyong:sdo, dolma} requires at what point of instruction execution is effected by variable resource (such that to delay execution only as late as possible).
    % static 
    \item Some works~\cite{Bourgeat:m16, yu:oisa, jiyong:stt,choudhary:2021:spt, Schwarz:ConTExT, jiyong:sdo, dolma} also requires enumerating transmit instructions that induce statefule modulation versus not. 
    \item We discuss in more details in \S\ref{sec:related}, but we note that these details enable these proposal to attain both performance and security.
    \end{enumerate}

Common to both software and hardware based defenses is \textit{leakage contracts} of varying granularity that describe leakage on a microarchitecture.
    \begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
    %\item However, , but there exists yet an automatic and scalable tool to synthesize or verify a CT contract against hardware, not to mention the exact details on channels required by hardware-based defenses.
    \item These defenses are effective only if leakage contracts are provably upheld by the hardware. 
    \item However, for software-based defense, there exists no automatic and scalable way to synthesize/verify a CT contracts that they depend on. 
    \item For hardware-based defense, it remains challenging to implement these proposals on existing hardware when there exists no tool that exhaustively collects details for every channel on a given microarchitecture. 
%contracts to enable complete way to collect exhaustively all channels on a given microarchitecture, not to mention the fine-grained details about each channel including the condition under which modulation is induced, instruction execution that are effected by the channel, and more.
    \end{enumerate}
%(informal and implicit in the case of hardware-based defense).
%    \item It thus remains challenging to implement these proposals on existing hardware.


\textbf{This Paper.} A fundamental challenge in constructing and verifying leakage contracts is that there exits no formal way to describe side-channel leakage.  
    \begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
    \item Specifically, both software-based and hardware-based defenses require verification engineers or architects to reason about when and how leakage are induced and manifest. % 
    \item Such task is complicated by the vague notion of the channels themselves, how their modulation is controlled by transmit instruction operands, and how their modulation manifests as distinct receiver observations. 
    %\item Without enumerating all channels and the operands of transmitters, CT contracts will be incomplete and render software-based defense void. 
    %\item Similarly, hardware-based defense will be ineffective if channels are not exhaustively identified and classified to be addressed according to each defense proposal.
    \end{enumerate}
%  Transmitter -> Channel modulation -> Channel observation -> Leakage
\textbf{Insight 1: \upaths{} Enable Channel Observation.}
    \begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
    \item To formally reason about leakage, we observe that a transmit instruction's execution creates \upath{} variability for one or more \textit{transponder instructions}, or simply \textit{transponders},\footnote{In telecommunications~\cite{roddy2006satellite}, ``a transponder is the series of interconnected units which forms a single communications channel between the receive and transmit antennas in a communications satellite.''} 
    executed by the victim or receiver. A receiver ultimately observes a transmit instruction's channel modulations by detecting which \upath(s) its transponder(s) took at runtime, e.g., by measuring transponder execution time. 
    \item \inst{MUL-ADD} example.  
    \end{enumerate}
    
\textbf{Insight 2: Leakage Functions Supports Enforcement of Defenses.}
    \begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
    \item With \upaths{} providing channel and leakage observation capability, to define leakage regarding each channel reduces to collecting leakage functions (Fig.~\ref{fig:leak_fun_muladd}) that define how a channel, modulated by transmit instructions (function arguments), creates \upath{} variability (function outputs) for a transponder with respect to some phase of the transponder's execution (function name).
    
    \item \inst{MUL-ADD} example's leakage function. 
    \end{enumerate}


\textbf{Insight 3: \upaths{} Enable Synthesis of Leakage Function.}
    \begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
    \item  A key benefit of \upaths{} and transponders is that they enable an automated procedure for synthesizing leakage functions from processor RTL that relies \textit{primarily} on evaluating simple \textit{(single-)trace properties} on the design under verification (DUV).  In contrast, all existing leakage contract verification approaches, which target \ct{} contracts, \textit{exclusively} evaluate \textit{2-safety hyperproperties}~\cite{gleissenthall:iodine,gleissenthall:xenon,wang2023specification,deutschmann:upec-do, deutschmann2023scalable}.
    \end{enumerate}

\textbf{Putting it all Together.} In addressing the challenge, we propose 1) \upaths{}-based \textit{per-channel leakage function} as a unifying framework to captures what operand(s) of transmitter(s) induces modulation of channels that render distinct observation, and 2) an automatic tool that synthesizes and verifies leakage function against the hardware. We summarize our contributions as follows.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%        % [ ] the correpsonidgly term in each work  STT,SDO, 
%        % set of intrinsic or non-intrinsic (which requires the transponder set)
%        % channel modlation and observation in same instruction or not
%        % how variable manifest example
%            %, through its own execution or effects on subtle effects as a result of interaction with other instructions. 
%        % -> intrinsinc for us:  explicit channel
%        % -> dynamic: STT, SDO, SPT, Dolma, MI6
%        % -> static:  
%        % -> decision src PL
%        \item When channel is induced from ``instruction interaction'', defenses~\cite{MI6, STT, SDO, SPT} requires at what point of instruction execution is effected by variable resource (such that to delay execution only as late as possible).
%        % where operand dependent modulation first manifest, decision source PL + transponder
%        % [ ] example of concrete terms for each work in (..)
%    \item Some works~\cite{MI6, OISA, STT, SDO, SPT, Dolma} asks architect to enumerate all possible ``stateful'' channels  and ensure they are not modulated by speculative instructions. % intel 
%    \item Beyond identifying channels, some works requires the architect to know if a channel is share-resources among instructions such as queue~\cite{MI6}, functional units~\cite{Dolma}
%    %, or ``persistent states'' such as caches.
%    \end{enumerate}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    \item Initially the transmitters were often \textit{transmit instructions} whose execution make the program execution time a direct function of its operands. The attacker can learn the secrets by simply observing the victim program's execution time.
%    \item the introduction of 
%execution createsvariable  
%    \item In Kocher's seminal attack and many that followed, transmitters are often \textit{transmit instructions} whose execution creates variable time usage of hardware and are observed by the attacker (via program execution time) to infer the secret they process.
%    \item While these older attacks exploit the timing variation induced by transmit instruction executed by the victim,
%and are timed by the attacker and  
%Kocher’s seminal attack exploit transmit instruction
%trasnmitter  Transmitter is initially a \textit{transmit instruction}
%This enables automatic synthesis of \upaths{} .
%, and design an automatic procedure to synthesizes all possible \upaths{} for each instruction automatically from RTL design.

%multi-\upaths{} further facilitates precise definition of hardware side-channels, when one can verify the path variability is \textit{operand-dependent} or not.
%, this implies a hardware side-channel, from which we can for the first time precisely define hardware side-channel leakage in terms of which instruction(s) respectively induces the channel modulation and enables the channel observation.



\section{From 02-background}
\yao{Kinda not really helpful in understanding since main use is the 3.1 as long as the next paragraph uses $m$ and $\mu$ directly which is also well-defined as mappings. \textgreater{}\textgreater{}\textgreater{}}
Consider state $s = \langle \sigma, \mu \rangle$, where $\sigma = \langle m, a \rangle$. We use $s(\sigma)$ and $s(\mu)$ to refer to the architectural and microarchitectural state components of $s$; $\sigma(m)$ and $\sigma(a)$ to refer to the main memory and architectural register file components of $\sigma$; $m(j)$% , $a(k)$, and $\mu(l)$
to refer to the value assumed by memory location $j$ in $m$;
% , architectural register, and microarchitectural register;
$s(\sigma)(m)(j)$ to refer to the value assumed by memory location $j$ in $s$; and so on.
\yao{\textless{}\textless{}\textless{}}

\section{From 03-spec}
\yao{To remove \textgreater{}\textgreater{}\textgreater{}}To construct these definitions, we define a \textit{dynamic privacy policy} $\phi = \{loc \cup reg_a \cup reg_{\mu} \} \rightarrow \{\textsc{l}, \textsc{h}, \textsc{o}, \textsc{t}\}$, which is updated synchronously with state transitions. We adopt the taint algebra from \textit{gate-level information-flow tracking} (GLIFT) under security lattice $\mathnormal{L} = \{\mathnormal{S}, \sqsubseteq\} = \{\{\textsc{l}, \textsc{h}, \textsc{o}, \textsc{t}\}, \{(\textsc{l}, \textsc{h}), (\textsc{l}, \textsc{o}), (\textsc{h}, \textsc{t}), (\textsc{o}, \textsc{t})\}\}$, where $(a, b) \in\hspace{3pt} \sqsubseteq$ indicates that information flow from $a$ to $b$ is allowed~\cite{GLIFT:lattice,lattice}.
% does not violate the privacy policy~\cite{GLIFT:lattice,lattice}.
Given $t = \lbbar p \rbbar_{\mathnormal{M}}^{\langle\sigma, \mu\rangle}$,
all state elements are \textsc{l}-labeled in $\phi$ initially (in state $\langle\sigma, \mu\rangle$), except for elements that overlap with $\pi$ (\S\ref{sec:background:sec-def}), whose labels are defined by 
$\pi$.
% Given $\lbbar p \rbbar_{\mathnormal{M}}^{\langle\sigma_0, \mu_0\rangle}$, dynamic privacy policy $\phi$ is an extension of static privacy policy $\pi$ initializes $\phi$, i.e., , $\phi = \pi$ in $\langle\sigma_0, \mu_0\rangle$. 
When $\phi$-labeled state mixes in step $k$ of trace $t$, $\phi$ is updated per the taint algebra in step $k+1$.

As before (\S\ref{sec:background:sec-def}), 
\textsc{l}- and \textsc{h}-labeled state elements contain low and high data, respectively. 
Label \textsc{o} is given to a specific decoded source register field $op_{xmit}$ of a specific decoded transmit instruction $I_{xmit}$. 
% \chris{prev sentence: don't we taint the src op for all instructions, not just transmitters?}
% \yao{I believe here we give O only when transmitter is decoded? Possibly add "is only given to"?}
When \textsc{h}-labeled state mixes with \textsc{o}-labeled state, indicating that operand $op_{xmit}$ of instruction $I_{xmit}$ is supplied with high data, the result is \textsc{t}-labeled state.
We can now define a predicate to denote if high data \textit{reaches} operand $op$ of instruction $I$ in execution trace $t$, which satisfies some leakage condition $c$:
%\footnote{{\color{myorange}Orange} highlights leakage conditions, which are new in this paper.}
% \textsc{T}-labeled state in \M{} 
% Instructions in $p$ read their operands from, and write their operands to, state elements in $\{loc \cup reg_a \cup reg_{op}\}$. 
% A register instruction with at least one \textsc{h}-labeled operand in $\phi$ will \textsc{h}-label its output in $\phi$.
% A memory load that reads \textsc{h}-labeled from memory will \textsc{h}-label its output in $\phi$.
% We define a predicate to determine if \textsc{h}-labeled data ever reaches operand $op$ of \textit{instruction} $i \in p$ in trace $t$:
% \caroline{I will change this to refer to just architectural operands and check the taint values of operands right before comment.}
% during an execution on \M{}:
% \chris{could we say "adopt the taint algebra from GLIFT" as a catch all?  This covers how taint flows in other operations (e.g., what happens if the PC gets tainted) that we don't explicitly mention.}
% \chris{is there an implicit quantifier over $loc$, $reg_a$ and $reg_\mu$?}
% \chris{For doing multiple levels of indexing into a state, e.g., $\sigma(m(loc))$, it isn't clear by the S2.2 notation whether it should look like $\sigma(m(loc))$ or $\sigma(m)(loc)$.}
\begin{equation}
\begin{split}
      \mathnormal{X}_\pi(I, op, t, {c}) =
      \begin{cases}
      true & \hspace{-7pt} \textcolor{ForestGreen}{//~I_{xmit} = I \land op_{xmit} = op} \\
      & \hspace{-7pt} \mathrm{if}~\exists n.\exists j. \exists k. \exists l. 
      t \vdash {c} \land t[n] = \langle \sigma, \mu \rangle  \\
      & \land~ \sigma = \langle m, a \rangle ~\land
      % i \in \mu_k \\
       (\phi(\sigma(m)(j)) = \textsc{t} \\
       & \lor~\phi(\sigma(a)(k)) = \textsc{t} \lor
       \phi(\mu(l)) = \textsc{t})\\
       % \mu_k(\mathtt{ROB[head]}) = i \\
       % & \land~\phi(reg_{a}(I, op)) = \textsc{h}\\
       % & (i \in \mu(rs) \land \phi(reg_{op}(rs, i, op)) = \textsc{h})) \\
      false &  \hspace{-7pt} \mathrm{otherwise}
    \end{cases}
\end{split}
\label{eq:access-policy}
\end{equation}
% \chris{this text needs a pass w/ the new eqn 3:}
% This function checks to see if there exists a state $\langle \sigma_k, \mu_k \rangle \in t$ that satisfies condition $c$, such that $i$ is in the \textit{read register (rr)} phase of its execution and accesses \textsc{h}-labeled data from $reg_a$, or if $i$ is in a \textit{reservation station (rs)} and accesses \textsc{h}-labeled data from $reg_{op}$, located in $rs$.
% \chris{is the dysjunction to handle things like bypassing?  I'm worried about whether this is complete / whether that will be clear to people.}
% \chris{Suggest changing bot and top to False and True to avoid confusion}
Recall that \ctC{} is the set of all $(I, op)$ pairs, such that $I$ is a transmitter with unsafe operand $op$ (\S\ref{sec:background:hw-sc-defense}).
% With this information and Eq.~\ref{eq:access-policy}, we define the \ct{} defense, parameterized by \ctC{}, below.
\pct{} contracts permit high data to reach transmitter operands in some circumstances, so we define \tspecC{} as the set of all $(I, op, c)$ tuples, such that instruction $I$'s operand $op$ is \textit{unsafe} in an execution trace that satisfies leakage condition $c$. We define \tshieldD{},
% the \pct{}  defense,
parameterized by \tspecC{}, below.
\yao{\textless{}\textless{}\textless{}}


\subsubsection{\upaths{} Formalized}
\label{sec:tspec:upathsdef}
\yao{Remove \textgreater{}\textgreater{}\textgreater{}}
%\rsout{
We define 
% A dynamic instruction $i$ with type $I$ exhibits one out of a set
$\boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathnormal{M}$ as the set of all possible possible \upaths{} that a dynamic instance of $I$ may exhibit when it runs on micraorchitecture \M{} (\S\ref{sec:tspec:upaths:op-packing}).
% ; $\boldsymbol{\mu \textsc{\textbf{path}}^i_\mathnormal{M}}$ as the set of all \upaths{} that $i$ may exhibit on \M{}.
% more than one \upath{} when it runs on a microarchitecture \M{}.
% }\yao{already mentioned in scene setting text earlier}
% We now
% \caroline{Please use this notation below:}
%we formally define the set $\mu \textsc{path}^{I}_\mathnormal{M}$ of all \upaths{} that instruction $i$ may exhibit on microarchitecture \M{}.
% define the set $\boldsymbol{\mu \textsc{\textbf{path}}^i_\mathnormal{M}}$ of all \upaths{} that instruction $i$ may exhibit on \M{}.
%
%
% \rsout{
% Then, $\upath_i = \{(pl, pl') \mid \exists t. con(pl, pl') \wedge visit(i, pl, t[k]) \wedge
% visit(i, pl', t[k+1])\}$.} \caroline{This is not capturing a notion of edge weights/revisits.}
% %
%\yao{$pl$ can be equal to $pl'$; we summarize consecutive revisits using node weight $w: (nodes ,\mathbb{N}) = \{ (pl, n) | \arg\max_n \exists t. (\forall j. 0 \le j < n, visit(i, pl, t[k+j])) \}$}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%To define a \upath{} for $i$, we first collect an ordered sequence of PLs visited by $i$ in trace $t$: $V = (s_0, s_1, .. s_j)$ where $ s_j = \{pl \mid visit(i, pl, t[k+j]\}\}$. The \upath{} for $i$ is thus an ordered list of tuples $E = (e_1, e_2, ..)$ where $e_j = \{(pl, pl')  \mid conn(pl, pl') \wedge pl \in s_{j-1} \wedge pl' \in s_j\} $
%\\
%\\
% \yao{
% As described below, e
Each
$p \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathnormal{M}$ 
% $\mu \textsc{path}^{I}_\mathnormal{M} \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathnormal{M}$ 
% represents some \upath{} that $i$ may exhibit on \M{} in some trace $t$. It
is a tuple $(V, E)$, where $V$ and 
$E$ are sequences of \textit{sets of PLs} and \textit{sets of happens-before edges}, respectively, as defined below.

% \chris{how are edge weights/time encoded in this representation?}
%\yao{A post-processing pass summarizes the revisited PLs using the node weight (numbers after row labels) for consecutively-visited (non-consecutively-visited) PLs.}
% is a sequence of partial orders defined as follows. 
Consider an execution trace $t$, where $i_I$ materializes in \M{} (i.e., appears in some PL) in state $t[j]$, and dematerializes (i.e., disappears from all PLs) in state $t[k]$, where $j<k$.
Suppose $i_I$ exhibits $p = (V, E) \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathnormal{M}$ from $t[j]$ through $t[k-1]$.
We define $V = (v_0, v_1, ..., v_{k-j-1})$, where $v_n = \{pl \mid visit(i_I, pl, t[j+n]) \}$ captures the set of PLs visited by $i_I$ in step $n$ of its execution.
% , sequenced sets of PLs visited at $n$-step of $i$'s execution.   
We define $E = (e_0, e_1, ..., e_{k-j-2})$, where $e_n = \{(pl, pl') \mid con(pl, pl') \wedge pl \in v_n  \wedge pl' \in v_{n+1}\}$ captures happens-before ordering between $i_I$'s visits to PLs in consecutive trace steps.
% captures happens-before ordering between \upath{} nodes. 
% We use dashed edge with label \inst{l} in Fig.~\ref{fig:upaths-example} to summarize \inst{l} consecutive revisits to the same PL where only first or last visit is incident with any edge. 
% Old def w/o weights:
% We define $V = (v_0, v_1, ..., v_{k-j-1})$, where $v_n = \{pl \mid \exists i. visit(i, pl, t[j+n])\}$ captures the set of PLs visited by $i$ in step $n$ of its execution. We define $E = (e_0, e_1, ..., e_{k-j-2})$, where $e_n = \{(pl, pl') \mid  con(pl, pl') \wedge pl \in v_n  \wedge pl' \in v_{n+1}\}$ captures happens-before ordering between $i$'s visits to PLs in consecutive trace steps.
% \yao{remove $\exists i.$ since this is constrained under an $i$}.  
 %\yao{Updated to match figure: }
%  New def w/weights:
% \rsout{We define $V = (v_0, v_1, ..., v_{k-j-1})$, where $v_n = \{(pl, l) \mid l > 0 \land \neg visit(i, pl, t[j+n-1]) \wedge (\wedge_{q = 0}^{l} visit(i, pl, t[j+n+q]))\} \cup \{(pl, 1) \mid visit(i, pl, t[j+n]) \wedge \neg visit(i, pl, t[j+n+1])\}$. The first set builder captures consecutively revisited PLs that are newly visited in $t[j+n]$ and assigns them label $l$. The second set builder captures all PLs visited for the last consecutive cycle in $t[j+n]$ and assigns them label $1$.
% We define $E = (e_0, e_1, ..., e_{k-j-2})$, where $e_n = \{(pl, pl') \mid  \exists l, l'. \land con(pl, pl') \wedge (pl, l) \in v_n  \wedge (pl', l') \in v_{n+1}\}$ captures happens-before ordering between \upath{} nodes.}
% \yao{FIGTWO:
% We define $V = (v_0, v_1, ..., v_{k-j-1})$, where $v_n = \{pl \mid visit(i, pl, t[j+n]) \}$, sequenced sets of PLs visited at $n$-step of $i$'s execution.   
% We define $E = (e_0, e_1, ..., e_{k-j-2})$, where $e_n = \{(pl, pl') \mid con(pl, pl') \wedge pl \in v_n  \wedge pl' \in v_{n+1}\}$ captures happens-before ordering between \upath{} nodes. 
% We use dashed edge with label \inst{l} in Fig.~\ref{fig:upaths-example} to summarize \inst{l} consecutive revisits to the same PL where only first or last visit is incident with any edge. 
% If there is not out/in-going edges to $pl$ across multiple visits $\wedge_{n=k}^{n=k+l} (pl, pl)$ we summarize using 
% } 
% $i$'s first/final visits to PLs in consecutive trace steps.
% visited captures PLs visited across $l$ consecutive cycles as one PL with node label $l$ and another with node label $1$ (representing final visit), for a total of $l+1$ consecutive visits. \caroline{All pls such that its the first cycle we visit them plus all pls such that it is the last cycle we visit them.}
% \yao{Maybe obvious as from bottom of p.5 when \inst{l} is first used, $l > 0$}
%\yao{Add quantified $l > 0$ (Or maybe obvious, then can be omitted): 
%We define $V = (v_0, v_1, ..., v_{k-j-1})$, where $v_n = \{(pl, l)\mid \exists l > 0. \neg visit(i, pl, t[j+n-1]) \wedge (\wedge_{q = 0}^{l} visit(i, pl, t[j+n+q]))\} \cup \{(pl, 1) \mid visit(i, pl, t[j+n]) \wedge \neg visit(i, pl, t[j+n+1])\} $ captures PLs visited across $l$ consecutive cycles as one PL with node label $l$ and another with node label $1$ (representing final visit), for a total of $l+1$ consecutive visits.
%}
% \yao{the q should be range from 0 to $l-1$ so the total number is $l$ cycles.}
% the set of PLs visited by $i$ consecutively starting in step $n$ of its execution via the first $w-1$ and the final visits. 

% We define $V = (v_0, v_1, ..., v_{k-j-1})$, where $v_n = \{(pl, w-1)\mid \neg visit(i, pl, t[j+n-1]) \wedge (\wedge_{q = 0}^{w-1} visit(i, pl, t[j+n+q]))\} \cup \{(pl, 0) \mid visit(i, pl, t[j+n]) \wedge \neg visit(i, pl, t[j+n+1])\} $ captures the set of PLs visited by $i$ consecutively starting in step $n$ of its execution via the first $w-1$ and the final visits.

%We define $E = (e_0, e_1, ..., e_{k-j-2})$, where $e_n = \{(pl, pl') \mid  \exists l. l'. m. m \le n + l \land con(pl, pl') \wedge (pl, l) \in v_n  \wedge (pl', l') \in v_{m}\}$ captures happens-before ordering between $i$'s visits to PLs in consecutive trace steps.
% We define $E = (e_0, e_1, ..., e_{k-j-2})$, where $e_n = \{(pl, pl') \mid  \exists l, l', m. n < m \le n + l \land con(pl, pl') \wedge (pl, l) \in v_n  \wedge (pl', l') \in v_{m}\}$ captures happens-before ordering between $i$'s first/final visits to PLs in consecutive trace steps.

% We define $E = (e_0, e_1, ..., e_{k-j-2})$, where $e_n = \{(pl, pl') \mid  \exists l, l'. con(pl, pl') \wedge (pl, l) \in v_n  \wedge (pl', l') \in v_{n+1}\}$ captures happens-before ordering between $i$'s visits to PLs in consecutive trace steps.
% \caroline{Yao: fix.}
%Then, a \upath{} for $i$ within a trace $t$, $ \mu \textsc{path}^{I}_\mathnormal{M}$, is $(V, E)$: $V$ is a sequence of node sets $\exists k, (v_0, v_1, ...)$, where $v_j = \{pl \mid visit(i, pl, t[k+j])\}$.
%$E$ is a sequence of partial orders set $(e_0, e_1, ..)$ where $e_j = \{(pl, pl') \mid  con(pl, pl') \wedge pl \in v_j  \wedge pl' \in v_{j+1}\}$. 
% In short, $\mu \textsc{path}^{I}_\mathnormal{M}$ collects the set of partial orders among $pl$ visited by $i$ in two consecutive steps. 
% }
%We define a \upath{} exhibited by $i$ within a trace $t$, 
%$ \mu \textsc{path}^{I}_\mathnormal{M}$, as $(V, E)$, where 
%$V = \{ (pl, r) \mid \forall r. 1 \le r \le (\sum_k visit(i, pl, t[k]))  \}$,  and \\
%$E = \{ ((pl, r), (pl', r')) \mid con(pl, pl') \wedge visit(i, pl, t[k]) \wedge visit(i, pl', t[k+1]) \wedge \sum_{l < k} visit(i, pl, t[l]) = r-1\;\wedge $ \\
%$ \sum_{l' < k} visit(i, pl', t[l']) = r'-1 \}$. \\
%In other words, a path $p \in \boldsymbol{\mu \textsc{\textbf{path}}^i_\mathnormal{M}}$ is a set of tuples $((pl, r), (pl', r'))$, where $i$'s $r$-th visit to $pl$ happens one cycle before $r'$-th visit to $pl'$ in some execution trace $t$.
%$\boldsymbol{\mu \textsc{\textbf{path}}^i_\mathnormal{M}}$ is thus the set of $\mu \textsc{path}^{I}_\mathnormal{M}$ under any trace $t$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \rsout{In other words, a path $p \in \upath_i$ is a set of tuples $(pl, pl')$, where $i$ visits $pl$ one cycle before $pl'$ in some execution trace $t$.}

Above, the predicate $con(pl, pl')$ returns true iff \ufsms{} corresponding to $pl$ and $pl'$ are connected purely by combinational logic in \M{}'s netlist. It requires that \upaths{} exclusively capture \textit{causal} happens-before relationships among visited PLs.
\yao{\textless{}\textless{}\textless{}}



\yao{Remove \textgreater{}\textgreater{}\textgreater{}}
A \textit{\upath{} decision}
$d^{I}_\mathnormal{M} = (src, \mathbf{dst})$ 
% $d^{I}_\mathnormal{M} = (src^{I}_\mathnormal{M}, \mathbf{dst}^{I}_\mathnormal{M})$
made by an instruction $I$ on microarchitecture \M{} is a tuple, where 
% $src^{I}_\mathnormal{M}$
$src$
is a single \textit{decision source} PL and $\mathbf{dst}$
% $\mathbf{dst}^{I}_\mathnormal{M}$
is a set of \textit{decision destination} PLs, that 
distinguishes \textit{at least two} of $I$'s \upaths{} on \M{}.
% of instruction $i$.
% localizes variability in one \upath{} compared to another \upath{} for the same instruction $i$.
We define the set of all decisions $\mathbf{d}^{I}_\mathnormal{M}$ that $I$ makes on \M{} below.
% Given an instruction $i$ (e.g., \inst{ADD} in our running example), we can define the set of decisions $\mathbf{d_i}$ across all of $i$'s \upaths{} as follows.
% , corresponding to two dynamic instances of the same instruction.
% \chris{define $\upath_i$}
% \yao{new subsubsection\S\ref{sec:tspec:upathsdef}}

% \rsout{First, we define the set of $i$'s \textit{decision source} PLs as}
% % consider all pairs of $i$'s \upaths{}, $p$ and $p'$, to derive the set of \textit{decision sources}
% \caroline{Please fix this definition:}
% \rsout{$\mathbf{src}^I_\mathnormal{M} = \{ pl \mid \forall p, p' \in \upath_i, ~pl \in p.nodes \land pl \in p'.nodes \land next(p, pl) \neq next(p', pl)\}$.
% In other words, a decision source PL $src^{I}_\mathnormal{M} \in \mathbf{src}^I_\mathnormal{M}$ is followed by a distinct set of \textit{decision destination} PLs in at least two of $i$'s \upaths{} on \M{}.
% Next, we can construct the set of decisions \caroline{Please fix this definition:}
% $\mathbf{d}^{I}_\mathnormal{M} = \{(src^{I}_\mathnormal{M}, \mathbf{dst}^{I}_\mathnormal{M}) \mid \forall  p \in \upath_i, \forall src^{I}_\mathnormal{M} \in \mathbf{src}^I_\mathnormal{M}, ~\mathbf{dst}^{I}_\mathnormal{M} = next (src^{I}_\mathnormal{M}, p) \}$.}
% \yao{Below is new text \textgreater\textgreater\textgreater} 
% % $\mu \textsc{path}^{I}_\mathnormal{M}

For \upath{} $p = (V, E)$, let 
% $\mathbf{pl}_p = \{pl \mid \exists v_n \in V. pl \in v_n \}$
% \yao{
$\mathbf{pl}_p = \{pl \mid \exists v_n \in V. pl \in v_n \}$
% }
select the set of all PLs that are visited
in $p$.
Let  $next(p, pl) = \{pl' \mid \exists e_n \in E. (pl, pl') \in e_n \}$ select the set of all PLs visited the cycle after $pl$ in $p$.
%\yao{Let  $next(p, pl) = \{pl' \mid \exists e_n \in E. ((pl, w), (pl', w')) \in e_n \}$ select the set of all PLs visited the cycle after $pl$ in $p$.}
We define the set of $I$'s decision source PLs on \M{} as $\mathbf{src}^I_\mathnormal{M} = \{ pl \mid \exists p, p' \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathnormal{M}. ~pl \in \mathbf{pl}_p \land pl \in \mathbf{pl}_{p'} \land next(p, pl) \neq next(p', pl)\}$.
%For a \upath{} $p = (V, E)$, $v_k \in V, e_k \in E$, %\upath{} of $i$, $p$, 
%%and $pl \in .v_k$, then 
%let $p.e_k(pl) = \{pl' \mid pl \in v_k \wedge (pl, pl') \in e_k \}$, the set of connected PLs visited by $i$ after visiting $pl$ in $v_k$.
%The set of $i$'s \textit{decision source} PLs, $\mathbf{src}^I_\mathnormal{M} = \{pl \mid  \forall p, p' \in \boldsymbol{\mu \textsc{\textbf{path}}^i_\mathnormal{M}}, \exists k, k', ~pl \in p.v_k \land pl \in p'.v_{k'} \land p.e_k(pl) \neq p'.e_{k'}(pl)\}$.
%% $\mu \textsc{path}^{I}_\mathnormal{M}
In other words, a decision source
$src \in \mathbf{src}^I_\mathnormal{M}$ 
% $src^{I}_\mathnormal{M} \in \mathbf{src}^I_\mathnormal{M}$
is followed by a distinct set of \textit{decision destinations} in at least two of $I$'s \upaths{} on \M{}.
We then define the set of \upath{} decisions for $I$ on \M{} as 
$\mathbf{d}^{I}_\mathnormal{M} = \{(src, \mathbf{dst}) \mid \exists p \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathnormal{M}. src \in \mathbf{src}^I_\mathnormal{M} \land 
\mathbf{dst} = \{pl \mid pl \in next(p, src)\}
\}$.
% \yao{%no $\cup$. \\%just $\mathbf{dst} = \{pl \mid \exists (V, E) \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathnormal{M}. \exists e_n \in E. (src, pl) \in e_n\}$; %why not use $\mathbf{dst} = \{pl \mid \exists p \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathnormal{M}. pl \in next(p, src)$?
% It should be:
% $\mathbf{d}^{I}_\mathnormal{M} = \{(src, \mathbf{dst}) \mid \exists p \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathnormal{M}. src \in \mathbf{src}^I_\mathnormal{M} \land 
% \mathbf{dst} = \{pl \mid pl \in next(p, src)\}
% \}$.
% %$\mathbf{dst} = \exists p \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathnormal{M}. \{pl \mid  pl \in next(p, src)$
% }
% \yao{there shouldn't be any $src^I_\mathnormal{M}$ to refer to element of $\mathbf{src}^I_\mathnormal{M} $}
% \caroline{Check}
% $\mathbf{d}^{I}_\mathnormal{M} = \{(src^{I}_\mathnormal{M}, \mathbf{dst}^{I}_\mathnormal{M}) \mid src^{I}_\mathnormal{M} \in \mathbf{src}^I_\mathnormal{M} \land \mathbf{dst}^{I}_\mathnormal{M} = \bigcup \{pl \mid \exists (V, E) \in \boldsymbol{\mu \textsc{\textbf{path}}}^{I}_\mathnormal{M}. \exists e_n \in E. (src^{I}_\mathnormal{M}, pl) \in e_n\}\}$.
% $ \forall  p \in \boldsymbol{\mu \textsc{\textbf{path}}^i_\mathnormal{M}}. \forall src^{I}_\mathnormal{M} \in \mathbf{src}^I_\mathnormal{M}, ~\mathbf{dst}^{I}_\mathnormal{M} = next (p, src^{I}_\mathnormal{M}) \}$.
%
%Next, we can construct the set of decisions 
%$\mathbf{d}^{I}_\mathnormal{M} = \{(src^{I}_\mathnormal{M}, \mathbf{dst}^{I}_\mathnormal{M}) \mid \forall  p \in \boldsymbol{\mu \textsc{\textbf{path}}^i_\mathnormal{M}}, \forall src^{I}_\mathnormal{M} \in \mathbf{src}^I_\mathnormal{M}, \forall k, \mathbf{dst}^{I}_\mathnormal{M} = p.e_k(src^{I}_\mathnormal{M}) \}$.
%src^{I}_\mathnormal{M} \in p.v_k,
%
%First, we define the set of $i$'s \textit{decision source} PLs as
%$\mathbf{src}^I_\mathnormal{M} = \{ pl \mid \forall p, p' \in \boldsymbol{\mu \textsc{\textbf{path}}^i_\mathnormal{M}}, \exists r_j \in p, r_{j'} \in p', ~pl \in p.nodes \land pl \in p'.nodes \land (next(pl, r_j) \neq next(pl, r_{j'}))\}$, where $p.nodes$ are all $pl$ visited by $i$ in $p$, and $next(pl, r_j)$ is the set $\{pl' \mid (pl, pl') \in r_j\}$. % for $r_j \in p$. %the $j$-th step for $i$ in $p$. 
%In other words, a decision source PL $src^{I}_\mathnormal{M} \in \mathbf{src}^I_\mathnormal{M}$ is followed by a distinct set of \textit{decision destination} PLs in at least two of $i$'s \upaths{} on \M{}.
%Next, we can construct the set of decisions 
%$\mathbf{d}^{I}_\mathnormal{M} = \{(src^{I}_\mathnormal{M}, \mathbf{dst}^{I}_\mathnormal{M}) \mid \forall  p \in \boldsymbol{\mu \textsc{\textbf{path}}^i_\mathnormal{M}}, \forall r_j \in p, \forall src^{I}_\mathnormal{M} \in \mathbf{src}^I_\mathnormal{M}, ~\mathbf{dst}^{I}_\mathnormal{M} = next (src^{I}_\mathnormal{M}, r_j) \}$.
%%%%%%%%
%First, for a path $p \in \boldsymbol{\mu \textsc{\textbf{path}}^i_\mathnormal{M}}$, let $next(p, pl)$ be the set $\{\{pl' \mid \forall pl'. \exists r'. ((pl, r), (pl', r')) \in p.E \} \mid \forall r. (pl, r) \in p.V \}$. 
%We define the set of $i$'s \textit{decision source} PLs as
%$\mathbf{src}^I_\mathnormal{M} = \{ pl \mid \forall p, p' \in \allpaths. \exists s, s'. s \in next(p, pl) \wedge s' \in next(p', pl) \wedge s \neq s'\}$. 
%%$. (pl,r) \in p.V \land (pl, r') \in p'.V \land next(p, (pl,r)) \neq next(p', (pl, r'))\}$.
%In other words, a decision source PL $src^{I}_\mathnormal{M} \in \mathbf{src}^I_\mathnormal{M}$ is followed by a distinct set of \textit{decision destination} PLs in at least two of $i$'s \upaths{} on \M{}.
%Next, we can construct the set of decisions 
%%\caroline{Please fix this definition:}
%$\mathbf{d}^{I}_\mathnormal{M} = \{(src^{I}_\mathnormal{M}, \mathbf{dst}^{I}_\mathnormal{M}) \mid \forall  p \in \upath_i. \forall src^{I}_\mathnormal{M} \in \mathbf{src}^I_\mathnormal{M}.\forall  ~\mathbf{dst}^{I}_\mathnormal{M} \in next (p, src^{I}_\mathnormal{M}) \}$.
%%Next, we can construct the set of decisions 
%%%\caroline{Please fix this definition:}
%%$\mathbf{d}^{I}_\mathnormal{M} = \{(src^{I}_\mathnormal{M}. \mathbf{dst}^{I}_\mathnormal{M}) \mid \forall  p \in \upath_i. \forall src^{I}_\mathnormal{M} \in \mathbf{src}^I_\mathnormal{M}.\forall r.  ~\mathbf{dst}^{I}_\mathnormal{M} = next (p, (src^{I}_\mathnormal{M}, r)) \}$.
% \\ \yao{\textless\textless\textless}

% \caroline{Check once we make other minor changes:}
% Fig.~\ref{fig:upaths-example} highlights decision source PLs (\textcolor{orange}{orange} nodes) and decision destination PLs (\textcolor{Cerulean}{blue} nodes) in the \upaths{} of various instructions according to their execution on CVA6-OP (from our running example) and the original CVA6 design.
With respect to its two \upaths{} in Fig.~\ref{fig:upaths-example}, \inst{ADD} on CVA6-OP (\M{}) has $\mathbf{src^\mathtt{ADD}_{\mathnormal{M}}} = \{\mathtt{ID}\}$ and $\mathbf{d^\mathtt{ADD}_\mathnormal{M}} = \{(\mathtt{ID}, \{\mathtt{issue}, \mathtt{scbIss}\}), (\mathtt{ID}, \{\mathtt{ID}\})\}$.
\yao{\textless{}\textless{}\textless{}} \\




\subsection{From Leakage Functions to \pct{} contracts}
\label{sec:tspec:lf-to-tspec}
% By precisely modeling how channel modulations manifest as receiver observations, l
% Furthermore, \inst{{I_P\_src^{I_P}_M}} highlights two classes of conditional leakage discussed in the 

% The function body captures leakage conditions related to particular transmit instruction \textit{operand values}.
% Input labels capture leakage conditions related to particular \textit{scheduling decisions}.

Leakage functions are useful, because they expose precise conditions under which transmit instructions leak their unsafe operands, thereby enabling the design of precise \pct{} contracts.\footnote{Leakage functions also enable formally defining static/dynamic channels (\S\ref{sec:background:telecom:channels}) and passive/active attacks (\S\ref{sec:background:telecom:receiver})---see \rsout{\S\ref{sec:tspec:static-dynamic} and \S\ref{sec:tspec:active-passive}, respectively}.\yao{TBD...}}
% Plus, they expose two flavors of \textit{leakage conditions}, which we use to construct \pct{} contracts in \S\ref{sec:tspec:lf-to-tspec}.
In particular, their function body captures conditions related to particular transmitter \textit{operand values}, while labels on their explicit inputs capture
% Input labels capture 
conditions related to microarchitectural \textit{scheduling decisions}.
% Leakage functions enable us to define the conditions under which transmit instructions leak their unsafe operands.\footnote{They also enable formally defining static/dynamic channels (\S\ref{sec:background:telecom:channels}) and passive/active attacks (\S\ref{sec:background:telecom:receiver})---see \S\ref{sec:tspec:static-dynamic} and \S\ref{sec:tspec:active-passive}, respectively.}

Given a set of leakage functions for a microarchitecture \M{}, we can define \tspecCupath{} for receiver \Rupath{} as follows. 

First, initialize \tspecCupath{} to $\{ (I, op, false) \mid \exists f, I \in f.args \land I.op \in f.body \}$, i.e., the set of all tuples $(I, op, false)$, where $I$ 
is an argument (explicit input) to some leakage function $f$ and $I.op$ appears in $f$'s function body. 
% This initial contract is the same as an empty \pct{} contract.
Recall that $(I, op, c) \in \mathnormal{C}_{pct}^\mathnormal{M,R_{\upath}}$ indicates that secrets \textit{may not} be supplied to operand $op$ of instruction $i$ in traces that satisfy $c$ (\S\ref{sec:tspec:formal-def}). % Since no trace satisfies $false$, o
Hence, our initial (``empty'') contract permits all transmitters to process secrets in \textit{all circumstances}.
% since all conditions that preclude supplying secrets to unsafe transmitter operands are $false$.
% since all the conditions under which transmitters $i$ may \textit{not} be supplied secrets in thier unsafe $op$
% This initial contract captures the same information as a transmitter-centric leakage contract \ctCupath{} (\S\ref{sec:tspec:upaths}).

% \chris{break out (i) (ii) etc into more visible bullets.}
% \yao{Line breaks added}

Next, for each $(I, op, c) \in \mathnormal{C}_{pct}^\mathnormal{M,R_{\upath}}$, consider every transponder $P$ along with every one of its leakage functions \inst{P\_src}, where $src \in \mathbf{src}^{P}_\mathnormal{M}$.
% \inst{I_P\_src^{I_P}_M}.
% that may contribute to its \upath{} variability on \M{}.
% it may query throughout its execution on \M{}.
% each of its associated leakage functions $f_{leak}$\yao{for some decision source PL $src_{i_p}$ }, and 
For each such function, $I$ may appear as an argument to 
% \inst{I_P\_src^{I_P}_M}
\inst{P\_src} zero or more times (e.g., corresponding to different dynamic instructions, possibly with different labels, as in \inst{ADD\_ID} in Fig.~\ref{fig:leakage_func_examples}).
For each instance of input $I$ in the argument list, if $op$ appears in the function body,
% , consider each instance of input $i$, and 
% For each time that $i$ appears as an input to \inst{I_P\_src^{I_P}_M} and $op$ appears in the function body,
replace $(I, op, c)\in \mathnormal{C}_{pct}^\mathnormal{M,R_{\upath}}$ with $(I, op, c \lor (s \land v))$,
% update $c$ with $c \lor c'$
% add $(I, op, c)$ to \tspecCupath{}
where $s \land v$ extends the (existing) leakage condition $c$ to rule out some situation in which supplying a secret to $op$ is unsafe.


Assertions $v$ and $s$ denote unsafe transmitter operand values and an unsafe microarchitectural scheduling decision, respectively.
Conservatively, $v$ and/or $s$ may be assigned $true$.
% , eventually resulting in a \pct{} contract that is logically equivalent to a \ct{} contract (\S\ref{}).
But, using leakage functions, both assertions can be defined more precisely as follows.

We identify three variants of $s$ based on $I$'s label in 
% \inst{I_P\_src^{I_P}_M}
\inst{P\_src}:


% \yao{If one ignores fine-grained leakage conditions that arises from unsafe scheduling decision/supplying of unsafe values, we set $s = true$/$v = true$. Otherwise, we construct $s$ and $v$ as follows. }
% Assertion $s$, denotes an unsafe \textbf{scheduling decision}:
% for which there are two options:
% as follows. \caroline{Need to communicate that we will consider $i$ for each time that it appears in \inst{I_P\_src^{I_P}_M}'s argument list. For each instance we will consider 1a or 1b and 2 to produce $s \land v$ to append to our leakage condition. States that if both $s$ and $v$ hold, $i$ cannot safely accept a secret in $op$.}
% \textbf{Rule 1a (Dynamic):}
\begin{itemize}
    \item If $I$ is intrinsic (\inst{I^N}),
    % in \inst{I_P\_src^{I_P}_M},
    then $s$ asserts ``$i_I$ visits \textit{src}.''
    % \inst{src^{I_P}_M}.''
    % This condition likely precludes secrets from being pass to $op$ from ever accepting secrets unless particular secret values are deemed safe (see below) or .
    \item If $I$ is dynamic (\inst{I^D}), then $s$ asserts ``$i_I$ is in-flight (visiting some PL) when  $i_{P}$\yao{$\neq i_I$} visits \textit{src}.'' \yao{Otherwise, when I and P is of same type it will be ambiguous}
    \item  If $I$ is static (\inst{I^S}), then the function body will indicate that (a function of) $op$ has persisted in some hardware structure $r$. Here, $s$ asserts ``$r$ is not overwritten between when it is updated by $i_I$ and when $i_{P}$ visits \textit{src}.''
    % \chris{does flushed include intervening writes by other instructions?}
    % \yao{Yes, possibly change to cleared or flushed?}
    % \item \color{olive}{\sout{If ignoring leakage conditions that arise due to scheduling decisions, $s = true$.}}\yao{I think this part starts with $s$ denotes unsafe scheduling decision but then this rule ignores unsafe scheduling decision; I put at top. }
\end{itemize}

Regardless of $I$'s input label in \inst{P\_src}, it may be safe for $I$ to compute on some secret values of $op$ (e.g., non-zero values for zero-skip multiply, \S\ref{sec:intro:this-paper:spec-challenge}), but not others, as far as leakage via transponder $P$ is concerned. Information theoretic approaches like multiplicative gain leakage~\cite{alvim2014additive}, mutual information~\cite{shannon1948mathematical}, or maximal leakage~\cite{wu2020case} may be used to characterize which operand values for $I$ % \yao{I?} 
result in  unacceptable privacy leakage. An operand range that yields a single decision may also be selected (\S\ref{sec:intro:this-paper}).
Several variants of $v$ may be constructed as follows:
\begin{itemize}
    \item  For all values $V = \{val_0, ..., val_n\}$ that are deemed unsafe for $op$ with respect to $P$, $v$ asserts ``$op$ is supplied some $val_j \in V$.''
    % \item \color{olive}{\sout{If ignoring leakage conditions that arise due to usafe operand values, $v = true$.}}
\end{itemize}

\yao{
Consider the running example \inst{ADD}'s argument \inst{arg0} and its leakage function \inst{ADD\_ID} in Fig.~\ref{fig:leakage_func_examples}. Since the first/second input is an intrinsic/dynamic \inst{ADD} (\inst{ADD^N\;i0}/\inst{ADD^D\;i1}), $c$ of $(\mathtt{ADD}, \mathtt{arg0}, c) $ will be extended to be disjunctive with $(\mathtt{i_{ADD}\;\mathsf{visits}\;ID})$ and $(\mathtt{i_{ADD}}\;\mathsf{is\;inflight\; when\;other}\;\mathtt{i'_{ADD}}\;\mathsf{visits}\;\mathtt{ID})$, assuming value condition $v$ to be \textit{true}. 
% \\ TODO! value condition \inst{msb(arg0) < 32} ? since \inst{msb(arg0) > 32} always results in slow path whereas \inst{msb(arg0) < 322} may or may not result in slow path. 
}
% \yao{Could we change $val_i$ to $val_n$ just not to confuse $i$}
The procedure above highlights the fact that \pct{} contracts represent a \textit{family} of leakage contracts that may account for a range of leakage conditions. For example,
% In particular, each $v$ and $s$ may be assigned $true$ (conservatively) or a more precise assertion, as defined above. Always 
always (conservatively) assigning $true$ to $v$ and $s$ will result in a 
% \yao{If leakage conditions only includes scheduling decisions (derivable from abstract leakage functions), the result contract is a family of \tspecHat{}.}
% If leakage conditions corresponding to scheduling decisions and unsafe operand values are both ignored, the resulting
\pct{} contract that is logically equivalent to a  \ct{} contract (\S\ref{sec:tspec:formal-def}).
\rsout{Overall, \pct{} contracts enable hardware and software to collaborate towards providing precise and performant hardware side-channel defenses (\S\ref{sec:contracts-to-defenses}).}
\yao{Move to the new subsection (along message in appendix) at the beginning of this section that indicates how the information can be used for side-channel defense.}

% 

% \begin{figure}[t!]
%     \centering
%      \includegraphics[width=0.9\linewidth]{figs/cva6_pls2.png}
%      \caption{
%      CVA6 block diagram. 1-21: $\langle \mathtt{IIR}, \mu \mathtt{FSM} \rangle$ pairs (\S\ref{sec:tspec:pls}). Bit-widths of \ufsm{} state variable(s) are given in parentheses.     %$\mathtt{PCR}$ and $\mu \mathtt{FSM}$ 
%      % defined by state variable(s) with bit width in parentheses.
%      %\inst{PCR_i} and $\mu FSM_i$ 
%      %followed by \ufsm{} consisting of state variables 
%      %CVA6 block diagram. 1-21:is a (PCR, \ufsm{}) tuple, where \ufsm{} are defined by state variables.
%      %(PCR, \ufsm{}) tuples. 
%      %A sample of synthesized \upaths{} on CVA6 with respect to data cache (for \inst{SW}) and core (for \inst{BEQ}, \inst{LW}, \inst{ADD}).
%      % Row(F/L): an exec. phase (first/last consecutive visit). 
%      }
%      \label{fig:cva6_block_diag}

% \end{figure}

\subsection{Formal Foundation}
\label{sec:tspec:formal-def}

We now define \textit{\pct{} contracts} \tspecC{} and the \textit{\pct{} defense} \tshieldD{}.

\yao{
To construct these definitions, we use $\mathnormal{X}_\pi(I, op, t, {c})$ to denote if high data with respect to $\pi$ \textit{reaches}\footnote{By reaching we mean taint of high data can propagate to some signal based on gate-level information-flow tracking~\cite{GLIFT:lattice,lattice}.} operand $op$ of instruction $I$ in an execution trace $t$ that satisfies some leakage condition $c$. 
}
% they enable.
% We show that \ct{} contracts are a special case of \pct{} contracts, and thus the \ct{} defense 
% % \ctD{} 
% can be defined analogously to the \pct{} defense.
% \tshieldD{}.
% also illustrate how their 
% \chris{we will show how the constant-time definitions can be expressed as a special case.}
% comparing both to their 
% constant-time counterparts, \ctC{} and \ctD{}, can be viewed as a special case.
% \chris{"conditionally constant-time" sounds like we are "conditionally sound"}
% \textit{conditionally constant-time} 
 %  we formally define both defense strategies in this section
% \caroline{TODO: I think we do need $reg_{op}$ after all...otherwise we I think we will not capture speculative transmitters.}\chris{agree.  Idea: Use the following lattice: L -> H, L -> O, H -> T, O -> T.  H = high operand data as before.  O = a label given to the decoded source register fields of decoded transmitter instructions.  When H mixes with O (meaning an in-flight transmitter touched H data), we get T.  Presence of T labeled data is a violation.}
\yao{Removed $X_\pi$ (in 11-depr now)}

% , as follows.
% \yao{1. To make sure I understand, $op$ is not used anywhere but its implicitly used because the ``assume xmit = i'' that introduces label \textsc{o} at $op$, right?}
%2. I think then the predicate denote if high data reaches operand $op$ for $i$ or any state elements, but since \textsc{t} is only introduced from \textsc{o} at $op$}

% \chris{if we are short on space, I think we can drop Def 3.1 and just keep the brief mention of it at the beginning of Sec 3.2.}
% \begin{definition}[Constant-Time Defense $\mathnormal{D}_{ct}^{\textcolor{MidnightBlue}{\mathnormal{M}}, \textcolor{MidnightBlue}{\mathnormal{R}}, \textcolor{MidnightBlue}{\pi}}$]
% With respect to receiver \textcolor{MidnightBlue}{\R{}} and security policy \textcolor{MidnightBlue}{$\pi$}, program \textcolor{MidnightBlue}{$p$} running on microarchitecture \textcolor{MidnightBlue}{\M{}} from initial state \textcolor{MidnightBlue}{$\langle \sigma, \mu \rangle$} enforces the \textit{constant-time (\ct{}) defense} $\mathnormal{D}_{ct}^{\textcolor{MidnightBlue}{\mathnormal{M}}, \textcolor{MidnightBlue}{\mathnormal{R}}, \textcolor{MidnightBlue}{\pi}}$, 
% parameterized by $\mathnormal{C}^\mathnormal{M, R}_{xmit}$, 
% or $\mathnormal{D}_{ct}^{\textcolor{MidnightBlue}{\mathnormal{M}}, \textcolor{MidnightBlue}{\mathnormal{R}}, \textcolor{MidnightBlue}{\pi}}(\lbbar \textcolor{MidnightBlue}{p} \rbbar_{\textcolor{MidnightBlue}{\mathnormal{M}}}^{\color{MidnightBlue}\langle \sigma, \mu \rangle})$, iff:

% \chris{pedantic notation comment: would we say $c=true$ or $c=\lambda(t):true$?}
% \begin{equation}
% \begin{split}
%       % (\lbbar p \rbbar_{\mathnormal{M}} \vdash \mathnormal{D}_{(s)ct}^{\mathnormal{R}, \pi}) \iff 
%       % \forall p.
%       % \forall \sigma_0. \forall \mu_0. 
%       \forall i. \forall op. 
%       i \in \textcolor{MidnightBlue}{p} \land (I, op)\in \mathnormal{C}^{\textcolor{MidnightBlue}{\mathnormal{M}}, \textcolor{MidnightBlue}{\mathnormal{R}}}_{ct} \hspace{-2pt} \implies \hspace{-2pt} \neg \mathnormal{X}_\pi(I, op, \lbbar \textcolor{MidnightBlue}{p} \rbbar_{\mathnormal{M}}^{\color{MidnightBlue}\langle \sigma, \mu \rangle}, {true})
%       % \\
%       % \land~({i.op1 \in \mathnormal{C}^\mathnormal{R}_{ct}}\implies \mathnormal{X}_\pi(I, op1, \lbbar p \rbbar_{\mathnormal{M}}^{s_0}))
% \end{split}
% \label{eq:ct-defense}
% \end{equation}
% \end{definition}
% Eq.~\ref{eq:ct-defense} says for all instructions $i \in p$ and all operands $op$, if $i$ is a transmitter with unsafe operand $op$, then high data \textit{never} reaches $op$ in $\lbbar p \rbbar_{\mathnormal{M}}^{\langle \sigma, \mu \rangle}$, i.e., the leakage condition ${c = true}$.


% As discussed in \S\ref{sec:intro:this-paper:spec-challenge} and the start of this section, 

% below.

% Eq.~\ref{eq:ct-defense} solves the second challenge associated with Eq.~\ref{eq:non-interference}, since it is a trace property.
% (i.e., a hyperproperty involving a single trace, $\lbbar p \rbbar_{\mathnormal{M}}^{\langle \sigma_0, \mu_0 \rangle}$).
% We can use Eq.~\ref{eq:ct-defense}, instead of Eq.~\ref{eq:non-interference}, to verify a that a program $p$ is hardware side-channel safe with respect to receiver \R and privacy policy $\pi$ when it runs on \M{}. The catch is that we need to verify \textit{once} that \M{} upholds its leakage contract $\mathnormal{C}_{ct}^\mathnormal{R}$, i.e., \textcolor{Orange}{$\mathnormal{M} \vdash_{\mathnormal{C}^\mathnormal{R}_{ct}}\mathnormal{D}[hw]^{\mathnormal{R},\pi}$} from
% Eq.~\ref{eq:security-contract}. Verifying that \M{} upholds its execution contract is also important, but we focus on leakage contract verification in this per which spans many important defenses~\cite{defenses-that-depend-on-ct-contracts}.


% Our first contribution is a novel class of leakage contracts, called \pct{} contracts, which add to $\mathnormal{C}_{ct}^\mathnormal{R}$ the \textit{conditions} under which transmitters can safely process secrets.
% Thus, we can define a \textit{conditional constant-time defense} $\mathnormal{D}^{\mathnormal{R}, \pi}_{\tau}$ based on \pct{} contract $\mathnormal{C}_{\tau}^\mathnormal{R}$ for program $p$ running on microarchitecture \M{} as:

\begin{definition}[Permissive Constant-Time Defense $\mathnormal{D}_{pct}^{\textcolor{MidnightBlue}{\mathnormal{M}}, \textcolor{MidnightBlue}{\mathnormal{R}}, \textcolor{MidnightBlue}{\pi}}$]
With respect to receiver \textcolor{MidnightBlue}{\R{}} and security policy \textcolor{MidnightBlue}{$\pi$},
program \textcolor{MidnightBlue}{$p$} running on microarchitecture \textcolor{MidnightBlue}{\M{}} from initial state \textcolor{MidnightBlue}{$\langle \sigma, \mu \rangle$} enforces the \textit{\pct{} defense} $\mathnormal{D}_{pct}^{\textcolor{MidnightBlue}{\mathnormal{M}}, \textcolor{MidnightBlue}{\mathnormal{R}}, \textcolor{MidnightBlue}{\pi}}$, 
% parameterized by \tspecC{},
or $\mathnormal{D}_{pct}^{\textcolor{MidnightBlue}{\mathnormal{M}}, \textcolor{MidnightBlue}{\mathnormal{R}}, \textcolor{MidnightBlue}{\pi}}(\lbbar \textcolor{MidnightBlue}{p} \rbbar_{\textcolor{MidnightBlue}{\mathnormal{M}}}^{\textcolor{MidnightBlue}{\langle \sigma, \mu \rangle}})$, iff:
\begin{equation}
\begin{split}
      % (\lbbar p \rbbar_{\mathnormal{M}} \vdash \mathnormal{D}_{(s)ct}^{\mathnormal{R}, \pi}) \iff 
      % \forall p. 
      % \forall \sigma_0. \forall \mu_0.
      \forall I. \forall op. \forall {c}. 
      % i \hspace{-1pt} \in \textcolor{MidnightBlue}{p} \hspace{-1pt} \land
      (I, op, {c}) \in \mathnormal{C}^{\textcolor{MidnightBlue}{\mathnormal{M}},\textcolor{MidnightBlue}{\mathnormal{R}}}_{pct} \implies  \neg \mathnormal{X}_\pi(I, op, \lbbar \textcolor{MidnightBlue}{p} \rbbar_{\textcolor{MidnightBlue}{\mathnormal{M}}}^{\textcolor{MidnightBlue}{\langle \sigma, \mu \rangle}}, {c})
\end{split}
\label{eq:tspec-defense}
\end{equation}
\end{definition}
% \yao{From our discussion that defense is a function of M and R only, then shouldn't here the permissive constant-time defense be parameterized only by M and R only, and thus $\pi$ should not be colored?}


%\yao{Maybe its common/less confusing to use $.$ instead or $,$ as quantifier separation? But I sometimes confuse $c.i$ as some entity and realize there is not such child property exists for $c$. }
% Clearly, Eq.~\ref{eq:tspec-defense} prevents high data from reaching the unsafe operands of transmitters under \textit{certain conditions}, as specified in $\mathnormal{C}_{\tau}^\mathnormal{R}$.

% In a passive attaick the transpoder
% Define active/passive attacks.  T is victim instruction, by definition. However, P may be a victim instruction or an attacker instruction.
% \begin{itemize}
%     \item In a passive attack, P is a victim instruction.
%     \item In an active attack, P is an attacker instruction.
% \end{itemize}
% \subsubsection{\upath{} Divergences and Path Selector Functions}
% \subsubsection{Modeling Channels with Leakage Functions}
% \subsubsection{Defining Circumstantial Leakage with \pct{} contracts}
% Given our observations, \pct{} contracts are \textit{transponder-centric}, enumerating transponders and a set of leakage functions for each. 
% Leakage function arguments are instructions, which are distinguished as the \textit{transponder} itself ($\mathtt{OP_P}$) or other \textit{dynamic} ($\mathtt{OP_D}$) or \textit{static} ($\mathtt{OP_S}$) instructions that it may interact with.
% Classifying arguments in this way
% enables hardware side-channel defenses that are tailored to particular \textit{threat models}, or which \textit{conditionally} pass secrets to transmit instructions or \textit{periodically} obfuscate hardware state.
% \caroline{Our Goal: We want to make programmers aware of the conditions under which transmit instructions leak their operand(s), so that can use them to process secrets safely. This can be accomplished with per-channel leakage functions that map the operand space of a transmit instruction that modulates some channel onto the observation space of a receiver that observes this channel. To do this, however, we must first (1) precisely define the notion of a channel which has been used to represent a range of hardware resources from ports to full modules, and (2) precisely define how channel modulations manifest as receiver observations.}
% Both the zero skip and operand packing examples highlight conditional leakage. Note scheduling for operand packing. Also highlight how channel modulations manifest as receiver observations. 
% What is a \upath{}? We proposed that \upaths{} should be modeled at the granularity of instructions projecting state updates onto the design. \ufsms{} can help us do this. 
% Given all of this information, we can define \pct{} contracts. 
% \suksection{\pct{} contracts by Example}
% \label{sec:tspec:examples}
% \caroline{Illustrate/explain leakage functions for a a microarchitecture that implements a variety of optimizations (e.g., those from Pandora~\cite{pandora:isca:21}).}
% \caroline{\pct{} contracts: 2 pages}

\section{From 04-tsynth}

In theory, the various instances of Eq.~\ref{eq:non-interference-cex} described in \S\ref{sec:checking-eq-8} can checked on \M{} by: (i) constructing a \textit{product circuit}, where \M{} is instantiated twice, to check the property directly~\cite{wang2023specification, deutschmann:upec-do}, or (ii) augmenting \M{} with \textit{information flow tracking} (IFT) circuitry to check the property indirectly~\cite{gleissenthall:xenon, gleissenthall:iodine}.
The first strategy is regarded as more precise~\cite{yang2018lazy}. However, with our goal of attributing transponder decisions to transmitter operands, it exhibits a soundness limitation \rsout{(\S\ref{sec:product-circuit-limitations})}\yao{TBD}.
% We refer the interested reader to \S\ref{} for more details.
% Due to issues outlined in 
% the limitations associated with the product circuit formulation of % these limitations, we decide to instantiate
% \S\ref{sec:product-circuit-limitations}, 

\section{from previous appendix}
\subsection{From \pct{} Contracts to Hardware Side-Channel Defenses}
\label{sec:contracts-to-defenses}
\pct{} contracts enable hardware and software to collaborate towards providing precise and performant hardware side-channel defenses. For example, program transformations may be able to constrain transmitter operand values. Hardware designers can provide targeted instructions for flushing microarchitectural state from software that may leak the operands of static transmitters. Hardware can schedule instructions from victim and attacker processes such that dynamic transmitters in the victim never create \upath{} variability for transponders executed by the attacker. \pct{} contracts enable these defense strategies towards co-optimizing for security and performance in a post-Moore's Law world.

\section{Caroline dump}
Eq.~\ref{eq:non-interference} presents two key challenges.
% , e.g., due to operand-dependent fast and slow paths for many instructions~\cite{arm:dit,intel:doit,riscv_zkt,pandora:isca:21}. 
First, it is a \textit{hyperproperty}~\cite{clarkson2010hyperproperties} (over two traces),
% , $\lbbar p \rbbar_{\mathnormal{M}}^{\langle \sigma, \mu \rangle}$ and $\lbbar p \rbbar_{\mathnormal{M}}^{\langle \sigma', \mu \rangle}$,
which is notoriously difficult to check.
Second, most microarchitecture does not enforce Eq.~\ref{eq:non-interference} for an arbitrary program (satisfying our assumptions in \S\ref{sec:background:sec-def:program}) and privacy policy, given a realistic receiver, like $\mathnormal{R}_C$~\cite{arm:dit,intel:doit,riscv_zkt,pandora:isca:21}.
Hardware side-channel defenses address both issues.
% ---the former by being sufficiently conservative so as to be checkable as (single-)trace properties.
% \chris{by being sufficiently conservative to be checkable as (single-)trace properties.}

\begin{definition}[Hardware Side-Channel Defense]
\label{def:sc_defense}
% Given microarchitecture ${\color{MidnightBlue}\mathnormal{M}}$ and receiver ${\color{MidnightBlue}\mathnormal{R}}$, a 
A \textit{hardware side-channel defense} $\mathnormal{D}^{{\color{MidnightBlue}\mathnormal{M}},{\color{MidnightBlue}\mathnormal{R}},{\pi}}$ is a \textit{(single-)trace property} 
% (e.g., Eq.\ref{eq:ct-defense}, Eq.\ref{eq:tspec-defense})
of program {$p$} with privacy policy {$\pi$}, running on microarchitecture ${\color{MidnightBlue}\mathnormal{M}}$, with respect to receiver ${\color{MidnightBlue}\mathnormal{R}}$, such that:
% (e.g., Eq.~\ref{eq:ct-defense}), such that:
% of a program $p$ running on a microarchitecture \M, such that:
\begin{equation}
\begin{split}
     \forall p. \forall \pi.
     \left( \forall \sigma. \forall \mu.
     % \lbbar p \rbbar_{\mathnormal{M}}^{\langle \sigma, \mu \rangle} \vdash
     \mathnormal{D}^{{\color{MidnightBlue}\mathnormal{M}}, {\color{MidnightBlue}\mathnormal{R}}, {\pi}}
     (\lbbar {p} \rbbar_{{\color{MidnightBlue}\mathnormal{M}}}^{\langle \sigma, \mu \rangle})
     \right)
     \hspace{-4pt}
     \implies
     \hspace{-4pt}
     \mathrm{SC\hbox{-}Safe}({\color{MidnightBlue}\mathnormal{M}}, {\color{MidnightBlue}\mathnormal{R}}, {p}, {\pi})
\end{split}
\label{eq:hw-sc-defense}
\end{equation}
\end{definition}
% \yao{From our discussion: we will change back to $\forall \forall$ }
Eq.~\ref{eq:hw-sc-defense} says that for 
every pair of a program 
{$p$} and a security policy {$\pi$}, if \textit{all} of {$p$}'s executions on \textcolor{MidnightBlue}{\M{}} uphold
$\mathnormal{D}^{{\color{MidnightBlue}\mathnormal{M}},{\color{MidnightBlue}\mathnormal{R}},{\pi}}$, then  
% for \textit{all of their executions} on \textcolor{MidnightBlue}{\M{}},
% (regardless of initial state $\langle \sigma, \mu \rangle$),
%satisfies $\mathnormal{D}^{\mathnormal{R},\pi}$,
hardware side-channel safety (Eq.~\ref{eq:non-interference}) holds for the same \textcolor{MidnightBlue}{\M{}}, \textcolor{MidnightBlue}{\R{}}, $p$, and {$\pi$}.

% \yao{I think we already discussed in our discussion.
% My confusion is from terms: Def 2.2 is defining defense ``w.r.t hardware'', is parameterized by M and R, makes sense to quantify over all pi, and requires eqn 3 to satisfy but is a two-trace property (eqn 3) \\ 
% However a defense w.r.t a program and a policy, facilitated by hardware and software, is just a single trace property. 
% }
% \yao{Regardless of initial state deviate from the equation; this quantifier in the description seems a bit different from the equation itself; a $p$ satisfies $D$ only under certain $\mu_0$ is more sensible. Suggest: ``
% Eq.~\ref{eq:hw-sc-defense} says that for all programs $p$, for any initial state such that $\mathnormal{D}^{\mathnormal{R},\pi}$ is enforced, microarchitectural non-interference (Eq.~\ref{eq:uni}) holds. 
% ''
% }


% \chris{The below makes sense, but I'm wondering whether its too general / adding too much notational complexity for this paper.  How about: 
% - We define the contract as the set of instructions that are transmitters / unsafe.  I don't even think we need operand granularity here (that's something we will cover in S3).
% - Give Eqn 3, but say that both SW and HW have the same responsibility: ensure that given architectural semantics (SW) and microarchitectural semantics (HW), don't pass H to unsafe/transmit instructions.  
% - Existing contracts say an instruction is unsafe/a transmitter if there exists an execution whereby passing H data to said instruction creates a timing difference, it is considered a transmitter.  This is overly restrictive; the next section develops tsynth models....}


As a trace property,
% checking that a program $p$ running on a microarchitecture \M{} enforces
$\mathnormal{D}^{\mathnormal{M},\mathnormal{R},\pi}$ resolves the first challenge associated with Eq.\ref{eq:non-interference}, as it is much easier to check. 
% \yao{w.r.t program verification?}
To address the second challenge, hardware side-channel defenses solicit cooperation from hardware and software, facilitated by a \textit{leakage contract} $\mathnormal{C}^{\mathnormal{M}, \mathnormal{R}}$. Informally, a leakage contract exposes information about how a particular microarchitecture \M{} may leak the data it processes to a particular receiver \R{} via hardware side-channels.
% \caroline{I think contracts should be parameterized by the microarchitecture - I will  update this notation throughout.}
% $\mathnormal{C}^\mathnormal{R}$ as follows.

For example, consider the \ct{} defense \ctD{}, which is enabled by a \ct{} contract \ctC{} (\S\ref{sec:background:telecom:transmit-lc}). We define \ctC{} as the set of all $(I, op)$
pairs, such that with respect to \R{}, $I$ is transmitter with unsafe operand $op$ on \M{}. % Specifically, $i$ denotes a particular instruction opcode and function.
Given \ctC{}, hardware and software cooperate to enforce \ctD{} for a program $p$ when it runs on \M{}. This involves preventing data that depends on $p$'s private inputs (i.e., high data in $\pi$)
% (i.e., programs' private inputs) from ever reaching
% $p$'s private inputs (i.e., high data in $\pi$) from reaching
from ever \textit{reaching} 
operand $op$ of a dynamic instruction $i_I \in p$ at runtime, where $(I, op) \in \mctC$ (\S\ref{sec:tspec:formal-def}). 

Note that we use upper-case, like $I$, to denote an instruction \textit{type} (e.g., \rsout{\inst{MUL~rd, rs1, rd2}}\yao{\inst{MUL}, \inst{ADD}, etc.}) and lower-case, like $i$ to denote a \textit{dynamic} instruction; $i_I$ denotes a \textit{dynamic} instruction of type $I$.
% \yao{I feel this footnote could be in main text, unlike the others being supplemantary, this one is some convention we will use throughout?}
% We use $(i, op) \in \mctC$, where $i$ has type $I$, to denote $(I, op) \in \mctC$. The notation $i \in p$ returns $true$ iff $i$ belongs to program $p$.}
% instruction  $I =_t i$ denotes that dynamic instruction $I$ is of type $i$.


%\footnote{We use lower-case $i$ to denote an instruction \textit{type} (e.g., \inst{MUL}) and upper-case $I$ to denote a \textit{dynamic} instruction; $I =_t i$ denotes that dynamic instruction $I$ is of type $i$.}
% ; \S\ref{sec:tspec:formal-def} formalizes this defense strategy.
%\mathnormal{C}^{\mathnormal{M}, \mathnormal{R}}_{xmit} 
% as one of our contributions.

\yao{\textgreater{}\textgreater{}\textgreater{} Remove following?}

\ct{} contracts often assume $\mathnormal{R}_C$. Thus,
% \yao{assume execution time observability for the receiver ($\mathnormal{R} = \mathnormal{R}_C$) (\S\ref{sec:background:sec-def}) and } have
$(I, op) \in \mathnormal{C}^{\mathnormal{M}, {\mathnormal{R}_C}}_{ct}$ iff there exists a program $p$ with privacy policy $\pi$, such that data derived from $p$'s private inputs reaching operand $op$ of dynamic instruction $i_I \in p$ 
implies a violation of $\mathrm{SC\hbox{-}Safe}(\mathnormal{M}, \mathnormal{R}_C, \pi, p)$.
Informally, $i_I$ creates timing variability for $p$ as a function of $op$'s data value.
Interestingly,
% when high data is supplied to $op$. 
% \rsout{That is, $\mathnormal{R} = \mathnormal{R}_C$.}
% \chris{unclear that '$\mathnormal{R} = \mathnormal{R}_C$' is due to 'execution time variability' as opposed to something else in the first sentence}
% \yao{It is due to 'execution time variability'. Addressed w/ new text above}
this approach is simultaneously too strong and too weak.
% both \textit{overly-restrictive} and \textit{narrow} in threat model scope. In particular, 
First, instruction operands are assumed \textit{entirely} safe or unsafe (i.e., they create timing variability, or they do not), when in reality hardware side-channel leakage is highly circumstantial (too strong). Second, many practical threat models assume more powerful receivers than $\mathnormal{R}_C$ (too weak)~\cite{perf_counter_sc,powerexploit, acousticexploit, radiationexploit,KocherDPA,sok_em_side_channels,branchpred_sc, portsmash, memjam, xu:controlledchannelattacks, drama, tlb_bleed}.
%resource contention~\cite{branchpred_sc, portsmash, memjam, xu:controlledchannelattacks, drama, tlb_bleed}, etc.
%~\cite{perf_counter_sc,powerexploit, acousticexploit, radiationexploit,KocherDPA,sok_em_side_channels}.
%todo}.
Plus, an automated approach for formally verifying hardware adherence to \ct{} leakage contracts remains elusive (Table~\ref{table:relatedwork}).

We develop \pct{} contracts (\S\ref{sec:tspec}) and \tsynth{} (\S\ref{sec:tsynth-approach})
% develop \tspec{} models and the \tsynth{} approach,
to resolve these leakage contract specification and verification challenges.
\yao{\textless{}\textless{}\textless{}}



% Typically software and hardware have the same responsibility when enforcing $\mathnormal{D}^\mathnormal{R}_{ct}$: $p \vdash_{\mathnormal{C}^{\mathnormal{R}}} \mathnormal{D}[sw]^{\mathnormal{R},\pi}$ iff $p$ ($\mathnormal{M} \vdash_{\mathnormal{C}^{\mathnormal{R}}} \mathnormal{D}[hw]^{\mathnormal{R},\pi})\implies\mathrm{Eq.~\ref{eq:non-interference}}$) iff $p$ (\M{}) never passes high data to transmitters architecturally (microarchitecturally).

% To address the second challenge, hardware side-channel defenses solicit cooperation from hardware and software, facilitated by a \textit{leakage contract} $\mathnormal{C}^\mathnormal{R}$, such that for a receiver \R{}, privacy policy $\pi$, and microarchitecture \M{}: 
% \begin{equation}
% \begin{split}
%       % (\lbbar p \rbbar_{\mathnormal{M}} \vdash % \mathnormal{D}^{\mathnormal{R},\pi}) \\ \iff
%       % \forall \mathnormal{M}. 
%       \forall p. (p \vdash_{\mathnormal{C}^{\mathnormal{R}}} \mathnormal{D}[sw]^{\mathnormal{R},\pi} \land \mathnormal{M} \vdash_{\mathnormal{C}^{\mathnormal{R}}} \mathnormal{D}[hw]^{\mathnormal{R},\pi})\implies\mathrm{Eq.~\ref{eq:non-interference}})
% \end{split}
% \label{eq:security-contract}
% \end{equation}
% Eq.~\ref{eq:security-contract} says that
% % every execution of $p$ on \M{} upholds defense $\mathnormal{D}^{\mathnormal{R},\pi}$ iff 
% for all programs $p$, which enforce \textit{software} component of the defense $\mathnormal{D}[sw]^{\mathnormal{R},\pi}$ with respect to $\mathnormal{C}^\mathnormal{R}$ and run on \M{} that upholds the \textit{hardware} component of the defense $\mathnormal{D}[hw]^{\mathnormal{R},\pi}$ with respect to $\mathnormal{C}^\mathnormal{R}$, Eq.~\ref{eq:non-interference} holds, assuming the same \M{}, \R{}, and $\pi$.

% For the \textit{constant-time defense} $\mathnormal{D}^\mathnormal{R}_{ct}$ (\S\ref{sec:background:telecom:transmit-lc}), we define contract $\mathnormal{C}^\mathnormal{R}_{ct}$ as a set of $(I, op)$ pairs, denoting that instruction $i$ is a transmitter with unsafe operand $op$. 
% Typically software and hardware have the same responsibility when enforcing $\mathnormal{D}^\mathnormal{R}_{ct}$: $p \vdash_{\mathnormal{C}^{\mathnormal{R}}} \mathnormal{D}[sw]^{\mathnormal{R},\pi}$ iff $p$ ($\mathnormal{M} \vdash_{\mathnormal{C}^{\mathnormal{R}}} \mathnormal{D}[hw]^{\mathnormal{R},\pi})\implies\mathrm{Eq.~\ref{eq:non-interference}}$) iff $p$ (\M{}) never passes high data to transmitters architecturally (microarchitecturally).
% , and 

% \M{} never passes high data tor

% : ensure that given architectural semantics (sw) and microarchitectural semantics (hw) don't pass high data to unsafe operands of transmitters.
% Existing contracts say an instruction is unsafe if there exits an execution whereby passing H data to said instruction creates a timing difference. This is both overly restrictive and narrow in threat model scope. The next section develops \tspec{} models.

% The former (\textit{our focus}) defines what program data may leak to a receiver.


% A security contract is composed of a \textit{leakage contract} and an \textit{execution contract}, i.e., $\mathnormal{C}^\mathnormal{R} = \langle \mathnormal{C}^\mathnormal{R}_{lc}$, $\mathnormal{C}^\mathnormal{R}_{ex} \rangle$~\cite{guarnieri:contracts,cauligi:sok-spectre-sw-defense,serberus:mosier:2024}.
% The former (\textit{our focus}) defines what program data may leak to a receiver.
% The latter defines what (possibly speculative) control- and data-flow a program may exhibit runtime.
% Table~\ref{tab:hw-sc-defenses} highlights two hardware side-channel defenses from the literature which use the transmitter-centric leakage contract $\mathnormal{C}^\mathnormal{R}_{ct}$ that we study in this paper.

% \subsection{Threat Model Summary}
% \label{sec:background:threat-model-summary}
% \chris{we need to define what the type of $\mathnormal{C}^\mathnormal{R}_{lc}, \mathnormal{C}^\mathnormal{R}_{ct}$ is.}
% We study variants of transmitter-centric leakage contracts $\mathnormal{C}^\mathnormal{R}_{lc} = \mathnormal{C}^\mathnormal{R}_{ct}$, which support constant-time defenses $\mathnormal{D}_{ct}^{\mathnormal{R}, \pi}$ (\S\ref{sec:background:telecom:transmit-lc}).
% We can define any such defense in a manner that abstracts away details of the assumed execution contract.

% To do this, w


% Only control-flow instructions may update the $pc$'s $\phi$-labeling.

% When a $p$ first begins executing, instructions will access their operands via architectural state $\{loc \cup reg_a\}$.
% However, due to out-of-order execution and speculation, instructions will largely access their operands from $reg_{op}$.

% That is $\phi$ is initialized with the state privacy policy $\pi$.

% All arithmetic operations in \ourmodel{} propagate security labels in this way (\S\ref{sec:asm-other-inst}), as in prior work \cite{ctfoundations:pldi:20}.

% All arithmetic operations in \ourmodel{} propagate security labels in this way (\S\ref{sec:asm-other-inst}), as in prior work \cite{ctfoundations:pldi:20}.
% \chris{how about tweaking $\mathnormal{X}$ to be a predicate?}

% \footnote{Eq.~\ref{eq:access-policy} may be adapted to accommodate any execution phases during which an instruction may access operands via non-architectural operand registers.}
% , $i \in \mu_k$ evaluates to true if $i$ is currently in-flight in $M$.
% $reg_{op}(i, arg)$ returns the \textit{operand register} identifier $reg_{op} \in reg_{\mu}$ (\S\ref{}) for the state element that holds $i$'s argument $arg$ in $\mu_k$ (if such a state element exists), and $i \in \mu_k$ evaluates to true if $i$ is currently in-flight in $M$. 


% $\mathnormal{C}_{ct}^\mathnormal{R}$ or \M{} upholds $\mathnormal{C}_{ct}^\mathnormal{R}$

% \begin{figure}
%     \begin{tcolorbox}[left=0pt,right=0pt,top=2pt,bottom=2pt]
%     %\begin{framed}
%     \small
%     %\noindent\textcolor{ForestGreen}{{\RaggedLeft// \textbf{\inst{SW} in CVA6}: \inst{SW} updates non-write-allocate 4-way set-associative cache if there exists a prior \inst{LD} whose address overlaps. Data are stored in two-parallel banks.}}\\
%     %: LD in `LdUnit' phase taking path 0 for cache miss or path 1-4 for cache-read paths of corresponding data banks. Assume each way is in a separate bank and a write-no-allocate 4-way set associative cache)}}\\
%     %\noindent\textcolor{ForestGreen}{{\RaggedLeft// Precondition}}\\
    
%         \noindent\textcolor{ForestGreen}{{\RaggedLeft// \textbf{Operand packing:} \inst{ADD_P} in ID0 takes \upath{} 1 if it is the only instruction in ID queue or eligible to be packed with another dynamic \inst{ADD_D}, else it takes \upath{} 0 to be head of the ID FIFO.}}\\
%            {
%        \renewcommand{\arraystretch}{1.3}
%     \setlength{\arrayrulewidth}{1pt}
%      \begin{tabular}[t]{
%        @{}>{\raggedright\arraybackslash} m{0.95\linewidth}
%        }
%     \centering\arraybackslash $\mathsf{visit(i0, ID0)}$ \\[2pt]
%     \hline
%     \noindent\hlt{$\mathsf{path\_id\;ADD\_ID0(ADD_I\;i0,\;ADD_D\;i1)}$}$\mathsf{\;:}$ \newline
%     \indent$\;\;\mathsf{path\_id= (IDCnt == 1\;\vee (IDCnt == 2\;\wedge\; visit(i1, ID1) \;\wedge}$\newline 
%     \indent$\;\;\;\;\mathsf{(\forall arg \in \{}$\hlt{$\mathsf{i0.\iparg{op0}, i0.\iparg{op1}, i1.\itarg{op0}, i1.\itarg{op1}}$}$\mathsf{\}, msb(arg) < 32)))}$\newline
%     \indent$\;\;\mathsf{\textcolor{blue}{return}\;ite(path\_id, }$\hlt{$\mathsf{\{issueALU\}, \{ID1\}}$}$\mathsf{)}$\\
%        \end{tabular}
%    } 
%    \end{tcolorbox}
% \end{figure}





% such that $\mathnormal{M} \vdash_{\mathnormal{C}^\mathnormal{R}_{ct}}\mathnormal{D}[hw]^{\mathnormal{R},\pi}$
% \M{}'s adherence to a (partial) \tspec{} model and constant-time contracts $\mathnormal{C}_{ct}$, which \tspec{} models subsume.

% Our work defines (\tspec{}) and verifies (with \tsynth{}) $LC_P$-style (transponder-centric, \S\ref{}) leakage contracts under the assumption of receiver $\mathnormal{R}_{\mu \textsc{path}}$.

% $\mathnormal{M} \vdash_\mathnormal{C}_{ct} \mathnormal{D}^{\mathnormal{R},\pi}_{hw}$, we just need to verify that $\mathrm{Eq.~\ref{eq:ct-defense}} \implies \mathrm{Eq.~\ref{eq:non-interference}}$

% from satisfy that holds for all execution traces (starting in any initial state)
% that holds for all execution traces (starting in any initial state).
% \yao{so its meaning this? 
% A \textit{hardware side-channel defense} $\mathnormal{D}$ w.r.t a contract C is a property of a program $p$ running on a microarchitecture $M$ that holds for all execution traces (starting in any initial state). 
% }
% % \chris{Doesn't the above need to be w.r.t. a specific policy $\pi$?  Then below, the implication will imply that Property 1 holds w.r.t. the same $\pi$.}
% \begin{definition}[Effectiveness]
% Hardware side-channel defense $\mathnormal{D}$ parameterized by contract $\mathnormal{C}$ is \textit{effective} for program $p$ on microarchitecture $M$ iff $(\lbbar p \rbbar_{M} \vdash_{\mathnormal{C}} \mathnormal{D}) \rightarrow \mathrm{Eq.~\ref{eq:non-interference}}$.
% \end{definition}


% First, they solicit cooperation from hardware and software to enforce Eq.~\ref{eq:non-interference}.
% Typically, hardware enforces Eq.~\ref{eq:non-interference} for a subset of \textit{safe} execution traces and software emits code that is guaranteed to generate one of these safe traces.
% This coordination is facilitated by a hardware-software contract $\mathnormal{C}$.
% Second, a hardware side-channel defense $\mathnormal{D}$, parameterized by a contract $\mathnormal{C}$, is a \textit{trace property} of a program running on a microarchitecture, such that $\lbbar p \rbbar_{M} \vdash_\mathnormal{C} \mathnormal{D} \implies Eq.~\ref{eq:non-interference}$. Checking $\lbbar p \rbbar_{M} \vdash_\mathnormal{C} \mathnormal{D} \implies Eq.~\ref{eq:non-interference}$ is hyperproperty that need only be checked once when a defense is first proposed. Checking $\lbbar p \rbbar_{M} \vdash_\mathnormal{C} \mathnormal{D}$ is a trace property that can be more easily checked for each $p$ running on \M{}. For some microarchitecture, checking this property may only require checkin...


% We can verify that $\lbbar p \rbbar_{M} \vdash \mathnormal{D} \implies$ Eq.~\ref{eq:non-interference} once and then verify that our program running on the microarchitecture satisfies the defense.


% \artem{So one execution is from $(\sigma_0, \mu_0)$ to $(\sigma\_m, \mu\_m)$. What is the other execution? Is it not just a safety property?}



 % (\lbbar p \rbbar_{M} \vdash_{\mathnormal{C}_{ct}} \mathnormal{D}_{ct}) \iff \\
 %      \forall \sigma_0, \sigma_m. \forall \mu_0, \mu_m. \forall i.
 %      (\langle \sigma_0, \mu_0 \rangle \Downarrow_M^p \langle \sigma_m, \mu_m \rangle  \land i \in \mu_m) \\
 %      \implies ((i.op0 \in \mathnormal{C}_{ct}) \rightarrow \pi(\mu_m(src(i.op0))) = \textsc{l}~ \\ 
 %      \land~(i.op1 \in \mathnormal{C}_{ct}) \rightarrow \pi(\mu_m(src(i.op1))) = \textsc{l})
      
% \artem{(I know this will be getting more attention soon, so this might be premature, but) two things stand out to me:
% (1) is that I am curious what math object $\mathnormal{C}_{ct}$ is, and
% (2) is that I guess the idea is to assert that $\pi(\mu_m(i.argN))$ remain low under certain conditions. Is it obvious that it then implies $\pi(\textrm{arch part of the state at m-th step})$ is all low?}



% We write $\lbbar p \rbbar_{M} \vdash_\mathnormal{C} \mathnormal{D}$ to denote that $\mathnormal{D}$ parameterized by $\mathnormal{C}$ holds for all executions of $p$ on $M$.


% As an example, consider the constant-time defense $\mathnormal{D}_{CT}$~\cite{..}. We say that $\lbbar p \rbbar_{M} \vdash_{LC_T} \mathnormal{D}_{CT}$ iff $p$ never passes a secret to the unsafe operand of a transmitter, as defined in $LC_T$, in any execution on $M$.
% \chris{not clear how "passed to a transmitter" is represented.}
% % from any initial state $\langle \sigma, \mu \rangle$.
% The constant-time defense enforces $(\lbbar p \rbbar_{M} \vdash_{LC_T} \mathnormal{D}_{CT}) \rightarrow \mathrm{Eq.~\ref{eq:non-interference}}$.\footnote{Orthogonal to our work, $\mathnormal{D}_{CT}$ may be constructed differently depending on the degree to which $M$ may execute transiently~\cite{guarnieri:contracts,cauligi:sok-spectre-sw-defense,serberus:mosier:2024}.}

% With respect to the orange colored text, Eq.~\ref{eq:non-interference} is a more precise definition of hardware side-channel than appears in recent related work~\cite{guarnieri:contracts, others}.


% , when \R's observations can be solely attributed to microarchitectural state.

% Consider a program $p_{\mathtt{ADD}}$ which contains a single instruction, $\mathtt{ADD, r3, r1, r2}$, which sums the contents of $\mathtt{r1}$ and $\mathtt{r2}$ and writes the result to $\mathtt{r3}$ (where $\mathtt{r1}, \mathtt{r2}, \mathtt{r3} \in reg$).
% Suppose we want to determine if $p$ is hardware side-channel safe on the same CVA6 CPU variant from \S\ref{sec:intro:this-paper:spec-challenge} with respect to receiver $\mathnormal{R}_C$ (\S\ref{sec:background:observer-model}). Consider a pair of initial architectural states, $\sigma$ and $\sigma'$, where the $\mathtt{ADD}$'s two register operands are \textsc{h}-labeled and thus may take on different values (e.g., $\sigma(\mathtt{r1}) = 5$, $\sigma(\mathtt{r2}) = 2$, $\sigma'(\mathtt{r1}) = 7$, $\sigma'(\mathtt{r2}) = 3$).
% Consider also a pair of initial microarchitectural states, $\mu$ and $\mu'$, which feature in-flight $\mathtt{MUL}$s that have just reached the $\mathtt{mulUnit.mul(first)}$ execution phase. 
% Suppose that 

% In $\mu$, the $\mathtt{MUL}$ features a zero operands; in $\mu'$ both operands are non-zero. 

% Intuitively, Eq.~\ref{eq:non-interference} defines a program $p$ as safe with respect to $mathnormal{R}$ when it runs on $\uarch$ as long as any pair of executions




% that $p$'s execution on $M$ can create a pair of distinct observation traces for \R can can be directly attributed to $p$'s operands.

% Without leakage contract 
% O(uarch(P(p, s), u)) != O(uarch(P(p, s’), u’))
% Cache hit/ miss

% \chris{I suggest we split this into 2 sections:
% % - Section 2: Execution semantics
% % - New Section 3: Security definition
%  %And consolidate the new OD-style property 1 / subsequent new definitions to the new Section 3.
% % \\
% For this new Section 3, we can frame it like this:
% - Verifying the absence of side channels is done through hyper-properties.  We propose a new hyper-property, inspired by OD, that more precisely captures the desired absence of H-dependent uarch leakage.
% - Hyper-properties are difficult to check, so contracts/defenses instead are described as trace properties.  Frame Definition II.2 $\mathnormal{C}$ as a trace property.
% - Our contribution: More precise trace properties for contract construction.  Show a concrete example of a safe trace disallowed by LC\_T and allowed by LC\_P.
% }


% \textbf{Selecting an Observer Model  ($\mathnormal{O_R}$)}
% \label{sec:background:observer-model}
% Consider an omniscient receiver $\mathnormal{R}_O$ that observes the entire processor state at every step of an execution trace, i.e.,  $\mathnormal{O}_{\mathnormal{R}_O}(\langle \sigma, \mu \rangle) = \langle \sigma, \mu \rangle$. For $\mathnormal{R}_O$, Eq.~\ref{eq:non-interference} is trivially invalid for all microarchitecture.
% \caroline{Assumes not computing on encrypted data.}
% In practice, receivers are less powerful than this. 


% on $M$ as a function.


% \caroline{Industrial observer models assume that channel modulations manifest as execution latency variability for
% committed instructions or instruction sequences.
% Hence, an instruction's safe operand(s) are guaranteed to not impact the \textit{execution time} (in cycles) of any in-flight instruction including themselves~\cite{arm:dit,intel:doit,riscv_zkt}.}
% instructions/programs.
% additionally capturing a receiver that perceives channel modulations through hardware resource contention for example.

% O is value of uFSM state variables - a handful of state elements in the design which are sufficient for understanding an instruction’s execution progress / phase. We adopt a more precise notion of how channel modulations are observable - via upath variability. Allows us to capture transmitters beyond those which create operand dependent timing variability. Because our observer sees a superset of microarchitectural state of the commit based observer, we’ll find all of the same transmit instructions.



% With ct contract on program
% O(uarch(P(p, s), u)) = O(uarch(P(p, s’), u’))
% For seq processor

% O(uarch(P(p, s), u)) != O(uarch(P(p, s’), u’))
% For spec processor, because misprediction can supply two different secrets to loads

% With sct contract on software and Serberus hardware restrictions
% O(uarch(P(p, s), u)) = O(uarch(P(p, s’), u’))

% All of the above are for O = commit times

% We’re interpreting O as execution paths which is a superset of commit times

% Leave tries to fine a set of instructions for which the above holds if the classify them / their operand as transmitters

% We find a strictly richer contract
% More nuanced definition contact satisfaction for the program execution on the microarch

% Uspec says internal control signals are observable via impact on time - not totally accurate 

% Contract satisfaction involves cooperation between hardware and software

% Secrets never reach transmitters can be satisfied by the program for seq processors but requires hardware/software cooperation at min for speculative processors 

% Maybe the contract is what’s supplied to software and what we’re talking about is a defense enabled by a contract Defense involves hardware and software. Facilitated by the contract which supplies relevant hardware semantics to software.


% So far, we've decribed the basic mechanics of a hrdware side-channel attack. 
% Our most significant contributions in this paper are tspec models for exposing the cricumstances under which transmitters leak their oeprands to programmers and hardware designser and the tsynth approach and tool for tspec model (and state-of-the-art leakage contract0 veirifcation.
% In this section, we now provide some brief formal notion to more precsiely compare tspec models with state-of-the-art leakage contracts and tsynth with state-of-the-art contract verification approaches.






% \textbf{Formalizing Hardware Side-Channel Defenses}
% \label{sec:background:leakage-contracts}
% M% ost microarchitecture does not enforce Eq.~\ref{eq:non-interference} for a realistic receiver like $\mathnormal{R}_C$ or $\mathnormal{R}_{\upath{}}$, e.g., due to operand-dependent optimizations that create fast and slow paths for many instructions~\cite{arm:dit,intel:doit,riscv_zkt,pandora:isca:21}.
% Thus, hardware side-channel defenses elicit cooperation from hardware and software.
% to enforce Eq.~\ref{eq:non-interference}.
% , facilitated by a hardware-software contract.
% Typically, hardware enforces Eq.~\ref{eq:non-interference} for a subset of \textit{safe} execution traces and software emits code that is guaranteed to generate one of these safe traces.
% This coordination is facilitated by a hardware-software contract. 


% \yao{Dumb question: Is this $D_{CT}$ a sequential constant-time defence? Because only $p$ not passing secret is a sequential constant time but if the $uarch$ is speculative, the property does not automatically holds?}


% \textbf{Our work} enables hardware and software designers to explore new \textit{conditional} constant-time defenses enabled by transponder-centric leakage contracts $LC_P$. Consider such a defense $\mathnormal{D}_{CT_C}$, where $\lbbar p \rbbar_{M} \vdash_{LC_T} \mathnormal{D}_{CT_C}$ iff $p$ never passes a secret to the unsafe operand of a transmitter \textit{whenever leakage conditions are met} in any execution on $M$. Similarly, $(\lbbar p \rbbar_{M} \vdash_{LC_P} \mathnormal{D}_{CT_C}) \rightarrow \mathrm{Eq.~\ref{eq:non-interference}}$.
% Note that for the same microarchitecture $M$, $\mathnormal{D}_{{CT}_C}$ parameterized by $LC_P$ admits a superset of execution traces for a program $p$ compared to $\mathnormal{D}_{CT}$ parameterized by $LC_T$.



% In doing so, we implicitly verify $LC_T$-style (transmitter-centric) leakage contracts with respect to receivers $\mathnormal{R}_C$ and $\mathnormal{R}_{\mu path}$.
 
% However, $\mathnormal{D}_{CT}$ (parameterized by $LC_P$) 
% has some advantages over
% $\mathnormal{D}_{CT_C}$ (parameterized by $LC_T$). 
% Compared to $LC_T$, $LC_P$ has the benefit that permits more programs and/or microarchitectures. It also enables new defenses based on selectively flushing microarchitectural state or controlling scheduling decisions.

% \newcommand{\cmark}{\ding{51}}
% \textbf{Threat Model Summary}
% % \begin{table}[]
% %     \centering 
% %     \begin{tabular}{|c|c|c|}\hline
% %          & $LC_T$ & $LC_P$ \\ \hline
% %         $\mathnormal{R}_C$ & \cmark & \cmark\\ \hline
% %         $\mathnormal{R}_{\mu \mathtt{path}}$ & \cmark & \cellcolor{Gray}\cmark \\ \hline
% %     \end{tabular}
% %     \caption{\caroline{Breifly mention that \tsynth{}'s focus is synthesizing $LC_P$ contracts for the $\mathnormal{R}_{\mu \mathtt{path}}$ receiver, but that in doing so it also synthesizes the other three contract flavors.}\yao{I agree we need to mention your comment($\leftarrow$), but I'm not sure I get the table...it seemed it can be put in main text? without taking another space?}}
% %     \label{tab:my_label}
% % \end{table}

% We highlight three key distinct features of our threat model compared to prior work. First, 
% Eq.~\ref{eq:non-interference} features a more precise definition of side-channel safety; prior work omits the orange text~\cite{guarnieri:contracts, others}.
% We find that the orange text is required to avoid \textit{mis-classifying} a safe program $p$ running on microarchitecture $M$ as \textit{unsafe} with respect to receiver \R.
% % Prior work presents an imprecise definition of hardware side-channel safety that restricts
% % Eq.~\ref{eq:non-interference} to just the black text~\cite{guarnieri:contracts, others}.
% % gives a more precise definition of hardware side-channel safety than prior work~\cite{guarnieri:contracts, others}, which restricts our definition to just the black text. 
% Second, we assume a more powerful receiver $\mathnormal{R}_{\mu \textsc{path}}$
% that can perceive
% channel modulations through means other than execution time.
% Third, we design and automatically synthesize (from RTL) leakage contracts that support conditional constant-time defenses. 
% % capturing a receiver that perceives channel modulations through means other than execution time.

% Our observer function assumes that instruction execution paths are observable to a receiver. For a transmitter-centric contract, we’d need to find the instructions that can create path variability as a function of their operands. For our transponder-centric contract, we also want to expose the conditions under which this can happen.




% \caroline{Prior work presents an imprecise definition of hardware side-channel safety that restricts
% Eq.~\ref{eq:non-interference} to just the black text~\cite{guarnieri:contracts, others}.
% % gives a more precise definition of hardware side-channel safety than prior work~\cite{guarnieri:contracts, others}, which restricts our definition to just the black text. 
% We find that the orange text is required to avoid \textit{mis-classifying} a safe program $p$ running on microarchitecture $M$ as \textit{unsafe} with respect to receiver \R.}

% \yao{
% We say that a program p is not susceptible to hardware side-channel attack with respect to a receiver R when p runs on a uarch iff the observation traces of running p from two differing $\mu, \mu'$ states with different $\sigma, \sigma'$ should either yield the same trace or \textit{can not be} attributed to the secret data in the $\sigma$.
% Naturally, receiver may have distinct observation because of differing $\mu$: the $\mu$ and $\mu'$ is processing a MUL with different public value and is at source of path divergence \mymath{mulUnit.mul(first)} when we run program p consisting of an ADD that process secret and commit at different time point due to modulation from in-flight MUL. 
% The distinct observation in this case is a result of differing uarch but not a result of the secret value supplied to ADD. \\
% %
% Thus. w.r.t a receiver, the side-channel free program execution on uarch requires that if same p yield two identical traces running from any $\mu, \mu'$ (to isolate out the influence of uarch state) then two differing $sigma/sigma'$ running from $mu/mu'$ should yield the same observation trace  %
% %
% % \uarch{} can have  instead of differing secret value in $\sigma$s. 
% % Prior interference: A program p is not susceptible to hw side-channel attack w.r.t a receiver R when P runs on uarch iff for any two arch. states differing in some secret value, the receiver observation of running P from the ``same uarch state'' on the uarch should be the same in regardless of secret.  \\ 
% % However, following the example of zero-skip MUL, this constrain the uarch from even ever processing secret, as it will violates the ``same uarch'' when it is in-flight.  
% %This restricts one from using MUL processing secret since it wil violates the ``same uarch''.  (i.e. a restriction on the program that can be run on uarch)
% % To have a more relax program that are eligibal to run MUL and have two uarch potentially diverging with a multiplicastion already in flight but still able to issue ADD without leaking the secret
% The key takeaway: ... \\
% Selecting an Observer Model: ... \\ 
% Our work assumes 
% }
% %A defense is  property of a program running on a microarchitecture. 

% % Hardware side-channel defenses aim to restore Eq.~\ref{eq:non-interference} for a realistic receiver, when the microarchitecture cannot enforce it by default.
% % They require some cooperation between hardware and software.

% % For example, with industrial leakage contracts, hardware promises that Eq.~\ref{eq:non-interference} will be valid as long as secret data. Given such a transmitter-centric leakage contract $LC_T$, a program $p$ that is written according to the constant-time programming discipline (i.e., $p \vDash_{LC_T} CT$) can enforce  Eq.~\ref{eq:non-interference} for all \textit{sequential} processors.
% % Enforcing Eq.~\ref{eq:non-interference} for \textit{speculative} processors requires additional hardware and software coordination~\cite{} with respect to the same style of leakage contract.
 
% % \begin{equation}
% % \label{eq:non-interference-seq}
% % \begin{split}
% %       \forall \sigma, \sigma'. \forall \mu, \mu'. \sigma \approx_{\pi} \sigma' \land \\
% %       \mathnormal{R}(\lbbar p_{ct} \rbbar_{seq}^{\langle \sigma, \mu \rangle}) = \mathnormal{R}(\lbbar p_{ct} \rbbar_{seq}^{\langle\sigma, \mu'\rangle}) \rightarrow \\
% %       \mathnormal{R}(\lbbar p_{ct} \rbbar_{seq}^{\langle\sigma, \mu\rangle}) = \mathnormal{R}(\lbbar p_{ct} \rbbar_{seq}^{\langle\sigma', \mu'\rangle})
% % \end{split}
% % \end{equation}

% % Note that Eq.~\ref{eq:non-interference-seq} considers executions on a \textit{sequential} microarchitecture $seq$ that is free from transient execution. If $seq$ is replaced with a microarchitecture $spec$ that features transient execution, Eq.~\ref{eq:non-interference-seq} can again be trivially violated. In particular, constant-time programming prevents secrets from reaching transmit instruction operands during \textit{sequential execution only} but not not transient execution.

% % Mitigating transient execution attacks typically requires additional cooperation from hardware. This is because it is impractical to reason about unconstrained speculative control- and data-flow in software...


% % A For example, recent work enforces the following for a \textit{speculative constant-time}  program $p_{sct}$, a slight strengthening of a constant-time program:
% % \begin{equation}
% % \label{eq:non-interference-sct}
% % \begin{split}
% %       \forall \sigma, \sigma'. \forall \mu, \mu'. \sigma \approx_{\pi} \sigma' \land \\
% %       \mathnormal{R}(\lbbar p_{sct} \rbbar_{asp}^{\langle \sigma, \mu \rangle}) = \mathnormal{R}(\lbbar p_{sct} \rbbar_{asp}^{\langle\sigma, \mu'\rangle}) \rightarrow \\
% %       \mathnormal{R}(\lbbar p_{sct} \rbbar_{asp}^{\langle\sigma, \mu\rangle}) = \mathnormal{R}(\lbbar p_{ct} \rbbar_{asp}^{\langle\sigma', \mu'\rangle})
% % \end{split}
% % \end{equation}


% % Recent work can enforce Eq.~\ref{eq:non-interference-seq} if $p_{ct}$ is replaced with $p_{sct}$ and the microarchitecture offers particular features for constraining speculative control 


% % $\lbbar p \rbbar_{seq}^{ct}(\sigma, \mu)$ returns the hardware trace obtained from running program $p$ on a microarchitecture with a sequential execution semantics ($seq$) under the constant-time programming defense.



% % \textbf{Refining and Verifying Receiver Assumptions}
% % \label{sec:background:receiver}
% % With microarchitects deploying increasingly exotic, data-dependent hardware optimizations to harvest any available performance in a post-Moore era, we observe that transmitter-centric leakage contracts face a critical challenge.
% % In particular, a receiver $\mathnormal{R_A}(\langle \sigma, \mu \rangle) = \sigma$ that observes all architectural state is becoming increasingly realistic. In the worst case, we cannot enforce Eq.~\ref{eq:non-interference}. In the best case, enforcing Eq.~\ref{eq:non-interference}. will come at a significant performance cost.

% % In this paper, we:
% % \begin{itemize}
% %  \item Consider a more powerful receiver $\mathnormal{R_{P}}(\langle \sigma, \mu \rangle) = \mu(\mu FSMs)$. At each time step the receiver can observe the \ufsms{} in the design. \caroline{Could also say that the receiver can see execution paths, but this is trickier to map onto a trace.}
% %  \item Propose that programs satisfy transponder-centric leakage contracts in order to defend against hardware side-channel attacks. That is, $p \vDash_{LC_P} CT$, where $LC_P$ is a transponder-centric leakage contract.
% %  \item Propose an approach to synthesize $\mathnormal{R_{P}}$ from a microarchitecture. In doing so, we verify other realistic receivers, like  $\mathnormal{R_{C}}$ which is the focus of prior work and industry contracts
% % \end{itemize}

% % We also propose that programmers enforce a transponder centric contract that permit secrets to be passed to transmitters in some circumstances. 
% % that can observe the microarchitectural execution paths of all in-flight instructions at each time


% % In general, we lack scalable and automated approaches for formally verifying microarchitectural adherence to \leakagecontracts{}~\cite{arm:dit,intel:doit,riscv_zkt}---\textit{the verification challenge}.
% % A few \textit{contract satisfaction} methodologies have been proposed~\cite{gleissenthall:iodine, gleissenthall:xenon, guaniere:leave, upec-dit-v2}, where a circuit's adherence to a \leakagecontract{} is formally proven or refuted. However, these schemes either target \textit{signal-centric} \leakagecontracts{}~\cite{gleissenthall:iodine,gleissenthall:xenon}, which are too coarse-grained to support CT code, or require significant \textit{manual effort and designer knowledge} to formulate inductive invariants, inspect (possibly spurious) counterexamples, and generally guide the proof effort~\cite{guaniere:leave, deutschmann:upec-do, upec-dit-v2}.

% % Prior work which aims to verify microarchitectural satisfaction of transmitter-centric leakage contracts considers $\mathnormal{A}=\{commit_0, commit_1, ...\}$~\cite{leave} or $\mathnormal{A}=\{ctrl_0, ctrl_1, ...\}$~\cite{deutschmann:upec-do,upecv2}. The contract synthesis approach we present in this paper considers $\mathnormal{A}=\{\upath_0, \upath_1, ...\}$---a trace of execution paths for every fetched instruction, ordered by fetch order. Execution paths can be used to derive contracts from prior work.

% \begin{itemize}
%     % \item Non-Interference \label{sec:background:non-interference}
%     \item Leakage Contracts \label{sec:background:leakage-contracts}
%     \item Hardware Side-Channel Defenses \label{sec:background:defense}
% \end{itemize}

\subsubsection{Other Security Definitions} \caroline{Agree - this subsubsection can move to the appendix.}
\label{sec:background:sec-def:imprecise}
Some prior definitions of hardware side-channel safety omit $\mu$ in Eq.~\ref{eq:non-interference}, leaving the initial microarchitectural states for pairs of traces compared by the consequent implicitly unconstrained~\cite{deutschmann:upec-do, deutschmann2023scalable, gleissenthall:iodine, gleissenthall:xenon}.
%\yao{removed from previous and add to next \cite{guarnieri:contracts}}
% do not explicitly require the pairs of compared traces in Eq.\rsout{~\ref{eq:non-interference}}\yao{~\ref{def:hw-sc-safety}} to be run from the \textit{same} initial microarchitectural states, i.e., \rsout{the red text}\yao{$\mu_0$} is omitted~\cite{guarnieri:contracts, deutschmann:upec-do, deutschmann2023scalable, gleissenthall:iodine, gleissenthall:xenon}.
% \chris{people may get confused here because low equivalence is well known.  should we say prior work doesn't say anything about uarch state? (just arch state)}
% \yao{I think the text above already indicates that prior work doesn't say anything about "uarch"(?).}
% work omits details of the initial microarchitectural state (the red text in Eq.~\ref{eq:non-interference}) when \textit{defining} hardware side-channel safety~\cite{guarnieri:contracts, gleissenthall:iodine, gleissenthall:xenon, deutschmann:upec-do, deutschmann2023scalable}.
However, like prior work~\cite{guarnieri:contracts, wang2023specification}, we observe that constraining these traces' initial microarchitectural states (e.g., to be equivalent)\footnote{Eq.~\ref{eq:non-interference} must constrain the initial microarchitectural states in both traces to be \textit{non-interfering w.r.t. $p$ and $\pi$}. Any $\mu$ and $\mu'$ for which $\mathnormal{O_R}(\lbbar p \rbbar_{\mathnormal{M}}^{\langle \sigma, \mu \rangle}) = \mathnormal{O_R}(\lbbar p \rbbar_{\mathnormal{M}}^{\langle\sigma, \mu'\rangle})$ holds in the antecedent of Eq.~\ref{eq:non-interference} suffices,
% to prove hardware side-channel safety of $p$,
% evaluates to true form an equivalence class of microarchitectural states which are \textit{non-interfering w.r.t. $p$}. Any such pair is sufficient
% to prove hardware side-channel safety of $p$, 
but we select $\mu = \mu'$ for simplicity.} is required to prevent Eq.~\ref{eq:non-interference} from \textit{mis-classifying} a safe program $p$ running on microarchitecture \M{} as \textit{unsafe} with respect to security policy $\pi$ and receiver \R{}.
\yao{We provide example and detailed discussion for interested reader in an online appendix (\S\ref{TODO}). }
\yao{TODO refer to appendix for the example}. 
\yao{\textless{}\textless{}\textless{}}
% \yao{HW-SW contract~\cite{guarnieri:contracts} does leave uarch unconstrained. But in this paragraph we want to cite LEAVE though. LEAVE requires initial uarch to be the same as precondition for ''contract satisfaction'', which in our framework boils down to side-channel free though, without mentioning why. 
%%Prior definitions of hardware side-channel safety omit $\mu$ in Eq.~\ref{eq:non-interference}, leaving the initial microarchitectural states for pairs of traces compared by the consequent implicitly unconstrained~\cite{guarnieri:contracts, deutschmann:upec-do, deutschmann2023scalable, gleissenthall:iodine, gleissenthall:xenon}.
%%Prior definitions of hardware side-channel safety either omit $\mu$ in Eq.~\ref{eq:non-interference} and left the initial microarchitectural states for pairs of traces compared by the consequent implicitly unconstrained~\cite{deutschmann:upec-do, deutschmann2023scalable, gleissenthall:iodine, gleissenthall:xenon}.
% }
% this imprecision when verifying hardware side-channel safety~\cite{gleissenthall:iodine, gleissenthall:xenon}.


\subsection{Overview and Running Example}
\label{sec:tspec:upaths}
% \chris{add to section title: "...and overview"?}
% Defining a \pct{} contract \tspecC{} requires defining leakage conditions $c$ for transmitters' unsafe operands. As alluded above, 
Observe that \ct{} contracts are a class of \pct{} contracts where {$c = true$} for all $(I, op, {c}) \in \mathnormal{C}_{pct}^{\mathnormal{M}, \mathnormal{R}}$.
However, we seek \pct{} contracts with more precise leakage conditions that permit transmitters to process secrets safely whenever possible.
% \yao{Possibly above can be remove and replace with "Allude above, \ctC{} is a class of \tspec{} that has all $c = true$. However, we seek \pct{} contracts with more precise (i.e., minimal) leakage conditions that permit transmitters to process secrets safely as often as possible." merged with next paragraph?}
Formulating precise leakage conditions requires characterizing how channel modulations ultimately manifest as receiver observations. A core contribution of this paper is devising such a characterization based on a \textit{microarchitectural execution path} (\upath{}) abstraction, inspired by prior work~\cite{pipecheck, ccicheck, coatcheck, rtlcheck, checkmate, rtl2uspec:hsiao:2021}, that encodes an instruction's hardware resource usage (restricted to state elements) when it executes.
% Towards this goal, we leverage a \textit{microarchitectural execution path} (\upath{}) abstraction inspired by prior work~\cite{pipecheck, ccicheck, coatcheck, rtlcheck, checkmate, rtl2uspec:hsiao:2021} to help us define a receiver's perception of channel modulations. 
% Before presenting \upaths{}, we introduce a running example, which we will use to build intuition in this and later sections.

\subsubsection{\upaths{} by Example}
\label{sec:tspec:upaths:op-packing}
We first introduce a running example to build intuition for \upaths{} and related concepts.
% \begin{figure}[t!]
%     \centering
%      \includegraphics[width=0.95\linewidth]{figs/paths_3_9_2.png}
%      \caption{Left: \inst{ADD} \upaths{} on CVA6-OP (\S\ref{sec:tspec:upaths}). 
%      Right: A sample of synthesized \upaths{} (\S\ref{sec:results}) on CVA6 with respect core (for \inst{BEQ}, \inst{LD}) and data cache (for \inst{ST}). 
%      Row\textsubscript{\inst{f}}: PL (\inst{f}:final). \inst{n} in a node: First to \inst{n}-th consecutive visit. 
%      %Row($f$/$l$): PL (first up to \inst{n}-th/last consecutive visit; \inst{n}: \# in a node)
%      % \rsout{Row(\textsubscript{n}):  %PL (\S\ref{sec:tspec:pls}) 
%      % an exec. phase 
%      % ($\mathsf{n}$: \# in a node, one up to n-th consecutive revisit).} %. OP: Operand-packing. % extension. % t=67/68 for original/operand-packing extended CVA6 
%      %Paths for \inst{ADD} are potential paths running on CVA6 augmented with operand-packing based on the synthesized paths:  ID1 is additional decode slot to enable multi-issue. Row(F/L): an exec. phase (first/last consecutive visit)
%      %\yao{edge label, n; }
%      % A sample of synthesized \upaths{} on CVA6 with respect to data cache (for \inst{SW}) and core (for \inst{BEQ}, \inst{LW}, \inst{ADD}).
%      % % Row(F/L): an exec. phase (first/last consecutive visit). 
%      %\chris{sentence to define the yellow/green node coloring.}
%      Yellow/green nodes: decision source/destination PLs (\S\ref{sec:tspec:transponders}).
%      }
%      \label{fig:upaths-example}

% \end{figure}



% \begin{figure}[t!]
% %        \captionsetup[subfigure]{aboveskip=-4pt,belowskip=1pt}
% %            \begin{subfigure}{1.0\linewidth} 
% %            \centering
% %            \begin{tcolorbox}[left=0pt,right=0pt,top=2pt,bottom=2pt]
% %            \footnotesize
% %            \noindent\textcolor{ForestGreen}{{\RaggedLeft// \textbf{Operand packing~\cite{brooks:operand-packing}:} \inst{ADD_I} in \inst{ID} is issued if it is ready to be issued or eligible for operand packing; otherwise it is stalled. %$\mathsf{msb}$: Most significant bit.
% %            %    %\inst{ADD_I} in \inst{ID} gets issued if it is the only instruction in ID queue or eligible to be packed with another dynamic \inst{ADD_D}, else it is stalled and moved to head of ID queue.
% %                }}\\
% %            \noindent\hlt{$\mathsf{dst\;ADD\_ID(ADD_I\;i0,\;ADD_D\;i1)}$}$\mathsf{\;:}$ \newline
% %            \indent$\;\;\mathsf{path\_id= (PO(i0, i1)\;\vee (visit(i1, ID) \;\wedge\; PO(i1, i0)\;\wedge}$\newline 
% %            \indent$\;\;\;\;\mathsf{(\forall arg \in \{}$\hlt{$\mathsf{i0.\iparg{arg0}, i0.\iparg{arg1}, i1.\itarg{arg0}, i1.\itarg{arg1}}$}$\mathsf{\}, msb(arg) < 32)))}$\newline
% %            \indent$\;\;\mathsf{\textcolor{blue}{return}\;ite(path\_id, }$\hlt{$\mathsf{\{scbIss, issue\}, \{ID\}}$}$\mathsf{)}$
% %            \end{tcolorbox} 
% %             \caption{Leakage function for operand packing on CVA6-OP (\S\ref{sec:tspec:upaths:op-packing})}
% %             \label{fig:op-f-leak}
% %        \end{subfigure}%
% %        \\[1pt] 
% %            \begin{subfigure}{1.0\linewidth} 
% %            \centering
%     \begin{tcolorbox}[left=0pt,right=0pt,top=2pt,bottom=2pt]
%     %\begin{framed}
%     \footnotesize
%     %\noindent\textcolor{ForestGreen}{{\RaggedLeft// \textbf{\inst{SW} in CVA6}: \inst{SW} updates non-write-allocate 4-way set-associative cache if there exists a prior \inst{LD} whose address overlaps. Data are stored in two-parallel banks.}}\\
%     %: LD in `LdUnit' phase taking path 0 for cache miss or path 1-4 for cache-read paths of corresponding data banks. Assume each way is in a separate bank and a write-no-allocate 4-way set associative cache)}}\\
%     %\noindent\textcolor{ForestGreen}{{\RaggedLeft// Precondition}}\\
%         \noindent\textcolor{ForestGreen}{{\RaggedLeft// \textbf{Operand packing~\cite{brooks:operand-packing}:} \inst{ADD_I} in \inst{ID} is issued if it is ready to be issued or eligible for operand packing; otherwise it is stalled. %$\mathsf{msb}$: Most significant bit.
%         %\inst{ADD_I} in \inst{ID} gets issued if it is the only instruction in ID queue or eligible to be packed with another dynamic \inst{ADD_D}, else it is stalled and moved to head of ID queue.
%         }}\\
%     \noindent\hlt{$\mathsf{dst\;ADD\_ID(ADD_I\;i0,\;ADD_D\;i1)}$}$\mathsf{\;:}$ \newline
%     \indent$\;\;\mathsf{path\_id= (PO(i0, i1)\;\vee (visit(i1, ID) \;\wedge\; PO(i1, i0)\;\wedge}$\newline 
%     \indent$\;\;\;\;\mathsf{(\forall arg \in \{}$\hlt{$\mathsf{i0.\iparg{arg0}, i0.\iparg{arg1}, i1.\itarg{arg0}, i1.\itarg{arg1}}$}$\mathsf{\}, msb(arg) < 32)))}$\newline
%     \indent$\;\;\mathsf{\textcolor{blue}{return}\;ite(path\_id, }$\hlt{$\mathsf{\{scbIss, issue\}, \{ID\}}$}$\mathsf{)}$
%     \\[5pt]
%      % 
%     % {
%     %   %\renewcommand{\arraystretch}{1.3}
%     %\setlength{\arrayrulewidth}{1pt}
%     % \begin{tabular}[t]{
%     %   @{}>{\raggedright\arraybackslash} m{0.98\linewidth}
%     %  }
% %      \textcolor{ForestGreen}{{\RaggedLeft// \textbf{Register-file 0/1 compression~\cite{balakrishnan2003exploiting}}: \inst{ADD} in \inst{rename} stalls if no valid physical register or moves to \inst{issue} if available physical register.}}\\
% %      % free\_pool[idx] indicates if PRF[idx] is available for rename. ADD can substituted with any register-writing instruction. 
% %      %Any register-writing instruction can be a transmitter, but for illustration simplicity, we choose ADD as example
% %      %}}\\
% %     %\hline \\[-8pt]
% %     \noindent\hlt{$\mathsf{dst\;ADD\_rename(AND_S\;i1)}$}$\;\mathsf{:}$ \newline
% %     %\indent$\;\;\mathsf{path\_id = (\vee_i\;free\_pool[i] == 1)}$\\
% %     \indent$\;\;\mathsf{\textcolor{blue}{return}\;ite(((free\_pool[i1.PRF\_idx] == ite((}$\hlt{$\mathsf{i1.\itarg{arg0}}$}$\mathsf{ + }$\hlt{$\mathsf{i1.\itarg{arg1}}$}$\mathsf{) \le 1, }$\\[2pt]
% %     \indent$\;\;\;\;\mathsf{1, 0))\wedge\;\vee_{idx}\;free\_pool[idx] == 1), }$\hlt{$\mathsf{\{issue\}, \{rename\}}$}$\mathsf{)}$
% %     %   \end{tabular}
% %     %   } 
% %       \\[5pt]
% %       \noindent\textcolor{ForestGreen}{{\RaggedLeft// \textbf{Silent-store~\cite{silentstore,lepak2000value}:} %\inst{rdata} is returned by \inst{ST}'s earlier \inst{SS\hbox{-}load} micro-op. 
% %     \inst{ST} in \inst{SQCHit} completes silently on a match of \inst{rdata} returned by \inst{ST}'s earlier \inst{SS\hbox{-}load} micro-op. }}\\
% %     % at SQCacheHit cycle, ST is reading value in the cache
% % %{
% % %      % \renewcommand{\arraystretch}{1.3}
% % %    \setlength{\arrayrulewidth}{1pt}
% % %     \begin{tabular}[t]{
% % %       @{}>{\raggedright\arraybackslash} m{0.95\linewidth}
% % %       }
% %     %\noindent\textcolor{ForestGreen}{\RaggedLeft// Precondition}\newline
% % %    $\mathsf{Mem[}$\hlt{$\mathsf{i1.\itarg{addr}}$}$\mathsf{] ==\; }$\hlt{$\mathsf{i1.\itarg{data}}$}$\mathsf{\;\;cache[}$\hlt{$\mathsf{i0.\iparg{addr}}$}$\mathsf{] == Mem[}$\hlt{$\mathsf{i1.\itarg{addr}}$}$\mathsf{]}$$\mathsf{\;\;\;}$\\[2pt]
% % %     \hline \\[-8pt]
% %     \noindent\hlt{$\mathsf{dst\;ST\_SQCHit(ST_I\;i0, ST_S\;i1)}$}$\mathsf{\;:}$ \newline
% %     \indent$\;\;\mathsf{SS\_ld = (Mem[}$\hlt{$\mathsf{i1.\itarg{addr}}$}$\mathsf{] ==\; }$\hlt{$\mathsf{i1.\itarg{data}}$}$\mathsf{\;\wedge\;rdata == }$$\mathsf{\;\;cache[}$\hlt{$\mathsf{i0.\iparg{addr}}$}$\mathsf{])}$ \newline 
% % %    \hlt{$\mathsf{i0.\iparg{addr}}$}$\mathsf{\;==\; }$\hlt{$\mathsf{i1.\itarg{addr}}$}$\mathsf{\;\wedge \;}$\hlt{$\mathsf{i0.\iparg{data}}$}$\mathsf{\;== cache[}$\hlt{$\mathsf{i0.\iparg{addr}}$}$\mathsf{]}$\newline
% %     \indent$\;\;\mathsf{path\_id = (}$\hlt{$\mathsf{i0.\iparg{addr}}$}$\mathsf{\;==\; }$\hlt{$\mathsf{i1.\itarg{addr}}$}$\mathsf{\;\wedge \;}$\hlt{$\mathsf{i0.\iparg{data}}$}$\mathsf{\;== rdata)}$\newline
% %     \indent$\;\;\mathsf{\textcolor{blue}{return}\;ite((path\_id == 1), }$\hlt{$\mathsf{\{SQComp\}, \{reqWCache\}}$}$\mathsf{)}$ 
% %     \\ [5pt]
% %       \noindent\textcolor{ForestGreen}{{\RaggedLeft// \textbf{Dynamic inst. reuse~\cite{sodani1997dynamic}}: \inst{FP} in \inst{issue} computes (\inst{FPU}) or not depending on a single-entry reuse table that tracks prior \inst{FP} results.}}\\
% %    {
% %        \renewcommand{\arraystretch}{1.3}
% %     \setlength{\arrayrulewidth}{1pt}
% %      \begin{tabular}[t]{
% %        @{}>{\raggedright\arraybackslash} m{0.95\linewidth}
% %        }
% %     %\noindent\textcolor{ForestGreen}{\RaggedLeft// Precondition}\newline
% % % \\[2pt]
% %  %   \hline
% %         \noindent\hlt{$\mathsf{dst\;FP\_issue(FP_I\;i0, FP_S\;i1)}$}$\;\mathsf{:}$\newline
% %         \indent$\;\;\mathsf{path\_id = (}$$\mathsf{reuse\_buffer == \{}$\hlt{$\mathsf{i1.\itarg{res}}$}$\mathsf{,}$\hlt{$\mathsf{i1.\itarg{arg0}}$}$\mathsf{,}$\hlt{$\mathsf{i1.\itarg{arg1}}$}$\mathsf{,i1.op\}\;\wedge}$
% %         \indent$\;\;\;\;\mathsf{\{}$\hlt{$\mathsf{i0.\iparg{arg0},i0.\iparg{arg1}}$}$\mathsf{,i0.op\}== reuse\_buffer.\{arg0,arg1,op\})}$ \newline
% %     %\indent$\;\;\;\;\mathsf{}$\hlt{$\mathsf{i0.\iparg{arg1}}$}$\mathsf{ == i1.reuse\_buffer.arg1\;\wedge i0.op == reuse\_buffer.op})$ \newline
% %     \indent$\;\;\mathsf{\textcolor{blue}{return}\;ite((path\_id == 1), }$\hlt{$\mathsf{\{ROBComp\}, \{FPUnit\}}$}$\mathsf{)}$ \\
% %        \end{tabular}
% %    } 
% %     \\[5pt]
% %    % 
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
% % %       {
% % %       \renewcommand{\arraystretch}{1.3}
% % %    \setlength{\arrayrulewidth}{1pt}
% % %     \begin{tabular}[t]{
% % %       @{}>{\raggedright\arraybackslash} m{0.96\linewidth}
% % %       }
% % %    \textcolor{ForestGreen}{{\RaggedLeft// \textbf{\inst{DIV} in CVA6}: \inst{DIV} at `scbFin` can be flushed due to a mis-aligned taken-branch that is committing.}} \\ % mis-predict branch. }} \\
% % %    %if there exists a prior \inst{LD} whose address overlaps with its address.
% % %    \centering\arraybackslash$\mathsf{visit(i0, scbFin)\;\;\;(visit(i1, scbExcptn)\vee visit(i1, scbCommit))}$ \\[2pt]
% % %     \hline
% % %    \noindent\hlt{$\mathsf{dst\;DIV\_scbFin(BEQ_D\;i1)}$}$\mathsf{\;:}$ \newline %\textcolor{ForestGreen}{// Leakage function}\newline
% % %        \indent$\;\;\mathsf{flush = (}$\hlt{$\mathsf{i1.\iparg{arg0}}$}$\mathsf{\;==\; }$\hlt{$\mathsf{i1.\itarg{arg1}}$}$\mathsf{\;\wedge\;mis\_aligned(i1.jump\_addr))}$ \newline
% % %        \indent$\;\;\mathsf{\textcolor{blue}{return}\;ite(flush,\;}$\hlt{$\mathsf{\{\}}$}$\mathsf{, ite(headOfScb,}$\hlt{$\mathsf{\{scbCommit\}, \{scbFin\}\}}$}$\mathsf{)}$
% % %    \end{tabular}
% % %    }  \\[3pt]
% % %    {
% % %       \renewcommand{\arraystretch}{1.3}
% % %    \setlength{\arrayrulewidth}{1pt}
% % %     \begin{tabular}[t]{
% % %       @{}>{\raggedright\arraybackslash} m{0.96\linewidth}
% % %       }
%     \noindent\textcolor{ForestGreen}{{\RaggedLeft// \textbf{CVA6 \inst{LD}:} \inst{LD} in \inst{issue} finishes or is stalled depending on whether its address overlaps with a pending speculative or committed \inst{ST}.}}\\
%     \noindent\hlt{$\mathsf{dst\;LD\_issue(LD_I\;i0, ST_D\;i1)}$}$\;\mathsf{:}$ \newline
%     %\textcolor{ForestGreen}{// Leakage function} \newline
%         %\indent$\;\;\mathsf{match=(offset(
%         %}$$\mathsf{) \in offset(comSTB \cup specSTB))}$ \newline
%         \indent$\;\;\mathsf{\textcolor{blue}{return}\;ite((}$\hlt{$\mathsf{i1.\itarg{addr}}$}$\mathsf{\;\in (comSTB \cup specSTB)\;\wedge\;}$ \newline 
%         \indent$\;\;\;\;\mathsf{offset(}$\hlt{$\mathsf{i0.\iparg{addr}}$}$\mathsf{)== offset(}$\hlt{$\mathsf{i1.\itarg{addr}}$}$\mathsf{)),}$\hlt{$\mathsf{\{ldStall, LSQ\}, \{ldFin\}}$}$\mathsf{)}$
%        % 
%     \\[5pt]
%     \textcolor{ForestGreen}{{\RaggedLeft// \textbf{CVA6 \inst{ST} (cache):} A \inst{ST}, on a hit in the 4-way set-assoc. no-write-alloc. cache, will progress to update one of two data banks.}}\\ 
%     \noindent\hlt{$\mathsf{dst\;ST\_wBVld(ST_I\;i0, LD_S\;i1)}$}$\mathsf{\;:}$ \newline %\textcolor{ForestGreen}{// Leakage function}\newline
%         \indent$\;\;\mathsf{hit = (cacheTag[set(}$\hlt{$\mathsf{i1.\itarg{addr}}$}$\mathsf{)][way] == tag(}$\hlt{$\mathsf{i1.\itarg{addr}}$}$\mathsf{)\;\wedge}$\newline 
%         \indent$\;\;\;\;\mathsf{set(}$\hlt{$\mathsf{i0.\iparg{addr}}$}$\mathsf{) == set(}$\hlt{$\mathsf{i1.\itarg{addr}}$}$\mathsf{)\;\wedge\;tag(}$\hlt{$\mathsf{i0.\iparg{addr}}$}$\mathsf{) == tag(}$\hlt{$\mathsf{i1.\itarg{addr}}$}$\mathsf{))}$ \newline
%         \indent$\;\;\mathsf{\textcolor{blue}{return}\;ite(hit, }$\hlt{$\mathsf{\{wRTag, wr\$[way/2]\}, \{wRTag\}}$}$\mathsf{)}$ 
%         \\ [5pt]
%     \textcolor{ForestGreen}{{\RaggedLeft// \textbf{CVA6 \inst{ST} (core)}: \inst{ST} at \inst{comSTB} is stalled from draining to memory if its address offset does not match a younger \inst{LD}}.} \\ % mis-predict branch. }} \\
%     %if there exists a prior \inst{LD} whose address overlaps with its address.
% %    \centering\arraybackslash$\mathsf{visit(i0, comSTB)\;\;\;)}$ \\[2pt]
% %     \hline
%     \noindent\hlt{$\mathsf{dst\;ST\_comSTB(SW_I\;i0, LD_D\;i1)}$}$\mathsf{\;:}$ \newline %\textcolor{ForestGreen}{// Leakage function}\newline
%         \indent$\;\;\mathsf{\textcolor{blue}{return}\;ite((PO(i0, i1)\;\wedge\;offset(}$\hlt{$\mathsf{i0.\iparg{addr}}$}$\mathsf{)\;==\; offset(}$\hlt{$\mathsf{i1.\itarg{addr}}$}$\mathsf{)\;\wedge\;}$\newline
%         %\indent$\;\;\mathsf{\textcolor{blue}{return}\;ite(flush,\;}
%         \indent$\mathsf{\;\;\;\;visit(i1, issue)), }$\hlt{$\mathsf{\{memRq, comSTB\},\{comSTB\}\}}$}$\mathsf{)}$
% %    \end{tabular}
% %    } 
%     \end{tcolorbox}
% %    
% %       \end{subfigure}%
% %
%     \caption{(\hlt{Abstract}) leakage functions for CVA6 (\S\ref{sec:results}) and optimizations in ~\cite{pandora:isca:21}. $\mathsf{I_I/I_D/I_S}$: intrinsic/dynamic/static transmitter.
%     PO: Program order. \inst{ite(c,t,f)}: returns $t$ if $c$ is true or $f$ otherwise. $\mathsf{msb}$: Most significant bit.
%     % \chris{define all the terms: PO, ite, msb, etc.}\yao{fixed}
%     % \chris{I'm not sure this figure is adding much/whether people will read it beyond the ADD\_ID example}
%     }
%     % \yao{added a forward reference to result that discuss the leakage functions}
% %    \caption{(Abstract) leakage function for different instruction at differing phases as defined in a \pct{} contract w.r.t optimizations in pandoras;
% %    $\mathsf{I_P/I_I/I_D/I_S}$ is transponder/intrinsic transmitter/dynamic transmitter/static transmitter respectively. 
% %    }
%     \label{fig:leakage_func_examples}
% \end{figure}

%\input{fig-paths}


Consider an extension to the RISC-V CVA6 CPU~\cite{cva6}
% ---a 64-bit, 6-stage, single-issue RISC-V core featuring speculation and limited out-of-order write-back
(Fig.~\ref{fig:cva6_block_diag}) that we verify in \S\ref{sec:case-study}. The baseline design may fetch up to two compressed instructions per cycle or one uncompressed instruction per cycle, 
but only one instruction can be sent to decode per cycle. The CVA6 variant we consider, called CVA6-OP, is one where the ALU has been modified to support \textit{operand packing}~\cite{brooks:operand-packing,pandora:isca:21} for all operations, and up to \textit{two} instructions can be sent to decode per cycle.
That is, if a pair of (concurrently) decoded instructions perform identical ALU operations \textit{and} feature narrow width operands (32 bits or less), they will be packed into a single operation and executed together.

% \chris{we need some scene setting here to 
% - introduce uarch execution paths notationally (this part is probably best in S2)
% - discuss how we extend them (variable cycles, path selector functions, etc.)}
% \subsubsection{Microarchitectural Execution Paths}
% \label{sec:tspec:upaths-intuition}
% \chris{Is Fig.~\ref{fig:upaths-example} out of date?  (It looks like there is a lot going on besides the add.)}
% \subsubsection{\upaths{} by Example}
% \label{sec:tspec-upaths-by-example}
Fig.~\ref{fig:upaths-example} depicts two distinct (concrete) \upaths{} for an $\mathtt{ADD}$ executing on CVA6-OP---one which can manifest when \inst{ADD}s are packed (left) and the other when they are not packed (right)---using Lamport-style \textit{happens-before graph} notation~\cite{lamport:happensbefore}. 
% We depict \upaths{} as happens-before graphs~\cite{lamport:happensbefore} with labeled nodes.

Each of these two possible \upaths{} is shown as a vertically-oriented DAG (a column) in the figure.
Row labels (ignoring parentheticals)
% A \upath{} is oriented vertically. 
% \chris{Each column denotes a specific possible execution of an instruction.}
% Its column label denotes the instruction that exhibits the \upath{}, and its row labels
denote \textit{performing locations} (PLs, \S\ref{sec:tspec:pls}). % , \S\ref{sec:tspec:pls}).
%\chris{forward ref to III.B.2.}
A node indicates that an instruction \textit{visits} (\S\ref{sec:tspec:receiver-assumptions}) a PL during one cycle of its execution (in some state of an execution trace, \S\ref{sec:background:uarch-semantics}).
When an instruction visits a particular PL, it has the ability to \textit{perform updates} that target (i.e., it has \textit{ownership} of) a particular subset of state elements in the design.
% design states.
% in a given cycle (or state in an execution trace, \S\ref{sec:background:uarch-semantics}).
An instruction may visit multiple PLs in the same cycle, but any PL can be occupied by one instruction at a time.

A key contribution of this paper is to extend the \upath{} abstraction so that it can represent different attacker-distinguishable ways in which a particular instruction can execute.
% that \yao{in which} an instruction with a particular opcode can execute.

First, we provide semantics to express how an instruction can revisit the same PL in multiple (consecutive or non-consecutive) cycles.
% remain in a PL for multiple cycles.
This is needed to represent real designs, e.g., ones where an execution unit has variable execution time.
% In particular, an instruction may revisit a PL multiple times during its execution.
In general, we use row label \inst{PL(n)} to denote the \inst{n}-th visit to \inst{PL}. However, we use a special notation in Fig.~\ref{fig:upaths-example}  to succinctly denote \inst{n} \textit{consecutive} visits to the same PL. 
In particular, row labels \inst{PL(1)} and \inst{PL(}$l$\inst{)} denote the first and last consecutive visit to \inst{PL}. Node labels specify the concrete value of $l$ for a particular \upath{}, and red happens-before edges represent $l-2$ (implicit) totally-ordered nodes, order after \inst{PL(1)} and before \inst{PL(}$l$\inst{)}, with no other outgoing edges.

From the above, we can deduce that a node is visited in cycle $N$ of an instruction's execution if $N$ is the longest path from $\mathtt{IF}$ to the node in question, accounting for implicit nodes due to consecutive PL visits along the \upath{}. Further, an instruction's overall latency is given by the longest path from $\mathtt{IF}$ to $\mathtt{scbCmt}$---4 or 5 cycles for \inst{ADD}, depending on the outcome of the decision at \inst{ID(1)}.

% a node in a \upath{} that corresponds to a rows labeled \inst{PL(x)} is labeled with the value of \inst{x} for that concrete execuion. 
% Namely, an \inst{n}-labeled a bracket between the nodes corresponding to \inst{PL(1)} and \inst{PL(x)} denotes that there are \inst{n} totally ordered nodes, including \inst{PL(1)} and \inst{PL(x)}, with no other outgoing edges.
% \inst{x = n} (for that concrete \upath{}).
% the
% row label \inst{PL(x)} combined with an \inst{n}-labeled bracket between the nodes corresponding to \inst{PL(1)} and \inst{PL(x)} denotes \inst{x = n}.
% % for some concrete \upath{}. 
% For \inst{n>2}, nodes corresponding to \inst{PL(1)} and \inst{PL(x)} are connected by a dashed happens-before edge, which represents \inst{x} totally ordered nodes, including \inst{PL(1)} and \inst{PL(x)}, with no other outgoing edges.
% representing consecutive revisits to \inst{PL} across \inst{l} cycles.




\yao{
Propose the structure (after explaining background e.g., side-channel defenses ...):  \\
sec 3 (new): upath + PL formalism  to enable upathFNDR \\ 
sec 4: leakage function explain (table for on hw defenses) \\
sec 5: leakage function synthesis formal foundation \\ 
sec 6:  synthzigin leakage function from RTL a.k.a. implementation of upathfndr and symbolic ift; \\ 
sec 7: case study \\ 
sec 8: result \\ 
sec 9: related work \& conclusion \\ 
}

==> fig-paths.tex <==
\begin{figure}[t!]
    \centering
     %\includegraphics[width=0.95\linewidth]{figs/paths_3_9_3.png}
     %\includegraphics[width=0.95\linewidth]{figs/paths_3_9_5.png}
%     \includegraphics[width=0.93\linewidth]{figs/paths_5_3.png}
     %\includegraphics[width=1.0\linewidth]{figs/path_v5.png}
     \includegraphics[width=1.0\linewidth]{figs/path_v6.png}
     %\includegraphics[width=0.95\linewidth]{figs/paths_3_9_6.png}
     \caption{
     Left to the bar: \inst{ADD} \upaths{} on CVA6-OP (\S\ref{sec:upath_formal}). 
     %Gray: Original \uhb{} semantics. 
     Right to the bar: A sample of \upaths{} for the CVA6 core (for \inst{BEQ}, \inst{LD}) and data cache (for \inst{ST}) based on \PathFinder{} synthesis results (\S\ref{sec:results}). 
     Row({\inst{1}/\llt{}}): 1st/\llt{}-th visit to Row.
     %\llt{} is defined in node label. 
     Node label: value of \llt{} for \upath{}.
     % Node label \llt{}: Concrete value for Row (\llt{}).
     %1\textsuperscript{st} to \inst{n}\textsuperscript{th} consecutive visit to Row.
     %Subpath labeled \llt{}: \llt{} consecutive visits to Row.
     % \yao{Updated} 
     %Left: \inst{ADD} \upaths{} on CVA6-OP (\S\ref{sec:tspec:upaths}). 
     %Right: A sample of \upaths{} (\S\ref{sec:results}) synthesized by \tsynth{} from the CVA6 core (for \inst{BEQ}, \inst{LD}) and data cache (for \inst{ST}). 
     %Row\textsubscript{\inst{f}}: \textit{final} visit to Row. Node label \inst{n}: 1\textsuperscript{st} to \inst{n}\textsuperscript{th} consecutive visit to Row.
     %%Row($f$/$l$): PL (first up to \inst{n}-th/last consecutive visit; \inst{n}: \# in a node)
     %% \rsout{Row(\textsubscript{n}):  %PL (\S\ref{sec:tspec:pls}) 
     %% an exec. phase 
     %% ($\mathsf{n}$: \# in a node, one up to n-th consecutive revisit).} %. OP: Operand-packing. % extension. % t=67/68 for original/operand-packing extended CVA6 
     %%Paths for \inst{ADD} are potential paths running on CVA6 augmented with operand-packing based on the synthesized paths:  ID1 is additional decode slot to enable multi-issue. Row(F/L): an exec. phase (first/last consecutive visit)
     %%\yao{edge label, n; }
     %% A sample of synthesized \upaths{} on CVA6 with respect to data cache (for \inst{SW}) and core (for \inst{BEQ}, \inst{LW}, \inst{ADD}).
     %% % Row(F/L): an exec. phase (first/last consecutive visit). 
     %%\chris{sentence to define the yellow/green node coloring.}
     %Orange/Blue nodes: decision source/destination PLs (\S\ref{sec:tspec:transponders}).
     %\yao{dashed edge for edge for revisited nodes}
     % \yao{scbC}
     \chris{now that we have more space, I suggest we split this figure up into several.  E.g., it is unwieldy to talk about the "left" and "right" uPath in SIV when we have a bunch of different examples rammed into here.}
     }
     \label{fig:upaths-example}

\end{figure}

==> new-intro.tex <==
\section{Introduction}
% Same opening up as uspec rtl
A standard strategy to enhance the efficacy of formal verification procedures is to analyze an \textit{abstract model} of the target system, which omits irrelevant design details~\cite{todo}.
A particularly successful deployment of this strategy has emerged in the computer architecture community over the past decade, where abstract microarchitectural models that  omit irrelevant RTL implementation details have facilitated two traditionally challenging verification tasks.
In particular, \textit{\uspec{} models} enable the \textit{Check} family of tools to conduct 
formal memory consistency model~\cite{pipecheck, ccicheck, coatcheck, tricheck, rtlcheck, pipeproof} and security~\cite{checkmate} verification of processors efficiently and automatically.

\paragraph{The Check Tools}
A their core, the Check tools conduct \textit{microarchitectural happens-before} (\uhb{}) analysis, which
models hardware-specific program executions as directed \textit{\uhb{} graphs} (e.g., Fig.~\ref{}). 
Nodes in a \uhb{} graph represent microarchitectural events, namely, program instructions (column labels, with program order proceeding from left to right) updating \textit{sets} of hardware state elements (row labels).
Directed edges denote happens-before relationships between nodes. 
The utility of \uhb{} graphs comes from their ability to determine whether a microarchitectural execution of a program is \textit{observable}; a \textit{cyclic} \uhb{} graph encodes an \textit{unobservable} execution. 

To facilitate \uhb{} analysis, the Check tools are provided with microarchitecture in the guise of an an axiomatic \emph{\uspec{} model} (Fig.~\ref{uspec_extracted})---a collection of first-order logic axioms (i.e., rules), 
which describe how to construct \uhb{} graphs that encode hardware-specific program executions on the design.
More specifically, the axioms encode (1) all \textit{microarchitectural execution paths} for each implemented instruction (encoding column-wise nodes and edges), and (2) all possible \textit{structural} and \textit{data-flow} dependencies between pairs executing instructions (instantiating edges between graph columns)~\cite{rtl2uspec:hsiao:2021}.

Given a \uspec{} model, the Check tools
leverage automated reasoning engines (e.g., SAT~\cite{sat:chaff} or SMT~\cite{barrett:smt} solvers) to search the space of \textit{possible} hardware-specific program executions encoded by the model for those which exhibit memory consistency~\cite{pipecheck, ccicheck, coatcheck, tricheck, rtlcheck, pipeproof} or security~\cite{checkmate} bugs. Each  execution \textit{possibility} corresponds to a distinct \textit{acyclic} \uhb{} graph that satisfies all \uspec{} model axioms.






\paragraph{The \uspec{}-RTL Gap}
% No one wants to write these uspec models for RTL 
Despite their success in finding bugs in real hardware~\cite{pipecheck, tricheck, c11counterexamples, checkmate, spectremeltdownprime}, the \textit{Check} tools have not achieved widespread adoption due to a longstanding gap between \uspec{} models and the RTL they represent.

% While we can synthesize them given this work from micro 21
% Modern processors have multiple upaths through a microarchitecture
Recent work, called \rtltouspec{}, narrows this gap via a methodology for automatically synthesizing (i.e., ``reverse-engineering'') formally-verified \uspec{} models from SystemVerilog processor designs, using a combination of static netlist analysis, linear temporal logic (LTL) property generation~\cite{}, and model checking~\cite{rtl2uspec:hsiao:2021}.
However, \rtltouspec{} restricts the scope of designs it supports to those where each implemented instruction may exhibit exactly one \textit{microarchitectural execution path}, and thus one \uhb{} graph column, when it executes---coined the \textit{single-execution-path assumption} in the original paper. 
This restriction precludes pervasive hardware features like: caches, which create hit and miss paths for memory instructions; serial dividers, which create many execution path possibilities for division instructions; and speculation, which creates commit and squash paths for virtually all instructions.

Thus, deploying the \textit{Check} tools on advanced processors, currently requires constructing \uspec{} models \textit{by hand}.

% This paper's contribution is to extend from micro 21 to support multiple upaths for this
% * We present a formalisms for this
\paragraph{This Paper}
% Check tools which build out the \usepc{} model formalism, define \uspec{} models in terms of microarchitectural events and happens-before relationships betweeen events. Our formalism maps the notion of a microarchitectural event on to a state in a control-path finite state machine of a processor implemenation.
In this paper, \textbf{our primary contribution} is an extension to \rtltouspec{} that resolves its single-execution-path assumption.
% We achieve this goal through three steps.
This extension is made possible by a novel \upath{} abstraction, which effectively formalizes the notion of microarchitectural execution path as \textit{cycle-accurate} \uhb{} graph column. In other words, \upath{} nodes represent an instruction updating a particular set of hardware state elements in a given cycle, and edges encode one-cycle happens-before relationships between nodes. For example, Fig.~\ref{} illustrates two distinct \upaths{} for two different RISC-V instructions---\inst{MUL} and \inst{SUB}---as implemented on the CVA6 CPU~\cite{cva6}. \caroline{More explanation here...}

We further show that \upath{} nodes, as defined above, are precisely captured by \textit{distinct control states} in a subset of finite state machines (FSMs) within a processor's control path that instructions ``visits'' during their execution executions.
Such FSM, which we call \textit{micro-op FSMs} (\ufsms{}), orchestrate the execution of instructions from the time they are fetched until the time they perform their final state updates (possibly after they commit).

Hence, we design an automated procedure---based on static netlist analysis, LTL property generation, and model checking---for synthesizing a formally-verified set of \upaths{} (and their corresponding \uspec{} axioms) for each implemented instruction on a SystemVerilog processor design. 


% We demonstrate applications of this formalism to hardware security problems
% * If an instruction has multiple execution paths through a uarch its a strong signal it can leak the operands 
% * If you can further identify divergences you identify where to interlock instructions to prevent using 
% * if you can further differential SDO
\textbf{Our secondary contribution} is a demonstration of the utility of our \upath{} formalism beyond the realm of \uspec{} model synthesis. In particular, we observe that our automated procedure for synthesizing all \upaths{} per instruction on a microarchitecture lays the foundation for synthesizing formally-verified \textit{leakage contracts}~\cite{ct,} from the same designs.



% \paragraph{Verification of Microarchitectural Leakage Contracts}

If an instruction can exhibit multiple \upaths{} on a microarchitecture, it is a strong signal that it can leak its own and/or some other instruction(s)'s operands. 





% Multi-uspec formalisms with applications for hardware security 





% That is, we propose a formalism and associated analysis procedure to support synthesizing \uspec{} models that capture all des, for a particular hardware instruction, all microarchitectural execution paths it may exhibit on given SystemVerilog implementation.


% To this end, we first propose formal object, called a \upath{}, which encodes a specific cycle-accurate execution path of an instruction on a microarchitecture as a directed graph. Fig.~\ref{} illustrates two distinct \upaths{} for two different RISC-V instructions---\inst{MUL} and \inst{SUB}---as implemented on the CVA6 CPU~\cite{cva6}. 
% % As in prior work~\cite{pipecheck, ccicheck, coatcheck, tricheck, rtlcheck, pipeproof, checkmate},
% In general, \upaths{} are (slightly) more detailed variants of \textit{microarchitectural happens-before} (\uhb{}) graphs~\cite{pipecheck, ccicheck, coatcheck, tricheck, rtlcheck, pipeproof, checkmate} that encode the executions of individual instructions.
% Nodes in a \upath{} represent the microarchitectural execution phase of an instruction in a particular cycle, and edges represent one-cycle happes-before relationships between nodes. 



% The \textit{Check} verification tools~\cite{checkweb} show that various formal hardware verification tasks can be conducted efficiently and automatically when directed at abstract models of microarchitectures, instead of detailed RTL implementations. In particular, the Check tools conduct push-button memory consistency model~\cite{pipecheck, ccicheck, coatcheck, tricheck, rtlcheck, pipeproof} and security~\cite{checkmate} verification of a microarchitecture, supplied in the guise of an axiomatic specification, called a \uspec{} model.
% % s supplied in the guise of axiomatic \textit{\uspec{} models}. 


% % A large body of prior work shows that ciritcal formal hardware verification tasks can be conducted efficiently and automatically with respect to  when targetting an abstract microarchitectural specificaiton, called a \uspec{} model, instead of detailed RTL. Shows significant ef
% It has been shown that various formal hardware verification tasks can be conducted efficiently and automatically with respect to abstract models of microarchitectures, called \textit{\uspec{} models},  detailed RTL implementations~\cite{pipecheck, ccicheck, coatcheck, tricheck, rtlcheck, pipeproof, checkmate}. 
% % In particular, the \textit{Check} line of work first proposed

% ---i.e., which \textit{microarchitectural execution paths} (\upaths{}) instructions may exhibit---and interact with other instructions that are in-flight concurrently.
%with respect to which state elements it updates in which (partial) order (i.e., a microarchitectural execution path), 
% In doing so, 


% In particular, we first propose a novel \upath{} formalism for encoding an instruction's distinct \upath{} possibilities on a particular hardware implementation as a cycle-accurate \textit{microarchitectural happens-before} (\uhb{}) graph~\cite{lamport:happensbefore, pipecheck, ccicheck, coatcheck, tricheck, rtlcheck, pipeproof, checkmate}.
% Second, we show 




% In particular, we first propose a novel formalism for encoding an instruction's distinct microarchitectural execution path possibilities on a particular processor design. 




% In essence, \uspec{} models are first-order logic (FOL) \textit{ordering specifications} of a microarchitecture. They are composed of a set of \textit{axioms} that describe how each legal hardware instruction (1) flows through the microarchitecture during its execution, with respect to which state elements it updates in which (partial) order (i.e., a microarchitectural execution path), and (2) interacts with other in-flight instructions during its execution via \textit{structural} or \textit{data-flow} dependencies.
% The \textit{Check} tools use \uspec{} models to reason about each possible execution of a program on a microarchitecture as a \textit{directed acyclic graph}, called a \uhb{} graph. Nodes in a \uhb{} graph represent hardware events---namely, an instruction updating a particular state element during its execution; directed edges represent happens-before relationships between events. Fig.~\ref{fig:divopres} shows three enhanced \uhb{} graphs (featuring edge labels) which each represent an execution path of a single instruction.







% At a high level, a \upath{} can be visualized as a vertically-oriented directed graph (e.g., Fig.~\ref{}), where a node denotes the \textit{execution phase} of an instruction in a particular cycle, and edge represents a one-cycle \textit{happens-before} relationship between nodes~\cite{lamport:happensbefore}.




% Within the domain of hardware verification, a prominent abstract model of processor microarchitecture, which disregards irrelevant RTL implementation details, has emerged as a facilitator for tackling two traditionally challenging verification tasks. Specifically, \textit{\uspec{} models} empower the \textit{Check} suite of tools to efficiently and automatically conduct formal verification of processor microarchitectures for memory consistency models~\cite{pipecheck, ccicheck, coatcheck, tricheck, rtlcheck, pipeproof} and security properties~\cite{checkmate}.

% has emerged within the last ten years  of this strategy 
% Within the domain of hardware verification, one such abstract model of processor microarchitecture that
% eschews irrelevant RTL implementation details stands out as an enabler for two

==> table-hw-defense.tex <==
{
\renewcommand{\arraystretch}{1.12}
\begin{table}[t!]
\setlength\tabcolsep{1pt}
\centering
\footnotesize
%\scriptsize
%\tiny
\begin{tabular}[]{
        |>{\centering\arraybackslash} m{19mm} %0.001\textwidth}
        |>{\raggedright\arraybackslash} m{42mm}
        |>{\centering\arraybackslash} m{2mm}
        |>{\centering\arraybackslash} m{2mm}
        |>{\centering\arraybackslash} m{4.5mm}
        |>{\centering\arraybackslash} m{3mm}
        |>{\centering\arraybackslash} m{3mm}
        |>{\centering\arraybackslash} m{3mm}
        |>{\centering\arraybackslash} m{2mm}|
        }
        % in order to find left side, what do we need on right hand side?
        %& \textbf{Leakage Signatures}
%        & & & & & &  & \\
        \hline
\multirow{2}{19mm}{\centering \textbf{Defense}} & \multicolumn{1}{c|}{\multirow{2}{42mm}{\centering\textbf{Leakage Contract Components}}} & \multirow{2}{*}{\textbf{$\mu$}} & \multicolumn{6}{c|}{\textbf{Leakage Sig.}} \\ 
\cline{4-9}
& & & & & & & \\ [-9pt]
& & & 
%\hline 
\inst{P} & \inst{src} & $T^\mathtt{N}$ & $T^\mathtt{D}_\mathtt{O}$ & $T^\mathtt{S}$  & \inst{a} \\ 
\specialrule{.2em}{.1em}{.1em} 
%Defenses based on CT Contract$\diamond$
CT, SCT (\S\ref{sec:background:hw-sc-defenses}) \newline SpecShield~\cite{barber:specshield} \newline ConTExt~\cite{Schwarz:ConTExT} 
 & Constant-time contract (\S\ref{sec:background:hw-sc-defenses}) & - & - &  & \chkm{} & \chkm{} & \chkm{} & \chkm{} \\
\specialrule{.2em}{.1em}{.1em} 
%% \hline 
%%NDA~\cite{weisse:nda} & Identifying SSB  & \chkm{} & & & & & \\ % \& fixing
%\hline
\multirow{2}{*}{MI6~\cite{Bourgeat:m16}} & Contention-based dynamic channels & & \chkm{} & \chkm{} & & \chkm{} & & \chkm{} \\ 
\cline{2-9}
 & Static channels & & \chkm{} & \chkm{} & & & \chkm{} & \chkm{} \\
\specialrule{.2em}{.1em}{.1em} 
OISA~\cite{yu:oisa} & Input-dependent arithmetic units & &  & \chkm{} & \chkm{} & & & \chkm{} \\
\specialrule{.2em}{.1em}{.1em} 
\multirow{5}{13mm}{STT~\cite{jiyong:stt}
SDO~\cite{jiyong:sdo}
SPT~\cite{choudhary:2021:spt}} & Explicit channels & &  & &\chkm{} & & & \chkm{} \\
%\cline{2-9}
\hhline{~--------}
 & Explicit branches$*$ & \multicolumn{7}{c|}{\cellcolor{gray!30}}  \\
\cline{2-9}
 & Implicit branches & & \chkm{} & \chkm{} & & \chkm{} & \chkm{}  & \chkm{}\\
\cline{2-9}
 & Prediction-based channels & & \chkm{} & \chkm{} & & & \chkm{} & \chkm{}\\
\cline{2-9}
 & Resolution-based channels & & \chkm{} & \chkm{} & &  \chkm{} && \chkm{} \\
%\cline{2-9}
% & Branch resolution point & & \chkm{} & &  &  & \chkm{} \\
\specialrule{.2em}{.1em}{.1em} 
{\multirow{1}{13mm}{\centering SDO~\cite{jiyong:sdo}}} & Data-oblivious variants & \chkm{} &  &  &  & & & \chkm{} \\
%\cline{2-9}
%& DO control/prediction logic &  & & & & & \\ 
\specialrule{.2em}{.1em}{.1em} 

\multirow{6}{13mm}{Dolma~\cite{dolma}} & Variable-time micro-ops & &  & & \chkm{} & & & \chkm{}\\
\cline{2-9}
& Contention-based dynamic channels due to variable time micro-ops & & \chkm{} & \chkm{} & \chkm{} & \chkm{} & & \chkm{} \\ 
\cline{2-9}
& Inducive micro-ops & & \chkm{} & & & \chkm{} & & \chkm{}\\ 
\cline{2-9}
& Resolvent micro-ops & &  &  &  & \chkm{} & & \chkm{}\\ 
\cline{2-9}
& Prediction resolution points &  & \chkm{} & \chkm{}    &  & \chkm{} & & \chkm{}\\ 
\cline{2-9}
& Persistent state modifying micro-ops & & \chkm{} & \chkm{}  &  & & \chkm{}& \chkm{} \\ 
\hline
%% & Transmitters affecting uarch states & & \chkm{} & &  &  & \\
%\hline %, \yao{branch resolution point} % so to block younger instruction who can be influence by the branch resolution 
% \\ 
% \hline 
% MI6~\cite{Bourgeat:m16}& \gntxt{Strong timing independence}: [\inst{T^D}, $\mathbf{src}^I_\mathnormal{M}$], \newline \gntxt{microarchitectural state flushes}: [\inst{T^D}, \inst{T^S}] \\ 
% \hline 
% & \\[-8pt]
% OISA~\cite{oisa} & \gntxt{Safe mode for transmitters}: [\inst{T^N}, $\mathbf{src}^I_\mathnormal{M}$] \\ [2pt] %, \newline \gntxt{branch predictor requirement}: \inst{T^S}\\ 
% \hline 
% & \\[-8pt]
% STT~\cite{jiyong:stt}* & {\color{green!40!black}Explicit channels}: \inst{T^N}, {\color{green!40!black}implicit channels}: \inst{[T^S, T^D]}, \newline {\color{green!40!black}branch resolution effected point}: $\mathbf{src}^I_\mathnormal{M}$ \\
% %points at which is affected by implicit branch resolution
% & \\[-8pt]
% \hline
% & \\[-8pt]
% ConTExt \cite{Schwarz:ConTExT} & \gntxt{Instructions that requires stall}: \inst{T^D}, \gntxt{operations influencing microarchitectural elements}: \inst{T^D, T^S} \\
% \hline 
% & \\ [-8pt]
% SDO~\cite{jiyong:sdo} & \gntxt{DO control logics}: $\mathbf{src}^I_\mathnormal{M}$, \gntxt{DO invariants}: \upaths{}\\ 
% & \\[-8pt]
% \hline
% & \\ [-8pt]
% Dolma \cite{dolma} & \gntxt{Variable-time micro-ops}: \inst{T^N}, \gntxt{inducive micro-ops}: \inst{P}, % associated with some \inst{T^D},  % case for store-to-load bypass..
% \gntxt{resolvent micro-ops}: \inst{T^D}, \gntxt{persistent state modifying micro-ops}: \inst{T^S}, \gntxt{prediction resolution}: $\mathbf{src}^I_\mathnormal{M}$ \\ [10pt]
% \hline
% SPT & STT requirements\\
% \hline
% & \multicolumn{1}{c|}{\textbf{Terms From Prior Works}}   \\
%\hline
%\textbf{\inst{T^N}} & Variable-time micro-ops (Dolma), explicit channels (STT*), inducive micro-ops (Dolma) \\ 
%\hline
%\textbf{\inst{T^D}} & Strong timing independence (MI6), implicit channels (STT*), ConTExt (instructions that requires stall), resolvent micro-ops (Dolma)   \\ 
%\hline
%\textbf{\inst{T^S}} & Microarchitectural state flushes (MI6), branch predictor requirements (OISA), implicit channels (STT*), operations influencing "uncore" or off-core microarchitectural elements (ConTExt), micro-ops producing persistent state modifications (Dolma) \\
%\hline
%\textbf{$\mathbf{src}^I_\mathnormal{M}$} & Enforcement of strong timing independence (MI6), Points where the effects of branch resolution take place (STT*), DO invariants control logics (SDO), prediction resolution for inducive micro-ops (Dolma) \\
%\hline 
%\textbf{\upaths{}} & Checking if SSB is a thread (NDA), DO invariants (SDO) \\
%\hline
\end{tabular}
\caption{Six classes of hardware side-channel defenses, with leakage contract requirements mapped onto \upaths{} ($\mu$) and leakage signatures. \inst{a}: Arguments. $*$: In the ISA.
% \chris{It's not clear what the column labels \inst{a} $\mu$, \inst{P} mean or what some of the combinations (like the first row -- SRC unchecked) mean.  Maybe walk through an example or two in the main body text?}
% \yao{attempted at \S\ref{sec:leakage-signatures}}
%
%{\color{red}%\marginpar{R ?? }
%test %T-Y/T-O younger/older
%}
% Leakage contracts per mega row indexed by supported defenses. %STT*: Include STT~\cite{jiyong:stt}, SDO~\cite{jiyong:sdo}, and SPT~\cite{choudhary:2021:spt}. 
% $\diamond$: CT Programming, SCT Programming~\cite{serberus:mosier:2024}, SpecShield~\cite{barber:specshield}, ConTExt~\cite{Schwarz:ConTExT}. 
%
% \caroline{Let's put CT contracts and defenses that use them as the first row in the table. Also, we don't need commas in the defense row - let's just make sure they're all on different lines. And, these won't all be ``bespoke.''}
} %$\diamond$: STT leakage contract is also required. }
\label{table:defenses_map}
\end{table}
}

% NDA: 
%   For SSB, bypass restriction: Instead of SSBD (load does not exec until all older stores resolve), it allows speculative load to execute and bypass in presence of unresolved stores. But this speculative load cannot forward data to dependent instructions until all bypassed store addresses are resolved. If a store's address is not resolved, loads that follow the store may read stale data. That is, exe transmitter (only ld in this work) but delay exe of all dependent until transmitter(ld) becomes non-speculative 

% {
% \renewcommand{\arraystretch}{1.0}
% \begin{table}[t!]
% \setlength\tabcolsep{0.8pt}
% \centering
% \footnotesize
% %\scriptsize
% %\tiny
% \begin{tabular}[]{
%         |>{\centering\arraybackslash} m{13mm} %0.001\textwidth}
%         |>{\raggedright\arraybackslash} m{30mm}
%         |>{\centering\arraybackslash} m{10mm}
%         |>{\centering\arraybackslash} m{7mm}
%         |>{\centering\arraybackslash} m{3mm}
%         |>{\centering\arraybackslash} m{3mm}
%         |>{\centering\arraybackslash} m{3mm}
%         |>{\centering\arraybackslash} m{3mm}|
%         }
%         % \textbf{Leakage Signatures}
%         \hline
% \textbf{Defense} & \textbf{Features of Leakage Contract} & \textbf{\upaths{}} &  \textbf{$\mathbf{src}^I_\mathnormal{M}$} & \inst{T^N} & \inst{T^D} & \inst{T^S} & \inst{P} \\ 
% % \hline 
% % NDA~\cite{weisse:nda} & \gntxt{Speculative-load bypasses unresolved stores}: \upaths{} %, \yao{branch resolution point} % so to block younger instruction who can be influence by the branch resolution 
% % \\ 
% % \hline 
% % MI6~\cite{Bourgeat:m16}& \gntxt{Strong timing independence}: [\inst{T^D}, $\mathbf{src}^I_\mathnormal{M}$], \newline \gntxt{microarchitectural state flushes}: [\inst{T^D}, \inst{T^S}] \\ 
% % \hline 
% % & \\[-8pt]
% % OISA~\cite{oisa} & \gntxt{Safe mode for transmitters}: [\inst{T^N}, $\mathbf{src}^I_\mathnormal{M}$] \\ [2pt] %, \newline \gntxt{branch predictor requirement}: \inst{T^S}\\ 
% % \hline 
% % & \\[-8pt]
% % STT~\cite{jiyong:stt}* & {\color{green!40!black}Explicit channels}: \inst{T^N}, {\color{green!40!black}implicit channels}: \inst{[T^S, T^D]}, \newline {\color{green!40!black}branch resolution effected point}: $\mathbf{src}^I_\mathnormal{M}$ \\
% % %points at which is affected by implicit branch resolution
% % & \\[-8pt]
% % \hline
% % & \\[-8pt]
% % ConTExt \cite{Schwarz:ConTExT} & \gntxt{Instructions that requires stall}: \inst{T^D}, \gntxt{operations influencing microarchitectural elements}: \inst{T^D, T^S} \\
% % \hline 
% % & \\ [-8pt]
% % SDO~\cite{jiyong:sdo} & \gntxt{DO control logics}: $\mathbf{src}^I_\mathnormal{M}$, \gntxt{DO invariants}: \upaths{}\\ 
% % & \\[-8pt]
% % \hline
% % & \\ [-8pt]
% % Dolma \cite{dolma} & \gntxt{Variable-time micro-ops}: \inst{T^N}, \gntxt{inducive micro-ops}: \inst{P}, % associated with some \inst{T^D},  % case for store-to-load bypass..
% % \gntxt{resolvent micro-ops}: \inst{T^D}, \gntxt{persistent state modifying micro-ops}: \inst{T^S}, \gntxt{prediction resolution}: $\mathbf{src}^I_\mathnormal{M}$ \\ [10pt]
% % \hline
% % SPT & STT requirements\\
% % \hline
% % & \multicolumn{1}{c|}{\textbf{Terms From Prior Works}}   \\
% %\hline
% %\textbf{\inst{T^N}} & Variable-time micro-ops (Dolma), explicit channels (STT*), inducive micro-ops (Dolma) \\ 
% %\hline
% %\textbf{\inst{T^D}} & Strong timing independence (MI6), implicit channels (STT*), ConTExt (instructions that requires stall), resolvent micro-ops (Dolma)   \\ 
% %\hline
% %\textbf{\inst{T^S}} & Microarchitectural state flushes (MI6), branch predictor requirements (OISA), implicit channels (STT*), operations influencing "uncore" or off-core microarchitectural elements (ConTExt), micro-ops producing persistent state modifications (Dolma) \\
% %\hline
% %\textbf{$\mathbf{src}^I_\mathnormal{M}$} & Enforcement of strong timing independence (MI6), Points where the effects of branch resolution take place (STT*), DO invariants control logics (SDO), prediction resolution for inducive micro-ops (Dolma) \\
% %\hline 
% %\textbf{\upaths{}} & Checking if SSB is a thread (NDA), DO invariants (SDO) \\
% %\hline
% \end{tabular}
% \caption{Bespoke leakage contracts used in defenses. STT*: Include STT~\cite{jiyong:stt}, SDO~\cite{jiyong:sdo}, and SPT~\cite{choudhary:2021:spt}. }
% \label{table:defenses_map}
% \end{table}
% }
%{
%\renewcommand{\arraystretch}{1.0}
%\begin{table}[t!]
%\setlength\tabcolsep{0.8pt}
%\centering
%\footnotesize
%%\scriptsize
%%\tiny
%\begin{tabular}[]{
%        |>{\centering\arraybackslash} m{13mm} %0.001\textwidth}
%        |>{\raggedright\arraybackslash} m{65mm}|
%        %|>{\centering\arraybackslash} m{8mm} %0.001\textwidth}
%        %|>{\raggedright\arraybackslash} m{76mm}|
%        }
%        \hline
% \textbf{Defense} & \multicolumn{1}{c|}{\textbf{\gntxt{Terms/requirements} corresponding to terms}} \\        
% \hline 
% NDA~\cite{weisse:nda} & \gntxt{Speculative-load bypasses unresolved stores}: \upaths{} %, \yao{branch resolution point} % so to block younger instruction who can be influence by the branch resolution 
% \\ 
% \hline 
% % \gntxt{Strong timing independence}
% MI6~\cite{Bourgeat:m16}& \gntxt{Dynamic channels (contention-based)}: [\inst{T^D}, $\mathbf{src}^I_\mathnormal{M}$], \newline \gntxt{Static channels}: [\inst{T^S}] \\ 
% \hline 
% & \\[-8pt]
% OISA~\cite{oisa} & \gntxt{Input-dependent arithmetic unit}: [\inst{T^N}, $\mathbf{src}^I_\mathnormal{M}$] \\ [2pt] %, \newline \gntxt{branch predictor requirement}: \inst{T^S}\\ 
% \hline 
% & \\[-8pt]
% STT~\cite{jiyong:stt}* & \caroline{Explicit channels (Tn), explicit branch (comment - ISA), implicit branches (P, src, Td, Ts), prediction-based channels (P, src, Ts), resolution-based channels (P, src, Td)}{\color{green!40!black}Explicit channels}: \inst{T^N}, {\color{green!40!black}implicit channels}: \inst{[T^S, T^D]}, \newline {\color{green!40!black}branch resolution effected point}: $\mathbf{src}^I_\mathnormal{M}$ \\
% %points at which is affected by implicit branch resolution
% & \\[-8pt]
% \hline
% & \\[-8pt]
% ConTExt \cite{Schwarz:ConTExT} & \gntxt{Instructions that requires stall}: \inst{T^D}, \gntxt{operations influencing microarchitectural elements}: \inst{T^D, T^S} \\
% \hline 
% & \\ [-8pt]
% SDO~\cite{jiyong:sdo} & \gntxt{DO control logics}: $\mathbf{src}^I_\mathnormal{M}$, \gntxt{DO invariants}: \upaths{}\\ 
% & \\[-8pt]
% \hline
% & \\ [-8pt]
% Dolma \cite{dolma} & \gntxt{Variable-time micro-ops}: \inst{T^N}, \gntxt{inducive micro-ops}: \inst{P}, % associated with some \inst{T^D},  % case for store-to-load bypass..
% \gntxt{resolvent micro-ops}: \inst{T^D}, \gntxt{persistent state modifying micro-ops}: \inst{T^S}, \gntxt{prediction resolution}: $\mathbf{src}^I_\mathnormal{M}$ \\ [10pt]
% \hline
%% SPT & STT requirements\\
%% \hline
%% & \multicolumn{1}{c|}{\textbf{Terms From Prior Works}}   \\
%%\hline
%%\textbf{\inst{T^N}} & Variable-time micro-ops (Dolma), explicit channels (STT*), inducive micro-ops (Dolma) \\ 
%%\hline
%%\textbf{\inst{T^D}} & Strong timing independence (MI6), implicit channels (STT*), ConTExt (instructions that requires stall), resolvent micro-ops (Dolma)   \\ 
%%\hline
%%\textbf{\inst{T^S}} & Microarchitectural state flushes (MI6), branch predictor requirements (OISA), implicit channels (STT*), operations influencing "uncore" or off-core microarchitectural elements (ConTExt), micro-ops producing persistent state modifications (Dolma) \\
%%\hline
%%\textbf{$\mathbf{src}^I_\mathnormal{M}$} & Enforcement of strong timing independence (MI6), Points where the effects of branch resolution take place (STT*), DO invariants control logics (SDO), prediction resolution for inducive micro-ops (Dolma) \\
%%\hline 
%%\textbf{\upaths{}} & Checking if SSB is a thread (NDA), DO invariants (SDO) \\
%%\hline
%\end{tabular}
%\caption{Bespoke leakage contracts used in defenses. STT*: Include STT~\cite{jiyong:stt}, SDO~\cite{jiyong:sdo}, and SPT~\cite{choudhary:2021:spt}. }
%\label{table:f_leak_defense}
%\end{table}
%}
%        %SPT~\cite{choudhary:2021:spt}, Dolma~\cite{dolma}, STT~\cite{jiyong:stt}, SDO~\cite{jiyong:sdo}, MI6~\cite{Bourgeat:m16}, ConTExt~\cite{Schwarz:ConTExT}, OISA~\cite{yu:oisa}, NDA~\cite{weisse:nda} \\
%% \subsection{Bullets summarizing related works}
%% \begin{itemize} [topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
%% \item Intrinsic transmitters are required in Dolma (called variable-time micro-ops), STT family of works including STT, SDO, SPT (called explicit channels)
%% \item Dynamic transmitters are required in MI6 (called Strong Timing Independence), STT family of works (called implicit channels), ConTExt (called instruction that influece the microarchitectural state that it has to stall), and Dolma (called resolvent micro-ops). 
%% \item Static transmitter are required in MI6 (for its microarchitectural state flushes), OISA (for its requirement on branch predictor), STT family of works (included in the implicit channels), ConTExt (called operations that influence "uncore" or off-core microarchitectural elements), and Dolma (micro-ops that produce persistent state modifications).
%% \item Decisions source PL are required in MI6 (to enforce strong timing independence), STT family of works (for the point where ``the effects of branch resolution'' take place), SDO (for implementing the control to select DO invariants), and Dolma (for the poitn where ``prediction resolves for inducive micro-ops''). 
%% \item upaths are required in NDA (for checking if speculative-store-bypass is a threat), and SDO (for DO invariants). 
%% % decision source PL is not enough, take MUL for eample, one needs to know a total of 64 paths can spawn from the mulU corresponding to 64 DO invariants (non-interfereing w.r.t the input operand value)
%% \end{itemize}
